Firm Heterogeneity, Market Power and Macroeconomic Fragility

We study how firm heterogeneity and market power affect macroeconomic fragility, defined as the probability of long slumps. We propose a theory in which the positive interaction between firm entry, competition and factor supply can give rise to multiple steady-states. We show that when firms are highly heterogeneous in terms of productivities, even small temporary shocks can trigger firm exit and make the economy spiral in a competition-driven poverty trap. We calibrate our model to incorporate the well-documented trends on rising firm heterogeneity in the US economy, and show that they significantly increase the likelihood and length of slow recoveries. We use our framework to study the 2008-09 recession and show that the model can rationalize the persistent deviation of output and most macroeconomic aggregates from trend, including the behavior of net entry, markups and the labor share. Post-crisis cross-industry data corroborates our proposed mechanism. We conclude by showing that firm subsidies can be powerful in preventing long slumps and can lead to welfare gains between 10% and 50%.

==> TO_DO.tex <==
AEJ:MA Revision

writing/theory
%- eliminate S2 and introduce fragility in S3
%- write the full characterization without eta=1 and Gamma_i=Gamma and then have all comparative statics with those conditions 
%- cournot eqm, read fucking impulliti whatever  
%- proof of concavity of Omega for Prop 3

code/quantitative model
%- use a 1-5\% sample of the largest firms to compute moments for comparability with Compustat.
%as a first step we can just compute the markup of the top 1-5\% largest in the current calibration. 
- use a fixed cost distribution that takes value 0 for a fraction f and has a normal distribution for the remaining 1-f. ideally it should be centered at c and with a small variance
%- cost-weighted markup as target
- model versions without i) oligopolistic competition; ii) extensive margin; iii) endogenous factor supply
- run regressions on model data (R2 point 3)
- reverse engineer changes in f that generate the observed changes in measured TFP
- add shocks post recession (10-15 quarters of exog TFP variation to show that 1990 recovers quick)
- additional policy experiment
%- transition probs of upward changes



==> input/proof_prop4.tex <==
\begin{proof}[Proof of Proposition \ref{prop:MPS_BA}]
The proposition we set out to prove states that when we apply a mean-preserving spread to $n$ firms in the economy, the $n$-firms steady state becomes more fragile to negative shocks. 

Before diving in the proof we provide a brief sketch of the logic we will follow. Denote our steady state of interest as $K^\star_n$ and the unstable steady state to its left by $\tilde K_{n-1,n}$. 
We start by noting that the statement is equivalent to saying that $|K^\star_n-\tilde K_{n-1,n}|$ decreases. 

We apply a mean-preserving spread to $n$ firms, where $n$ is the number of firms in the highest steady state.
We prove via the following steps: 
\begin{enumerate}
\item we provide two preliminary remarks:
\begin{enumerate}
    \item we note that we can characterize movements in $K$ by means of movements in the the rental rate map $r(K)$ whose crossings with the horizontal line $r_{ss}$ define steady states.
    \item we note that the shifts in $r(K)$ following a MPS solely depend on the movements in the the aggregate factor cost index $\Theta(\Gamma,N)$.
    \end{enumerate}
    \item we show that in the symmetric region with $n$ firms $\Theta(n)$ decreases and, therefore, $K^\star_n$ decreases.
    \item we prove that $\Theta(\Gamma,N)$ does not increase in the region between $\tilde K_{n-1,n}$ and $K^\star_n$ when $n=2$ and that this holds a fortiori for any $n>2$.
\end{enumerate}
\vspace{5pt}
\noindent\textbf{Preliminaries}
\begin{remark}
The set of stable and unstable  steady states $\mathcal{K}$ is defined by zeros in the function $h(K,\Gamma,N)\equiv r(K, \Gamma, N)-r^{ss}$. As $r^{ss}$ is a constant we can study movements in elements of $\mathcal{K}$ by characterizing movements in $r(K, \Gamma, N)$.
\end{remark}
\begin{remark}
As discussed in the main body, $r_t=\alpha\;{A}_{t} \: \Theta(\Gamma,N)\;L_{t}^{1-\alpha}\,K_{t}^{\alpha-1}.$ As we are fixing $K$ and $L$ only moves with $K$, the whole function moves in the same direction as $\Theta(\Gamma, N)$.  
\end{remark}

Finally, note that the region of interest for the proof is the one between an unstable steady state and a stable one. We know that the former is given by a zero of $h(\cdot)$ ``from below'' and the latter by a zero ``from above''. Therefore we set out to show that, following an $n$-MPS the $r(\cdot)$ function shifts downward. This will imply that zeros ``from below'' move rightward and zeros ``from above'' move leftward, shrinking the distance between the two. We do so by characterizing how $\Theta$ moves after an $n$-MPS.\\

\vspace{5pt}
\noindent\textbf{$K^\star_n$ decreases}\\
When all industries are identical, stable steady states feature the same number of firms. In these symmetric regions if all industries have $n$ firms with productivities
$\gamma_{1}>\gamma_{2}>\cdots>\gamma_{n}$ we have
\[
\Theta\left(\mathbf{\Gamma},\mathbf{N}\right)=\Theta\left(n\right)=I^{\frac{1-\rho}{\rho}}\dfrac{n-\left(1-\rho\right)}{\sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}}}
\]
Since $f\left(\gamma\right)=1/\gamma$ is convex in $\gamma$, if
$\left\{ \gamma_{k}^{\prime}\right\} _{k=1}^{n}$ is a mean-preserving
spread of $\left\{ \gamma_{k}\right\} _{k=1}^{n}$ then 
%
\[
\begin{array}{rl}
 & \sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}^{\prime}}>\sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}}\\[2ex]
\Leftrightarrow & I^{\frac{1-\rho}{\rho}}\left(\dfrac{n-\left(1-\rho\right)}{\sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}^{\prime}}}\right)<I^{\frac{1-\rho}{\rho}}\left(\dfrac{n-\left(1-\rho\right)}{\sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}}}\right)\\[2ex]
\Leftrightarrow & \Theta^{\prime}\left(n\right)<\Theta\left(n\right)
\end{array}
\]
As $\Theta(n)$ decreases after the $n$-MPS, given the remarks above, $K^\star_n$ decreases.\\

\vspace{5pt}
\noindent\textbf{$\tilde K_{n-1,n}$  does not decrease}\\
Let us now analyze how $\Theta\left(\cdot\right)$ changes at the
unstable steady-state. The proof involves more steps in this region,
since we cannot obtain a closed-form expression for $\Theta\left(\cdot\right)$
when the equilibrium is not symmetric.

First note that when there are $m$ industries with $n$ firms ($n-$oligopolies)
and $I-m$ industries with $n-1$ firms ($\left(n-1\right)-$oligopolies),
we can write $\Theta\left(\cdot\right)$ as
\begin{equation}
\Theta\left(n,m\right)=\left\{ \left(I-m\right)g\left(n-1\right)^{\frac{\rho}{1-\rho}}+m\,g\left(n\right)^{\frac{\rho}{1-\rho}}\right\} ^{\frac{1-\rho}{\rho}}\label{eq:theta_asymmetric}
\end{equation}
where 
\[
g\left(n\right)\equiv\dfrac{n-\left(1-\rho\right)}{\sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}}}
\]
%
As we have proved above $g\left(n\right)$ always decreases following
a mean-preserving spread on $\left\{ \gamma_{k}\right\} _{k=1}^{n}$.
The difficulty in establishing a result in this case lies in two features
of the above expression for $\Theta\left(n,m\right)$. First we cannot
establish whether $g\left(n-1\right)$ increases or decreases after
a mean-preserving spread on all the $n$ firms. Second, $m$ is itself
an endogenous object and is likely to change after the mean-preserving
spread.

In this region, $\Theta\left(\cdot\right)$ is a step function, being
discontinuous at points
\[
\underline{K}\left(n,1\right),\underline{K}\left(n,2\right),\ldots,\underline{K}\left(n,I-1\right),\underline{K}\left(n,I\right)
\]
where $\underline{K}\left(n,m\right)$ is the level of aggregate capital
$K$ such that $n-$oligopolies exactly break-even when there are
$m$ of such $n-$oligopolies. This point is implicitly defined by
\[
\underbrace{\dfrac{1}{1-\rho}\left[1-\dfrac{n-\left(1-\rho\right)}{\sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}}}\dfrac{1}{\gamma_{j}}\right]^{2}\left[\dfrac{n-\left(1-\rho\right)}{\sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}}}\right]^{\frac{\rho}{1-\rho}}}_{\equiv\varLambda\left(j,n\right)}\Theta\left(n,m\right)^{-\frac{\rho}{1-\rho}}\underbrace{\Phi\left(n,m\right)\underline{K}\left(n,m\right)^{\alpha}L^{1-\alpha}}_{Y}-c_{f}=0
\]
%
This is illustrated in Figure \ref{fig:theta_proof}, where the blue
map shows $\Theta\left(\cdot\right)$ as a function of $K$ for an
initial combination of productivity values $\left\{ \gamma_{k}\right\} _{k=1}^{n}$.

\begin{figure}[H]
\begin{centering}
\includegraphics[scale=0.5]{input/theta_proof.eps}
\par\end{centering}
\caption{Factor Cost Index $\Theta$ (asymmetric region) \label{fig:theta_proof}}

\end{figure}

We want to show that, as we apply a mean-preserving spread, the new
map $\Theta^{\prime}$ is such that $\Theta^{\prime}<\Theta$ for
all $K$ with at least one $n-$oligopoly under $\left\{ \gamma_{k}^{\prime}\right\} _{k=1}^{n}$.
Let us take again a look at Figure \ref{fig:theta_proof}. First note
that, for all points below $\underline{K}\left(n,1\right)$, we have
$\Theta^{\prime}\left(n,0\right)>\Theta\left(n,0\right)$. From (\ref{eq:theta_asymmetric}),
this must be because $g^{\prime}\left(n-1\right)>g\left(n-1\right)$.
This indeed shows that, while it is always true that $g^{\prime}\left(n\right)<g\left(n\right)$
when we do a mean-preserving spread on the first $n$ firms, we can
however have $g^{\prime}\left(n-1\right)>g\left(n-1\right)$. So it
is not obvious in which direction $\Theta$, as defined in (\ref{eq:theta_asymmetric}),
will change.

Let us now analyze the interval $\left[\underline{K}\left(n,1\right),\underline{K}\left(n,2\right)\right)$.
In this interval, $\Theta$ takes value $\Theta\left(n,1\right)$
under $\left\{ \gamma_{k}\right\} _{k=1}^{n}$. However, under $\left\{ \gamma_{k}^{\prime}\right\} _{k=1}^{n}$,
the new value of $\Theta$ in this same interval is $\Theta^{\prime}\left(n,0\right)<\Theta\left(n,1\right)$.
This happens because the first $n-$oligopoly is only possible now
at 
\[
\underline{K}^{\prime}\left(n,1\right)>\underline{K}\left(n,2\right)
\]
In other words, while the economy could accommodate one $n-$oligopoly
at $\left[\underline{K}\left(n,1\right),\underline{K}\left(n,2\right)\right)$
with the resulting $\Theta\left(n,1\right)$, now it can only accommodate
$\left(n-1\right)-$oligopolies with the resulting $\Theta^{\prime}\left(n,0\right)<\Theta\left(n,1\right)$.

This happens because 
%
\[
\left.\dfrac{\underline{K}^{\prime}\left(n,m\right)}{\Theta^{\prime}\left(n,m-1\right)}\right|_{m=1}>\left.\dfrac{\underline{K}\left(n,m\right)}{\Theta\left(n,m-1\right)}\right|_{m=1}
\]
%
We will now prove that this must be always the case. We will show
this for the particular case $n=2$ and $m=1$ and then explain why
it must also hold for higher $m$ and $n$. 

\textbf{Proof for $n=2$ and $m=1$ }

Note that for $n=2$ and $m=1$ we have
$
\Theta(2,0)=\rho\gamma_{1}
$.
To obtain $\underline{K}\left(2,1\right)$ note that
\[
\begin{array}{rl}
 & c_{f}=\underbrace{\dfrac{1}{1-\rho}\left(1-\dfrac{1+\rho}{\dfrac{1}{\gamma_{2}}+\dfrac{1}{\gamma_{1}}}\dfrac{1}{\gamma_{2}}\right)^{2}\left(\dfrac{1+\rho}{\dfrac{1}{\gamma_{2}}+\dfrac{1}{\gamma_{1}}}\right)^{\frac{\rho}{1-\rho}}}_{\Lambda\left(2,2\right)}\Theta\left(1\right){}^{-\frac{\rho}{1-\rho}}\underbrace{\gamma_{1}\,\underline{K}\left(2,1\right)^{\alpha}}_{Y}\\
\Leftrightarrow & \underline{K}\left(2,1\right)^{\alpha}=c_{f}\left(1-\rho\right)\left(1-\dfrac{1+\rho}{1+\dfrac{\gamma_{2}}{\gamma_{1}}}\right)^{-2}\left(\dfrac{1+\rho}{\dfrac{1}{\gamma_{2}}+\dfrac{1}{\gamma_{1}}}\right)^{-\frac{\rho}{1-\rho}}\:\left(\rho\gamma_{1}\right){}^{\frac{\rho}{1-\rho}}\gamma_{1}^{-1}\\
\Leftrightarrow & \underline{K}\left(2,1\right)^{\alpha}=\left[c_{f}\left(1-\rho\right)\rho{}^{\frac{\rho}{1-\rho}}\left(1-\dfrac{1+\rho}{1+\dfrac{\gamma_{2}}{\gamma_{1}}}\right)^{-2}\left(\dfrac{1+\rho}{\dfrac{\gamma_{1}}{\gamma_{2}}+1}\right)^{-\frac{\rho}{1-\rho}}\:\gamma_{1}^{-1}\right]^{1/\alpha}
\end{array}
\]
When we do an MPS, we simply increase $\gamma_{1}$ holding $\gamma_{1}+\gamma_{2}$
fixed. Therefore, let
$ \gamma_{1}+\gamma_{2}=2x$ and substitute it in the previous equation we have
\[
\begin{array}{rl}
 %& \underline{K}\left(2,1\right)=\left[c_{f}\left(1-\rho\right)\rho{}^{\frac{\rho}{1-\rho}}\left(1-\dfrac{1+\rho}{1+\dfrac{2x-\gamma_{1}}{\gamma_{1}}}\right)^{-2}\left(\dfrac{1+\rho}{\dfrac{\gamma_{1}}{2x-\gamma_{1}}+1}\right)^{-\frac{\rho}{1-\rho}}\:\gamma_{1}^{-1}\right]^{1/\alpha}\\
%\Leftrightarrow &
\underline{K}\left(2,1\right)=\left\{ c_{f}\left(1-\rho\right)\rho{}^{\frac{\rho}{1-\rho}}\left(1-\left(1+\rho\right)\dfrac{\gamma_{1}}{2x}\right)^{-2}\left[\left(1+\rho\right)\dfrac{2x-\gamma_{1}}{2x}\right]^{-\frac{\rho}{1-\rho}}\gamma_{1}^{-1}\right\} ^{1/\alpha}
\end{array}
\]
Therefore, we have 
\[
\begin{array}{rl}
\dfrac{\underline{K}\left(2,1\right)}{\Theta\left(2,0\right)}%= & \left\{ c_{f}\left(1-\rho\right)\rho{}^{{\color{red}-\alpha}+\frac{\rho}{1-\rho}}\left(1-\left(1+\rho\right)\dfrac{\gamma_{1}}{2x}\right)^{-2}\left[\left(1+\rho\right)\dfrac{2x-\gamma_{1}}{2x}\right]^{-\frac{\rho}{1-\rho}}\gamma_{1}^{-1{\color{red}-\alpha}}\right\} ^{1/\alpha}\\
%= & \left\{ c_{f}\left(1-\rho\right)\rho{}^{-\alpha+\frac{\rho}{1-\rho}}\left(1+\rho\right)^{-\frac{\rho}{1-\rho}}\left(1-\left(1+\rho\right)\dfrac{\gamma_{1}}{2x}\right)^{-2}\left[\dfrac{2x-\gamma_{1}}{2x}\gamma_{1}^{\left(1+\alpha\right)\frac{1-\rho}{\rho}}\right]^{-\frac{\rho}{1-\rho}}\right\} ^{1/\alpha}\\
= & \left\{ c_{f}\left(1-\rho\right)\rho{}^{-\alpha+\frac{\rho}{1-\rho}}\left(1+\rho\right)^{-\frac{\rho}{1-\rho}}\left(1-\left(1+\rho\right)\dfrac{\gamma_{1}}{2x}\right)^{-2}\left[\gamma_{1}^{\left(1+\alpha\right)\frac{1-\rho}{\rho}}-\dfrac{\gamma_{1}^{\left(1+\alpha\right)\frac{1-\rho}{\rho}+1}}{2x}\right]^{-\frac{\rho}{1-\rho}}\right\} ^{1/\alpha}
\end{array}
\]
It follows that the term
\[
\underbrace{\left(1-\left(1+\rho\right)\dfrac{\gamma_{1}}{2x}\right)^{-2}}_{\left(1\right)}\underbrace{\left[\gamma_{1}^{\left(1+\alpha\right)\frac{1-\rho}{\rho}}-\dfrac{\gamma_{1}^{\left(1+\alpha\right)\frac{1-\rho}{\rho}+1}}{2x}\right]^{-\frac{\rho}{1-\rho}}}_{\left(2\right)}
\]
needs to be increasing in $\gamma_{1}$. The derivative of (1) is
\[
-2\left(1-\left(1+\rho\right)\dfrac{\gamma_{1}}{2x}\right)^{-2-1}\left(-\left(1+\rho\right)\dfrac{1}{2x}\right)
\]
and the derivative of (2) is
\[
\begin{array}{rl}
 %& \left(-\dfrac{\rho}{1-\rho}\right)\left[\gamma_{1}^{\left(1+\alpha\right)\frac{1-\rho}{\rho}}-\dfrac{\gamma_{1}^{\left(1+\alpha\right)\frac{1-\rho}{\rho}+1}}{2x}\right]^{-\frac{\rho}{1-\rho}-1}\;\left\{ \left(1+\alpha\right)\frac{1-\rho}{\rho}\gamma_{1}^{\left(1+\alpha\right)\frac{1-\rho}{\rho}-1}-\left[\left(1+\alpha\right)\frac{1-\rho}{\rho}+1\right]\dfrac{\gamma_{1}^{\left(1+\alpha\right)\frac{1-\rho}{\rho}}}{2x}\right\} \\
%= &
\left(-\dfrac{\rho}{1-\rho}\right)\left[\gamma_{1}^{\left(1+\alpha\right)\frac{1-\rho}{\rho}}-\dfrac{\gamma_{1}^{\left(1+\alpha\right)\frac{1-\rho}{\rho}+1}}{2x}\right]^{-\frac{\rho}{1-\rho}-1}\;\gamma_{1}^{\left(1+\alpha\right)\frac{1-\rho}{\rho}}\left\{ \left(1+\alpha\right)\frac{1-\rho}{\rho}\left(\gamma_{1}^{-1}-\dfrac{1}{2x}\right)-\dfrac{1}{2x}\right\} 
\end{array}
\]
Hence, the derivative of the ratio increases in $\gamma_{1}$ if
\[
\begin{array}{rl}
 & -2\left(1-\left(1+\rho\right)\dfrac{\gamma_{1}}{2x}\right)^{-1}\left(-\left(1+\rho\right)\dfrac{1}{2x}\right)+\\
+ & \left(-\dfrac{\rho}{1-\rho}\right)\left[\gamma_{1}^{\left(1+\alpha\right)\frac{1-\rho}{\rho}}-\dfrac{\gamma_{1}^{\left(1+\alpha\right)\frac{1-\rho}{\rho}+1}}{2x}\right]^{-1}\;\gamma_{1}^{\left(1+\alpha\right)\frac{1-\rho}{\rho}}\left\{ \left(1+\alpha\right)\frac{1-\rho}{\rho}\left(\gamma_{1}^{-1}-\dfrac{1}{2x}\right)-\dfrac{1}{2x}\right\} >0\\
%\Leftrightarrow & \left(1-\left(1+\rho\right)\dfrac{\gamma_{1}}{2x}\right)^{-1}\dfrac{1+\rho}{x}+\left[1-\dfrac{\gamma_{1}}{2x}\right]^{-1}\left\{ -\left(1+\alpha\right)\left(\gamma_{1}^{-1}-\dfrac{1}{2x}\right)+\dfrac{1}{2x}\dfrac{\rho}{1-\rho}\right\} >0\\
%\Leftrightarrow & \dfrac{\dfrac{1+\rho}{x}}{1-\left(1+\rho\right)\dfrac{\gamma_{1}}{2x}}+\dfrac{\dfrac{1}{2x}\dfrac{\rho}{1-\rho}-\left(1+\alpha\right)\left(\gamma_{1}^{-1}-\dfrac{1}{2x}\right)}{1-\dfrac{\gamma_{1}}{2x}}>0\\
%\Leftrightarrow & \dfrac{2\left(1+\rho\right)}{2x-\left(1+\rho\right)\gamma_{1}}+\dfrac{\dfrac{\rho}{1-\rho}-\left(1+\alpha\right)\left(\dfrac{2x}{\gamma_{1}}-1\right)}{2x-\gamma_{1}}>0\\
%\Leftrightarrow & \dfrac{2\left(1+\rho\right)}{\left(\gamma_{1}+\gamma_{2}\right)-\left(1+\rho\right)\gamma_{1}}+\dfrac{\dfrac{\rho}{1-\rho}-\left(1+\alpha\right)\dfrac{\gamma_{2}}{\gamma_{1}}}{\gamma_{2}}>0\\
\Leftrightarrow & \dfrac{2\left(1+\rho\right)}{\gamma_{2}-\rho\gamma_{1}}+\dfrac{\dfrac{\rho}{1-\rho}-\left(1+\alpha\right)\dfrac{\gamma_{2}}{\gamma_{1}}}{\gamma_{2}}>0
\end{array}
\]
Recall that we have imposed $\gamma_{2}>\rho\gamma_{1}$, for otherwise $\gamma_{2}$
has a negative market share. In the limit case of $\gamma_{2}=\rho\,\gamma_{1}$
the condition is always satisfied. When $\gamma_{1}=\gamma_{2}$ the
condition is also satisfied since
\[
\underbrace{2\dfrac{1+\rho}{1-\rho}}_{>2}+\dfrac{\rho}{1-\rho}-\underbrace{\left(1+\alpha\right)}_{<2}>0
\]
%
\textbf{Generalizing for $m>1$}

We proved that
\[
\dfrac{\underline{K}^{\prime}\left(n,m\right)}{\Theta^{\prime}\left(n,m-1\right)}>\dfrac{\underline{K}\left(n,m\right)}{\Theta\left(n,m-1\right)}
\]
%
for $m=1$ (i.e. when there exists just only one $n-$oligopoly).
Note that, for higher $m$, the ratio $\underline{K}\left(n,m\right)/\Theta\left(n,m-1\right)$
should increase even faster. This happens for two reasons. First,
as an immediate inspection of (\ref{eq:theta_asymmetric}) reveals,
the denominator $\Theta\left(n,m-1\right)$ should increase slower
(or even decrease) with high $m$. This is because we have a lower
share of industries with $g^{\prime}\left(n-1\right)$ and higher
share of industries with $g^{\prime}\left(n\right)<g\left(n\right)$.

Second, the numerator $\underline{K}\left(n,m\right)$ must increase
faster when $m$ is large. Note that when we only have $m=1$ duopolies,
the remaining $I-1$ industries are monopolies. In these last industries,
the MPS generates higher productivity (as we are increasing $\gamma_{1}$).
However, as we move to $m=2$, the positive impact of the MPS becomes
weaker in aggregate terms (now we have one less monopoly than before).
In other words, the production possibility frontier of the economy
should increase more slowly with $m=2$, making it increasingly difficult
for $m=2$ industries to be $n-$oligopolies.

Therefore, the ratio 
\[
\dfrac{\underline{K}\left(n,m\right)}{\Theta\left(n,m-1\right)}
\]
%
must increase faster as we consider higher $m$.\\
\vspace{5pt}
\noindent\textbf{Generalizing for $n>2$}

Suppose we have a sequence of positive values
$
\varepsilon_{1}>\varepsilon_{2}>\varepsilon_{3}>\cdots
$,
such that 
$
\dfrac{\varepsilon_{1}}{\gamma_{1}}>\dfrac{\varepsilon_{2}}{\gamma_{2}}>\dfrac{\varepsilon_{3}}{\gamma_{3}}>\cdots
$
%
Suppose the MPS is such that for the first $n/2$ values we increase
productivity by %$\varepsilon_{1}>\varepsilon_{2}>\varepsilon_{3}>\cdots>\varepsilon_{n/2}$
while for the last $n/2$ values we apply a symmetric decrease (starting
by the last firm).
\[
\begin{array}{rl}
\gamma_{1}^{\prime}= & \gamma_{n}+\varepsilon_{1}\\
\gamma_{2}^{\prime}= & \gamma_{2}+\varepsilon_{2}\\
%\gamma_{3}^{\prime}= & \gamma_{3}+\varepsilon_{3}\\
\vdots & \vdots\\
%\gamma_{n-2}^{\prime}= & \gamma_{n-2}-\varepsilon_{3}\\
\gamma_{n-1}^{\prime}= & \gamma_{n-1}-\varepsilon_{2}\\
\gamma_{n}^{\prime}= & \gamma_{n}-\varepsilon_{1}
\end{array}
\]
Note that we have
%
\[
\begin{array}{rl}
 & \dfrac{g^{\prime}\left(n-1\right)}{g\left(n-1\right)}>\dfrac{g^{\prime}\left(n\right)}{g\left(n\right)}\\[3ex]
%\Leftrightarrow & \dfrac{\dfrac{\left(n-1\right)-\left(1-\rho\right)}{\sum\limits _{k=1}^{n-1}\dfrac{1}{\gamma_{k}+\varepsilon_{k}}}}{\dfrac{\left(n-1\right)-\left(1-\rho\right)}{\sum\limits _{k=1}^{n-1}\dfrac{1}{\gamma_{k}}}}>\dfrac{\dfrac{n-\left(1-\rho\right)}{\sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}+\varepsilon_{k}}}}{\dfrac{n-\left(1-\rho\right)}{\sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}}}}\\[8ex]
\Leftrightarrow & \dfrac{\sum\limits _{k=1}^{n-1}\dfrac{1}{\gamma_{k}}}{\sum\limits _{k=1}^{n-1}\dfrac{1}{\gamma_{k}+\varepsilon_{k}}}>\dfrac{\sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}}}{\sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}+\varepsilon_{k}}}\\[8ex]
%\Leftrightarrow & \left(\sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}}-\dfrac{1}{\gamma_{n}}\right)\left(\sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}+\varepsilon_{k}}\right)>\left(\sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}}\right)\left(\sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}+\varepsilon_{k}}-\dfrac{1}{\gamma_{n}+\varepsilon_{n}}\right)\\[4ex]
\Leftrightarrow & \left(-\dfrac{1}{\gamma_{n}}\right)\left(\sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}+\varepsilon_{k}}\right)>\left(\sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}}\right)\left(-\dfrac{1}{\gamma_{n}+\varepsilon_{n}}\right)\\[4ex]
%\Leftrightarrow & \left(\sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}}\right)\dfrac{1}{\gamma_{n}+\varepsilon_{n}}>\dfrac{1}{}\left(\sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}+\varepsilon_{k}}\right)\\[4ex]
\Leftrightarrow & \sum\limits _{k=1}^{n}\dfrac{\gamma_{n}}{\gamma_{k}}>\sum\limits _{k=1}^{n}\dfrac{\gamma_{n}+\varepsilon_{n}}{\gamma_{k}+\varepsilon_{k}}=\sum\limits _{k=1}^{n}\dfrac{\gamma_{n}^{\prime}}{\gamma_{k}^{\prime}}
\end{array}
\]
which must be satisfied if $\left\{ \gamma_{k}^{\prime}\right\} _{k=1}^{n}$
results from a MPS on $\left\{ \gamma_{k}\right\} _{k=1}^{n}$. Therefore,
the higher is $n$, the lower is the increase in $g\left(n-1\right)$
following an MPS on $\left\{ \gamma_{k}\right\} _{k=1}^{n}$. A corollary
of this fact is that $\Theta\left(n,m-1\right)$ should increase slower
(or even decrease) as we increase $n$.

Furthermore, $\underline{K}\left(n,m\right)$ should increase faster
as we increase $n$ (i.e. the economy can only accommodate $m$ oligopolies
with $n$ firms at higher $K$). Clearly, the higher is $n$, the
lower is the potential technological benefit associated with the MPS
on $\left(n-1\right)-$oligopolies. When we have $n=2$, the productivity
of the first firm increases by $\varepsilon_{1}>0$. However, for
$n>2$ the productivity of this firm increases by the same $\varepsilon_{1}>0$,
but this firm has a market share lower than one; the productivity
of the other firms increases by some $\varepsilon_{k}<\varepsilon_{1}$
(which can be even negative). Therefore, the potential positive impact
of the MPS is now lower than before and $\underline{K}\left(n,m\right)$
should increase faster.

Therefore, the ratio 
\[
\dfrac{\underline{K}\left(n,m\right)}{\Theta\left(n,m-1\right)}
\]

must increase faster as we consider higher $n$. This completes our
proof.


\end{proof}



==> input/proof_prop4_old.tex <==
\section{Proof of our main proposition}

\textbf{\textcolor{black}{1. Symmetric Region}}

When all industries are identical and have $n$ firms with productivities
$\gamma_{1}>\gamma_{2}>\cdots>\gamma_{n}$ we have
\[
\Theta\left(\mathbf{\Gamma},\mathbf{N}\right)=\Theta\left(n\right)=I^{\frac{1-\rho}{\rho}}\dfrac{n-\left(1-\rho\right)}{\sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}}}
\]
Since $f\left(\gamma\right)=1/\gamma$ is convex in $\gamma$, if
$\left\{ \gamma_{k}^{\prime}\right\} _{k=1}^{n}$ is a mean-preserving
spread of $\left\{ \gamma_{k}\right\} _{k=1}^{n}$ then 

\[
\begin{array}{rl}
 & \sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}^{\prime}}>\sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}}\\[2ex]
\Leftrightarrow & I^{\frac{1-\rho}{\rho}}\left(\dfrac{n-\left(1-\rho\right)}{\sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}^{\prime}}}\right)<I^{\frac{1-\rho}{\rho}}\left(\dfrac{n-\left(1-\rho\right)}{\sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}}}\right)\\[2ex]
\Leftrightarrow & \Theta^{\prime}\left(n\right)<\Theta\left(n\right)
\end{array}
\]

\textbf{2. Asymmetric Region}

Let us now analyze how $\Theta\left(\cdot\right)$ changes at the
unstable steady-state. The proof involves more steps in this region,
since we cannot obtain a closed-form expression for $\Theta\left(\cdot\right)$
when the equilibrium is not symmetric.

First note that when there are $m$ industries with $n$ firms ($n-$oligopolies)
and $I-m$ industries with $n-1$ firms ($\left(n-1\right)-$oligopolies),
we can write $\Theta\left(\cdot\right)$ as
\begin{equation}
\Theta\left(n,m\right)=\left\{ \left(I-m\right)g\left(n-1\right)^{\frac{\rho}{1-\rho}}+m\,g\left(n\right)^{\frac{\rho}{1-\rho}}\right\} ^{\frac{1-\rho}{\rho}}\label{eq:theta_asymmetric}
\end{equation}
where 
\[
g\left(n\right)\equiv\dfrac{n-\left(1-\rho\right)}{\sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}}}
\]

As we have proved above $g\left(n\right)$ always decreases following
a mean-preserving spread on $\left\{ \gamma_{k}\right\} _{k=1}^{n}$.
The difficulty in establishing a result in this case lies in two features
of the above expression for $\Theta\left(n,m\right)$. First we cannot
establish whether $g\left(n-1\right)$ increases or decreases after
a mean-preserving spread on all the $n$ firms. Second, $m$ is itself
an endogenous object and is likely to change after the mean-preserving
spread.

In this region, $\Theta\left(\cdot\right)$ is a step function, being
discontinuous at points
\[
\underline{K}\left(n,1\right),\underline{K}\left(n,2\right),\ldots,\underline{K}\left(n,I-1\right),\underline{K}\left(n,I\right)
\]
where $\underline{K}\left(n,m\right)$ is the level of aggregate capital
$K$ such that $n-$oligopolies exactly break-even when there are
$m$ of such $n-$oligopolies. This point is implicitly defined by
\[
\underbrace{\dfrac{1}{1-\rho}\left[1-\dfrac{n-\left(1-\rho\right)}{\sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}}}\dfrac{1}{\gamma_{j}}\right]^{2}\left[\dfrac{n-\left(1-\rho\right)}{\sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}}}\right]^{\frac{\rho}{1-\rho}}}_{\equiv\varLambda\left(j,n\right)}\Theta\left(n,m\right)^{-\frac{\rho}{1-\rho}}\underbrace{\Phi\left(n,m\right)\underline{K}\left(n,m\right)^{\alpha}L^{1-\alpha}}_{Y}-c_{f}=0
\]

This is illustrated in Figure \ref{fig:theta_proof}, where the blue
map shows $\Theta\left(\cdot\right)$ as a function of $K$ for an
initial combination of productivity values $\left\{ \gamma_{k}\right\} _{k=1}^{n}$.

\begin{figure}[H]
\begin{centering}
\includegraphics[scale=0.6]{theta_proof.eps}
\par\end{centering}
\caption{Factor Cost Index $\Theta$ (asymmetric region) \label{fig:theta_proof}}

\end{figure}

We want to show that, as we apply a mean-preserving spread, the new
map $\Theta^{\prime}$ is such that $\Theta^{\prime}<\Theta$ for
all $K$ with at least one $n-$oligopoly under $\left\{ \gamma_{k}^{\prime}\right\} _{k=1}^{n}$.
Let us take again a look at Figure \ref{fig:theta_proof}. First note
that, for all points below $\underline{K}\left(n,1\right)$, we have
$\Theta^{\prime}\left(n,0\right)>\Theta\left(n,0\right)$. From (\ref{eq:theta_asymmetric}),
this must be because $g^{\prime}\left(n-1\right)>g\left(n-1\right)$.
This indeed shows that, while it is always true that $g^{\prime}\left(n\right)<g\left(n\right)$
when we do a mean-preserving spread on the first $n$ firms, we can
however have $g^{\prime}\left(n-1\right)>g\left(n-1\right)$. So it
is not obvious in which direction $\Theta$, as defined in (\ref{eq:theta_asymmetric}),
will change.

Let us now analyze the interval $\left[\underline{K}\left(n,1\right),\underline{K}\left(n,2\right)\right)$.
In this interval, $\Theta$ takes value $\Theta\left(n,1\right)$
under $\left\{ \gamma_{k}\right\} _{k=1}^{n}$. However, under $\left\{ \gamma_{k}^{\prime}\right\} _{k=1}^{n}$,
the new value of $\Theta$ in this same interval is $\Theta^{\prime}\left(n,0\right)<\Theta\left(n,1\right)$.
This happens because the first $n-$oligopoly is only possible now
at 
\[
\underline{K}^{\prime}\left(n,1\right)>\underline{K}\left(n,2\right)
\]
In other words, while the economy could accommodate one $n-$oligopoly
at $\left[\underline{K}\left(n,1\right),\underline{K}\left(n,2\right)\right)$
with the resulting $\Theta\left(n,1\right)$, now it can only accommodate
$\left(n-1\right)-$oligopolies with the resulting $\Theta^{\prime}\left(n,0\right)<\Theta\left(n,1\right)$.

This happens because 

\[
\left.\dfrac{\underline{K}^{\prime}\left(n,m\right)}{\Theta^{\prime}\left(n,m-1\right)}\right|_{m=1}>\left.\dfrac{\underline{K}\left(n,m\right)}{\Theta\left(n,m-1\right)}\right|_{m=1}
\]

We will now prove that this must be always the case. We will show
this for the particular case $n=2$ and $m=1$ and then explain why
it must also hold for higher $m$ and $n$. 

\subsubsection*{Proof for $n=2$ and $m=1$ }

Note that we have
\[
\Theta(2,0)=\rho\gamma_{1}
\]
To obtain $\underline{K}\left(2,1\right)$ note that
\[
\begin{array}{rl}
 & c_{f}=\underbrace{\dfrac{1}{1-\rho}\left(1-\dfrac{1+\rho}{\dfrac{1}{\gamma_{2}}+\dfrac{1}{\gamma_{1}}}\dfrac{1}{\gamma_{2}}\right)^{2}\left(\dfrac{1+\rho}{\dfrac{1}{\gamma_{2}}+\dfrac{1}{\gamma_{1}}}\right)^{\frac{\rho}{1-\rho}}}_{\Lambda\left(2,2\right)}\Theta\left(1\right){}^{-\frac{\rho}{1-\rho}}\underbrace{\gamma_{1}\,\underline{K}\left(2,1\right)^{\alpha}}_{Y}\\
\Leftrightarrow & \underline{K}\left(2,1\right)^{\alpha}=c_{f}\left(1-\rho\right)\left(1-\dfrac{1+\rho}{1+\dfrac{\gamma_{2}}{\gamma_{1}}}\right)^{-2}\left(\dfrac{1+\rho}{\dfrac{1}{\gamma_{2}}+\dfrac{1}{\gamma_{1}}}\right)^{-\frac{\rho}{1-\rho}}\:\left(\rho\gamma_{1}\right){}^{\frac{\rho}{1-\rho}}\gamma_{1}^{-1}\\
\Leftrightarrow & \underline{K}\left(2,1\right)^{\alpha}=\left[c_{f}\left(1-\rho\right)\rho{}^{\frac{\rho}{1-\rho}}\left(1-\dfrac{1+\rho}{1+\dfrac{\gamma_{2}}{\gamma_{1}}}\right)^{-2}\left(\dfrac{1+\rho}{\dfrac{\gamma_{1}}{\gamma_{2}}+1}\right)^{-\frac{\rho}{1-\rho}}\:\gamma_{1}^{-1}\right]^{1/\alpha}
\end{array}
\]
When we do an MPS, we simply increase $\gamma_{1}$ holding $\gamma_{1}+\gamma_{2}$
fixed. Therefore, let
\[
\begin{array}{rl}
 & \gamma_{1}+\gamma_{2}=2x\\
\Leftrightarrow & \gamma_{2}=2x-\gamma_{1}
\end{array}
\]
Substituting in the previous equation we have
\[
\begin{array}{rl}
 & \underline{K}\left(2,1\right)=\left[c_{f}\left(1-\rho\right)\rho{}^{\frac{\rho}{1-\rho}}\left(1-\dfrac{1+\rho}{1+\dfrac{2x-\gamma_{1}}{\gamma_{1}}}\right)^{-2}\left(\dfrac{1+\rho}{\dfrac{\gamma_{1}}{2x-\gamma_{1}}+1}\right)^{-\frac{\rho}{1-\rho}}\:\gamma_{1}^{-1}\right]^{1/\alpha}\\
\Leftrightarrow & \underline{K}\left(2,1\right)=\left\{ c_{f}\left(1-\rho\right)\rho{}^{\frac{\rho}{1-\rho}}\left(1-\left(1+\rho\right)\dfrac{\gamma_{1}}{2x}\right)^{-2}\left[\left(1+\rho\right)\dfrac{2x-\gamma_{1}}{2x}\right]^{-\frac{\rho}{1-\rho}}\gamma_{1}^{-1}\right\} ^{1/\alpha}
\end{array}
\]
Therefore, we have 
\[
\begin{array}{rl}
\dfrac{\underline{K}\left(2,1\right)}{\Theta\left(2,0\right)}= & \left\{ c_{f}\left(1-\rho\right)\rho{}^{{\color{red}-\alpha}+\frac{\rho}{1-\rho}}\left(1-\left(1+\rho\right)\dfrac{\gamma_{1}}{2x}\right)^{-2}\left[\left(1+\rho\right)\dfrac{2x-\gamma_{1}}{2x}\right]^{-\frac{\rho}{1-\rho}}\gamma_{1}^{-1{\color{red}-\alpha}}\right\} ^{1/\alpha}\\
= & \left\{ c_{f}\left(1-\rho\right)\rho{}^{-\alpha+\frac{\rho}{1-\rho}}\left(1+\rho\right)^{-\frac{\rho}{1-\rho}}\left(1-\left(1+\rho\right)\dfrac{\gamma_{1}}{2x}\right)^{-2}\left[\dfrac{2x-\gamma_{1}}{2x}\gamma_{1}^{\left(1+\alpha\right)\frac{1-\rho}{\rho}}\right]^{-\frac{\rho}{1-\rho}}\right\} ^{1/\alpha}\\
= & \left\{ c_{f}\left(1-\rho\right)\rho{}^{-\alpha+\frac{\rho}{1-\rho}}\left(1+\rho\right)^{-\frac{\rho}{1-\rho}}\left(1-\left(1+\rho\right)\dfrac{\gamma_{1}}{2x}\right)^{-2}\left[\gamma_{1}^{\left(1+\alpha\right)\frac{1-\rho}{\rho}}-\dfrac{\gamma_{1}^{\left(1+\alpha\right)\frac{1-\rho}{\rho}+1}}{2x}\right]^{-\frac{\rho}{1-\rho}}\right\} ^{1/\alpha}
\end{array}
\]
Therefore, the term
\[
\underbrace{\left(1-\left(1+\rho\right)\dfrac{\gamma_{1}}{2x}\right)^{-2}}_{\left(1\right)}\underbrace{\left[\gamma_{1}^{\left(1+\alpha\right)\frac{1-\rho}{\rho}}-\dfrac{\gamma_{1}^{\left(1+\alpha\right)\frac{1-\rho}{\rho}+1}}{2x}\right]^{-\frac{\rho}{1-\rho}}}_{\left(2\right)}
\]
needs to be increasing in $\gamma_{1}$. The derivative of (1) is
\[
-2\left(1-\left(1+\rho\right)\dfrac{\gamma_{1}}{2x}\right)^{-2-1}\left(-\left(1+\rho\right)\dfrac{1}{2x}\right)
\]
and the derivative of (2) is
\[
\begin{array}{rl}
 & \left(-\dfrac{\rho}{1-\rho}\right)\left[\gamma_{1}^{\left(1+\alpha\right)\frac{1-\rho}{\rho}}-\dfrac{\gamma_{1}^{\left(1+\alpha\right)\frac{1-\rho}{\rho}+1}}{2x}\right]^{-\frac{\rho}{1-\rho}-1}\;\left\{ \left(1+\alpha\right)\frac{1-\rho}{\rho}\gamma_{1}^{\left(1+\alpha\right)\frac{1-\rho}{\rho}-1}-\left[\left(1+\alpha\right)\frac{1-\rho}{\rho}+1\right]\dfrac{\gamma_{1}^{\left(1+\alpha\right)\frac{1-\rho}{\rho}}}{2x}\right\} \\
= & \left(-\dfrac{\rho}{1-\rho}\right)\left[\gamma_{1}^{\left(1+\alpha\right)\frac{1-\rho}{\rho}}-\dfrac{\gamma_{1}^{\left(1+\alpha\right)\frac{1-\rho}{\rho}+1}}{2x}\right]^{-\frac{\rho}{1-\rho}-1}\;\gamma_{1}^{\left(1+\alpha\right)\frac{1-\rho}{\rho}}\left\{ \left(1+\alpha\right)\frac{1-\rho}{\rho}\left(\gamma_{1}^{-1}-\dfrac{1}{2x}\right)-\dfrac{1}{2x}\right\} 
\end{array}
\]
Hence, the derivative of the ratio increases in $\gamma_{1}$ if
\[
\begin{array}{rl}
 & -2\left(1-\left(1+\rho\right)\dfrac{\gamma_{1}}{2x}\right)^{-1}\left(-\left(1+\rho\right)\dfrac{1}{2x}\right)+\\
+ & \left(-\dfrac{\rho}{1-\rho}\right)\left[\gamma_{1}^{\left(1+\alpha\right)\frac{1-\rho}{\rho}}-\dfrac{\gamma_{1}^{\left(1+\alpha\right)\frac{1-\rho}{\rho}+1}}{2x}\right]^{-1}\;\gamma_{1}^{\left(1+\alpha\right)\frac{1-\rho}{\rho}}\left\{ \left(1+\alpha\right)\frac{1-\rho}{\rho}\left(\gamma_{1}^{-1}-\dfrac{1}{2x}\right)-\dfrac{1}{2x}\right\} >0\\
\Leftrightarrow & \left(1-\left(1+\rho\right)\dfrac{\gamma_{1}}{2x}\right)^{-1}\dfrac{1+\rho}{x}+\left[1-\dfrac{\gamma_{1}}{2x}\right]^{-1}\left\{ -\left(1+\alpha\right)\left(\gamma_{1}^{-1}-\dfrac{1}{2x}\right)+\dfrac{1}{2x}\dfrac{\rho}{1-\rho}\right\} >0\\
\Leftrightarrow & \dfrac{\dfrac{1+\rho}{x}}{1-\left(1+\rho\right)\dfrac{\gamma_{1}}{2x}}+\dfrac{\dfrac{1}{2x}\dfrac{\rho}{1-\rho}-\left(1+\alpha\right)\left(\gamma_{1}^{-1}-\dfrac{1}{2x}\right)}{1-\dfrac{\gamma_{1}}{2x}}>0\\
\Leftrightarrow & \dfrac{2\left(1+\rho\right)}{2x-\left(1+\rho\right)\gamma_{1}}+\dfrac{\dfrac{\rho}{1-\rho}-\left(1+\alpha\right)\left(\dfrac{2x}{\gamma_{1}}-1\right)}{2x-\gamma_{1}}>0\\
\Leftrightarrow & \dfrac{2\left(1+\rho\right)}{\left(\gamma_{1}+\gamma_{2}\right)-\left(1+\rho\right)\gamma_{1}}+\dfrac{\dfrac{\rho}{1-\rho}-\left(1+\alpha\right)\dfrac{\gamma_{2}}{\gamma_{1}}}{\gamma_{2}}>0\\
\Leftrightarrow & \dfrac{2\left(1+\rho\right)}{\gamma_{2}-\rho\gamma_{1}}+\dfrac{\dfrac{\rho}{1-\rho}-\left(1+\alpha\right)\dfrac{\gamma_{2}}{\gamma_{1}}}{\gamma_{2}}>0
\end{array}
\]
We need to have $\gamma_{2}>\rho\gamma_{1}$, for otherwise $\gamma_{2}$
has a negative market share. In the limit case of $\gamma_{2}=\rho\,\gamma_{1}$
the condition is always satisfied. When $\gamma_{1}=\gamma_{2}$ the
condition is also satisfied since
\[
\underbrace{2\dfrac{1+\rho}{1-\rho}}_{>2}+\dfrac{\rho}{1-\rho}-\underbrace{\left(1+\alpha\right)}_{<2}>0
\]


\subsubsection*{Generalizing for $m>1$}

We proved that
\[
\dfrac{\underline{K}^{\prime}\left(n,m\right)}{\Theta^{\prime}\left(n,m-1\right)}>\dfrac{\underline{K}\left(n,m\right)}{\Theta\left(n,m-1\right)}
\]

for $m=1$ (i.e. when there exists just only one $n-$oligopoly).
Note that, for higher $m$, the ratio $\underline{K}\left(n,m\right)/\Theta\left(n,m-1\right)$
should increase even faster. This happens for two reasons. First,
as an immediate inspection of (\ref{eq:theta_asymmetric}) reveals,
the denominator $\Theta\left(n,m-1\right)$ should increase slower
(or even decrease) with high $m$. This is because we have a lower
share of industries with $g^{\prime}\left(n-1\right)$ and higher
share of industries with $g^{\prime}\left(n\right)<g\left(n\right)$.

Second, the numerator $\underline{K}\left(n,m\right)$ must increase
faster when $m$ is large. Note that when we only have $m=1$ duopolies,
the remaining $I-1$ industries are monopolies. In these last industries,
the MPS generates higher productivity (as we are increasing $\gamma_{1}$).
However, as we move to $m=2$, the positive impact of the MPS becomes
weaker in aggregate terms (now we have one less monopoly than before).
In other words, the production possibility frontier of the economy
should increase more slowly with $m=2$, making it increasingly difficult
for $m=2$ industries to be $n-$oligopolies.

Therefore, the ratio 
\[
\dfrac{\underline{K}\left(n,m\right)}{\Theta\left(n,m-1\right)}
\]

must increase faster as we consider higher $m$.

\subsubsection*{Generalization for $n>2$}

Suppose we have a sequence of positive values
\[
\varepsilon_{1}>\varepsilon_{2}>\varepsilon_{3}>\cdots
\]
such that 
\[
\dfrac{\varepsilon_{1}}{\gamma_{1}}>\dfrac{\varepsilon_{2}}{\gamma_{2}}>\dfrac{\varepsilon_{3}}{\gamma_{3}}>\cdots
\]

Suppose the MPS is such that for the first $n/2$ values we increase
productivity by
\[
\varepsilon_{1}>\varepsilon_{2}>\varepsilon_{3}>\cdots>\varepsilon_{n/2}
\]
while for the last $n/2$ values we apply a symmetric decrease (starting
by the last firm).
\[
\begin{array}{rl}
\gamma_{1}^{\prime}= & \gamma_{n}+\varepsilon_{1}\\
\gamma_{2}^{\prime}= & \gamma_{2}+\varepsilon_{2}\\
\gamma_{3}^{\prime}= & \gamma_{3}+\varepsilon_{3}\\
\vdots & \vdots\\
\gamma_{n-2}^{\prime}= & \gamma_{n-2}-\varepsilon_{3}\\
\gamma_{n-1}^{\prime}= & \gamma_{n-1}-\varepsilon_{2}\\
\gamma_{n}^{\prime}= & \gamma_{n}-\varepsilon_{1}
\end{array}
\]
Note that we have

\[
\begin{array}{rl}
 & \dfrac{g^{\prime}\left(n-1\right)}{g\left(n-1\right)}>\dfrac{g^{\prime}\left(n\right)}{g\left(n\right)}\\[3ex]
\Leftrightarrow & \dfrac{\dfrac{\left(n-1\right)-\left(1-\rho\right)}{\sum\limits _{k=1}^{n-1}\dfrac{1}{\gamma_{k}+\varepsilon_{k}}}}{\dfrac{\left(n-1\right)-\left(1-\rho\right)}{\sum\limits _{k=1}^{n-1}\dfrac{1}{\gamma_{k}}}}>\dfrac{\dfrac{n-\left(1-\rho\right)}{\sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}+\varepsilon_{k}}}}{\dfrac{n-\left(1-\rho\right)}{\sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}}}}\\[8ex]
\Leftrightarrow & \dfrac{\sum\limits _{k=1}^{n-1}\dfrac{1}{\gamma_{k}}}{\sum\limits _{k=1}^{n-1}\dfrac{1}{\gamma_{k}+\varepsilon_{k}}}>\dfrac{\sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}}}{\sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}+\varepsilon_{k}}}\\[8ex]
\Leftrightarrow & \left(\sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}}-\dfrac{1}{\gamma_{n}}\right)\left(\sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}+\varepsilon_{k}}\right)>\left(\sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}}\right)\left(\sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}+\varepsilon_{k}}-\dfrac{1}{\gamma_{n}+\varepsilon_{n}}\right)\\[4ex]
\Leftrightarrow & \left(-\dfrac{1}{\gamma_{n}}\right)\left(\sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}+\varepsilon_{k}}\right)>\left(\sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}}\right)\left(-\dfrac{1}{\gamma_{n}+\varepsilon_{n}}\right)\\[4ex]
\Leftrightarrow & \left(\sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}}\right)\dfrac{1}{\gamma_{n}+\varepsilon_{n}}>\dfrac{1}{}\left(\sum\limits _{k=1}^{n}\dfrac{1}{\gamma_{k}+\varepsilon_{k}}\right)\\[4ex]
\Leftrightarrow & \sum\limits _{k=1}^{n}\dfrac{\gamma_{n}}{\gamma_{k}}>\sum\limits _{k=1}^{n}\dfrac{\gamma_{n}+\varepsilon_{n}}{\gamma_{k}+\varepsilon_{k}}=\sum\limits _{k=1}^{n}\dfrac{\gamma_{n}^{\prime}}{\gamma_{k}^{\prime}}
\end{array}
\]
which must be satisfied if $\left\{ \gamma_{k}^{\prime}\right\} _{k=1}^{n}$
results from a MPS on $\left\{ \gamma_{k}\right\} _{k=1}^{n}$. Therefore,
the higher is $n$, the lower is the increase in $g\left(n-1\right)$
following an MPS on $\left\{ \gamma_{k}\right\} _{k=1}^{n}$. A corollary
of this fact is that $\Theta\left(n,m-1\right)$ should increase slower
(or even decrease) as we increase $n$.

Furthermore, $\underline{K}\left(n,m\right)$ should increase faster
as we increase $n$ (i.e. the economy can only accommodate $m$ oligopolies
with $n$ firms at higher $K$). Clearly, the higher is $n$, the
lower is the potential technological benefit associated with the MPS
on $\left(n-1\right)-$oligopolies. When we have $n=2$, the productivity
of the first firm increases by $\varepsilon_{1}>0$. However, for
$n>2$ the productivity of this firm increases by the same $\varepsilon_{1}>0$,
but this firm has a market share lower than one; the productivity
of the other firms increases by some $\varepsilon_{k}<\varepsilon_{1}$
(which can be even negative). Therefore, the potential positive impact
of the MPS is now lower than before and $\underline{K}\left(n,m\right)$
should increase faster.

Therefore, the ratio 
\[
\dfrac{\underline{K}\left(n,m\right)}{\Theta\left(n,m-1\right)}
\]

must increase faster as we consider higher $n$. This completes our
proof.

\newpage

==> input/regression_model.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\hline\hline
&\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
&\multicolumn{1}{c}{$\Delta\log output$}&\multicolumn{1}{c}{$\Delta\log firms$}&\multicolumn{1}{c}{$\Delta\text{ labor share}$}\\
\hline
concentration & -0.0180\sym{***}&     -0.0369\sym{***}&     -0.0112\sym{***}\\
&   (0.00115)         &   (0.00237)         &  (0.000720)         \\
[1em]
$\log \text{firms}$ &      0.0139\sym{***}&      0.0284\sym{***}&     0.00864\sym{***}\\
                    &   (0.00103)         &   (0.00211)         &  (0.000641)         \\
[1em]
Constant            &      -0.122\sym{***}&     -0.0748\sym{***}&     -0.0228\sym{***}\\
                    &   (0.00285)         &   (0.00585)         &   (0.00178)         \\
\hline
Observations        &        9875         &        9875         &        9875         \\
\(R^{2}\)           &       0.115         &       0.115         &       0.115         \\
\hline\hline
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> old_versions/1_Introduction6.tex <==
\section{Introduction}

%1. Study how firm heterogeneity affects the likelihood, magnitude and persistence of recessions

A growing body of evidence suggests that the US economy has been undergoing decades of increasing heterogeneity between firms along several dimensions (size, productivity, and markups among others). In this paper we ask what is the effect of these secular trends on likelihood, magnitude and persistence of recessions.  


%2. RA economy with endogenous factor supply; multi-industry setup, endogenous entry and oligopolistic competition
     %\footnotesize complementarity between competition and factor supply can generate multiple SS}
     % {\footnotesize $\uparrow$ heterogeneity $\Rightarrow$ $\uparrow$ markups $\Rightarrow$ $\downarrow$ factor share $\Rightarrow$ $\downarrow$ capital demand $\Rightarrow$ high SS more fragile}

We study this question in the context of an RBC model with oligopolistic competition, endogenous entry and factor supply. At the heart of our model is a complementarity between competition and factor supply. First, economies with intense competition in product markets feature low profit shares and high factor shares and prices, which sustain high factor supply. Second, high factor supply allows more firms to enter the market, which results in greater competition. This complementarity can give rise to multiple stochastic steady-states. A key contribution of our theory is to show that rising firm heterogeneity can make transitions from high to low steady-states more likely to occur. When firm heterogeneity increases, large, productive firms expand while small, unproductive firms contract. As a consequence, smaller negative shocks can trigger firm exit and make the economy transition to steady-states with lower competition, capital stock and output.

% QUANTITATIVE RESULTS

To quantify these economic forces, we calibrate our model to match firm level moments in 2007 (on markups and fixed costs). To compare the 2007 economy to one with lower heterogeneity, we recalibrate the model to match the same data moments observed in 1985. We subject the two model economies to the same shocks and observe that the 2007 economy exhibits significantly larger amplification and propagation. Quantitatively, the 2007 economy is between 5 and 9 times more likely to experience a deep and prolonged recession, relative to the 1985 economy.

We also use our model economy to study the aftermath of the Great Recession. We feed a sequence of shocks calibrated to match the behavior of aggregate TFP in 2008/9. Our model generates the observed persistent deviation from trend of GDP as well as of investment, hours and aggregate TFP. It also explains the sharp drop of the labor share after 2008. Importantly, when we subject our 1985 economy with the same shocks, our model does not predict a persistent deviation from trend.

%% POLICY

In terms of the policy lesson of our theory, we ask whether we can design an effective policy to curb the endogenous amplification of aggregate shocks. We show that a budget balanced firm subsidy is very effective in preventing deep recessions, leading to a welfare gain of 21\% in consumption-equivalent terms.

%% EMPIRICS

We conclude by providing empirical evidence in favor of our proposed mechanism. In particular, our theory provides sharp predictions in terms of across industries responses to the business cycle. We show that, consistent with our model, industries that were more concentrated before the 2008 crisis experienced larger declines in net entry and economic activity.

==> old_versions/1_introduction.tex <==
\section{Introduction\label{sec:Introduction}}

The US economy appears to have experienced a fundamental change over the past four decades. Several studies and indicators have highlighted different secular trends concerning the structure of product markets, the distribution of income across factors and the distribution of activity across firms.
Some of the trends attracting prominent attention in the recent debate include i) the decline in the labor share; ii) the increase in the profit share; iii) the increase in aggregate markups and iv) the decline in the firm entry rate.\footnote{See for example \cite{ERW}, \cite{ABBKL} and \cite{AA1}.}

Although these trends are still the object of discussion in the literature, two aspects are starting to gain consensus. First, they seem to be driven by a change in the market structure, and in particular an increasing share of large firms, with high markups and low labor shares, in production.\footnote{See for example \cite{ADKPR} and \cite{KV} for evidence on the labor share and \cite{LEU} for evidence on  markups.}

Second, they have become especially pronounced in the aftermath of the last two recessions \textendash{} the 2001 crisis and, in particular, the great recession of 2008. For example, Figure \ref{fig:labor_profit_shares_figure} shows that both the decline in the labor share and the increase in the profit share experienced a persistent deviation from their pre-crisis trends after 2008. An identical deviation can be observed in the decline of the firm entry rate.\footnote{See Appendix \ref{subsec:Number-of-Firms}. This has been associated with a persistent decline in the number of active firms after 2008. See Appendix \ref{sec:numberfirms} for the sectoral breakdown of the number of firms trend.} The 2008 recession had, however, a broader impact on the macroeconomy, with real GDP and most macroeconomic aggregates also deviating from their pre-crisis trends \textendash{} the so called \textit{great deviation} (Figure \ref{fig:great_deviation_figure}).



These observations suggest that the trends in the list above can be the consequence of forces operating at different frequencies \textendash{} long-run forces that have driven a slow process of reallocation towards large firm (i.e. the trend between 1980-2007), and the persistent impact of the 2008 recession on the economy (i.e. the deviation from trend after 2008). In this paper, we investigate a natural, yet unexplored, connection between these two sets of observations. First, we ask whether a recession can have a persistent impact on the macroeconomy, capable of explaining the persistent deviations from trend in both Figures \ref{fig:labor_profit_shares_figure} and \ref{fig:great_deviation_figure}. Second, we ask whether the long-run process of reallocation towards large firms (taking place already before the crisis) may have contributed to the severity and persistence of the crisis itself.

Our theory builds on the neoclassical growth model, with a representative household and the standard accumulation of capital. We depart, however, from the canonical model by introducing an endogenous market structure. We model a multi-industry economy, with endogenous entry and oligopolistic competition as in \cite{AB}. Firms face fixed production costs and make their entry decisions based on their idiosyncratic productivity draws and the state of the economy. The endogenous number of players in every market, together with the distribution of productivities, determines the overall distribution of markups and market shares.

In this environment there is a complementarity between capital accumulation and competition. To understand the mechanism, suppose that the economy experiences an increase in its capital stock. Holding fixed the set of active firms, a more abundant capital stock results in larger output and profit levels. This means that more firms will be willing to enter, so that the economy will end up having a more competitive market structure \textendash{} more firms enter, and markups and profit shares decline. Importantly, profit levels can still be higher in spite of lower profit margins because of larger sales/output. A higher level of competition will in turn increase the incentives for capital accumulation. Lower markups favor a reallocation of income from profits to factors of production, thereby resulting in greater factor prices (wages and rental rates) and factor shares (labor and capital shares). This increases  the supply of labor and capital by the representative household.

Two main insights emerge from our theory. The first is that the complementarity between capital accumulation and competition explained above may give rise to multiple competition regimes or stochastic steady-states. In particular, there can be regimes featuring a large stock of capital, a large number of firms and hence intense competition (low profit shares and high factor shares); and regimes featuring a low stock of capital, a small number of firms and weak competition (\textit{low competition traps}).\footnote{The existence of multiple regimes or stochastic steady-states does not rely on the existence of multiple equilibria. In other words, our economy can feature multiple steady-states in spite of the existence of a unique equilibrium path. The steady-state the economy will reach depends on the initial condition and the history of aggregate shocks.} Large (temporary) shocks can trigger a transition across regimes. In particular, when an economy in a high competition regime is hit by a negative shock that significantly depresses capital accumulation, it can experience a persistent transition to a low competition regime. In such a case, the economy follows a path that, in many aspects, resembles the 2008 recession and subsequent \textit{great deviation} \textendash{} there is a persistent decline in the labor share, an increase in the profit share, as well as a persistent drop in the number of firms.

The second insight to emerge from our theory concerns the long-run process of reallocation towards large firms. We model this trend by considering a comparative static that fattens the right tail of the firm productivity distribution.\footnote{In our model, firm heterogeneity is driven by differences in idiosyncratic productivity. Other sources of heterogeneity (e.g. firm-specific demand shifters) would yield identical results.} This shift has two main consequences. First, from a static point of view, it generates a reallocation of activity towards large, high markup firms, which is able to explain the first three facts listed above. Second, as firm heterogeneity increases, firms at the bottom of the distribution lose market share and reduce their markups. This makes them increasingly likely to exit the market upon a negative aggregate shock. In other words, a high competition regime becomes increasingly difficult to sustain, so that even a relatively small temporary shock can trigger a persistent transition to a \textit{low competition trap}. Our model therefore suggests that larger firm differences may have increased the likelihood of a recession like the 2008 crisis, with output experiencing a persistent deviation from trend.


We calibrate our model to match first and second moments of the markup distribution of public firms in 2007. The economy features two competition regimes. We then ask whether the model can generate a transition like the one in Figure \ref{fig:great_deviation_figure}. We feed the economy with a sequence of negative TFP shocks (to replicate the behavior of aggregate TFP in 2008-2009) and show that they can trigger a transition from the high to the low regime. Quantitatively, the model replicates the persistent drop in output, employment, investment and aggregate TFP observed in the data. It also generates a persistent drop in the labor share.

Furthermore, to evaluate the role of larger market power, we recalibrate our model to match the same moments of the markup distribution in 1985, when markups were lower and less dispersed. We show that, relative to the 2007 model, the 1985 economy exhibits lower amplification and persistence. Furthermore, the size of the shock needed to trigger a transition from the high to the low regime is larger in the 1985 economy. We estimate that the 2007 economy is between 3 and 8 times more likely to experience a deep recession than the 1985 economy.\footnote{In particular, the sequence of negative TFP shocks that we feed in the 2007 economy is not sufficient to generate a transition from the high to the low regime in 1985.} Overall, these results indicate that the increase in average markups and in markup dispersion may have rendered the US economy more vulnerable to aggregate shocks.

Finally, we present cross-industry evidence on our mechanism. Our model predicts that, for any two industries with the same number of firms, the one with initially higher concentration should experience a larger drop in activity (output, employment, number of firms) as the economy enters a low competition trap. The intuition behind this testable implication is that, fixing the number of firms, a larger dispersion in market shares implies that smaller/least productive firms are closer to their break-even point, and hence more sensitive to aggregate shocks. We test this prediction using data from the US census and focusing again on the 2008 crisis. Consistent with the predictions of the model, we find that, conditional on the pre-crisis number of firms, industries featuring a larger concentration in 2007 experienced a greater cumulative contraction over the 2007-2016 period, as well as a larger drop in the labor share.

The rest of the paper is organized as follows. Section \ref{sec:Model} presents the model. Section \ref{sec:Quantitative-Evaluation} discusses the calibration and presents the quantitative results. Section \ref{sec:aggregatefacts} focuses on the US great recession and its aftermath. Section \ref{sec:empiricalevidence} presents the cross-industry empirical evidence. Section \ref{sec:Conclusion} concludes.



\paragraph{Related Literature}

Our paper is related to three different strands of the literature. In the first place, there is a large literature studying the aggregate consequences of imperfect competition and variable markups. We are not the first to show how multiple equilibria and/or multiple steady-states can arise in a context of imperfect competition (see for example \cite{CJ1}, \cite{MP}, \cite{CCR}, \cite{GZ}, \cite{J}). As in our theory, these models typically rely on a complementarity between firm entry decisions in a context of variable markups and elastic factor supply.\footnote{Without relying on multiple equilibria or multiple steady-states, \cite{CJ2}, \cite{EC} and \cite{BGM} show that a combination of imperfect competition with endogenous entry can generate endogenous amplification and persistence of aggregate fluctuations.} We contribute to this literature, however, by discussing the role of firm heterogeneity in generating multiplicity and shaping the response of the economy to aggregate shocks. We also provide a quantification of our mechanism and link it to the 2008 crisis.\footnote{Our paper is also linked to the literature studying the cyclical properties of markups, which includes \cite{RS}, \cite{JF}, \cite{BKM} and \cite{AVB}.}
Second, this paper relates to a large and growing literature documenting long-run trends in firm heterogeneity and market power. There are several signs indicating rising market power in the US and other advanced economies. For example, \cite{ADKPR} use data from the US census and document rising sales and employment concentration, while \cite{AA2} document a rise in patenting concentration. Other studies have documented a secular rise in price-cost markups. Using data from national accounts, \cite{H} finds that the average sectoral markup
increased from 1.12 in 1988 to 1.38 in 2015. \cite{LEU} document a steady increase in sales-weighted average markups for US public firms between 1980 and 2016.\footnote{\cite{EMX} show that a cost-weighted average markup (as opposed to sales-weighted) displays a less pronounced upward trend. They show that a cost-weighted average markup is the one that is relevant for welfare analysis, as it accounts for the fact that high markup firms are also more productive. See also \cite{T}, \cite{KN2} and \cite{BHKZ} for a critique on the \cite{LEU} methodology.} This was driven by both an increasing share of large firms and by rising dispersion in the markup distribution.\footnote{Identical findings are obtained by \cite{DFVS} and by \cite{CCM}, who use data from ORBIS (Bureau van Dijk) and include different countries in their analysis.} In our model, rising dispersion in size and markups is driven by increasing productivity differences. Several studies have indeed documented a secular increase in productivity differences across firms (\cite{ACG}, \cite{K}, \cite{DHJM2}). We contribute to this literature by investigating the business cycle implications of these trends, and in particular their impact on the 2008 crisis and the subsequent \textit{great deviation}.

Lastly, this paper relates to the literature focusing on the persistent impact of the 2008 crisis. \cite{ST} study a model with endogenous capacity utilization. Their model features a complementarity between firms' capacity utilization and aggregate output, which gives rise to multiple steady-states. Like us, they interpret the post-2008 deviation as a transition to a low steady-state. Other authors have proposed explanations based on the complementarity between firms' innovation decisions and aggregate output (\cite{BF}, \cite{ACGM}). 
Finally, \cite{CPW} argue that the persistent decline in firm entry, observed after 2008, is crucial to understand the slow recovery. We contribute to this literature by linking the \textit{great deviation} to the well documented long-run increase in firm level heterogeneity. We  propose a mechanism based on the interactions between market size and market structure that can jointly account for the macroeconomic and the industry level responses to the recession. In particular, our model can jointly match the post crisis behaviour of output, markups, the labor share and the number of active firms.



==> old_versions/1_introduction2.tex <==
\section{Introduction\label{sec:Introduction}}

The US economy appears to have experienced a fundamental change over the past four decades. Several studies and indicators have highlighted different secular trends concerning the structure of product markets, the distribution of income across factors and the distribution of activity across firms.
Some of the trends attracting prominent attention in the recent debate include i) the decline in the labor share; ii) the increase in the profit share; iii) the increase in aggregate markups and iv) the decline in the firm entry rate.\footnote{See for example \cite{ERW}, \cite{ABBKL} and \cite{AA1}.} Although these trends are still the object of discussion in the literature, two aspects are starting to gain consensus. First, they seem to be driven by a change in the market structure, and in particular an increasing share of large firms, with high markups and low labor shares, in production.\footnote{See for example \cite{ADKPR} and \cite{KV} for evidence on the labor share and \cite{LEU} for evidence on  markups.}

In this paper we take the growing body of evidence of increased firm-level heterogeneity and ask what are its macroeconomic effects. In particular we study if and how the the long run process of reallocation of activity from towards large firms has contributed to properties of the business cycle. 

To analyse the interaction between competition and the macroeconomy, we start from a general framework of an economy with endogenous TFP. As it is well known, endogenous TFP can give rise to steady state multiplicity. In this context we ask how changes in the technology set of the economy affect transitions between steady states. In particular we study the economy \textit{fragility}, which we define as the probability of transitions to lower steady states. In this model we provide a sufficient condition for a change in technology to increase fragility which depends on movements in the capital share, in the allocative efficiency and in the net entry of firms. When we apply this general reasoning to increases in firm level heterogeneity, we note that it can increase fragility if the efficiency gains coming from the best firms becoming more productive are outweighed by their increase in market power and subsequent reallocation of factor shares from factor suppliers to owners. This mechanism is reinforced by the role of net entry: as firm heterogeneity increases, firms at the bottom of the distribution will permanently exit, thereby further increasing incumbents' market power.

With the goal of providing sharper theoretical and quantitative predictions we specify our model further. In particular we embed endogenous entry and oligopolistic competition  \`a la \cite{AB} in an otherwise standard neoclassical growth model. We assume that the production side of the economy is composed by firms which are heterogeneous in productivity and pay a fixed production cost every period. 

In this environment arises a natural complementarity between competition and capital accumulation. In particular the return to capital, and therefore the amount supplied by households, depends on the degree of competition in the production side and consequently how large factor shares are. Secondly, when the return to capital is high, households capital supply is large which facilitates entry of new firms. This, in turn, generates competitive pressure and increases factor shares and factor prices. This complementarity can give rise to stochastic steady state multiplicity, which allows us to study endogenous amplification and persistence of exogenous shocks depending of the degree of firm heterogeneity. 

In this context fragility is defined as the likelihood that, after a temporary exogenous drop in aggregate TFP, the economy suffers net exit and an increase in incumbents' market power such that it converges to a permanently lower level of capital and competition, which we label a \textit{low competition trap}. We show that the fragility of the economy increases when we apply a mean-preserving spread to the distribution of firms productivity or when we increase the fixed cost of production.

We then proceed to quantify these economic forces by calibrating a quantitative version of our model. In particular, we calibrate the key parameters of the firms' productivity distribution and the fixed cost of production to match moments of the markup distribution in 2007. To compare the 2007 economy with one with lower firm heterogeneity we recalibrate the model to the same moments in 1985, when markups were lower and less dispersed. Subjecting the two model economies with the same shock we note that the 2007 economy exhibits significantly larger endogenous amplification and persistence. Furthermore, it is between 3 and 8 times more likely to experience a deep and prolonged recession, relative to the 1985 economy. From this we conclude that firm level heterogeneity has a significant quantitative impact on an economy's fragility.

We conclude the paper with three further set of findings. First, we use our model to study the aftermath of the Great Recession in 2007. We feed a sequence of aggregate shocks to mimic the observed aggregate TFP behavior of the US economy in 2007. Our model economy is then able to replicate both qualitatively and quantitatively the permanent deviation from trend of GDP (\textit{great deviation} and the behavior of investment and labor in the aftermath of the Great Recession. As a robustness check we ask if the same large shocks would generate such deep and prolonged recession in a less fragility economy. To this end, we apply the same shocks to the 1985 economy and observe no permanent deviation from trend. This is again suggestive evidence that the key reason for which we observe the economy falling into a low competition trap is indeed firm heterogeneity. 

As the role of firm heterogeneity is paramount in our setting, we ask whether we can design an effective policy to curb the endogenous amplification of aggregate shocks. We show quantitatively that a small subsidy to firms goes a long way in preventing deep recessions. The intuition is somewhat simple, when firms are subsidized they are less likely to exit for a given negative aggregate shock. As the net entry margin becomes responsive over the business cycle we do not observe large market power during recessions and high competition during booms which increase the amplitude of fluctuations. 

Lastly, we provide suggestive evidence that our proposed mechanism is at play in the US economy. Our model predicts a sharp relationship in the industry cross-section between pre-shock concentration and response to the shock itself. In particular we should observe that highly concentrated industries pre-2007 feature the largest net exit flows and therefore the largest compression of output as incumbents gain market power.  We test this prediction using data from the US census and focusing again on the 2008 crisis. Consistent with the predictions of the model, we find that, conditional on the pre-crisis number of firms, industries featuring a larger concentration in 2007 experienced a greater cumulative contraction over the 2007-2016 period, as well as a larger drop in the labor share.

The rest of the paper is organized as follows. Section \ref{sec: general framework text} sets the general framework and provides the first result relating technology and fragility. Section \ref{sec:Model} presents the neoclassical growth model with oligopolistic competition and derives the main theoretical results. Section \ref{sec:Quantitative-Evaluation} discusses the calibration and presents the quantitative results. Section \ref{sec:aggregatefacts} focuses on the US great recession and its aftermath. Section \ref{sec:empiricalevidence} presents the cross-industry empirical evidence. Section \ref{sec:Conclusion} concludes.


\paragraph{Related Literature}

Our paper is related to three different strands of the literature. In the first place, there is a large literature studying the aggregate consequences of imperfect competition and variable markups. We are not the first to show how multiple equilibria and/or multiple steady-states can arise in a context of imperfect competition (see for example \cite{CJ1}, \cite{MP}, \cite{CCR}, \cite{GZ}, \cite{J}). As in our theory, these models typically rely on a complementarity between firm entry decisions in a context of variable markups and elastic factor supply.\footnote{Without relying on multiple equilibria or multiple steady-states, \cite{CJ2}, \cite{EC} and \cite{BGM} show that a combination of imperfect competition with endogenous entry can generate endogenous amplification and persistence of aggregate fluctuations.} We contribute to this literature, however, by discussing the role of firm heterogeneity in generating multiplicity and shaping the response of the economy to aggregate shocks. We also provide a quantification of our mechanism and link it to the 2008 crisis.\footnote{Our paper is also linked to the literature studying the cyclical properties of markups, which includes \cite{RS}, \cite{JF}, \cite{BKM} and \cite{AVB}.}
Second, this paper relates to a large and growing literature documenting long-run trends in firm heterogeneity and market power. There are several signs indicating rising market power in the US and other advanced economies. For example, \cite{ADKPR} use data from the US census and document rising sales and employment concentration, while \cite{AA2} document a rise in patenting concentration. Other studies have documented a secular rise in price-cost markups. Using data from national accounts, \cite{H} finds that the average sectoral markup
increased from 1.12 in 1988 to 1.38 in 2015. \cite{LEU} document a steady increase in sales-weighted average markups for US public firms between 1980 and 2016.\footnote{\cite{EMX} show that a cost-weighted average markup (as opposed to sales-weighted) displays a less pronounced upward trend. They show that a cost-weighted average markup is the one that is relevant for welfare analysis, as it accounts for the fact that high markup firms are also more productive. See also \cite{T}, \cite{KN2} and \cite{BHKZ} for a critique on the \cite{LEU} methodology.} This was driven by both an increasing share of large firms and by rising dispersion in the markup distribution.\footnote{Identical findings are obtained by \cite{DFVS} and by \cite{CCM}, who use data from ORBIS (Bureau van Dijk) and include different countries in their analysis.} In our model, rising dispersion in size and markups is driven by increasing productivity differences. Several studies have indeed documented a secular increase in productivity differences across firms (\cite{ACG}, \cite{K}, \cite{DHJM2}). We contribute to this literature by investigating the business cycle implications of these trends, and in particular their impact on the 2008 crisis and the subsequent \textit{great deviation}.

Lastly, this paper relates to the literature focusing on the persistent impact of the 2008 crisis. \cite{ST} study a model with endogenous capacity utilization. Their model features a complementarity between firms' capacity utilization and aggregate output, which gives rise to multiple steady-states. Like us, they interpret the post-2008 deviation as a transition to a low steady-state. Other authors have proposed explanations based on the complementarity between firms' innovation decisions and aggregate output (\cite{BF}, \cite{ACGM}). 
Finally, \cite{CPW} argue that the persistent decline in firm entry, observed after 2008, is crucial to understand the slow recovery. We contribute to this literature by linking the \textit{great deviation} to the well documented long-run increase in firm level heterogeneity. We  propose a mechanism based on the interactions between market size and market structure that can jointly account for the macroeconomic and the industry level responses to the recession. In particular, our model can jointly match the post crisis behaviour of output, markups, the labor share and the number of active firms.

\textbf{ADD SOMETHING ON FRAGILITY}




==> old_versions/1_introduction3.tex <==
\section{Introduction}
The US economy appears to have experienced a significant change in the last few decades. Some of the trends receiving prominent attention in the literature include both micro-level and macro-level phenomena.

At the micro/industry level, several studies have indicated a process of long-run change in the market structure, with firms becoming increasingly heterogeneous along different dimensions (size, markups and productivity, among others).\footnote{See \cite{VR} for a summary of the recent findings.} For example, research has shown that large firms have become relatively larger (i.e. industry concentration has risen), while the markup distribution has also become more dispersed. These observations seem to explain the rise in aggregate markups and the decline in the aggregate labor share \citep{LEU,KV,ADKPR}.

At the macro level, the US economy experienced a noticeable change in the aftermath of the 2008 crisis, with most aggregates displaying a persistent shift from trend (Figure \ref{fig:great_deviation_figure}). For example, as of 2019, real output was 14\% below its pre-crisis trend. Such a large and persistent deviation has not been observed in previous recessions. Despite much interest and debate about this fact, we still lack a complete understanding of its causes. 

In this paper, we investigate a connection between these two sets of trends. We ask whether the ongoing changes at the micro/industry level can shed light on the deviation from trend observed after 2008. More precisely, we ask whether rising firm heterogeneity and market power has made the US economy more prone to quasi-permanent recessions, as in 2008.

To answer this question, we start by analysing a general economy featuring capital accumulation, variable markups and endogenous TFP, where multiple steady-states can occur. Within this model, we ask how changes in the technology set (e.g. the degree of firm heterogeneity) affect the likelihood of moving from a high to a low steady-state \textendash{} what we call \textit{macroeconomic fragility}. We provide a sufficient condition for a change in technology to increase fragility. This condition depends on the behavior of the capital share, allocative efficiency and the net entry margin. In particular, a technology change increases fragility if it leads to a reduction in the aggregate capital share or a reduction in allocative efficiency.

With the goal of sharpening our theoretical and quantitative predictions we specify our model further. In particular, we embed endogenous entry and oligopolistic competition  \`a la \cite{AB} in an otherwise standard neoclassical growth model with stochastic aggregate TFP. We assume that the production side of the economy is composed by firms which are heterogeneous in idiosyncratic productivity and pay a fixed production cost every period. This model features a complementarity between capital accumulation and competition. On the one hand, a larger capital stock allows more firms to break even, thus resulting in a more competitive market structure. On the other hand, more intense competition, by favoring a reallocation of income from profits to factors of production (capital and labor), increases the incentives for capital accumulation. This complementarity between capital accumulation and competition can give rise to (stochastic) steady-state multiplicity. There can be high steady-states characterized by intense competition (large number of firms, low markups and high factor shares), and low steady-state characterized by weak competition (small number of firms, high markups and low factor shares). 

We then ask how changes in the technology set affect the likelihood of moving from a high to a low steady-state. We consider two comparative statics: i) an increase in firm heterogeneity via a mean-preserving spread to the distribution of productivities; ii) an increase in fixed costs. We show that in both cases the economy becomes more likely to experience a transition from a high to a low steady-state. As productivities become more dispersed or fixed costs increase, small firms become closer to their break-even thresholds. This implies that smaller aggregate shocks can now trigger a significant amount of exit. The exit of these firms can generate the vicious cycle leading to a lower steady-state.

To quantify these economic forces, we calibrate our model to match moments of the distribution of markups and market shares in 2007.  The existence of multiple steady-states introduces strong non-linearities in the response to temporary aggregate shocks. Small shocks generate fluctuations around one particular steady-state, as in a standard RBC model. On the other hand, sufficiently large shocks can have much stronger and long-lasting effects, by triggering a transition across steady-states. 

To compare the 2007 economy with one with lower firm heterogeneity we recalibrate the model to match the same data moments observed in 1985. We subject the two model economies to the same shocks and observe that the 2007 economy exhibits significantly larger amplification and propagation. Quantitatively, the 2007 economy is between 3 and 8 times more likely to experience a deep and prolonged recession, relative to the 1985 economy. From this we conclude that firm level heterogeneity has a significant quantitative impact on an economy's fragility.

Next, we use our model to study the aftermath of the Great Recession. We feed a sequence of shocks calibrated to match the behavior of aggregate TFP in 2008/9. Our model is able to replicate the permanent deviation from trend of GDP (\textit{great deviation}) as well as the behavior of investment, hours and aggregate TFP. When applying the same shocks to the 1985 economy, we observe no permanent deviation from trend. We take this as further evidence of the importance of firm heterogeneity to understand the post-2008 growth experience.

Moreover, we provide empirical evidence on our model's mechanism. According to our model, as the economy transitions from a high to a low steady-state, the degree of competition should weaken. Consistent with our model's predictions, we document a persistent decline in the number of firms after 2008, a decline of the labor share (relative to trend) and an increase in the aggregate profit share (also relative to trend). We further show that this effect is particularly strong in more concentrated industries, as our theory predicts.

Lastly, we ask whether we can design an effective policy to curb the endogenous amplification of aggregate shocks. We show that a small budget balanced subsidy to firms goes a long way in preventing deep recessions. When firms are subsidized, they are less likely to exit for a given negative aggregate shock. This prevents competition from falling significantly in bad times, thus reducing the size and duration of recessions. Such a policy lesson is specific to our model and to the pivotal role of the extensive margin in shaping the amount of market power in the economy. Its logic, however, is more general and fundamentally suggests that the cyclicality of market power represents a source of endogenous amplification over the business cycle. Therefore, policies reducing the cyclical response of market power can curb part of the volatility of the economy.


\paragraph{Related Literature}

Our paper is related to three different strands of the literature. In the first place, there is a large literature studying the aggregate consequences of imperfect competition and variable markups. We are not the first to show how multiple equilibria and/or multiple steady-states can arise in a context of imperfect competition (see for example \cite{CJ1}, \cite{MP}, \cite{CCR}, \cite{GZ}, \cite{J}). As in our theory, these models typically rely on a complementarity between firm entry decisions in a context of variable markups and elastic factor supply.\footnote{Without relying on multiple equilibria or multiple steady-states, \cite{CJ2}, \cite{EC} and \cite{BGM} show that a combination of imperfect competition with endogenous entry can generate endogenous amplification and persistence of aggregate fluctuations.} We contribute to this literature, however, by discussing the role of firm heterogeneity in generating multiplicity and shaping the response of the economy to aggregate shocks. We also provide a quantification of our mechanism and link it to the 2008 crisis.\footnote{Our paper is also linked to the literature studying the cyclical properties of markups, which includes \cite{RS}, \cite{JF}, \cite{BKM} and \cite{AVB}.}
Second, this paper relates to a large and growing literature documenting long-run trends in firm heterogeneity and market power. There are several signs indicating rising market power in the US and other advanced economies. For example, \cite{ADKPR} use data from the US census and document rising sales and employment concentration, while \cite{AA2} document a rise in patenting concentration. Other studies have documented a secular rise in price-cost markups. Using data from national accounts, \cite{H} finds that the average sectoral markup
increased from 1.12 in 1988 to 1.38 in 2015. \cite{LEU} document a steady increase in sales-weighted average markups for US public firms between 1980 and 2016.\footnote{\cite{EMX} show that a cost-weighted average markup (as opposed to sales-weighted) displays a less pronounced upward trend. They show that a cost-weighted average markup is the one that is relevant for welfare analysis, as it accounts for the fact that high markup firms are also more productive. See also \cite{T}, \cite{KN2} and \cite{BHKZ} for a critique on the \cite{LEU} methodology.} This was driven by both an increasing share of large firms and by rising dispersion in the markup distribution.\footnote{Identical findings are obtained by \cite{DFVS} and by \cite{CCM}, who use data from ORBIS (Bureau van Dijk) and include different countries in their analysis.} In our model, rising dispersion in size and markups is driven by increasing productivity differences. Several studies have indeed documented a secular increase in productivity differences across firms (\cite{ACG}, \cite{K}, \cite{DHJM2}). We contribute to this literature by investigating the business cycle implications of these trends, and in particular their impact on the 2008 crisis and the subsequent \textit{great deviation}.

Lastly, this paper relates to the literature focusing on the persistent impact of the 2008 crisis. \cite{ST} study a model with endogenous capacity utilization. Their model features a complementarity between firms' capacity utilization and aggregate output, which gives rise to multiple steady-states. Like us, they interpret the post-2008 deviation as a transition to a low steady-state. Other authors have proposed explanations based on the complementarity between firms' innovation decisions and aggregate output (\cite{BF}, \cite{ACGM}). 
Finally, \cite{CPW} argue that the persistent decline in firm entry, observed after 2008, is crucial to understand the slow recovery. We contribute to this literature by linking the \textit{great deviation} to the well documented long-run increase in firm level heterogeneity. We  propose a mechanism based on the interactions between market size and market structure that can jointly account for the macroeconomic and the industry level responses to the recession. In particular, our model can jointly match the post crisis behaviour of output, markups, the labor share and the number of active firms.


The rest of the paper is organized as follows. Section \ref{sec: general framework text} sets the general framework and provides the first result relating technology and fragility. Section \ref{sec:Model} presents the neoclassical growth model with oligopolistic competition and derives the main theoretical results. Section \ref{sec:Quantitative-Evaluation} discusses the calibration and presents the quantitative results. Section \ref{sec:aggregatefacts} focuses on the US great recession and its aftermath. Section \ref{sec:empiricalevidence} presents the cross-industry empirical evidence. Section \ref{sec:Conclusion} concludes.

==> old_versions/1_introduction4.tex <==
\section{Introduction}
The recent US growth experience has been marked by a secular change in market structure and a deviation of output from trend in the aftermath of the 2008 recession. In this paper, we investigate a connection between these two facts. We ask whether the ongoing changes at the micro/industry level can shed light on the deviation from trend observed after 2008. More precisely, we ask whether rising firm heterogeneity and market power have made the US economy more prone to persistent deviations from trend (which we refer to as quasi-permanent recessions), as in 2008.

At the micro/industry level, several studies have highlighted a long-run change in the market structure, with firms becoming increasingly heterogeneous along different dimensions (size, markups and productivity, among others). For example, industry concentration has risen and the markup distribution has become more dispersed. These observations have been used to explain the rise in aggregate markups and the decline in the aggregate labor share.\footnote{See \cite{LEU,KV,ADKPR} and \cite{VR}.}

At the macro level, after the 2008 crisis, most US aggregates displayed a persistent shift from trend (Figure \ref{fig:great_deviation_figure}). For example, in 2019, real output was 14\% below its pre-crisis trend, a deviation far larger and persistent than in previous recessions. Despite much debate, we still lack a complete understanding of the causes of this fact. 

In this paper, we combine these observations and investigate whether rising firm heterogeneity may have a role in shaping the likelihood, magnitude and persistence of recessions. To study this relation, we start by analysing a general economy featuring variable markups, endogenous capital accumulation and TFP, where multiple steady-states can arise. The framework features an infinitely lived household with time separable preferences, such that the supply of capital is infinitely-elastic in the long-run and independent of the market structure. Changes in the market structure will, however, shape the aggregate demand for capital, which, in turn, affects the likelihood that a high or a low steady-state is reached.
%Due to the infinitely-elastic supply of capital, steady states are demand determined. The product market structure shapes firms' demand for capital which, in turn, affects the likelihood that a high or a low steady-state is reached.

%Changes in the product market structure affect firms' demand for capital and hence the likelihood that a high or a low steady-state is reached.
% The framework features a representative household and an infinite time horizon, which makes the supply of capital infinitely-elastic in the long-run \textendash{} and independent of the market structure. Changes in the product market structure can, however, affect firms' demand for capital and hence the likelihood that a given steady-state is reached. In particular, a reduction in the aggregate demand for capital can make a high steady-state more difficult to sustain \textendash{} thereby increasing \textit{macroeconomic fragility}. For example, larger firm heterogeneity, by resulting in a reallocation towards large firms and hence greater market power, can reduce firms' incentives to invest. This makes it more likely for the economy to experience a transition to a steady-state with low capital after a negative shock. In other words, quasi-permanent recessions become more likely to occur.
Within this model, we ask how changes in the technology set (for example, an increase the degree of heterogeneity in firms productivity) affect the likelihood of moving from a high to a low steady-state \textendash{} which we refer to as macroeconomic fragility. 
We provide a sufficient condition for a change in technology to increase fragility. In particular, a technology change increases fragility if it leads to a reduction in the demand for capital. This can be triggered by a decrease in the factor share or in allocative efficiency. For example, an increase in firm heterogeneity will trigger a direct decrease of the factor share as economic activity is reallocated from high to low factor share firms. This effect can be, however, attenuated by higher allocative efficiency. The increase in heterogeneity can generate reallocation towards the most productive firms, thereby increasing the economy average productivity. This strengthens aggregate demand for capital and can make the economy less prone to persistent recessions.
%We provide a sufficient condition for a change in technology to increase fragility. In particular, a technology change increases fragility if it leads to a reduction in the aggregate factor share or a reduction in allocative efficiency. Intuitively, a lower factor share or allocative efficiency indicate a decreased demand for capital and hence a higher likelihood that a low steady-state level of capital is reached.
%This can result directly from the change in the technology set or through changes in the level of competition. For example, an increase in firm heterogeneity will trigger a direct decrease of the factor share as economic activity is reallocated from high to low factor share firms. 
%Furthermore, if the increased heterogeneity triggers firm exit, it will further increase the most productive firms market power, thereby reducing the capital share even more.
%This effect can be, however, attenuated by higher allocative efficiency. The increase in heterogeneity can generate reallocation towards the most productive firms. This strengthens aggregate demand for capital and can make the economy less prone to persistent recessions.

%Maybe we should omit the previous discussion on allocative efficiency, or replace it by something like (perhaps in a footnote)
%\footnote{As discussed in Section \ref{sec: general framework text}, the decrease in the aggregate factor share not be enough to generate an increase in fragility. This is because the increase in heterogeneity can generate reallocation towards the most productive firms, thus resulting in higher allocative efficiency. This strengthens aggregate demand for capital and can make the economy less prone to persistent recessions.}

%Within this model, we ask how changes in the technology set (for example, the degree of firm heterogeneity) affect the likelihood of moving from a high to a low steady-state \textendash{} what we call \textit{macroeconomic fragility}. We provide a sufficient condition for a change in technology to increase fragility. This condition depends on the behavior capital demand,  capital share, allocative efficiency and the net entry margin. In particular, a technology change increases fragility if it leads to a reduction in the aggregate capital share or a reduction in allocative efficiency. This can result directly from the change in the technology set or through changes in the level of competition. For example, an increase in firm heterogeneity will trigger a direct decrease of the capital share as economic activity is reallocated from high to low capital share firms.
%Furthermore, if the increased heterogeneity triggers firm exit, it will further increase the most productive firms market power, thereby reducing the capital share even more. On the other hand, the increase in heterogeneity can generate reallocation towards more productive firms, which allows the economy to sustain a higher level of capital and therefore be less prone to persistent recessions.
With the goal of sharpening our theoretical and quantitative predictions, we embed endogenous entry and oligopolistic competition  \`a la \cite{AB} in an otherwise standard neoclassical growth model with stochastic aggregate TFP. The production side of the economy is composed by firms which are heterogeneous in idiosyncratic productivity and pay a fixed production cost every period. This model features a complementarity between capital accumulation and competition. First, a larger capital stock allows more firms to break even, thus resulting in a more competitive market structure. Second, more intense competition, by favoring a reallocation of income from profits to factors of production (capital and labor), increases the incentives for capital accumulation. This complementarity between capital accumulation and competition can give rise to (stochastic) steady-state multiplicity. There can be high steady-states characterized by intense competition (large number of firms, low markups and high factor shares), and low steady-states characterized by weak competition (small number of firms, high markups and low factor shares). 

We ask how changes in the technology set affect the likelihood of moving from a high to a low steady-state. We consider two comparative statics motivated by the empirical literature on recent US trends: i) an increase in firm heterogeneity via a mean-preserving spread to the distribution of productivity; ii) an increase in fixed costs. We show that in both cases the economy becomes more likely to experience a transition from a high to a low steady-state. As productivities become more dispersed or fixed costs increase, small firms come closer to their break-even thresholds. This implies that smaller aggregate shocks can now generate the exit of more firms. As firms exit, incumbents gain market power and further depress output. This, in turn, can generate the vicious cycle leading to a lower steady-state.

The existence of multiple steady-states introduces strong non-linearities in the response to temporary aggregate shocks. Small shocks generate fluctuations around one particular steady-state, as in a standard RBC model. On the other hand, sufficiently large shocks can have much stronger and long-lasting effects, by triggering a transition across steady-states. 

To quantify these economic forces, we calibrate our model to match data on markups and fixed costs in 2007. To compare the 2007 economy to one with lower market power we recalibrate the model to match the same data moments observed in 1985. We subject the two model economies to the same shocks and observe that the 2007 economy exhibits significantly larger amplification and propagation. Quantitatively, the 2007 economy is between 5 and 9 times more likely to experience a deep and prolonged recession, relative to the 1985 economy. From this we conclude that firm-level heterogeneity has a significant quantitative impact on macroeconomic fragility.

Next, we use our model economy to study the aftermath of the Great Recession. We feed a sequence of shocks calibrated to match the behavior of aggregate TFP in 2008/9. Our model generates the observed persistent deviation from trend of GDP as well as of investment, hours and aggregate TFP. When applying the same shocks to the 1985 economy, we observe no permanent deviation from trend. We take this as further evidence of the importance of firm heterogeneity to understand the post-2008 growth experience.

Moreover, we provide empirical evidence on our model's mechanism. According to our model, as the economy transitions from a high to a low steady-state, the degree of competition should weaken. Consistent with our model's predictions, we document a persistent decline in the number of firms after 2008, a decline of the labor share (relative to trend) and an increase in the aggregate profit share and markups (also relative to trend). Furthermore, we use industry-level data to show that this effect is particularly strong in more concentrated industries, as our theory predicts. In our model this is driven by small firms in concentrated industries being more likely to exit for a given negative shock.

Lastly, we ask whether we can design an effective policy to curb the endogenous amplification of aggregate shocks. We show that a budget balanced firm subsidy goes a long way in preventing deep recessions, leading to a welfare gain of 21\% in consumption-equivalent terms. When firms are subsidized, competition is less likely to fall significantly in bad times, thus reducing the size and duration of recessions. In our economy firms entry and exit decisions have external effects as they change market power. A planner may then find beneficial to trade off the efficiency loss attached to less productive firms staying in the market with the reduction in the rents of productive firms. This policy lesson is specific to our model and to the pivotal role of the extensive margin in shaping the amount of market power in the economy. Its logic, however, is more general. The cyclical response of market power is a source of endogenous amplification of aggregate fluctuations. %Policies that reduce this response can curb the volatility of the economy and be welfare-improving.
Policies keeping the degree of product market competition high can prevent the economy from entering in low output regimes and improve welfare.

\paragraph{Related Literature}

Our paper speaks to three different strands of the literature. First, it is related to the macroeconomic literature studying models of coordination failures \citep{CJ1,Mat,BenhabibFarmer,FarmerGuo,herrendorf2000ruling}. We are not the first to show how multiple equilibria and/or multiple steady-states can arise in a context of imperfect competition and variable markups \citep{MP,CCR,GZ,J}.\footnote{Without relying on multiple equilibria or multiple steady-states, \cite{CJ2}, \cite{EC} and \cite{BGM} show that a combination of imperfect competition with endogenous entry can generate endogenous amplification and persistence of aggregate fluctuations.} We add to this literature by discussing the role of firm-level heterogeneity in shaping macroeconomic \textit{fragility}; as we discuss, this concept is distinct from \textit{existence} of steady-state multiplicity. We also provide a quantification of our mechanism and link it to the 2008 crisis.\footnote{Our paper is also linked to the literature studying the cyclical properties of markups, which includes \cite{RS}, \cite{JF}, \cite{BKM}, \cite{nekarda2020cyclical} and \cite{AVB}.}

Second, this paper relates to a large and growing literature documenting long-run trends in firm heterogeneity and market power. There are several signs indicating rising market power in the US and other advanced economies. For example, \cite{ADKPR} use data from the US census and document rising sales and employment concentration, while \cite{AA2} document a rise in patenting concentration. Other studies have documented a secular rise in price-cost markups. Using data from national accounts, \cite{H} finds that the average sectoral markup
increased from 1.12 in 1988 to 1.38 in 2015. \cite{LEU} document a steady increase in sales-weighted average markups for US public firms between 1980 and 2016.\footnote{\cite{EMX} show that a cost-weighted average markup displays a less pronounced upward trend. They show that the cost-weighted average markup is the relevant metric for welfare analysis. See also \cite{GP}, \cite{T}, \cite{KN2} and \cite{BHKZ} on trends in markups.} This was driven by both an increasing share of large firms and by rising dispersion in the markup distribution.\footnote{Identical findings are obtained by \cite{CCM} and \cite{DFVS} for different countries.} In our model, rising dispersion in size and markups is driven by increasing productivity differences. Several studies have documented a secular increase in productivity differences across firms \citep{ACG,K,DHJM2}. Close to our approach, \cite{de2021quantifying} argue that declining dynamism and rising market power can be explained, among other channels, by increasing productivity dispersion and fixed costs. \cite{EMX} estimate that the welfare cost of markups can be large and represent up to a 25\% loss in consumption-equivalent terms.\footnote{\cite{EGB} builds a search model with heterogeneous firms to study the impact of rising productivity dispersion on the labor share.}
%Lastly, \cite{EMX} use a model close to ours to compute the welfare costs generate by markups via three main channels: i) output reduction, ii) misallocation, and iii) distorted entry.
We contribute to this literature by investigating the business cycle implications of these trends, and in particular their impact on the 2008 crisis and the subsequent \textit{great deviation}. We also highlight that increased firm heterogeneity and market power may have negative welfare consequences through an increase in macroeconomic fragility.

Lastly, this paper relates to the literature focusing on the persistent impact of the 2008 crisis. \cite{ST} study a model with endogenous capacity utilization %Their model features a complementarity between firms' capacity utilization and aggregate output, which gives rise to multiple steady-states. 
and, like us, they interpret the post-2008 deviation as a transition to a low steady-state. Other authors have proposed explanations based on the complementarity between firms' innovation decisions and aggregate output \citep{BF,ACGM}. 
Finally, \cite{CPW} argue that the persistent decline in firm entry, observed after 2008, is crucial to understand the slow recovery. We add to this literature by arguing that rising firm-level heterogeneity has increased the likelihood of quasi-permanent recessions. We also propose a mechanism based on the interactions between market size and market structure that can jointly match the post crisis behaviour of output, markups, the labor share and the number of active firms.

The rest of the paper is organized as follows. Section \ref{sec: general framework text} sets the general framework and provides the first result relating technology and fragility. Section \ref{sec:Model} presents the neoclassical growth model with oligopolistic competition and derives the main theoretical results. Section \ref{sec:Quantitative-Evaluation} discusses the calibration and presents the quantitative results. Section \ref{sec:aggregatefacts} focuses on the US great recession and its aftermath. In Section \ref{policy}, we study the welfare effects of fiscal policy in our model. Section \ref{sec:empiricalevidence} presents the cross-industry empirical evidence. Finally, section \ref{sec:Conclusion} concludes.

==> old_versions/1_introduction5.tex <==
\section{Introduction}
The US economy has experienced a fundamental change over the past four decades. At the micro/industry level, firms have become increasingly heterogeneous along different dimensions (productivity, size and markups) and market power appears to have increased.\footnote{For example, industry concentration has risen and the markup distribution has become more dispersed. These observations have been used to explain the rise in aggregate markups and the decline in the aggregate labor share. See \cite{LEU,KV,ADKPR} and \cite{VR}.} At the macro level, after the 2008 crisis, most US aggregates displayed a persistent shift from trend (Figure \ref{fig:great_deviation_figure}). For example, in 2019, real output was 14\% below its pre-crisis trend, a deviation far larger and persistent than in previous postwar recessions. Despite much debate, we still lack a complete understanding of the causes of this fact. 


%In this paper, we combine these observations and investigate whether rising firm heterogeneity and market power may have a role in shaping the magnitude and persistence of recessions. To tackle this question, we study an economy featuring oligopolistic competition, endogenous entry and factor supply. At the center of our model is a complementarity between competition and factor supply. First, a larger factor supply allows more firms to break even, thus resulting in a more competitive market structure. Second, more intense competition, by favoring a reallocation of income from profits to factors of production, increases the supply of capital and labor. Such a complementarity can give rise to multiple (stochastic) steady-states, which opens the possibility of persistent recessions.
%A key contribution of our theory is to show that rising firm heterogeneity can make transitions from high to low steady-states more likely to occur. An increase in firm heterogeneity, reallocates activity towards firms with high markups and low factor shares, can result in a decline in the aggregate demand for capital. This makes high capital regimes or steady-states more difficult to sustain. In other words, the economy becomes more likely to experience a persistent transition to a low capital regime in the aftermath of a negative shock.

In this paper we study these phenomena jointly and ask what is the effect of rising firm heterogeneity and market power on the magnitude and persistence of recessions. We address this question in an economy with oligopolistic competition, endogenous entry and factor supply. At the heart of our model is a complementarity between competition and factor supply. First, economies with intense competition in product markets feature low profit shares and high factor shares and prices, which sustain high factor supply. Second, high factor supply allows more firms to enter the market, which results in greater competition. This complementarity can give rise to multiple stochastic steady-states. A key contribution of our theory is to show that rising firm heterogeneity can make transitions from high to low steady-states more likely to occur. When firm heterogeneity increases, large, productive firms expand while small, unproductive firms contract. As a consequence, smaller negative shocks can trigger firm exit and make the economy transition to steady-states with lower competition, capital stock and output.

To quantify these economic forces, we calibrate our model to match firm level moments in 2007 (on markups and fixed costs). To compare the 2007 economy to one with lower heterogeneity and market power we recalibrate the model to match the same data moments observed in 1985. We subject the two model economies to the same shocks and observe that the 2007 economy exhibits significantly larger amplification and propagation. Quantitatively, the 2007 economy is between 5 and 9 times more likely to experience a deep and prolonged recession, relative to the 1985 economy.


We also use our model economy to study the aftermath of the Great Recession. We feed a sequence of shocks calibrated to match the behavior of aggregate TFP in 2008/9. Our model generates the observed persistent deviation from trend of GDP as well as of investment, hours and aggregate TFP. It also explains the sharp drop of the labor share after 2008, as well different cross-industry patterns that we document.

Lastly, we ask whether we can design an effective policy to curb the endogenous amplification of aggregate shocks. We show that a budget balanced firm subsidy is very effective in preventing deep recessions, leading to a welfare gain of 21\% in consumption-equivalent terms.





==> old_versions/1_introduction7.tex <==
\section{Introduction}

%1. Study how firm heterogeneity affects the likelihood, magnitude and persistence of recessions

A growing body of evidence suggests that the US economy has been undergoing decades of increasing heterogeneity between firms along several dimensions, such as size, productivity, and markups among others.\footnote{\cite{ACG} and \cite{VR} show that across firms productivity dispersion has increased. \cite{LEU,KV,ADKPR} have shown that industry concentration has risen and the markup distribution has become more dispersed. These observations have been used to explain the rise in aggregate markups and the decline in the aggregate labor share.} Theoretically, increases in heterogeneity generate two opposing forces: i) making the best firms more productive creates increases aggregate TFP; ii) the higher competitive advantage of larger and more productive firms can generate higher market power and rent extraction. In this paper we formalize how, depending on which of these forces prevails, economies are more or less responsive to aggregate shocks. In particular, we show that these secular trends in firm-level heterogeneity increase the likelihood, magnitude and persistence of recessions.


%In this paper we show that which of these forces prevails is the key determinant of how increasing firm heterogeneity affects the economy's response to aggregate shocks over the business cycle. %In particular, we ask what is the effect of these secular trends in firm-level heterogeneity on the likelihood, magnitude and persistence of recessions. 
%In particular, we show that these secular trends in firm-level heterogeneity increase the likelihood, magnitude and persistence of recessions.
%In this paper  


%2. RA economy with endogenous factor supply; multi-industry setup, endogenous entry and oligopolistic competition
     %\footnotesize complementarity between competition and factor supply can generate multiple SS}
     % {\footnotesize $\uparrow$ heterogeneity $\Rightarrow$ $\uparrow$ markups $\Rightarrow$ $\downarrow$ factor share $\Rightarrow$ $\downarrow$ capital demand $\Rightarrow$ high SS more fragile}

We study this problem in the context of an RBC model with oligopolistic competition, endogenous firm entry and factor supply. At the heart of our model is a complementarity between competition and factor supply. First, economies with intense competition in product markets feature low profit shares and high factor shares and prices, which sustain high factor supply. Second, high factor supply allows more firms to enter the market, which results in greater competition. This complementarity can give rise to multiple stochastic steady-states. A key contribution of our theory is to show that rising firm heterogeneity can make transitions from high to low steady-states more likely to occur (we refer to these transitions as quasi-permanent recessions). When firm heterogeneity increases, large, productive firms expand while small, unproductive firms contract. As a consequence, smaller negative shocks can trigger firm exit and make the economy transition to steady-states with lower competition, capital stock and output. We characterize this result formally by showing that the minimal size of negative shocks required to trigger a transition to a lower steady-state decreases when firm heterogeneity rises or when fixed costs of production increase. We refer to this as an increase in macroeconomic fragility.

% QUANTITATIVE RESULTS

To quantify these economic forces, we calibrate our model to match firm level moments in 2007 (on markups and fixed costs). To compare the 2007 economy to one with lower heterogeneity, we recalibrate the model to match the same data moments observed in 1985. We subject the two model economies to the same shocks and observe that the 2007 economy exhibits significantly larger amplification and propagation. Quantitatively, the 2007 economy is between 5 and 9 times more likely to experience a deep and prolonged recession, relative to the 1985 economy. We conclude that the 2007 economy was significantly more fragile to negative shocks than the 1985 economy.

We also use our model economy as a laboratory to study the Great Recession and its aftermath. We feed a sequence of shocks calibrated to match the behavior of aggregate TFP in 2008/9. Our model generates the observed deviations from trend of GDP, investment, hours and aggregate TFP. It also explains the sharp drop of the labor share after 2008. Importantly, when we subject our 1985 economy with the same shocks, our model does not predict a persistent deviation from trend.

%% POLICY

In terms of the policy lesson of our theory, %we ask whether we can design an effective policy to curb the endogenous amplification of aggregate shocks. 
we show that a budget balanced firm subsidy is very effective in preventing deep recessions, leading to a welfare gain of 21\% in consumption-equivalent terms. The fundamental intuition behind this result is that in our economy firms entry and exit decisions have external effects as they change market power. A
planner may then find beneficial to trade off the efficiency loss attached to less productive firms staying in the market with the reduction in the rents of productive firms. This policy lesson is specific to our model and to the pivotal role of the extensive margin in shaping the amount of market power in the economy. Its logic, however, is more general. The cyclical response of market power is a source of endogenous amplification of aggregate fluctuations. Policies keeping the degree of product market competition high can prevent the economy from entering in low output regimes and improve welfare.

%% EMPIRICS

We conclude by providing empirical evidence in favor of our proposed mechanism. In particular, our theory provides sharp predictions in terms of across industries responses to the business cycle. Our model suggests that industries with higher pre-shock levels of concentration are more responsive to the shock itself. We show that, consistent with our model, industries that were more concentrated before the 2008 crisis experienced larger declines  net entry,  the labor share and economic activity, proxied by in employment and payroll.










\paragraph{Related Literature}

Our paper speaks to three different strands of the literature. First, it is related to the macroeconomic literature studying models of coordination failures \citep{CJ1,Mat,BenhabibFarmer,FarmerGuo,herrendorf2000ruling}. We are not the first to show how multiple equilibria and/or multiple steady-states can arise in a context of imperfect competition and variable markups \citep{MP,CCR,GZ,J}.\footnote{Without relying on multiple equilibria or multiple steady-states, \cite{CJ2}, \cite{EC} and \cite{BGM} show that a combination of imperfect competition with endogenous entry can generate endogenous amplification and persistence of aggregate fluctuations.} We add to this literature by discussing the role of firm-level heterogeneity in shaping macroeconomic \textit{fragility}; as we discuss, this concept is distinct from \textit{existence} of steady-state multiplicity. We also provide a quantification of our mechanism and link it to the 2008 crisis.\footnote{Our paper is also linked to the literature studying the cyclical properties of markups, which includes \cite{RS}, \cite{JF}, \cite{BKM}, \cite{nekarda2020cyclical} and \cite{AVB}.}

Second, this paper relates to a large and growing literature documenting long-run trends in firm heterogeneity and market power. There are several signs indicating rising market power in the US and other advanced economies. For example, \cite{ADKPR} use data from the US census and document rising sales and employment concentration, while \cite{AA2} document a rise in patenting concentration. Other studies have documented a secular rise in price-cost markups. Using data from national accounts, \cite{H} finds that the average sectoral markup
increased from 1.12 in 1988 to 1.38 in 2015. \cite{LEU} document a steady increase in sales-weighted average markups for US public firms between 1980 and 2016.\footnote{\cite{EMX} show that a cost-weighted average markup displays a less pronounced upward trend. They show that the cost-weighted average markup is the relevant metric for welfare analysis. See also \cite{GP}, \cite{T}, \cite{KN2} and \cite{BHKZ} on trends in markups.} This was driven by both an increasing share of large firms and by rising dispersion in the markup distribution.\footnote{Identical findings are obtained by \cite{CCM} and \cite{DFVS} for different countries.} In our model, rising dispersion in size and markups is driven by increasing productivity differences. Several studies have documented a secular increase in productivity differences across firms \citep{ACG,K,DHJM2}. Close to our approach, \cite{de2021quantifying} argue that declining dynamism and rising market power can be explained, among other channels, by increasing productivity dispersion and fixed costs. \cite{EMX} estimate that the welfare cost of markups can be large and represent up to a 25\% loss in consumption-equivalent terms.\footnote{\cite{EGB} builds a search model with heterogeneous firms to study the impact of rising productivity dispersion on the labor share.}
%Lastly, \cite{EMX} use a model close to ours to compute the welfare costs generate by markups via three main channels: i) output reduction, ii) misallocation, and iii) distorted entry.
We contribute to this literature by investigating the business cycle implications of these trends, and in particular their impact on the 2008 crisis and the subsequent \textit{great deviation}. We also highlight that increased firm heterogeneity and market power may have negative welfare consequences through an increase in macroeconomic fragility.

Lastly, this paper relates to the literature focusing on the persistent impact of the 2008 crisis. \cite{ST} study a model with endogenous capacity utilization %Their model features a complementarity between firms' capacity utilization and aggregate output, which gives rise to multiple steady-states. 
and, like us, they interpret the post-2008 deviation as a transition to a low steady-state. Other authors have proposed explanations based on the complementarity between firms' innovation decisions and aggregate output \citep{BF,ACGM}. 
Finally, \cite{CPW} argue that the persistent decline in firm entry, observed after 2008, is crucial to understand the slow recovery. We add to this literature by arguing that rising firm-level heterogeneity has increased the likelihood of quasi-permanent recessions. We also propose a mechanism based on the interactions between market size and market structure that can jointly match the post crisis behaviour of output, markups, the labor share and the number of active firms.

The rest of the paper is organized as follows. Section \ref{sec: general framework text} sets the general framework and provides the first result relating technology and fragility. Section \ref{sec:Model} presents the neoclassical growth model with oligopolistic competition and derives the main theoretical results. Section \ref{sec:Quantitative-Evaluation} discusses the calibration and presents the quantitative results. Section \ref{sec:aggregatefacts} focuses on the US great recession and its aftermath. In Section \ref{policy}, we study the welfare effects of fiscal policy in our model. Section \ref{sec:empiricalevidence} presents the cross-industry empirical evidence. Finally, section \ref{sec:Conclusion} concludes.

==> old_versions/1_introduction8.tex <==
\section{Introduction}

%1. Study how firm heterogeneity affects the likelihood, magnitude and persistence of recessions

A growing body of evidence suggests that the US and other advanced economies have been undergoing decades of increasing firm-level heterogeneity along several dimensions, such as productivity, size and markups.\footnote{Several studies have documented rising firm differences in terms of i) revenue TFP \citep{ACG,K, DHJM2}, ii) size \citep{BCG, ADKPR}, and iii) markups \citep{LEU,CCM,DLT}. 
%These observations have been used to explain the rise in aggregate markups and the decline in the labor share. 
See \cite{VR} for a summary of the recent findings.}
From a theoretical point of view, increases in firm heterogeneity can generate opposing forces. On the one hand, making the best firms more productive can result in higher aggregate TFP and output. On the other hand, the higher competitive advantage of larger and more productive firms can generate higher market power and rent extraction. This \textit{static} cost may result in lower output and welfare. In this paper, we highlight a different threat posed by rising firm heterogeneity, which is linked to the dynamics of business cycles. In particular, we show that rising firm heterogeneity can result in a higher probability of deep and long-lasting recessions. We refer to such a probability as \textit{macroeconomic fragility}.


%In this paper we show that which of these forces prevails is the key determinant of how increasing firm heterogeneity affects the economy's response to aggregate shocks over the business cycle. %In particular, we ask what is the effect of these secular trends in firm-level heterogeneity on the likelihood, magnitude and persistence of recessions. 
%In particular, we show that these secular trends in firm-level heterogeneity increase the likelihood, magnitude and persistence of recessions.
%In this paper  


%2. RA economy with endogenous factor supply; multi-industry setup, endogenous entry and oligopolistic competition
     %\footnotesize complementarity between competition and factor supply can generate multiple SS}
     % {\footnotesize $\uparrow$ heterogeneity $\Rightarrow$ $\uparrow$ markups $\Rightarrow$ $\downarrow$ factor share $\Rightarrow$ $\downarrow$ capital demand $\Rightarrow$ high SS more fragile}

We study an RBC model with oligopolistic competition, endogenous firm entry and factor supply. At the heart of our model is a complementarity between competition and factor supply. First, economies with intense competition in product markets feature low profit shares and high factor shares and factor prices, which induce high factor supply. Second, high factor supply allows more firms to enter the market, which results in greater competition. This complementarity can give rise to multiple competition regimes or (stochastic) steady-states. A key contribution of our theory is to show that rising heterogeneity in idiosyncratic TFP can make transitions from high to low steady-states more likely to occur. When firm heterogeneity increases, large, productive firms expand while small, unproductive firms contract. As a consequence, smaller negative shocks can be enough to trigger firm exit and a transition to a steady-state featuring lower competition, capital and output. An identical result is obtained when fixed costs of production increase. We characterize these results formally by showing that the minimum size (negative) shock required to trigger a transition from a high to a low steady-state decreases when firm TFP heterogeneity rises or when fixed costs increase.

% QUANTITATIVE RESULTS

To quantify these economic forces, we provide three calibrations of our model, where we target US firm-level moments in 1975, 1990 and 2007. These different calibrated models differ in the level of fixed costs and in the degree of TFP dispersion (which both increase over time). We first find that, while the 1975 economy is characterized by a unimodal ergodic distribution of output, the 1990 and 2007 feature bimodal distributions (an indication of two stochastic steady-states). Second, when we subject the three model economies to the same shocks, we observe that the 2007 economy exhibits significantly greater amplification and propagation. For example, we find that the 2007 economy experiences a recession greater than 10\% every 75 years, while the 1990 and 1975 economies experiences one every 120 and 735 years respectively. This suggests that rising firm heterogeneity and fixed costs made the US economy significantly more fragile and more prone to long-lasting recessions.

We also use our model economy as a laboratory to study the Great Recession and its aftermath. The 2008 crisis was marked by a large and persistent deviation of output and other aggregates from trend, something unusual in the entire postwar period. For example, in 2019, output per capita was 14\% below its pre\textendash2007 trend, a deviation far larger and persistent than in previous recessions (Figure \ref{fig:great_deviation_figure}). We ask whether our model can replicate such a quasi-permanent drop in aggregate output and other aggregate variables. To this end, we feed our 2007 economy a sequence of shocks calibrated to match the behavior of aggregate TFP in 2008\textendash9 and study the economy's response. The model generates the observed persistent deviation from trend of GDP as well as of investment, hours and aggregate TFP. It also explains the sharp and persistent drop of the labor share after 2008. Importantly, when we subject the 1990 and 1975 economies to the same shocks, the model does not predict such a persistent deviation from trend. %This suggests that rising firm heterogeneity has rendered the US economy more vulnerable to quasi-permanent recessions as in 2008.


%% EMPIRICS

We also provide empirical evidence in favor of our proposed mechanism. Our theory provides predictions in terms of cross-industry responses to the business cycle. In particular, for any two industries with the same number of firms, the one with a higher level of heterogeneity reacts more to a negative shock. We test this prediction in the data using concentration as a proxy for heterogeneity in US 6-digit industries. Consistent with our model predictions, we show that industries that were more concentrated in 2007 experienced greater cumulative declines in the number of firms, the labor share and economic activity over the 2008-2016 period.

%% POLICY

In terms of policy lessons from our theory, %we ask whether we can design an effective policy to curb the endogenous amplification of aggregate shocks. 
we show that firm subsidies can be effective in preventing deep recessions, leading to a welfare gain of up to 21\% in consumption-equivalent terms. The fundamental intuition behind this result is that in our economy firms' entry and exit decisions have externalities as they change market power. A planner may then find it beneficial to trade off the efficiency loss attached to less productive firms staying in the market with the reduction in the rents of more productive firms. This policy lesson is specific to our model and to the pivotal role of the extensive margin in shaping the degree of aggregate market power. Its logic, however, is more general. Cyclical changes in market power can amplify aggregate fluctuations. Policies that aim to keep the degree of product market competition high can prevent the economy from entering into low output regimes and thereby improve welfare.



\paragraph{Related Literature}

Our paper speaks to three different strands of the literature. First, it is related to the macroeconomic literature studying models of coordination failures \citep{CJ1,Mat,BenhabibFarmer,FarmerGuo,herrendorf2000ruling}. While we are not the first to show how multiple equilibria and/or steady-states can arise in a context of imperfect competition and variable markups \citep{MP,CCR,RW,GZ,J},\footnote{Without relying on multiple equilibria or steady-states, \cite{CJ2}, \cite{EC} and \cite{BGM} show that a combination of imperfect competition with endogenous entry amplifies aggregate fluctuations.} we contribute to this literature by studying the role of firm-level heterogeneity in shaping macroeconomic \textit{fragility}. As we discuss, this concept is distinct from the \textit{existence} of steady-state multiplicity. We also provide a quantification of our mechanism and link it to the 2008 crisis.\footnote{Our paper speaks to the literature on the cyclicality of markups, which includes \cite{RS}, \cite{rotemberg1991markups}, \cite{JF}, \cite{BKM}, \cite{nekarda2020cyclical} and \cite{AVB}.}

Second, this paper relates to a large and growing literature documenting long-term trends in firm heterogeneity and market power. There are several signs that indicate rising market power in the US and other advanced economies. For example, \cite{ADKPR} use data from the US census to document rising sales and employment concentration, while \cite{AA2} document a rise in patenting concentration. Other studies have documented a secular rise in price-cost markups. Using data from national accounts, \cite{H} finds that the average sectoral markup
increased from 1.12 in 1988 to 1.38 in 2015. \cite{LEU} document a steady increase in sales-weighted average markups for US public firms between 1980 and 2016.\footnote{\cite{EMX} show that a cost-weighted average markup displays a less pronounced upward trend. See also \cite{GP}, \cite{T}, \cite{KN2} and \cite{BHKZ} on trends in markups.} This was driven by both an increasing share of large firms and by rising dispersion in the markup distribution.
%\footnote{Identical findings are obtained by \cite{CCM} and \cite{DFVS} for different countries.} 
%In our model, rising dispersion in size and markups is driven by increasing productivity differences. Several studies have documented a secular increase in productivity differences across firms \citep{ACG,K,DHJM2}. 
Close to our approach, \cite{de2021quantifying} argue that declining dynamism and rising market power can be explained, among other channels, by increasing productivity dispersion and fixed costs. \cite{EMX} estimate that the welfare cost of markups can be large and represent a loss of up to 25\% in consumption-equivalent terms.%\footnote{\cite{EGB} builds a search model with heterogeneous firms to study the impact of rising productivity dispersion on the labor share.}
%Lastly, \cite{EMX} use a model close to ours to compute the welfare costs generate by markups via three main channels: i) output reduction, ii) misallocation, and iii) distorted entry.
We contribute to this literature by investigating the business cycle implications of these trends, and in particular their impact on the 2008 crisis and the subsequent \textit{great deviation}. We emphasize that increased firm heterogeneity and market power may have negative welfare consequences through an increase in macroeconomic fragility.

Lastly, this paper relates to the literature studying the persistent impact of the 2008 crisis. A large part of this literature has focused on the secular decline in interest rates and/or the possibility of liquidity traps, which constrains monetary policy \citep{BF,guerrieri_lorenzoni,eggertsson_et_al,mian_sufi_straub}, or endogenous R\&D as in \cite{fasil2021heterogeneous}. Close to this paper, \cite{ST} build an RBC with endogenous capacity utilization
and, as we do, they interpret the post\textendash{}2008 deviation as a transition to a low steady-state. We complement this literature by arguing that rising firm-level heterogeneity has increased the likelihood of quasi-permanent recessions. Our theory can also account for number of trends observed after 2008, related to the behavior of markups, the labor share, concentration and the number of firms.

The rest of the paper is organized as follows. Section \ref{sec: general framework text} sets the general framework and provides the first result relating to technology and fragility. Section \ref{sec:Model} presents a growth model with oligopolistic competition and derives the main theoretical results. Section \ref{sec:Quantitative-Evaluation} discusses the calibration and presents the quantitative results. Section \ref{sec:aggregatefacts} provides and extended application to the US great recession and its aftermath, and presents the cross-industry empirical evidence. In Section \ref{policy}, we study the welfare effects of fiscal policy in our model. Finally, section \ref{sec:Conclusion} concludes.

==> old_versions/1_introduction9.tex <==
\section{Introduction}

%1. Study how firm heterogeneity affects the likelihood, magnitude and persistence of recessions
The US economy appears to be recovering more slowly from its recessions. The left panel of Figure \ref{intro_figure} shows, for different recessions, the change in detrended output in the first two years after the trough. While in the first postwar recessions output recovered relatively quickly, this pace has significantly slowed down in the last decades. Indeed, considering the last three recessions, output grew below its trend in the first two years after the trough. This last observation is further illustrated in the right panel of Figure \ref{intro_figure}, which shows the evolution of detrended output for these three recessions (1990-1991, 2001 and 2008-2009). Four years since the beginning of each recession, detrended output was still below its pre-crisis value. Considering the 2008-2009 crisis, the gap is substantial (about 10 log points below trend) and, in fact, did never close or reduce. This has been called the \textit{long slump} or \textit{great deviation} \citep{H_slump}.
\begin{figure}[H]
\centering{}%
\begin{tabular}{ccc}
     \hspace{-1cm} \includegraphics*[scale=0.5]{input/US_postwar_recoveries} &
     \hspace{0.25cm}
     \includegraphics*[scale=0.5]{input/US_last_3_recessions}
\end{tabular}
\caption{Motivating Facts: Recovery from US Recessions\protect \\ {Note: \small{}\small{} The left panel shows, for each US postwar recession, the change in detrended output in the first two years after the trough. We use quarterly real GDP per capita (in logs, from BEA) and compute a linear trend for the period 1947-2019. We consider all recessions that the lasted longer than 6 months according to the NBER. The right panel shows the evolution of detrended output for the last 1990-1991, 2001 and 2008-2009 recessions.}} 
\label{intro_figure}
\end{figure}

In this paper, we argue that the slowdown in the pace of US recoveries can be partially explained by changes in the supply side of the US economy and in its product market structure \textendash{} namely, the fact that firms have become increasingly heterogeneous and large firms have gained market power. A growing body of evidence suggests that the US and other advanced economies have been undergoing decades of increasing firm-level heterogeneity along several dimensions, such as productivity, size and markups.\footnote{Several studies have documented rising firm differences in terms of i) revenue TFP \citep{ACG,K, DHJM2}, ii) size \citep{BCG, ADKPR}, and iii) markups \citep{LEU,CCM,DLT}. See \cite{VR} for a summary of the recent findings.} To give an illustration of these trends, Figure \ref{intro_figure_2} shows the evolution of the standard deviation of sales for US public firms. The figure focuses on listed firms, but increasing firm-level dispersion has been documented using census data, and focusing on narrowly defined industries.\footnote{See \cite{K} on TFP differences and \cite{ADKPR} on size/concentration.} The central message of this paper is to show that rising firm heterogeneity can have a significant impact on business cycle fluctuations, and in particular result in a higher probability of long slumps. We refer to such a probability as \textit{macroeconomic fragility}. These trends, we find, are quantitatively important, and can rationalize episodes such as the 2008-2009 recession and its aftermath.

\begin{figure}[H]
\centering{}%
\includegraphics*[scale=0.75]{input/std_log_ms_1960}
\caption{Motivating Facts: Dispersion in Sales for US Public Firms\protect \\ {Note: \small{}\small{} The figure shows the standard deviation of log sales for US public firms. Data is from COMPUSTAT.}} 
\label{intro_figure_2}
\end{figure}


%A growing body of evidence suggests that the US and other advanced economies have been undergoing decades of increasing firm-level heterogeneity along several dimensions, such as productivity, size and markups as shown in Figure \ref{intro_figure}.\footnote{Several studies have documented rising firm differences in terms of i) revenue TFP \citep{ACG,K, DHJM2}, ii) size \citep{BCG, ADKPR}, and iii) markups \citep{LEU,CCM,DLT}.  See \cite{VR} for a summary of the recent findings.} A seemingly unrelated observation is that over the last century the length and depth of recessions has been growing, as evidenced by Figure \ref{intro_figure}. In this paper we argue that the rise in firm heterogeneity can potentially explain the increasing occurrence of slow recoveries. We show that, beyond the well understood static effects, these trends can significantly alter the dynamic behavior of an economy. In particular, we show that rising firm heterogeneity can result in a higher probability of deep and long-lasting recessions. We refer to such a probability as \textit{macroeconomic fragility}. These effects, we find, are quantitatively important and can can rationalize the increasing occurrence of slow recoveries.  


We study an RBC model with oligopolistic competition, endogenous firm entry and factor supply. At the heart of our model is a complementarity between competition and factor supply. First, economies with intense competition in product markets feature low profit shares and high factor shares and factor prices, which induce high factor supply. Second, high factor supply allows more firms to enter the market, which results in greater competition. This complementarity can give rise to multiple competition regimes or (stochastic) steady-states. A key contribution of our theory is to show that rising heterogeneity in idiosyncratic TFP can make transitions from high to low steady-states more likely to occur. When firm heterogeneity increases, large, productive firms expand while small, unproductive firms contract. As a consequence, smaller negative shocks can be enough to trigger firm exit and a transition to a steady-state featuring lower competition, capital and output. An identical result is obtained when fixed costs of production increase. We characterize these results formally by showing that the minimum size (negative) shock required to trigger a transition from a high to a low steady-state decreases when firm TFP heterogeneity rises or when fixed costs increase. 

% QUANTITATIVE RESULTS

To quantify these economic forces, we provide three calibrations of our model, where we target US firm-level moments in 1975, 1990 and 2007. These different calibrated models differ in the level of fixed costs and in the degree of TFP dispersion (which both increase over time). We first find that, while the 1975 economy is characterized by a unimodal ergodic distribution of output, the 1990 and 2007 feature bimodal distributions (an indication of two stochastic steady-states). Second, when we subject the three model economies to the same shocks, we observe that the 2007 economy exhibits significantly greater amplification and propagation. For example, we find that the 2007 economy experiences a recession greater than 10\% every 75 years, while the 1990 and 1975 economies experiences one every 120 and 735 years respectively. This suggests that rising firm heterogeneity and fixed costs made the US economy significantly more fragile and more prone to long-lasting slumps.

We also use our model economy as a laboratory to study the Great Recession and its aftermath. The 2008 crisis was marked by a large and persistent deviation of output and other aggregates from trend, something unusual in the entire postwar period. For example, in 2019, output per capita was 14\% below its pre\textendash2007 trend, a deviation far larger and persistent than in previous recessions (Figure \ref{fig:great_deviation_figure}). We ask whether our model can replicate such a quasi-permanent drop in aggregate output and other aggregate variables. To this end, we feed our 2007 economy a sequence of shocks calibrated to match the behavior of aggregate TFP in 2008\textendash9 and study the economy's response. The model generates the observed persistent deviation from trend of GDP as well as of investment, hours and aggregate TFP. It also explains the sharp and persistent drop of the labor share after 2008. Importantly, when we subject the 1990 and 1975 economies to the same shocks, the model does not predict such a persistent deviation from trend. %This suggests that rising firm heterogeneity has rendered the US economy more vulnerable to quasi-permanent recessions as in 2008.


%% EMPIRICS

We also provide empirical evidence in favor of our proposed mechanism. Our theory provides predictions in terms of cross-industry responses to the business cycle. In particular, for any two industries with the same number of firms, the one with a higher level of heterogeneity reacts more to a negative shock. We test this prediction in the data using concentration as a proxy for heterogeneity in US 6-digit industries. Consistent with our model predictions, we show that industries that were more concentrated in 2007 experienced greater cumulative declines in the number of firms, the labor share and economic activity over the 2008-2016 period.

%% POLICY

In terms of policy lessons from our theory, %we ask whether we can design an effective policy to curb the endogenous amplification of aggregate shocks. 
we show that firm subsidies can be effective in preventing deep recessions, leading to a welfare gain of up to 21\% in consumption-equivalent terms. The fundamental intuition behind this result is that in our economy firms' entry and exit decisions have externalities as they change market power. A planner may then find it beneficial to trade off the efficiency loss attached to less productive firms staying in the market with the reduction in the rents of more productive firms. This policy lesson is specific to our model and to the pivotal role of the extensive margin in shaping the degree of aggregate market power. Its logic, however, is more general. Cyclical changes in market power can amplify aggregate fluctuations. Policies that aim to keep the degree of product market competition high can prevent the economy from entering into low output regimes and thereby improve welfare.



\paragraph{Related Literature}

Our paper speaks to three different strands of the literature. First, it is related to the macroeconomic literature studying models of coordination failures \citep{CJ1,Mat,BenhabibFarmer,FarmerGuo,herrendorf2000ruling}. While we are not the first to show how multiple equilibria and/or steady-states can arise in a context of imperfect competition and variable markups \citep{MP,CCR,RW,GZ,J},\footnote{Without relying on multiple equilibria or steady-states, \cite{CJ2}, \cite{EC} and \cite{BGM} show that a combination of imperfect competition with endogenous entry amplifies aggregate fluctuations.} we contribute to this literature by studying the role of firm-level heterogeneity in shaping macroeconomic \textit{fragility}. As we discuss, this concept is distinct from the \textit{existence} of steady-state multiplicity. We also provide a quantification of our mechanism and link it to the 2008 crisis.\footnote{Our paper speaks to the literature on the cyclicality of markups, which includes \cite{RS}, \cite{rotemberg1991markups}, \cite{JF}, \cite{BKM}, \cite{nekarda2020cyclical} and \cite{AVB}.}

Second, this paper relates to a large and growing literature documenting long-term trends in firm heterogeneity and market power. There are several signs that indicate rising market power in the US and other advanced economies. For example, \cite{ADKPR} use data from the US census to document rising sales and employment concentration, while \cite{AA2} document a rise in patenting concentration. Other studies have documented a secular rise in price-cost markups. Using data from national accounts, \cite{H} finds that the average sectoral markup
increased from 1.12 in 1988 to 1.38 in 2015. \cite{LEU} document a steady increase in sales-weighted average markups for US public firms between 1980 and 2016.\footnote{\cite{EMX} show that a cost-weighted average markup displays a less pronounced upward trend. See also \cite{GP}, \cite{T}, \cite{KN2} and \cite{BHKZ} on trends in markups.} This was driven by both an increasing share of large firms and by rising dispersion in the markup distribution.
%\footnote{Identical findings are obtained by \cite{CCM} and \cite{DFVS} for different countries.} 
%In our model, rising dispersion in size and markups is driven by increasing productivity differences. Several studies have documented a secular increase in productivity differences across firms \citep{ACG,K,DHJM2}. 
Close to our approach, \cite{de2021quantifying} argue that declining dynamism and rising market power can be explained, among other channels, by increasing productivity dispersion and fixed costs. \cite{EMX} estimate that the welfare cost of markups can be large and represent a loss of up to 25\% in consumption-equivalent terms.%\footnote{\cite{EGB} builds a search model with heterogeneous firms to study the impact of rising productivity dispersion on the labor share.}
%Lastly, \cite{EMX} use a model close to ours to compute the welfare costs generate by markups via three main channels: i) output reduction, ii) misallocation, and iii) distorted entry.
We contribute to this literature by investigating the business cycle implications of these trends, and in particular their impact on the 2008 crisis and the subsequent \textit{great deviation}. We emphasize that increased firm heterogeneity and market power may have negative welfare consequences through an increase in macroeconomic fragility.

Lastly, this paper relates to the literature studying the persistent impact of the 2008 crisis. A large part of this literature has focused on the secular decline in interest rates and/or the possibility of liquidity traps, which constrains monetary policy \citep{BF,guerrieri_lorenzoni,eggertsson_et_al,mian_sufi_straub}, or endogenous R\&D as in \cite{fasil2021heterogeneous}. Close to this paper, \cite{ST} build an RBC with endogenous capacity utilization
and, as we do, they interpret the post\textendash{}2008 deviation as a transition to a low steady-state. We complement this literature by arguing that rising firm-level heterogeneity has increased the likelihood of quasi-permanent slumps. Our theory can also account for number of trends observed after 2008, related to the behavior of markups, the labor share, concentration and the number of firms.

The rest of the paper is organized as follows. Section \ref{sec: general framework text} sets the general framework and provides the first result relating to technology and fragility. Section \ref{sec:Model} presents a growth model with oligopolistic competition and derives the main theoretical results. Section \ref{sec:Quantitative-Evaluation} discusses the calibration and presents the quantitative results. Section \ref{sec:aggregatefacts} provides and extended application to the US great recession and its aftermath, and presents the cross-industry empirical evidence. In Section \ref{policy}, we study the welfare effects of fiscal policy in our model. Finally, section \ref{sec:Conclusion} concludes.

==> old_versions/3_model.tex <==

\section{A Growth Model with Variable Markups\label{sec:Model}}
This section presents our theoretical framework. We start by describing the demand side and the technology structure. Then we analyze the equilibrium of a particular industry (taking aggregate variables as given). Finally, we characterize the general equilibrium.

\subsection{Preferences}
Time is discrete and indexed by $t=0,1,2,\ldots$.
There is a representative, infinitely-lived household with lifetime utility
\[
U_{t}=\mathbb{E}\sum_{t=0}^{\infty}\:\beta^{t}\:U\left(C_{t},L_{t}\right),
\]
where $0 < \beta < 1$ is the discount factor, $C_{t} \geq 0$ is consumption of the final good and $L_{t} \geq 0$ is labor.
We adopt a period utility function as in \cite{GHH}
\begin{equation}
U\left(C_{t},L_{t}\right)=\dfrac{1}{1-\psi}\left(C_{t}-\dfrac{L_{t}^{1+\nu}}{1+\nu}\right)^{1-\psi},
\label{eq:HH_utility}
\end{equation}
where $0\leq\psi\leq1$ and $\nu>0$. 

The representative household contains many individual members, which will be denoted by $j$. Each individual member can run a firm in the corporate sector. We assume that if two or more individuals run a firm in the same industry, they will behave in a non-cooperative way \textendash{} i.e. they will compete against each other and will not collude. Nevertheless, all individuals will pool together the profits they make. Hence there is a single dynamic budget constraint
\begin{equation}
K_{t+1}=\left[R_{t}+\left(1-\delta\right)\right]K_{t}+W_{t}L_{t}+\Pi^{N}_{t}-C_{t},
\label{eq:budget_constraint}
\end{equation}
where $K_t$ is capital, $R_t$ is the rental rate, $W_{t}$ is the wage rate and $\Pi^{N}_{t}=\sum_{j} \Pi_{j}^{N}$ are the profits accruing from all the firms in the economy net of fixed production costs. Capital depreciates at rate $0\leq\delta\leq1$ and factor prices $R_{t}$ and $W_{t}$ are taken as given. The representative household therefore maximizes (\ref{eq:HH_utility}) subject to (\ref{eq:budget_constraint}). Our choice of GHH preferences implies that the aggregate labor supply is a simple function of the wage rate $L_{t} = W_{t}^{1/\nu}$, where $\nu$ is the inverse of the wage elasticity of labor supply.\footnote{
From the perspective of the household, labor and entrepreneurial decisions are separable. We abstract from an occupational decision problem (becoming an entrepreneur \textit{versus} working) for simplicity. This assumption does not however imply that there is a fixed supply of entrepreneurs, since the equilibrium number of firms/entrepreneurs will be endogenous.}

\subsection{Technology}

There is a final good (the \textit{numeraire}), which is a CES aggregate of $I$ different industries $ Y_{t}=\left(\sum_{i=1}^{I}{\vphantom{\Pi^P}y}_{it}^{\rho}\right)^{1/\rho}, $ where $y_{it}$ is the quantity of industry $i\in\left[0,1\right]$, and $\sigma_{I} = {1}/{(1-\rho)}>1$ is the elasticity of substitution
across industries.

$I$ is assumed to be large, so that each individual industry has a negligible size in the economy. The output of each industry $i$ is itself a CES
composite of differentiated goods or varieties $ y_{it}=\left(\sum_{j=1}^{n_{it}}{\vphantom{\Pi^P}y}_{jit}^{\eta}\right) ^{1/\eta}, $ where $n_{it}$ is the number of active firms in industry $i$ at time $t$ (to be determined endogenously) and $\sigma_{G} = 1/(1-\eta) > 1$ is the within-industry
elasticity of substitution. Following \cite{AB},
we assume that goods are more easily substitutable within industries than across industries: 
%\begin{assumptionf} 
$0<\rho<\eta\leq1$.
%\end{assumptionf} 
Given these assumptions, the inverse demand for each variety $j$ in industry $i$ is given by
\begin{equation}
p_{ijt}=\left(\dfrac{Y_{t}}{y_{it}}\right)^{1-\rho}\left(\dfrac{y_{it}}{y_{ijt}}\right)^{1-\eta}.\label{eq:inv_demand_good}
\end{equation}
We assume that in every industry $i\in\left\{0,\ldots,I\right\}$ there is a maximum number of entrepreneurs $N \in \mathbb{N}$, so that $n_{it} \leq N$. Entrepreneur $j$ can produce his variety
by combining capital $k_{ijt}$ and labor $l_{ijt}$ through a Cobb-Douglas
technology
\begin{equation}
y_{it}=\underbrace{e^{a_{t}}\;\gamma_{ij}}_{\tau_{ijt}}\left(k_{ijt}\right)^{\alpha}\left(l_{ijt}\right)^{1-\alpha}.\label{eq:CD_pf}
\end{equation}
Note that the productivity of each entrepreneur $\tau_{ijt}$ is the product of two terms (i) a time-varying aggregate component $e^{z_{t}}$
(common to all industries and types) and (ii) a time-invariant idiosyncratic
term $\gamma_{ij}$. We refer to $z_{t}$ as aggregate productivity and to $\gamma_{ij}$ as $j$'s idiosyncratic productivity. Aggregate productivity $a_{t}$ follows an auto-regressive process $ a_{t}=\phi_{a}a_{t-1}+\varepsilon_{t}$, with $\varepsilon_{t}\sim N \left(0,\sigma_{\varepsilon}^{2}\right)$. With no loss of generality,
we order idiosyncratic productivities according to $\gamma_{i1}\geq\gamma_{i2}\geq\gamma_{i3}>\cdots.$ 
Labor is hired at the competitive wage $W_{t}$ and capital at the
rental rate $R_{t}$. Entrepreneur $j$ can thus produce
her variety with marginal cost $\Theta_{t} / \tau_{ijt}$,
where 
\[
\Theta_{t}\equiv\left(\frac{R_{t}}{\alpha}\right)^{\alpha}\left(\frac{W_{t}}{1-\alpha}\right)^{1-\alpha}
\]
is the marginal cost function for a Cobb-Douglas technology with unit
productivity. We refer to $\Theta_{t}$ as the \textit{factor
cost index}. In addition to all variable costs, the production of each variety entails a fixed production cost $c_{i} \geq 0$ per period (which can be possibly different across industries). Such a cost is in units of the \textit{numeraire}.\footnote{According to this formulation, fixed production costs do not change with factor prices. We introduce variable fixed costs in an extension (Appendix \ref{subsec:var_fixed_costs}).}


\subsection{Market Structure \label{subsec:Market-Structure}}

To conclude the description of the model, we must specify the way firms interact. We assume that all firms that enter (and thus incur the fixed cost $c_{i}$) play a static Cournot game: they will simultaneously announce quantities,
taking the output of the other competitors as given.\footnote{We follow \cite{AB} and assume
that firms enter sequentially in reverse order of productivity.} 
Therefore, each entrepreneur $j$ solves 
\begin{equation}
\begin{array}{cl}
\underset{y_{ijt}}{\textrm{max}}\quad\left(p_{ijt}-\dfrac{\Theta_{t}}{\tau_{ijt}}\right)y_{ijt}\qquad\text{s.t.}\; & p_{ijt}=\left(\dfrac{Y_{t}}{y_{it}}\right)^{1-\rho}\left(\dfrac{y_{it}}{y_{ijt}}\right)^{1-\eta}\\
& y_{it}=\left(\sum\limits_{k=1}^{n_{it}}y_{kit}^{\eta}\right)^{\frac{1}{\eta}}.
\end{array} \label{eq:Cournot_problem}
\end{equation}
The solution to (\ref{eq:Cournot_problem}) yields a system of $n_{it}$ non-linear equations in $\left\{ p_{ijt}\right\}_{j=1}^{n_{it}}$ (one for each firm)\footnote{
This system of first order conditions admits a close-form solution only in the limit case in which there is no differentiation within an industry ($\eta = 1$), as shown in Appendix \ref{Cournot_eta_1}.}
\begin{equation}
p_{ijt} = \underbrace{\dfrac{1}{\eta-\left(\eta-\rho\right)s_{ijt}}}_{\mu_{ijt}} \,  \dfrac{\Theta_{t}}{\tau_{ijt}},\label{eq:firm_FOC}
\end{equation}
where $s_{ijt}$ is the market share of firm $j=1,\ldots,n_{it}$ and $\mu_{ijt}$ is the markup. Equation (\ref{eq:firm_FOC}) establishes a positive relationship between market shares and markups. This happens because firms internalize the impact of size on the price they charge $p_{ijt}$; large firms end up restricting output disproportionately more (relative to productivity), thereby charging a high markup. 
Moreover, as equation (\ref{eq:firm_FOC}) also highlights, market shares are themselves a positive function of RTFP $p_{ijt} \: \tau_{ijt}$. Our model thus features a positive association between revenue productivity, size and markups. Therefore, a shock that generates larger productivity differences across firms will also lead to larger markup dispersion.

To conclude the description of the industry equilibrium, we need to determine the number of active firms $n_{it}$. To this end, let $ \Pi\left( \, j \, , \, n_{it} \, , \, \mathcal{F}_{it} \, , \, X_{t} \, \right) \coloneqq \left(p_{it}-{\Theta_{t}}/{\tau_{ijt}}\right)y_{ijt}$ denote the equilibrium profits of firm $j\leq n_{it}$ in industry $i$ (gross of the fixed production cost), when there are $n_{it}$
active firms, given a productivity distribution $\mathcal{F}_{it} \coloneqq \left\{ \, \gamma_{i1} \, , \, \gamma_{i2} \, , \, \ldots  \, \right\}$ and a vector of aggregate variables $X_{t}\coloneqq\left[ \, a_{t} \, , \, Y_{t} \, , \, \Theta_{t} \, \right]$. The equilibrium number of firms must be such that (i) the profits of each active firm are not lower than the fixed cost $c_{i}$ and (ii) if an additional firm were to enter, its profits would be lower than the fixed cost. Mathematically, an interior solution $n^{*}_{it} < N$ to the equilibrium number of firms must satisfy
\begin{equation}
\left[\Pi\left({\color{blue}n_{it}^{*}},{\color{blue}n_{it}^{*}},\mathcal{F}_{i},X_{t}\right)-c_{i}\right]\left[\Pi\left({\color{blue}n_{it}^{*}+1},{\color{blue}n_{it}^{*}+1},\mathcal{F}_{i},X_{t}\right)-c_{i}\right]\leq0 .\label{eq:eqm_n_firm}
\end{equation}
Lemma \ref{lemma:(Profit-Function)} in Appendix \ref{subsec:Profits} provides an analytical characterization of the profit function under the special case of $\eta=1$. In particular, we show that the profits of any firm $j$ increase in its own idiosyncratic productivity $\gamma_{ij}$ and decrease in the idiosyncratic productivity
of all the other firms $\gamma_{ik}$. Therefore, as top firms increase their productivity level, small firms make lower profits and become closer to their break even point (\textit{ceteris paribus}). This is key to understand some aggregate results that we describe next.

\subsection{General Equilibrium}
\paragraph{Equilibrium Definition}
We start by defining an equilibrium for this economy. Denoting the history of
aggregate productivity shocks by $ A^{t} = \{ a_{t}, a_{t-1}, ...\} $ we have the following definition.
\begin{definition}[Equilibrium]
A general equilibrium consists of a sequence of household policies  $ \left\{ C_{t}\left(A^{t}\right), K_{t}\left(A^{t}\right), L_{t}\left(A^{t}\right)\right\} $, firm policies $ \left\{ y_{ijt}\left(A^{t}\right), k_{ijt}\left(A^{t}\right), l_{ijt}\left(A^{t}\right)\right\} $, and a set of active firms $\left\{ n_{it}\left(A^{t}\right)\right\}_{i=1}^{I}$ such that i) households optimize; ii) all active firms optimize; iii) all active firms do not make a loss: iv) no additional firm is willing to enter; v) capital and labor markets clear.
\end{definition}


\subsubsection{Static Equilibrium}
We now describe the general equilibrium of this economy. We start by focusing on a static equilibrium, in which we describe production and labor supply decisions, taking the aggregate level of capital $K_{t}$ as given. Later on, we describe the equilibrium dynamics.

\paragraph{Aggregate Production Function} Given a $\left(I\times N\right)$
matrix of productivity draws $\mathbf{A}_{t}$ and a vector of active firms
$\mathbf{N}_{t} \equiv \left\{ n_{it}\right\}_{i=1}^{I}$, aggregate output can be written as 
\begin{equation}
Y_{t}={A}_{t}\Phi\left(\mathbf{\Gamma},\mathbf{N}_{t} \right)\;L_{t}^{1-\alpha}K_{t}^{\alpha} .\label{eq:agg_prod_fct}  
\end{equation}
The term $\Phi\left(\cdot\right)$ 
represents the endogenous component of aggregate TFP and is a function of the number of active firms, individual firm productivities and market shares. An expression for $\Phi\left(\mathbf{\Gamma},\mathbf{N}_{t}\right)$ is provided in Appendix \ref{subsec:Aggregate-TFP}.

\paragraph{Factor Markets}
The aggregate factor demand schedules for labor $L_t$ and capital $K_t$ are given by
\begin{equation}
\begin{array}{cl}
W_{t} \; = &  \left(1-\alpha\right)\;{A}_{t} \: \Omega\left(\mathbf{\Gamma},\mathbf{N}_{t}\right)\;\Phi\left(\mathbf{\Gamma},\mathbf{N}_{t}\right)\;L_{t}^{-\alpha}\,K_{t}^{\alpha},\\[1ex]
R_{t} \; = &  \alpha\;{A}_{t} \: \Omega\left(\mathbf{\Gamma}, \mathbf{N}_{t}\right)\;\Phi\left(\mathbf{\Gamma},\mathbf{N}_{t}\right)\;L_{t}^{1-\alpha}\,K_{t}^{\alpha-1}.
\end{array} \label{eq:factor_demand}  
\end{equation}
where $\Omega\left(\cdot\right) = \left(W_{t}\,L_{t} + R_{t}\,K_{t} \right)/Y_{t} $ is the aggregate factor share. An analytical expression for $\Omega\left(\mathbf{\Gamma}, \mathbf{N}_{t} \right)$ in provided in Appendix \ref{subsec:Factor-Prices}. These two demand schedules can be combined with the labor and capital supply equations
\begin{align}
     L_{t}^{S} = W_{t}^{1 / \nu}  \quad \text{and} \quad K_{t}^{S} = K_{t} 
\label{eq:factor_supply}  
\end{align}
to determine the factor market equilibrium.
% Combining equations (\ref{eq:factor_demand}) and (\ref{eq:factor_supply}) we can obtain an expression for equilibrium employment
% \begin{equation}
% L_{t} = \left[\left(1-\alpha\right)\Theta\left(\mathbf{A}_{t},\mathbf{N}_{t}\right)\right]^{\frac{1}{\nu+\alpha}}K_{t}^{\frac{\alpha}{\nu+\alpha}}. \label{eq:labor_mkt_eq}  
% \end{equation}
Combining equations (\ref{eq:factor_demand}) and (\ref{eq:factor_supply})  with (\ref{eq:agg_prod_fct}), we can write aggregate output as a function of the aggregate capital stock $K_t$, the productivity distribution $\mathbf{\Gamma}$ and the set of active firms $\mathbf{N}_{t}$
\begin{equation}
Y_{t}=\left[\left(1-\alpha\right)\Omega\left(\mathbf{\Gamma},\mathbf{N}_{t}\right)\right]^{\left(1-\alpha\right)/\left(\nu+\alpha\right)}\left[ {A}_{t} \, \Phi\left(\mathbf{\Gamma},\mathbf{N}_{t}\right) K_{t}^{\alpha}\right]^{\left(1+\nu\right)/\left(\nu+\alpha\right)}. \label{eq:agg_output_capital}
\end{equation}
To conclude the characterization of the static equilibrium, we must determine the set of active firms $\mathbf{N}_{t}$.

\paragraph{Equilibrium Set of Firms}

The number of active firms in each industry $i$ is  jointly determined by equations (\ref{eq:factor_demand}),  (\ref{eq:agg_output_capital}) and the set of inequalities defined in (\ref{eq:eqm_n_firm}). Such a joint system does not admit a general analytical characterization. We can nevertheless characterize the particular case in which all industries are identical. Proposition \ref{A-symmetric-equilibrium} states the conditions for a symmetric equilibrium with $n$ firms per industry.

\begin{prop}[Existence of Symmetric Equilibrium]
\label{A-symmetric-equilibrium} Suppose that all industries have the same distribution of idiosyncratic productivities $\mathcal{F}_{i}=\mathcal{F}$. Then, there can be a symmetric equilibrium with $n$ firms per industry if $K_{t}$ is such that
\[
\underline{K}\left(\mathcal{F},n\right)\leq K_{t}\leq\overline{K}\left(\mathcal{F},n\right),
\]

The bounds $\overline{K}\left(\cdot\right)$ and $\underline{K}\left(\cdot\right)$ are both increasing in $n$.
\end{prop}
\begin{proof}
See Appendix \ref{subsec:numb-active-firms}.
\end{proof}
Intuitively, $K_{t}$ must be (i) sufficiently large so that all existing $n$ firms can break even, (ii) but cannot be too high, for otherwise an additional firm could profitably enter in at least one industry.

\subsubsection{Equilibrium Dynamics}
We are now ready to explore the dynamic properties of our economy. To determine the model dynamics we need to characterize the law of motion
\begin{align*}
    K_{t+1} = \left(1-\delta\right) K_{t} + s_{t} \cdot Y_{t}
\end{align*}
where $s_{t}$ is the aggregate savings rate. 
We start by observing a necessary condition for the existence of multiple steady states.
\begin{remark}\label{remarkmultiplicity}
Steady state multiplicity can arise provided that either of the following is holds:
\begin{itemize}
    \item the saving rate $s$ can be locally increasing in capital;
    \item output $Y$ is not a strictly concave function of capital.
\end{itemize}
\end{remark}
This remark simply provides necessary conditions for the capital law of motion to feature non-concavities. When the law of motion is not strictly concave it can cross the 45 degree line multiple times, which is the definition of steady state multiplicity.
We now formalize in two propositions that both necessary conditions in Remark \ref{remarkmultiplicity} can hold in our model. 

Even though we cannot derive an analytical expression for the savings rate, we can nevertheless characterize it on a steady-state. In particular we are interested in how it changes with the number of active firms, and therefore with capital, and with the degree of firm heterogeneity. In the Appendix we provide two intermediate Lemmas which we summarise here. Lemma \ref{prop:ss_agg_s_rate} shows that the steady-state savings rate is proportional to the aggregate factor share $\Omega^{*}$. Lemma \ref{prop:The-aggregate-factor-share} shows that $\Omega(\cdot)$ increases in the number of active firms and decreases in the level of firm heterogeneity. The following proposition is an immediate consequence.

\begin{prop}\label{heterogeneity_savings} [Steady-State Savings Rate]
The steady-state savings rate $s^*=s\left(\mathbf{\Gamma},\mathbf{N}^{*}\right)$
\begin{enumerate}
    \item increases in the number of active firms. As the number of firms is weakly increasing in capital, the saving rate can increase in capital.
    \item decreases in the level of firm heterogeneity. 
\end{enumerate}
\end{prop}

\begin{proof}
Follows immediately from Lemma \ref{prop:ss_agg_s_rate} and \ref{prop:The-aggregate-factor-share}.
\end{proof}

The previous proposition states two important results. First, from Lemma \ref{prop:The-aggregate-factor-share} the larger is the number of firms per industry, the more intense is the degree of product market competition and hence the aggregate factor share $\Omega\left(\cdot\right)$. Second, the aggregate factor share decreases when the distribution of individual productivities becomes more dispersed. Intuitively, in every industry, high productivity firms are larger and charge higher markups. As large firms are able to increase their markups even further, the aggregate profit share increases and the aggregate factor share decreases. Proposition \ref{heterogeneity_savings} states that these changes in capital and labor shares translate into a changes in the steady-state savings rate. In turn, this implies that we can have multiplicity of steady states as the saving rate can increase in capital.

We now turn to the second condition of Remark \ref{remarkmultiplicity} and formalize the relationship between output and capital in the next Proposition.

This result is the cornerstone on which we build our multiplicity argument. As firm heterogeneity increases, this compresses factor shares, thereby decreasing the saving rate. As the saving rate declines it is harder for firm 

\paragraph*{Law of Motion}
To better illustrate some of the model dynamics, let us consider the example of an economy where all industries are ex-ante identical (i.e. same distribution idiosyncratic productivities $\mathcal{F}_{i}=\mathcal{F}$) and with no aggregate productivity shocks (i.e. $a_{t} = 1$). Furthermore, let us set $\eta=1$ so that there is no love for variety within an industry.
Figure \ref{fig:Law-of-Motion-Homog-UE} below shows the law of motion for a particular parameter configuration. For low values of the capital stock, all industries consist of a monopoly, whereas for higher values they consist of a duopoly.
Note that the law of motion is not globally concave and exhibits a convex region for $K_{t} \in \left[\overline{K}\left(1\right), \underline{K}\left(2\right)\right]$.\footnote{In this region, a symmetric equilibrium is not possible. In such a case, some industries will consist of a monopoly, and some other of a duopoly. A detailed characterization of this non-symmetric equilibrium is provided in online appendix \ref{subsec:Asymmetric Equilibrium}.} Such a convexity occurs because of the interplay between factor supply and competition. As $K_{t}$ increases, the economy moves towards a more competitive regime, with a larger factor share $\Omega\left(\mathbf{\Gamma},2\right) > \Omega\left(\mathbf{\Gamma},1\right)$. A larger factor share results in a higher wage and labor supply (resulting in larger $Y_{t}$ for a given $K_{t}$), but also in a higher savings rate (resulting in larger $K_{t+1}$ for a given $Y_{t}$).
Because of this complementarity between capital accumulation and competition, the law of motion exhibits two steady-states: one where all industries are a monopoly $\left(K_{1}^{\textrm{ss}}\right)$, and another where all industries are a duopoly $\left(K_{2}^{\textrm{ss}}\right)$.\footnote{The existence of exactly two steady-states is obviously not guaranteed. Figures \ref{fig:Unique_ss} and \ref{fig:Three_ss} in Appendix \ref{subsec:Steady-State} show examples of economies with one or three steady-states.} The steady-state to which the economy will converge depend on its initial condition $K_{0}$.\footnote{Figure \ref{fig:Law-of-Motion-Homog-UE} represents the law of motion for a fixed value of aggregate productivity $z_{t} = 1$. However, the law of motion will change with aggregate productivity $z_{t}$. Appendix \ref{law-of-motion-stochastic-productivity} shows an example with stochastic productivity.}  
Note that despite the existence of two steady-states, this example features a unique equilibrium: there is a unique value of $K_{t+1}$ for each value of $K_{t}$ (the state
variable). Figure \ref{fig:Static-Equilibrium} in Appendix \ref{subsec:Static-Equilibrium-Characterization} characterizes the behavior of the rental rate.

\begin{figure}[ht!]
\centering{}
 \includegraphics[scale=0.55]{input/lom_ue}
\caption{Law of motion
\protect \\ {Note: \small{} the figure plots the law of motion of capital. This example features two stable steady states and an unstable one. We use $\psi \, = \, 1 \,$, $\delta \, = \, 1 \,$, $\alpha \, = \, 1/3 \,$, $\rho \, = \, 0.6 \,$, $\eta \, = \, 1 \,$, $\nu \, = \, 0.4 \,$, $\gamma_{ij} \, = \, 1 \,$ and $ c_{i} \, = \, 0.015 \,$.}} 
\end{figure}

\begin{figure}[ht!]
\centering{}
\hspace{-0.2cm}
 \includegraphics[scale=0.475]{input/LOM_baseline}
 \hspace{0.4cm}
 \includegraphics[scale=0.475]{input/RR_baseline}
\caption{Rental rate and law of motion\label{fig:Law-of-Motion-Homog-UE}
\protect \\ {Note: \small{} the figure plots the law of motion of capital. This example features two stable steady states and an unstable one. We use $\psi \, = \, 1 \,$, $\delta \, = \, 1 \,$, $\alpha \, = \, 1/3 \,$, $\rho \, = \, 0.6 \,$, $\eta \, = \, 1 \,$, $\nu \, = \, 0.4 \,$, $\gamma_{ij} \, = \, 1 \,$ and $ c_{i} \, = \, 0.015 \,$.}} 
\end{figure}
This simple law of motion already provides a theory for some of the facts described in the introduction. Suppose that the economy starts in a neighborhood of the high steady-state $K^{SS}_{2}$ but is hit by a temporary shock that brings capital close to $\overline{K}\left(1\right)$. The economy will then enter the basin of attraction of the low steady-state $K^{SS}_{1}$ and experience a persistent drop in aggregate output, a persistent decline in the labor share and an increase in the profit share. Viewed through the lens of this model, a transition to a less competitive regime can explain the deviation of output from trend after 2008. 

However, as discussed in the introduction, several signs suggest a long-run increase in market power since at least the 1980. This seems to be associated with rising firm heterogeneity and a reallocation of activity towards large firms (\cite{VR}). Since these trends can have a direct impact on our mechanism, we ask what are the dynamics consequences of rising firm heterogeneity. We will also discuss the consequences of rising fixed costs.

We next consider two comparative statics exercises: a mean-preserving spread to the distribution of productivities, and an increase in fixed costs of production. We ask how these technological shifts affect the basin of attraction of the highest steady-state.

\paragraph*{Rising Firm Differences}

Let us now revisit the example of Figure \ref{fig:Law-of-Motion-Homog-UE}. Suppose  that in each industry there is a productive firm with productivity $\gamma_{1}=\gamma \geq 1$
(the leader), while all the other firms $j=2,3,\ldots$ have productivity $\gamma_{j}=1$ (the followers). Figure \ref{fig:Comparative-Statics-MPS} represents the effects of an increase in $\gamma$. 

Two facts stand out. First, the two concave segments of the law of motion (representing the symmetric equilibria with $n = 1$ and with $n = 2$ firms) move up. This fact simply represents an expansion in the economy's production possibility frontier \textendash{} because of the larger productivity advantage of the leaders, aggregate output will increase for any fixed number of active firms $n$. Second, part of the convex segment lying between $\overline{K}\left(1\right)$ and $\underline{K}\left(2\right)$ lies below the initial law of motion. This change reflects the fact that the leaders increase their productivity over the followers. Because of such a larger advantage, the followers can only enter at increasingly larger levels of aggregate capital, which results in a simultaneous increase in $\overline{K}\left(1\right)$ and $\underline{K}\left(2\right)$. Therefore, the increase in $\gamma$ has two effects on the law of motion: (i) for a fixed number of firms, it results in an expansion of the production possibility frontier, (ii) however an equilibrium with $n \geq 2$ can only be sustained with larger values of aggregate capital.

Recall that
\begin{equation*}
    R_{t} \: = \: \alpha\;{A}_{t} \: \Omega\left(\mathbf{\Gamma}, \mathbf{N}_{t}\right)\;\Phi\left(\mathbf{\Gamma},\mathbf{N}_{t}\right)\;L_{t}^{1-\alpha}\,K_{t}^{\alpha-1}.
\end{equation*}

As Lemma \ref{prop:The-aggregate-factor-share} shows, $\Omega\left(\mathbf{A},\mathbf{N}\right)$ necessarily declines when all industries have $\mathbf{N} = n = 2$ firms.

\begin{figure}[ht!]
\centering{}%
\begin{tabular}{cc}
	\hspace{-1cm} \includegraphics[scale=0.45]{input/RR_cf} &  \hspace{-0.2cm}
	\includegraphics[scale=0.45]{input/RR_MPS} \\
	\hspace{-1cm} 
	\includegraphics[scale=0.45]{input/LOM_cf.eps} & 
	\hspace{-0.2cm}
	\includegraphics[scale=0.45]{input/LOM_MPS}
\end{tabular}
\caption{Static equilibrium \protect \\ {Note: \small{} the figure shows how output, the profit share and input prices move with capital. Solid segments represent economies with symmetric market structure (same number of firms), while dotted segments represent non-symmetric equilibria. We use $\alpha \, = \, 1/3 \,$, $\rho \, = \, 0.6 \,$, $\eta \, = \, 1 \,$, $\nu \, = \, 0.4 \,$, $\pi_{ij} \, = \, 1 \,$ and $ c_{i} \, = \, 0.015 \,$.}} 
\label{fig:Comparative-Statics-MPS}
\end{figure}


% \begin{figure}[ht!]
% \begin{minipage}[b]{.5\linewidth}
% \centering{}\includegraphics[scale=0.465]{input/lom_lf_2_paper.eps}\subcaption{Larger productivity differences \label{fig:Law-of-Motion-Heterog}}
% \end{minipage}%
% \begin{minipage}[b]{.5\linewidth}
% \centering{}\includegraphics[scale=0.465]{input/lom_fc.eps}\subcaption{Larger fixed costs \label{fig:Law-of-Motion-Fixed-Cost}}
% \end{minipage}
% \caption{Law of motion (comparative statics) \protect \\ {Note: \small{} the figure shows changes in the law of motion of capital after an increase in productivity differences (Panel (a)) and in fixed costs (Panel (b)). We use $\psi \, = \, 1 \,$, $\delta \, = \, 1 \,$, $\alpha \, = \, 1/3 \,$, $\rho \, = \, 0.6 \,$, $\eta \, = \, 1 \,$ and $\nu \, = \, 0.4 \,$.}} \label{fig:lom_comp_statics}
% \end{figure}



% \begin{figure}[ht!]
% \begin{minipage}[b]{.5\linewidth}
% \centering{}\includegraphics[scale=0.465]{input/rr_leader_follower.eps}\subcaption{Larger productivity differences}
% \end{minipage}%
% \begin{minipage}[b]{.5\linewidth}
% \centering{}\includegraphics[scale=0.465]{input/rr_leader_follower_2.eps}\subcaption{Mean-preserving spread }
% \end{minipage}
% \end{figure}

Note that the increase in $\gamma$ results in a reduction of the basin of attraction of the high steady-state. Although we cannot provide a full analytical characterization of the impact of $\gamma$ on the basin of attraction (i.e. whether it always shrinks or can actually increase), we can nevertheless characterize its impact on the subset of the basin of attraction that falls under a symmetric equilibrium. This is done in Proposition \ref{prop:basin_attraction}.


\textbf{We prove this for a specific MPS. Add to proposition}

\begin{prop} [Mean Preserving Spreads and Basins of Attraction] \label{prop:basin_attraction_MPS} Let $\eta = 1$ and suppose that all industries are identical to start ($\gamma_{ij} = \gamma_{j} \; \forall i$). Let ${K}^{*}\left(n\right)$ be a steady-state with $n$ firms and basin of attraction $\left( \underline{B}\left(n\right),\overline{B}\left(n\right) \right)$. Let $\lambda$ be a mean-preserving spread on the distribution $\left\{\gamma_1,\ldots,\gamma_n\right\}$ of active firms. Then
\[ \dfrac{\partial \underline{B}\left(n\right)}{\partial\lambda} \geq 0 \quad \text{and} \quad \dfrac{\partial {K}^{*}\left(n\right)}{\partial\lambda} \leq 0. \]
\end{prop}
\begin{proof}
See Appendix \ref{subsec:basin_attraction}.
\end{proof}

\textbf{SKETCH OF THE PROOF}

\begin{corollary} If ${K}^{*}\left(n\right)$ is the highest steady-state, then its basin of attraction $\left(\underline{B}\left(n\right),\infty \right)$ shrinks.
\end{corollary}

\begin{corollary}
The following holds:
\begin{itemize}
    \item if labor supply is inelastic ($\nu\rightarrow\infty$), an MPS increases fragility  if $\alpha<1/(2-\rho)$ ;
    \item if labor supply is isoelastic ($\nu=1$), an MPS increases fragility  if $\alpha<\rho/(2-\rho)$;
    \item if labor supply is perfectly elastic ($\nu=0$), an MPS increases fragility  if $\alpha(1-\alpha)>(1-\rho)/(2-\rho)$.
\end{itemize}
Finally, fixing $\rho$,
$\nu^\star(\alpha)$: the pair $(\nu^\star(\alpha),\alpha)$ satisfies the condition in Proposition \ref{prop:basin_attraction_MPS} is increasing and convex in $\alpha$.
\end{corollary}

\textbf{DISCUSSION OF PROPOSITION AND COROLLARIES}

Let us sketch a proof for Proposition \ref{prop:basin_attraction_MPS}. To show that $\dfrac{\partial{K}^{*}\left(n\right)}{\partial\lambda} \leq 0$, we simply need to show that $\Theta\left(\Gamma,n\right)$ decreases after we apply the MPS, something we already did. 

To show that $\dfrac{\partial \underline{B}\left(n\right)}{\partial\lambda} \geq 0$ we need to go in steps. First note that $\underline{B}\left(n\right)$ is the unstable steady-state. We have to show that at the initial $\underline{B}\left(n\right)$, $\Theta\left( \cdot\right)$ is increasing in the average number of firms (something we already did), and that the average number of firms decreases (i.e. the number of industries with n-1 firms increases). This second part we haven't done, but we should be able to do it.

\begin{prop} [Firm Heterogeneity and Fragility]  Let \label{prop:basin_attraction} $\eta = 1$ and suppose that all industries and firms are identical to start ($\gamma_{j} = \gamma \; \forall j$). Let ${K}^{*}\left(n\right)$ be a steady-state with $n$ firms. Then we have that
\[	\dfrac{\partial}{\partial\gamma_{k}}\left[\dfrac{{K}^{*}\left(n\right)}{\underline{K}\left(n\right)}\right]<0.
\]	
if and only if
\[
\dfrac{1/ \nu +\alpha}{1-\alpha}<\dfrac{\left(4 + 1/n \right)\left[n-\left(1-\rho\right)\right]-n}{1-\rho}.
\]	
\end{prop}
\begin{proof}
See Appendix \ref{subsec:basin_attraction}.
\end{proof}
To understand Proposition \ref{prop:basin_attraction}, suppose that some type $\gamma_{k}$ experiences a productivity increase, while the productivity of all other types remains constant. Proposition \ref{prop:basin_attraction} gives the condition under which the basin of attraction falling under $\bigl[\underline{K}\left(n\right), K^{*}\left(n\right)\bigr]$ shrinks. This is satisfied provided that (i) labor supply is relatively inelastic (low $1/\nu$), (ii) there are strong diminishing returns to capital (low $\alpha$) and (iii) a low degree of product differentiation (high $\rho$). To have an intuition, note that labor supply needs to be relatively rigid for types $\gamma_n$ to be crowded out as types $\gamma_k \geq \gamma_n $ expand. The degree of product differentiation cannot be too high so that markups are low and industries are characterized by a \textit{winner-takes-it-all} type of dynamics.\footnote{When this condition is not satisfied, an increase in the productivity of the leader may increase the basin of attraction of the high steady-state. In this case, a larger production possibility frontier makes entry easier for the followers.}

\paragraph*{Rising Fixed Costs} The decline in product market competition since the 1980s may be also explained, through the lens of our model, by rising fixed costs. How can larger fixed costs affect the law of motion represented in Figure \ref{fig:Law-of-Motion-Homog-UE}? First, we can show that if a steady-state with $n$ firms exists, and all firms make strictly positive profits, the existence and level of such a steady-state $\left(K^{SS}_{n}\right)$ will not be affected by a marginal increase in $c_f$ (see Appendix \ref{subsec:basin_attraction} for a proof). A larger fixed cost will however result in a larger level of aggregate capital consistent with $n$ firms per industry, $\underline{K}\left(n\right)$ (see Appendix \ref{subsec:numb-active-firms}). Therefore, the basin of attraction of the largest steady-state shrinks, as shown in Figure \ref{fig:Comparative-Statics-MPS}. This means that rising fixed costs also make the highest steady-state more fragile, so that now even relatively small shocks can trigger a transition to the the low competition trap. This result is stated in the next proposition.

\begin{prop}[Fixed Cost and Fragility] \label{prop:basin_attraction_cf} Let $\eta = 1$. Let ${K}^{*}\left(n\right)$ be a steady-state with $n$ firms and suppose all firms make strictly positive profits. Then we have that
\[	\dfrac{\partial}{\partial c_{i}} \left[\dfrac{{K}^{*} \left(n\right)} {\underline{K}\left(n\right)}\right]<0.
\]	
\end{prop}
\begin{proof}
See Appendix \ref{subsec:basin_attraction}.
\end{proof}


\paragraph{Discussion}
We conclude by summarizing two keys insights of our theory, which we think are relevant to understand the US growth experience after 2008. The first is that a complementarity between competition and factor supply can generate multiple competition regimes or steady-states. A transition from a high competition to a low competition regime can in many aspects describe the 2008 recession and the subsequent great deviation. Second, changes in technology that result in larger market power (e.g. larger productivity differences across firms or larger fixed costs) make high competition regimes more difficult to sustain, and transitions to low competition traps easier to occur. Our model therefore suggests that the US economy, experiencing a long-run increase in markups and concentration since the 1980s, became increasing vulnerable to transitions like this.

We next use a calibrated version of our model to ask whether it can replicate the behaviour of the US economy in the aftermath of the 2008 crisis. We also perform some counterfactual exercises to quantify the impact of rising market power.


==> old_versions/3_model2.tex <==

\section{A Growth Model with Variable Markups\label{sec:Model}}
This section presents our theoretical framework. We start by describing the demand side and the technology structure. Then we analyze the equilibrium of a particular industry (taking aggregate variables as given). Finally, we characterize the general equilibrium.

\subsection{Preferences}
Time is discrete and indexed by $t=0,1,2,\ldots$.
There is a representative, infinitely-lived household with lifetime utility
\[
U_{t}=\mathbb{E}\sum_{t=0}^{\infty}\:\beta^{t}\:U\left(C_{t},L_{t}\right),
\]
where $0 < \beta < 1$ is the discount factor, $C_{t} \geq 0$ is consumption of the final good and $L_{t} \geq 0$ is labor.
We adopt a period utility function as in \cite{GHH}
\begin{equation}
U\left(C_{t},L_{t}\right)=\dfrac{1}{1-\psi}\left(C_{t}-\dfrac{L_{t}^{1+\nu}}{1+\nu}\right)^{1-\psi},
\label{eq:HH_utility}
\end{equation}
where $0\leq\psi\leq1$ and $\nu>0$. 

The representative household contains many individual members, which will be denoted by $j$. Each individual member can run a firm in the corporate sector. We assume that if two or more individuals run a firm in the same industry, they will behave in a non-cooperative way \textendash{} i.e. they will compete against each other and will not collude. Nevertheless, all individuals will pool together the profits they make. Hence there is a single dynamic budget constraint
\begin{equation}
K_{t+1}=\left[R_{t}+\left(1-\delta\right)\right]K_{t}+W_{t}L_{t}+\Pi^{N}_{t}-C_{t},
\label{eq:budget_constraint}
\end{equation}
where $K_t$ is capital, $R_t$ is the rental rate, $W_{t}$ is the wage rate and $\Pi^{N}_{t}=\sum_{j} \Pi_{j}^{N}$ are the profits accruing from all the firms in the economy net of fixed production costs. Capital depreciates at rate $0\leq\delta\leq1$ and factor prices $R_{t}$ and $W_{t}$ are taken as given. The representative household therefore maximizes (\ref{eq:HH_utility}) subject to (\ref{eq:budget_constraint}). Our choice of GHH preferences implies that the aggregate labor supply is a simple function of the wage rate $L_{t} = W_{t}^{1/\nu}$, where $\nu$ is the inverse of the wage elasticity of labor supply.\footnote{
From the perspective of the household, labor and entrepreneurial decisions are separable. We abstract from an occupational decision problem (becoming an entrepreneur \textit{versus} working) for simplicity. This assumption does not however imply that there is a fixed supply of entrepreneurs, since the equilibrium number of firms/entrepreneurs will be endogenous.}

\subsection{Technology}

There is a final good (the \textit{numeraire}), which is a CES aggregate of $I$ different industries $ Y_{t}=\left(\sum_{i=1}^{I}{\vphantom{\Pi^P}y}_{it}^{\rho}\right)^{1/\rho}, $ where $y_{it}$ is the quantity of industry $i\in\left[0,1\right]$, and $\sigma_{I} = {1}/{(1-\rho)}>1$ is the elasticity of substitution
across industries.

$I$ is assumed to be large, so that each individual industry has a negligible size in the economy. The output of each industry $i$ is itself a CES
composite of differentiated goods or varieties $ y_{it}=\left(\sum_{j=1}^{n_{it}}{\vphantom{\Pi^P}y}_{jit}^{\eta}\right) ^{1/\eta}, $ where $n_{it}$ is the number of active firms in industry $i$ at time $t$ (to be determined endogenously) and $\sigma_{G} = 1/(1-\eta) > 1$ is the within-industry
elasticity of substitution. Following \cite{AB},
we assume that goods are more easily substitutable within industries than across industries: 
%\begin{assumptionf} 
$0<\rho<\eta\leq1$.
%\end{assumptionf} 
Given these assumptions, the inverse demand for each variety $j$ in industry $i$ is given by
\begin{equation}
p_{ijt}=\left(\dfrac{Y_{t}}{y_{it}}\right)^{1-\rho}\left(\dfrac{y_{it}}{y_{ijt}}\right)^{1-\eta}.\label{eq:inv_demand_good}
\end{equation}
We assume that in every industry $i\in\left\{0,\ldots,I\right\}$ there is a maximum number of entrepreneurs $N \in \mathbb{N}$, so that $n_{it} \leq N$. Entrepreneur $j$ can produce his variety
by combining capital $k_{ijt}$ and labor $l_{ijt}$ through a Cobb-Douglas
technology
\begin{equation}
y_{it}=\underbrace{e^{a_{t}}\;\gamma_{ij}}_{\tau_{ijt}}\left(k_{ijt}\right)^{\alpha}\left(l_{ijt}\right)^{1-\alpha}.\label{eq:CD_pf}
\end{equation}
Note that the productivity of each entrepreneur $\tau_{ijt}$ is the product of two terms (i) a time-varying aggregate component $e^{z_{t}}$
(common to all industries and types) and (ii) a time-invariant idiosyncratic
term $\gamma_{ij}$. We refer to $z_{t}$ as aggregate productivity and to $\gamma_{ij}$ as $j$'s idiosyncratic productivity. Aggregate productivity $a_{t}$ follows an auto-regressive process $ a_{t}=\phi_{a}a_{t-1}+\varepsilon_{t}$, with $\varepsilon_{t}\sim N \left(0,\sigma_{\varepsilon}^{2}\right)$. With no loss of generality,
we order idiosyncratic productivities according to $\gamma_{i1}\geq\gamma_{i2}\geq\gamma_{i3}>\cdots.$ 
Labor is hired at the competitive wage $W_{t}$ and capital at the
rental rate $R_{t}$. Entrepreneur $j$ can thus produce
her variety with marginal cost $\Theta_{t} / \tau_{ijt}$,
where 
\[
\Theta_{t}\equiv\left(\frac{R_{t}}{\alpha}\right)^{\alpha}\left(\frac{W_{t}}{1-\alpha}\right)^{1-\alpha}
\]
is the marginal cost function for a Cobb-Douglas technology with unit
productivity. We refer to $\Theta_{t}$ as the \textit{factor
cost index}. In addition to all variable costs, the production of each variety entails a fixed production cost $c_{i} \geq 0$ per period (which can be possibly different across industries). Such a cost is in units of the \textit{numeraire}.\footnote{According to this formulation, fixed production costs do not change with factor prices. We introduce variable fixed costs in an extension (Appendix \ref{subsec:var_fixed_costs}).}


\subsection{Market Structure \label{subsec:Market-Structure}}

To conclude the description of the model, we must specify the way firms interact. We assume that all firms that enter (and thus incur the fixed cost $c_{i}$) play a static Cournot game: they will simultaneously announce quantities,
taking the output of the other competitors as given.\footnote{We follow \cite{AB} and assume
that firms enter sequentially in reverse order of productivity.} 
Therefore, each entrepreneur $j$ solves 
\begin{equation}
\begin{array}{cl}
\underset{y_{ijt}}{\textrm{max}}\quad\left(p_{ijt}-\dfrac{\Theta_{t}}{\tau_{ijt}}\right)y_{ijt}\qquad\text{s.t.}\; & p_{ijt}=\left(\dfrac{Y_{t}}{y_{it}}\right)^{1-\rho}\left(\dfrac{y_{it}}{y_{ijt}}\right)^{1-\eta}\\
& y_{it}=\left(\sum\limits_{k=1}^{n_{it}}y_{kit}^{\eta}\right)^{\frac{1}{\eta}}.
\end{array} \label{eq:Cournot_problem}
\end{equation}
The solution to (\ref{eq:Cournot_problem}) yields a system of $n_{it}$ non-linear equations in $\left\{ p_{ijt}\right\}_{j=1}^{n_{it}}$ (one for each firm)\footnote{
This system of first order conditions admits a close-form solution only in the limit case in which there is no differentiation within an industry ($\eta = 1$), as shown in Appendix \ref{Cournot_eta_1}.}
\begin{equation}
p_{ijt} = \underbrace{\dfrac{1}{\eta-\left(\eta-\rho\right)s_{ijt}}}_{\mu_{ijt}} \,  \dfrac{\Theta_{t}}{\tau_{ijt}},\label{eq:firm_FOC}
\end{equation}
where $s_{ijt}$ is the market share of firm $j=1,\ldots,n_{it}$ and $\mu_{ijt}$ is the markup. Equation (\ref{eq:firm_FOC}) establishes a positive relationship between market shares and markups. This happens because firms internalize the impact of size on the price they charge $p_{ijt}$; large firms end up restricting output disproportionately more (relative to productivity), thereby charging a high markup. 
Moreover, as equation (\ref{eq:firm_FOC}) also highlights, market shares are themselves a positive function of RTFP $p_{ijt} \: \tau_{ijt}$. Our model thus features a positive association between revenue productivity, size and markups. Therefore, a shock that generates larger productivity differences across firms will also lead to larger markup dispersion.

To conclude the description of the industry equilibrium, we need to determine the number of active firms $n_{it}$. To this end, let $ \Pi\left( \, j \, , \, n_{it} \, , \, \mathcal{F}_{it} \, , \, X_{t} \, \right) \coloneqq \left(p_{it}-{\Theta_{t}}/{\tau_{ijt}}\right)y_{ijt}$ denote the equilibrium profits of firm $j\leq n_{it}$ in industry $i$ (gross of the fixed production cost), when there are $n_{it}$
active firms, given a productivity distribution $\mathcal{F}_{it} \coloneqq \left\{ \, \gamma_{i1} \, , \, \gamma_{i2} \, , \, \ldots  \, \right\}$ and a vector of aggregate variables $X_{t}\coloneqq\left[ \, a_{t} \, , \, Y_{t} \, , \, \Theta_{t} \, \right]$. The equilibrium number of firms must be such that (i) the profits of each active firm are not lower than the fixed cost $c_{i}$ and (ii) if an additional firm were to enter, its profits would be lower than the fixed cost. Mathematically, an interior solution $n^{*}_{it} < N$ to the equilibrium number of firms must satisfy
\begin{equation}
\left[\Pi\left({\color{blue}n_{it}^{*}},{\color{blue}n_{it}^{*}},\mathcal{F}_{i},X_{t}\right)-c_{i}\right]\left[\Pi\left({\color{blue}n_{it}^{*}+1},{\color{blue}n_{it}^{*}+1},\mathcal{F}_{i},X_{t}\right)-c_{i}\right]\leq0 .\label{eq:eqm_n_firm}
\end{equation}
Lemma \ref{lemma:(Profit-Function)} in Appendix \ref{subsec:Profits} provides an analytical characterization of the profit function under the special case of $\eta=1$. In particular, we show that the profits of any firm $j$ increase in its own idiosyncratic productivity $\gamma_{ij}$ and decrease in the idiosyncratic productivity
of all the other firms $\gamma_{ik}$. Therefore, as top firms increase their productivity level, small firms make lower profits and become closer to their break even point (\textit{ceteris paribus}). This is key to understand some aggregate results that we describe next.

\subsection{General Equilibrium}
\paragraph{Equilibrium Definition}
We start by defining an equilibrium for this economy. Denoting the history of
aggregate productivity shocks by $ A^{t} = \{ a_{t}, a_{t-1}, ...\} $ we have the following definition.
\begin{definition}[Equilibrium]
A general equilibrium consists of a sequence of household policies  $ \left\{ C_{t}\left(A^{t}\right), K_{t}\left(A^{t}\right), L_{t}\left(A^{t}\right)\right\} $, firm policies $ \left\{ y_{ijt}\left(A^{t}\right), k_{ijt}\left(A^{t}\right), l_{ijt}\left(A^{t}\right)\right\} $, and a set of active firms $\left\{ n_{it}\left(A^{t}\right)\right\}_{i=1}^{I}$ such that i) households optimize; ii) all active firms optimize; iii) all active firms do not make a loss: iv) no additional firm is willing to enter; v) capital and labor markets clear.
\end{definition}


\subsubsection{Static Equilibrium}
We now describe the general equilibrium of this economy. We start by focusing on a static equilibrium, in which we describe production and labor supply decisions, taking the aggregate level of capital $K_{t}$ as given. Later on, we describe the equilibrium dynamics.

\paragraph{Aggregate Production Function} Given a $\left(I\times N\right)$
matrix of productivity draws $\mathbf{A}_{t}$ and a vector of active firms
$\mathbf{N}_{t} \equiv \left\{ n_{it}\right\}_{i=1}^{I}$, aggregate output can be written as 
\begin{equation}
Y_{t}={A}_{t}\Phi\left(\mathbf{\Gamma},\mathbf{N}_{t} \right)\;L_{t}^{1-\alpha}K_{t}^{\alpha} .\label{eq:agg_prod_fct}  
\end{equation}
The term $\Phi\left(\cdot\right)$ 
represents the endogenous component of aggregate TFP and is a function of the number of active firms, individual firm productivities and market shares. An expression for $\Phi\left(\mathbf{\Gamma},\mathbf{N}_{t}\right)$ is provided in Appendix \ref{subsec:Aggregate-TFP}.

\paragraph{Factor Markets}
The aggregate factor demand schedules for labor $L_t$ and capital $K_t$ are given by
\begin{equation}
\begin{array}{cl}
W_{t} \; = &  \left(1-\alpha\right)\;{A}_{t} \: \Omega\left(\mathbf{\Gamma},\mathbf{N}_{t}\right)\;\Phi\left(\mathbf{\Gamma},\mathbf{N}_{t}\right)\;L_{t}^{-\alpha}\,K_{t}^{\alpha},\\[1ex]
R_{t} \; = &  \alpha\;{A}_{t} \: \Omega\left(\mathbf{\Gamma}, \mathbf{N}_{t}\right)\;\Phi\left(\mathbf{\Gamma},\mathbf{N}_{t}\right)\;L_{t}^{1-\alpha}\,K_{t}^{\alpha-1}.
\end{array} \label{eq:factor_demand}  
\end{equation}
where $\Omega\left(\cdot\right) = \left(W_{t}\,L_{t} + R_{t}\,K_{t} \right)/Y_{t} $ is the aggregate factor share. An analytical expression for $\Omega\left(\mathbf{\Gamma}, \mathbf{N}_{t} \right)$ in provided in Appendix \ref{subsec:Factor-Prices}. These two demand schedules can be combined with the labor and capital supply equations
\begin{align}
     L_{t}^{S} = W_{t}^{1 / \nu}  \quad \text{and} \quad K_{t}^{S} = K_{t} 
\label{eq:factor_supply}  
\end{align}
to determine the factor market equilibrium.
% Combining equations (\ref{eq:factor_demand}) and (\ref{eq:factor_supply}) we can obtain an expression for equilibrium employment
% \begin{equation}
% L_{t} = \left[\left(1-\alpha\right)\Theta\left(\mathbf{A}_{t},\mathbf{N}_{t}\right)\right]^{\frac{1}{\nu+\alpha}}K_{t}^{\frac{\alpha}{\nu+\alpha}}. \label{eq:labor_mkt_eq}  
% \end{equation}
Combining equations (\ref{eq:factor_demand}) and (\ref{eq:factor_supply})  with (\ref{eq:agg_prod_fct}), we can write aggregate output as a function of the aggregate capital stock $K_t$, the productivity distribution $\mathbf{\Gamma}$ and the set of active firms $\mathbf{N}_{t}$
\begin{equation}
Y_{t}=\left[\left(1-\alpha\right)\Omega\left(\mathbf{\Gamma},\mathbf{N}_{t}\right)\right]^{\left(1-\alpha\right)/\left(\nu+\alpha\right)}\left[ {A}_{t} \, \Phi\left(\mathbf{\Gamma},\mathbf{N}_{t}\right) K_{t}^{\alpha}\right]^{\left(1+\nu\right)/\left(\nu+\alpha\right)}. \label{eq:agg_output_capital}
\end{equation}
To conclude the characterization of the static equilibrium, we must determine the set of active firms $\mathbf{N}_{t}$.

\paragraph{Equilibrium Set of Firms}

The number of active firms in each industry $i$ is  jointly determined by equations (\ref{eq:factor_demand}),  (\ref{eq:agg_output_capital}) and the set of inequalities defined in (\ref{eq:eqm_n_firm}). Such a joint system does not admit a general analytical characterization. We can nevertheless characterize the particular case in which all industries are identical. Proposition \ref{A-symmetric-equilibrium} states the conditions for a symmetric equilibrium with $n$ firms per industry.

\begin{prop}[Existence of Symmetric Equilibrium]
\label{A-symmetric-equilibrium} Suppose that all industries have the same distribution of idiosyncratic productivities $\mathcal{F}_{i}=\mathcal{F}$. Then, there can be a symmetric equilibrium with $n$ firms per industry if $K_{t}$ is such that
\[
\underline{K}\left(\mathcal{F},n\right)\leq K_{t}\leq\overline{K}\left(\mathcal{F},n\right),
\]

The bounds $\overline{K}\left(\cdot\right)$ and $\underline{K}\left(\cdot\right)$ are both increasing in $n$.
\end{prop}
\begin{proof}
See Appendix \ref{subsec:numb-active-firms}.
\end{proof}
Intuitively, $K_{t}$ must be (i) sufficiently large so that all existing $n$ firms can break even, (ii) but cannot be too high, for otherwise an additional firm could profitably enter in at least one industry.

\subsubsection{Equilibrium Dynamics}
We are now ready to explore the dynamic properties of our economy. To determine the model dynamics we need to characterize the law of motion
\begin{align*}
    K_{t+1} = \left(1-\delta\right) K_{t} + s_{t} \cdot Y_{t}
\end{align*}
where $s_{t}$ is the aggregate savings rate. 
We start by observing a necessary condition for the existence of multiple steady states.
\begin{remark}\label{remarkmultiplicity}
Steady state multiplicity can arise provided that either of the following is holds:
\begin{itemize}
    \item the saving rate $s$ can be locally increasing in capital;
    \item output $Y$ is not a strictly concave function of capital.
\end{itemize}
\end{remark}
This remark simply provides necessary conditions for the capital law of motion to feature non-concavities. When the law of motion is not strictly concave it can cross the 45 degree line multiple times, which is the definition of steady state multiplicity.
We now formalize in two propositions that both necessary conditions in Remark \ref{remarkmultiplicity} can hold in our model. 

Even though we cannot derive an analytical expression for the savings rate, we can nevertheless characterize it on a steady-state. In particular we are interested in how it changes with the number of active firms, and therefore with capital, and with the degree of firm heterogeneity. In the Appendix we provide two intermediate Lemmas which we summarise here. Lemma \ref{prop:ss_agg_s_rate} shows that the steady-state savings rate is proportional to the aggregate factor share $\Omega^{*}$. Lemma \ref{prop:The-aggregate-factor-share} shows that $\Omega(\cdot)$ increases in the number of active firms and decreases in the level of firm heterogeneity. The following proposition is an immediate consequence.

\begin{prop}\label{heterogeneity_savings} [Steady-State Savings Rate]
The steady-state savings rate $s^*=s\left(\mathbf{\Gamma},\mathbf{N}^{*}\right)$
\begin{enumerate}
    \item increases in the number of active firms. As the number of firms is weakly increasing in capital, the saving rate can increase in capital.
    \item decreases in the level of firm heterogeneity. 
\end{enumerate}
\end{prop}

\begin{proof}
Follows immediately from Lemma \ref{prop:ss_agg_s_rate} and \ref{prop:The-aggregate-factor-share}.
\end{proof}

The previous proposition states two important results. First, from Lemma \ref{prop:The-aggregate-factor-share} the larger is the number of firms per industry, the more intense is the degree of product market competition and hence the aggregate factor share $\Omega\left(\cdot\right)$. Second, the aggregate factor share decreases when the distribution of individual productivities becomes more dispersed. Intuitively, in every industry, high productivity firms are larger and charge higher markups. As large firms are able to increase their markups even further, the aggregate profit share increases and the aggregate factor share decreases. Proposition \ref{heterogeneity_savings} states that these changes in capital and labor shares translate into a changes in the steady-state savings rate. In turn, this implies that we can have multiplicity of steady states as the saving rate can increase in capital.

We now turn to the second condition of Remark \ref{remarkmultiplicity} and formalize the relationship between output and capital in the next Proposition.

This result is the cornerstone on which we build our multiplicity argument. As firm heterogeneity increases, this compresses factor shares, thereby decreasing the saving rate. As the saving rate declines it is harder for firm 

\paragraph*{Law of Motion}
To better illustrate some of the model dynamics, let us consider the example of an economy where all industries are ex-ante identical (i.e. same distribution idiosyncratic productivities $\mathcal{F}_{i}=\mathcal{F}$) and with no aggregate productivity shocks (i.e. $a_{t} = 1$). Furthermore, let us set $\eta=1$ so that there is no love for variety within an industry.
The left panel of Figure \ref{fig:Law-of-Motion-Homog-UE} shows the law of motion for a particular parameter configuration.
The law of motion is not globally concave and exhibits two steady-states: one where all industries are a monopoly, $K^{*}\left(1\right)$, and another where all industries are a duopoly, $K^{*}\left(2\right)$.\footnote{The existence of exactly two steady-states is obviously not guaranteed. Figures \ref{fig:Unique_ss} and \ref{fig:Three_ss} in Appendix \ref{subsec:Steady-State} show examples of economies with one or three steady-states.} The steady-state to which the economy will converge depend on its initial condition. 
The right panel of Figure \ref{fig:Law-of-Motion-Homog-UE} represents $K_{t+1}$ and a function of $R_{t+1}$. As one can see, the rental rate is not strictly decreasing in the capital stock. It contains an increasing segment in the region consisting of the \textit{transition} from full monopolies to full duopolies. This can be understood from equation (\ref{eq:factor_demand}) \textendash{} a larger capital stock, by allowing more firms to break even and enter, results in a higher aggregate factor share $\Omega\left(\cdot\right)$; this can in turn result in a higher rental rate. Steady-state multiplicity occurs whenever the rental rate map in the right panel of Figure \ref{fig:Law-of-Motion-Homog-UE} crosses the steady-state rental rate more than once.\footnote{Evaluating the steady-state Euler equation we obtain $R^{*} = \beta^{-1} - \left(1-\delta\right)$}

Such a convexity occurs because of the interplay between factor supply and competition. As $K_{t}$ increases, the economy moves towards a more competitive regime, with a larger factor share $\Omega\left(\mathbf{\Gamma},2\right) > \Omega\left(\mathbf{\Gamma},1\right)$. A larger factor share results in a higher wage and labor supply (resulting in larger $Y_{t}$ for a given $K_{t}$), but also in a higher savings rate (resulting in larger $K_{t+1}$ for a given $Y_{t}$).

Note that despite the existence of two steady-states, this example features a unique equilibrium: there is a unique value of $K_{t+1}$ for each value of $K_{t}$ (the state
variable). Figure \ref{fig:Static-Equilibrium} in Appendix \ref{subsec:Static-Equilibrium-Characterization} characterizes the behavior of the rental rate.


\begin{figure}[ht!]
\centering{}
\hspace{-0.2cm}
 \includegraphics[scale=0.475]{input/LOM_baseline}
 \hspace{0.4cm}
 \includegraphics[scale=0.475]{input/RR_baseline}
\caption{Law of Motion and Rental Rate Map \label{fig:Law-of-Motion-Homog-UE}
\protect \\ {This example features two stable steady states and an unstable one. We use $\psi \, = \, 1 \,$, $\delta \, = \, 1 \,$, $\alpha \, = \, 1/3 \,$, $\rho \, = \, 3/4 \,$, $\eta \, = \, 1 \,$, $\nu \, = \, 2/5 \,$ and $ c_{i} \, = \, 0.015 \,$.}} 
\end{figure}



This simple law of motion already provides a theory for some of the facts described in the introduction. Suppose that the economy starts in a neighborhood of the high steady-state $K^{SS}_{2}$ but is hit by a temporary shock that brings capital close to $\overline{K}\left(1\right)$. The economy will then enter the basin of attraction of the low steady-state $K^{SS}_{1}$ and experience a persistent drop in aggregate output, a persistent decline in the labor share and an increase in the profit share. Viewed through the lens of this model, a transition to a less competitive regime can explain the deviation of output from trend after 2008. 

However, as discussed in the introduction, several signs suggest a long-run increase in market power since at least the 1980. This seems to be associated with rising firm heterogeneity and a reallocation of activity towards large firms (\cite{VR}). Since these trends can have a direct impact on our mechanism, we ask what are the dynamics consequences of rising firm heterogeneity. We will also discuss the consequences of rising fixed costs.

\paragraph*{Mean Preserving Spread}

We start by discussing the impact of a mean-preserving spread (MPS) to the distribution of productivities [FOR ACTIVE FIRMS?]. We will assume that all industries are identical and there is no within-industry product differentiation $\left(\eta=1\right)$. These two assumptions are crucial to obtain an analytical characterization of the model's steady-state(s). The first result pertains to the impact of an MPS on the steady-state level of capital.

\begin{prop} [Mean Preserving Spread and Steady-State Capital] \label{prop:MPS} Let $\eta = 1$ and suppose that all industries are identical to start ($\gamma_{ij} = \gamma_{j} \; \forall i$). Let ${K}^{*}\left(n\right)$ be a steady-state with $n$ firms in every industry. Let $\Gamma_n=\left\{\gamma_1,\ldots,\gamma_n\right\}$ be the vector of productivity of the $n$ active firms and $\tilde\Gamma_n$ be a mean-preserving spread of $\Gamma_n$. The following holds
\begin{enumerate}[label=\alph*)]
    \item $K^{*}(\tilde\Gamma,n)<K^{*}(\Gamma,n)$.
    \item Suppose $n=2$, if $\rho>1-\nu\frac{1-\alpha}{1+\nu\alpha}$, then $\chi_2(\tilde\Gamma)<\chi_2(\Gamma)$.
\end{enumerate}
%\[ \dfrac{\partial {K}^{*}\left(n\right)}{\partial\lambda} \leq 0. \]
\end{prop}
\begin{proof}
See Appendix \ref{subsec:basin_attraction}.
\end{proof}

Proposition \ref{prop:MPS_Kss} states that, if there exists a steady-state where all industries are identical and have $n$ firms, the steady-state level of capital necessarily shrinks after a MPS to the productivities of these $n$ firms. The proof of this proposition is illustrated in the top left panel of Figure \ref{fig:Comparative-Statics}. We show

A MPS results in a lower factor cost index $\Theta\left(\mathbf{\Gamma}, \mathbf{N}_{t}\right) \; = \; \Omega\left(\mathbf{\Gamma}, \mathbf{N}_{t}\right)\;\Phi\left(\mathbf{\Gamma},\mathbf{N}_{t}\right)$. This depresses the rental rate for all levels of capital with $n$ firms. Therefore, the new steady-state (given by the intersection with $R^{ss}$ necessarily shrinks. 

The previous proposition characterizes the behavior of the steady-state level of capital ${K}^{*}\left(n\right)$. To evaluate fragility, one needs however to study the behavior of the unstable steady-state $\underline{B}\left(n\right)$. This is crucial to know whether the left side of the basin of attraction $\left[\underline{B}\left(n\right), {K}^{*}\left(n\right)\right]$ shrinks. If $\underline{B}\left(n\right)$ does not fall as fast as ${K}^{*}\left(n\right)$ (or increases), the basin of attraction necessarily shrinks. 
Note that, even when all industries are ex-ante identical, an unstable steady-state necessarily features industry heterogeneity: some industries will have $n$ firms, while others will have $n-1$ firms. This makes it impossible to give a full analytical characterization of its properties. Nevertheless, we can provide a sufficient condition under which $\underline{B}\left(n\right)$ increases. This is stated in the next proposition for the particular case of $n=2$ firms. Proposition \ref{prop:MPS_BA_n} in Appendix \ref{Proofs-Additional-Results} extends the result for $n$ firms.

\begin{prop} [Mean Preserving Spread and Fragility, n=2] \label{prop:MPS_BA} Let $\eta = 1$ and suppose that all industries are identical to start ($\gamma_{ij} = \gamma_{j} \; \forall i$). Let ${K}^{*}\left(n\right)$ be a steady-state with $n=2$ firms. Let $\lambda$ be a mean-preserving spread on $\left\{\gamma_1,\gamma_2\right\}$. Then, if
\[
\rho>1-\nu\frac{1-\alpha}{1+\nu\alpha}
\]
we have that
\[ \dfrac{\partial \underline{B}\left(2\right)}{\partial\lambda} > 0. \]
\end{prop}
\begin{proof}
See Appendix \ref{subsec:basin_attraction}.
\end{proof}
The proof of Proposition \ref{prop:MPS_BA} is provided in Appendix . The proof provides a sufficient condition under which an MPS shifts down the increasing part of the rental rate map in Figure \ref{fig:Comparative-Statics}.

We should stress that Proposition \ref{prop:MPS_BA} provides a sufficient condition under which $\underline{B}\left(n\right)$ increases after an MPS. It is therefore possible that $\underline{B}\left(n\right)$ even when the previous condition is not satisfied. Furthermore, the basin of attraction can also increase even when $\underline{B}\left(n\right)$ shrinks (provided that it does not shrink as fast as ${K}^{*}\left(n\right)$).


\begin{corollary} Suppose that the condition in Proposition \ref{prop:MPS_BA} is satisfied, then
% \[
% \rho>1-\nu\frac{1-\alpha}{1+\nu\alpha}
% \]
if ${K}^{*}\left(n\right)$ is the highest steady-state, then its basin of attraction $\left(\underline{B}\left(n\right),\infty \right)$ shrinks.
\end{corollary}

% \begin{corollary}
% The following holds:
% \begin{itemize}
%     \item if labor supply is inelastic ($\nu\rightarrow\infty$), an MPS increases fragility  if $\alpha<1/(2-\rho)$ ;
%     \item if labor supply is isoelastic ($\nu=1$), an MPS increases fragility  if $\alpha<\rho/(2-\rho)$;
%     \item if labor supply is perfectly elastic ($\nu=0$), an MPS increases fragility  if $\rho>1$, which is impossible.
% \end{itemize}
% Finally, fixing $\rho$,
% $\nu^\star(\alpha)$: the pair $(\nu^\star(\alpha),\alpha)$ satisfies the condition in Proposition \ref{prop:basin_attraction_MPS} is increasing and convex in $\alpha$.
% \end{corollary}

\textbf{DISCUSSION OF PROPOSITION AND COROLLARIES}


\begin{figure}[ht!]
\centering{}%
\begin{tabular}{cc}
	\hspace{-1cm} \includegraphics[scale=0.45]{input/RR_MPS} &  \hspace{-0.2cm}
	\includegraphics[scale=0.45]{input/RR_cf} \\
	\hspace{-1cm} 
	\includegraphics[scale=0.45]{input/LOM_MPS.eps} & 
	\hspace{-0.2cm}
	\includegraphics[scale=0.45]{input/LOM_cf}
\end{tabular}
\caption{Comparative Statics \protect \\ {The left panels represent the effect of a MPS on the rental rate and the law of motion of capital (in an economy with two steady-states). The right panels represent the effect of an increase in fixed costs. We use $\alpha \, = \, 1/3 \,$, $\rho \, = \, 3/4 \,$, $\eta \, = \, 1 \,$, $\nu \, = \, 2/5 \,$ and $ c_{i} \, = \, 0.015 \,$.}} 
\label{fig:Comparative-Statics}
\end{figure}


% \begin{figure}[ht!]
% \begin{minipage}[b]{.5\linewidth}
% \centering{}\includegraphics[scale=0.465]{input/lom_lf_2_paper.eps}\subcaption{Larger productivity differences \label{fig:Law-of-Motion-Heterog}}
% \end{minipage}%
% \begin{minipage}[b]{.5\linewidth}
% \centering{}\includegraphics[scale=0.465]{input/lom_fc.eps}\subcaption{Larger fixed costs \label{fig:Law-of-Motion-Fixed-Cost}}
% \end{minipage}
% \caption{Law of motion (comparative statics) \protect \\ {Note: \small{} the figure shows changes in the law of motion of capital after an increase in productivity differences (Panel (a)) and in fixed costs (Panel (b)). We use $\psi \, = \, 1 \,$, $\delta \, = \, 1 \,$, $\alpha \, = \, 1/3 \,$, $\rho \, = \, 0.6 \,$, $\eta \, = \, 1 \,$ and $\nu \, = \, 0.4 \,$.}} \label{fig:lom_comp_statics}
% \end{figure}



% \begin{figure}[ht!]
% \begin{minipage}[b]{.5\linewidth}
% \centering{}\includegraphics[scale=0.465]{input/rr_leader_follower.eps}\subcaption{Larger productivity differences}
% \end{minipage}%
% \begin{minipage}[b]{.5\linewidth}
% \centering{}\includegraphics[scale=0.465]{input/rr_leader_follower_2.eps}\subcaption{Mean-preserving spread }
% \end{minipage}
% \end{figure}



\paragraph*{Rising Fixed Costs} The decline in product market competition since the 1980s may be also explained, through the lens of our model, by rising fixed costs. Higher fixed costs, will drive out of the market firms that exactly break even. This will result in higher average markups and concentration. How can larger fixed costs affect the law of motion represented in Figure \ref{fig:Law-of-Motion-Homog-UE}? First, we can show that if a steady-state with $n$ firms exists, and all firms make strictly positive profits, the existence and level of such a steady-state $\left(K^{SS}_{n}\right)$ will not be affected by a marginal increase in $c_f$ (see Appendix \ref{subsec:basin_attraction} for a proof). A larger fixed cost will however result in a larger level of aggregate capital consistent with $n$ firms per industry, $\underline{K}\left(n\right)$ (see Appendix \ref{subsec:numb-active-firms}). Therefore, the basin of attraction of the largest steady-state shrinks, as shown in Figure \ref{fig:Comparative-Statics}. This means that rising fixed costs also make the highest steady-state more fragile, so that now even relatively small shocks can trigger a transition to the the low competition trap. This result is stated in the next proposition.

\begin{prop}[Fixed Cost and Fragility] \label{prop:basin_attraction_cf} Let ${K}^{*}\left(\mathbf{\Gamma}, \mathbf{N}_{t}\right) $ be a steady-state with a set of active firms $\mathbf{N}_{t}$. Then we have that

\[ \dfrac{\partial \underline{B}\left(n\right)}{\partial c_{i} } > 0 \quad \text{and} \quad \dfrac{\partial {K}^{*}\left(n\right)}{\partial c_{i}} \leq 0. \]

\end{prop}
\begin{proof} See Appendix \ref{subsec:basin_attraction}.
 \end{proof}

The left panels of Figure \ref{fig:Comparative-Statics} illustrates the effect of an increase in fixed costs. For simplicity, we represent an economy where all industries are ex-ante identical (same distribution of productivities and identical fixed costs). The two declining segments of the rental rate map represent a situation of full monopoly and full duopoly; since all firms make strictly positive profits in these regions, the equilibrium is unchanged as $c$ increases marginally. Things are however different in the increasing segment, where some firms are exactly breaking even. In this case, some firms are driven out of the market. The rental rate is lower and the unstable steady-state increases.


\paragraph{Discussion}
We conclude by summarizing two keys insights of our theory, which we think are relevant to understand the US growth experience after 2008. The first is that a complementarity between competition and factor supply can generate multiple competition regimes or steady-states. A transition from a high competition to a low competition regime can in many aspects describe the 2008 recession and the subsequent great deviation. Second, changes in technology that result in larger market power (e.g. larger productivity differences across firms or larger fixed costs) make high competition regimes more difficult to sustain, and transitions to low competition traps easier to occur. Our model therefore suggests that the US economy, experiencing a long-run increase in markups and concentration since the 1980s, became increasing vulnerable to transitions like this.

We next use a calibrated version of our model to ask whether it can replicate the behaviour of the US economy in the aftermath of the 2008 crisis. We also perform some counterfactual exercises to quantify the impact of rising market power.


==> submitted_version/0_z_abstract.tex <==
We study how firm heterogeneity and market power affect macroeconomic fragility, defined as the probability of long slumps. We propose a theory in which the positive interaction between firm entry, competition and factor supply can give rise to multiple steady-states. We show that when firms are highly heterogeneous in terms of productivities, even small temporary shocks can trigger firm exit and make the economy spiral in a competition-driven poverty trap. We calibrate our model to incorporate the well-documented trends on rising firm heterogeneity in the US economy, and show that they significantly increase the likelihood and length of slow recoveries. We use our framework to study the 2008\textendash{}09 recession and show that the model can rationalize the persistent deviation of output and most macroeconomic aggregates from trend, including the behavior of net entry, markups and the labor share. Post-crisis cross-industry data corroborates our proposed mechanism. We conclude by showing that firm subsidies can be powerful in preventing long slumps and can lead to up to a 21\% increase in welfare.


% abstract till 02/10/2022
%%We study how firm heterogeneity and market power affect macroeconomic fragility, defined as the probability of long-lasting recessions. We propose a theory in which the positive interaction between firm entry, competition and factor supply can give rise to multiple steady-states. We show that when firm heterogeneity is large, even small temporary shocks can trigger firm exit and make the economy spiral in a competition-driven poverty trap. Calibrating our model to incorporate the well-documented trends in increasing firm heterogeneity in the US economy, we find that, relative to 2007, an economy with the 1990 level of firm heterogeneity is 1.5 to 2 times less likely to experience a deep recession. We use our framework to study the 2008\textendash{}09 recession and show that the model can rationalize the persistent deviation of output and most macroeconomic aggregates from trend, including the behavior of net entry, markups and the labor share. Post-crisis cross-industry data corroborates our proposed mechanism. We conclude by showing that firm subsidies can be powerful in preventing quasi-permanent recessions and can lead to up to a 21\% increase in welfare.


%% abstract till 29/09/21

% We investigate how firm heterogeneity and market power affect macroeconomic fragility, defined as the probability of persistent recessions. 
% We provide a theory in which temporary aggregate shocks trigger changes in competition and can lead to quasi-permanent recessions. In our RBC model with oligopolistic competition and free entry, high firm heterogeneity increases the sensitivity of the entry margin to business cycle fluctuations. This, in turn, acts as an amplifier of aggregate fluctuations and can lead to deep and long-lasting downturns. 
% We use a quantitative version of our model to study the response of the US economy to the Great Recession of 2008-09. The model can rationalize the persistent deviation of output and most macroeconomic aggregates from trend. In counterfactual exercises, we find that, relative to 2007, an economy with the 1985 level of firm heterogeneity is 5 to 9 times less likely to experience a recession like 2008-9. Cross-industry data corroborates our proposed mechanism.
% Policy can help escape these Firm subsidies can be effective in preventing quasi-permanent recessions and can lead to a 21\% increase in welfare.




%Policies targeted at reducing the responsiveness of the competitive environment to aggregate shocks can increase welfare by avoiding quasi-permanent downturns.


%% abstract 16/07/21
% We investigate the connection between long-run changes in market structure and the deviation of the US economy from its long run trend after the 2008-9 crisis. 
% We provide a theory in which temporary negative aggregate shocks trigger changes in the competitive environment that can lead to deep quasi-permanent recessions. In our RBC model with oligopolistic competition and free entry, the magnitude of the changes in the market structure increases with the degree of firm heterogeneity in the economy. 
% We use a quantitative version of our model to study the response of the US economy to the Great Recession of 2008-09. The model can rationalize the persistent deviation of output and most macroeconomic aggregates from trend. In counterfactual exercises, we find that if the aggregate shocks of 2008-9 had hit an economy with lower firm heterogeneity we would not have observed such a deep and persistent recession. Quantitatively, an economy with the 1985 level of firm heterogeneity is 5-9 less likely to experience a recession like 2008-9.
% We show that policies targeted at reducing the responsiveness of the competitive environment to aggregate shocks can significantly increase welfare by avoiding quasi-permanent recessions.





%%% OLD ABSTRACT %%%%

%We study the impact of firm heterogeneity and market power on aggregate fluctuations. We build a multi-industry growth model with oligopolistic competition, endogenous entry and variable markups. Our model features a complementarity between capital accumulation and competition, which can give rise to multiple competition regimes. Some regimes are characterized by a large capital stock and strong competition while others feature low capital and weak competition. We show that the degree of firm heterogeneity, through its effects on competition, significantly changes the endogenous response to aggregate fluctuations. In particular, when firm heterogeneity is high, the economy becomes significantly more likely to move from a high to a low competition regime in the aftermath of a negative aggregate shock. 
%We use a quantitative version of our model to study the response of the US economy to the Great Recession of 2008-09. We show that our model can rationalize the persistent deviations of output and most macroeconomic aggregates from trend. In counterfactual exercises, we show that if the aggregate shocks of 2007 had hit an economy with lower firm heterogeneity we would not have observed such a deep and persistent recession. Quantitatively, an economy with the 1985 level of firm heterogeneity is 63\% less likely to experience a fall in output larger than 10\%. %We conclude by providing suggesting cross-industry evidence of our mechanism and by studying the ability of policy to alleviate the endogenous amplification of negative shocks.
%We conclude by providing cross-industry evidence in support of our model and by studying different policy interventions.
%We develop a multi-industry growth model with oligopolistic competition and variable markups. Our model features a complementarity between capital accumulation and competition, which can give rise to multiple competition regimes \textendash{} regimes characterized by a large capital stock and strong competition and regimes featuring low capital and weak competition (\textit{low competition traps}).
%Negative transitory shocks can trigger a transition from a high to a low competition regime. We also show that, as the firm size/markup distribution becomes more dispersed, the economy is increasingly likely to enter a \textit{low competition trap}. 
%In a calibrated version of our model, a transition from a high to a low competition regime rationalizes important features of the US great recession and its aftermath, such as the persistent drop in output and aggregate TFP, the decline of the labor share, the increase in the profit share, and the decline in the number of firms.

==> submitted_version/1_introduction10.tex <==
\section{Introduction}

The US economy appears to be recovering more slowly from its recessions. The left panel of Figure \ref{intro_figure} shows, for different recessions, the change in detrended output in the first two years after the trough. Over the postwar period the pace of recoveries has significantly slowed down. 
This has been especially clear for the last three recessions \citep[][]{gali2012slow}. As shown in the right panel of Figure \ref{intro_figure}, four years after the beginning of each recession, detrended output was still below its pre-crisis value. For the 2008-2009 crisis, the gap is substantial (about 10 log points below trend) and has been referred to as the \textit{long slump} or \textit{great deviation} \citep[][]{H_slump}. During the same period, the US experienced a significant increase in firm heterogeneity along several dimensions, such as productivity, size and markups. This is illustrated in Figure \ref{intro_figure_2}, which shows the evolution of the standard deviation of sales for US public firms.\footnote{The figure focuses on listed firms, but increasing firm-level dispersion has been documented using census data, and focusing on narrowly defined industries. Several studies have documented rising firm differences in terms of i) revenue TFP \citep{ACG,K, DHJM2}, ii) size \citep{BCG, ADKPR}, and iii) markups \citep{LEU,CCM,DLT}. See \cite{VR} for a summary of the recent findings.} In this paper we argue that the slowdown in the pace of US recoveries can be partially explained by the rise of firm heterogeneity.
\begin{figure}[H]
\centering{}%
\begin{tabular}{ccc}
     \hspace{-1cm} \includegraphics*[scale=0.4]{input/US_postwar_recoveries} &
     \hspace{0.75cm}
     \includegraphics*[scale=0.4]{input/US_last_3_recessions}
\end{tabular}
\caption{\small{} Recovery from US Recessions\protect \\ {Note: \footnotesize{} The left panel shows, for each US postwar recession, the change in detrended output in the first two years after the trough. We use quarterly real GDP per capita (in logs, from BEA) and compute a linear trend for the period 1947-2019. We consider all recessions that lasted longer than 6 months according to the NBER. The right panel shows the evolution of detrended output for the 1990-1991, 2001 and 2008-2009 recessions.}} 
\label{intro_figure}
\end{figure}

The main contribution of this paper is to show that rising firm heterogeneity can have a significant impact on business cycle fluctuations, and result in a higher probability of long slumps. We refer to such a probability as \textit{macroeconomic fragility}. We show this in the context of an RBC model with oligopolistic competition, endogenous firm entry and elastic capital and labor supply. We use a quantitative version of our framework to study the effects of the trends in rising firm heterogeneity. We find that these forces are quantitatively important, they can rationalize episodes such as the 2008-2009 recession and its aftermath and are consistent with cross-industry empirical evidence from the \textit{great deviation}.

\begin{figure}[htb]
\centering{}%
\includegraphics*[scale=0.6]{input/std_log_ms_1960} 
\hspace{0.4cm}
\includegraphics*[scale=0.6]{input/ratio_fixed_costs}
\caption{\small {}Long-Run Trends for US Public Firms\protect \\ {Note: \footnotesize{} Data is from COMPUSTAT. The left panel shows the standard deviation of log sales for US public firms. The right panel shows the average ratio of fixed to total costs. Following \cite{GW}, we define fixed costs as the sum of `Selling, General and Administrative Expenses' (COMPUSTAT item XSGA), `Advertising Expenses'
(Compustat item XAD) and `R\&D Expenditures'  (Compustat item XRD). Total costs are the sum of fixed costs and variable costs, where the latter correspond to the `Cost of Goods Sold' (Compustat item COGS).}} 
\label{intro_figure_2}
\end{figure}


%A growing body of evidence suggests that the US and other advanced economies have been undergoing decades of increasing firm-level heterogeneity along several dimensions, such as productivity, size and markups as shown in Figure \ref{intro_figure}.\footnote{Several studies have documented rising firm differences in terms of i) revenue TFP \citep{ACG,K, DHJM2}, ii) size \citep{BCG, ADKPR}, and iii) markups \citep{LEU,CCM,DLT}.  See \cite{VR} for a summary of the recent findings.} A seemingly unrelated observation is that over the last century the length and depth of recessions has been growing, as evidenced by Figure \ref{intro_figure}. In this paper we argue that the rise in firm heterogeneity can potentially explain the increasing occurrence of slow recoveries. We show that, beyond the well understood static effects, these trends can significantly alter the dynamic behavior of an economy. In particular, we show that rising firm heterogeneity can result in a higher probability of deep and long-lasting recessions. We refer to such a probability as \textit{macroeconomic fragility}. These effects, we find, are quantitatively important and can can rationalize the increasing occurrence of slow recoveries.  


At the heart of our model is a complementarity between competition and factor supply. First, economies with intense competition in product markets feature low profit shares and high factor shares and factor prices, which induce high factor supply. Second, high factor supply allows more firms to enter the market, which results in greater competition. This complementarity can give rise to multiple competition regimes or (stochastic) steady-states. A key contribution of our theory is to show that rising heterogeneity in idiosyncratic TFP can make transitions from high to low steady-states more likely to occur. When firm heterogeneity increases, large, productive firms expand, while small, unproductive firms contract. As a consequence, smaller negative shocks can be enough to trigger firm exit and a transition to a steady-state featuring lower competition, capital and output. An identical result is obtained when fixed costs of production increase. We characterize these results formally by showing that the minimum size (negative) shock required to trigger a transition from a high to a low steady-state decreases when firm TFP heterogeneity rises or when fixed costs increase. 

% QUANTITATIVE RESULTS

To quantify these economic forces, we provide three calibrations of our model, where we target US firm-level moments in 1975, 1990 and 2007. These different calibrations differ in the level of fixed costs and in the degree of TFP dispersion (which both increase over time). We first find that, while the 1975 economy is characterized by a unimodal ergodic distribution of output, the 1990 and 2007 feature bimodal distributions (an indication of two stochastic steady-states). Second, when we subject the three economies to the same shocks, the 2007 economy exhibits significantly greater amplification and propagation. For example, we find that the 2007 economy experiences a recession greater than 10\% every 75 years, while the 1990 and 1975 economies experiences one every 120 and 735 years respectively. This suggests that rising firm heterogeneity and fixed costs made the US economy significantly more fragile and more prone to long-lasting slumps.

We also use our model economy as a laboratory to study the Great Recession and its aftermath. The 2008 crisis was marked by a large and persistent deviation of output and other aggregates from trend, something unusual in the entire postwar period. For example, in 2019, output per capita was 14\% below its pre\textendash2007 trend, a deviation far larger and persistent than in previous recessions (Figure \ref{fig:great_deviation_figure}). We ask whether our model can replicate such a quasi-permanent drop in aggregate output and other aggregate variables. To this end, we feed our 2007 economy a sequence of shocks calibrated to match the behavior of aggregate TFP in 2008\textendash9 and study the economy's response. The model generates the observed persistent deviation from trend of GDP as well as of investment, hours and aggregate TFP. It also explains the sharp and persistent drop of the labor share after 2008. Importantly, when we subject the 1990 and 1975 economies to the same shocks, the model does not predict such a persistent deviation from trend. %This suggests that rising firm heterogeneity has rendered the US economy more vulnerable to quasi-permanent recessions as in 2008.


%% EMPIRICS

We also provide empirical evidence in favor of our proposed mechanism. Our theory provides predictions in terms of cross-industry responses to the business cycle. In particular, for any two industries with the same number of firms, the one with a higher level of heterogeneity reacts more to a negative shock. We test this prediction in the data using concentration as a proxy for heterogeneity in US 6-digit industries. Consistent with our model predictions, we show that industries that were more concentrated in 2007 experienced greater cumulative declines in the number of firms, the labor share and economic activity over the 2008-2016 period.

%% POLICY

In terms of policy lessons from our theory, %we ask whether we can design an effective policy to curb the endogenous amplification of aggregate shocks. 
we show that firm subsidies can be effective in preventing deep recessions, leading to a welfare gain of up to 21\% in consumption-equivalent terms. The fundamental intuition behind this result is that in our economy firms' entry and exit decisions have externalities as they change market power. A planner may then find it beneficial to trade off the efficiency loss attached to less productive firms staying in the market with the reduction in the rents of more productive firms. This policy lesson is specific to our model and to the pivotal role of the extensive margin in shaping the degree of aggregate market power. Its logic, however, is more general. Cyclical changes in market power can amplify aggregate fluctuations. Policies that aim to keep the degree of product market competition high can prevent the economy from entering into low output regimes and thereby improve welfare.



\paragraph{Related Literature}

Our paper speaks to three different strands of the literature. First, it is related to the macroeconomic literature studying models of coordination failures \citep{CJ1,Mat,BenhabibFarmer,FarmerGuo,herrendorf2000ruling,big_push_distorted_economies}. While we are not the first to show how multiple equilibria and/or steady-states can arise in a context of imperfect competition and variable markups \citep{MP,CCR,RW,GZ,J},\footnote{Without relying on multiple equilibria or steady-states, \cite{CJ2}, \cite{EC}, \cite{BGM} and \cite{Gamber} show that a combination of imperfect competition with endogenous entry amplifies aggregate fluctuations.} we contribute to this literature by studying the role of firm-level heterogeneity in shaping macroeconomic \textit{fragility}. As we discuss, this concept is distinct from the \textit{existence} of steady-state multiplicity. We also provide a quantification of our mechanism and link it to the 2008 crisis.\footnote{Our paper speaks to the literature on the cyclicality of markups, which includes \cite{RS}, \cite{rotemberg1991markups}, \cite{JF}, \cite{BKM}, \cite{nekarda2020cyclical} and \cite{AVB}.}

Second, this paper relates to a large and growing literature documenting long-term trends in firm heterogeneity and market power. There are several signs that indicate rising market power in the US and other advanced economies. For example, \cite{ADKPR} use data from the US census to document rising sales and employment concentration, while \cite{AA2} document a rise in patenting concentration. Other studies have documented a secular rise in price-cost markups. Using data from national accounts, \cite{H} finds that the average sectoral markup
increased from 1.12 in 1988 to 1.38 in 2015. \cite{LEU} document a steady increase in sales-weighted average markups for US public firms between 1980 and 2016.\footnote{\cite{EMX} show that a cost-weighted average markup displays a less pronounced trend. See also \cite{T}, \cite{KN2} and \cite{BHKZ} on trends in markups.} This was driven by both an increasing share of large firms and by rising dispersion in the markup distribution.
%\footnote{Identical findings are obtained by \cite{CCM} and \cite{DFVS} for different countries.} 
%In our model, rising dispersion in size and markups is driven by increasing productivity differences. Several studies have documented a secular increase in productivity differences across firms \citep{ACG,K,DHJM2}. 
Close to our approach, \cite{de2021quantifying} argue that declining dynamism and rising market power can be explained, among other channels, by increasing productivity dispersion and fixed costs. \cite{EMX} estimate that the welfare cost of markups can be large and represent a loss of up to 25\% in consumption-equivalent terms.%\footnote{\cite{EGB} builds a search model with heterogeneous firms to study the impact of rising productivity dispersion on the labor share.}
%Lastly, \cite{EMX} use a model close to ours to compute the welfare costs generate by markups via three main channels: i) output reduction, ii) misallocation, and iii) distorted entry.
We contribute to this literature by investigating the business cycle implications of these trends, and in particular their impact on the 2008 crisis and the subsequent \textit{great deviation}. We emphasize that increased firm heterogeneity and market power may have negative welfare consequences through an increase in macroeconomic fragility.

Lastly, this paper relates to the literature studying slow recoveries and the persistent impact of the 2008 crisis. A large part of this literature has focused on the secular decline in interest rates and/or the possibility of liquidity traps, which constrains monetary policy \citep{gali2012slow,BF,guerrieri_lorenzoni,eggertsson_et_al,mian_sufi_straub}, or on the long-run consequences of R\&D decisions \citep{queralto2020model,fasil2021heterogeneous}. Close to this paper, \cite{ST} build an RBC model with complementarities in capacity utilization choices among monopolistic firms to generate multiple steady-states. We too use coordination to obtain multiplicity and interpret the post\textendash{}2008 deviation as a transition to a low steady-state. Differently from their work, we study the role of heterogeneity in productivities in oligopolistic markets with variables markups. We complement their analysis, and the aforementioned literature, by arguing that rising firm-level heterogeneity has increased the likelihood of slumps. Our theory can also account for number of trends observed after 2008, such as the acceleration in the labor share decline, the acceleration of markup growth, and the decline in the number of firms.

The rest of the paper is organized as follows. Section \ref{sec: general framework text} sets the general framework and provides the first result relating to technology and fragility. Section \ref{sec:Model} presents a growth model with oligopolistic competition and derives the main theoretical results. Section \ref{sec:Quantitative-Evaluation} discusses the calibration and presents the quantitative results. Section \ref{sec:aggregatefacts} provides and extended application to the US great recession and its aftermath, and presents the cross-industry empirical evidence. In Section \ref{policy}, we study the welfare effects of fiscal policy in our model. Finally, section \ref{sec:Conclusion} concludes.

==> submitted_version/2_general_problem.tex <==
\section{General Framework}\label{sec: general framework text}
In this section we introduce the concept of macroeconomic fragility. We do so in the context of a general economy, featuring a representative household, endogenous factor supply, and a large number of product markets (characterized by an endogenous number of firms, variable markups and love-for-variety).
We proceed by first describing the economy. We then define macroeconomic fragility and study how it changes with firm-level heterogeneity. In Section \ref{sec:Model} we impose additional structure to this general framework, by developing an RBC model with oligopolistic competition.  This allows us to derive sharper predictions and analytical results.

\subsection{Primitives}\label{general_description}
\paragraph{Demographics}
The economy contains an infinitely-lived representative household, who has time separable utility $U = \sum_{t=0}^{\infty} \beta^{t}u\left(C_{t},L_{t}\right)$.  The household can save by investing in capital, which depreciates at rate $\delta$. The household earns rental and wage rates $R_{t}$ and $w_{t}$, determined in competitive factor markets.
\paragraph{Technology}
There is a final good (used for consumption and investment), which is given by a homothetic aggregator of different varieties. The economy contains $I \in \mathbb{N}^{+}$ product markets and within each product market there is a unit mass of identical submarkets or locations (e.g. different towns where a supermarket can locate).\footnote{We adopt this formulation only for tractability reasons, to make the aggregate number of firms a continuously differentiable variable, in spite of the existence of a finite number of product markets $I$.} Every product submarket is characterized by a maximum number of players $M \in \mathbb{N}^{+}$, each of which can produce a differentiated variety. Operating in a given submarket of product market $i$ requires a per period fixed cost $c_i$ (in units of the final good). Firms purchase factors of production in competitive factor markets, but imperfectly compete in product markets. Firms produce according to $\tilde{F}\left(\gamma,L,K\right) = \gamma \cdot F\left(L,K\right)$ where $\gamma$ is idiosyncratic TFP and $ F\left(L,K\right)$ is a constant returns to scale production function satisfying the Inada conditions.
The technology set is further described by a matrix of Hicks-neutral idiosyncratic productivities $\Gamma \coloneqq \big[\gamma_{ij}\big]_{\left(I\times M\right)}$ and a vector of fixed costs $\mathcal{C} \coloneqq \big[c_{i}\big]_{\left(I\times 1\right)}$. 
%The elements of each row of $\Gamma$ appear in decreasing order, so that $\gamma_{ij} \geq \gamma_{ij+1}$ (i.e. more productive firms are ranked first).\footnote{These assumptions are with no loss of generality. If an industry can only have a maximum of $M<N$ firms, this can be modeled as $\gamma_{ij}=0 \; \forall j \geq M+1$.} To simplify the exposition, we assume that firms have identical fixed costs $c_{ij} = c$ and that, within a market, firms enter sequentially in decreasing order of productivity.\footnote{Therefore, if firm $\gamma_{ij}$ is active, all firms $k$ with $\gamma_{ik}>\gamma_{ij}$ are also active.}
Given these definitions, the technology set is summarized by $\Lambda \coloneqq \left[\:\Gamma\,,\:\mathcal{C}\,\right]$.
The aggregate mass of firms can be written as $ n =
\sum_{i=1}^{I} \, \sum_{m=1}^{M} \, \eta_{im} \, m$, where $\eta_{im}\in\left[0,1\right]$ is the share of locations within product market $i$ with $m=1,\ldots,M$ firms. We assume that firms enter sequentially and that firms making higher profits enter first. Given these assumptions, the aggregate mass of firms $n$ and the technology set $\Lambda$ fully characterize the set of active firms. For exposition purposes, we work with a deterministic setting subject to one time unexpected shocks. In particular, we think of the possibility of shocks that destroy a fraction $1 -\chi \in \left[0,1\right]$ of the capital stock. Aggregate uncertainty, by means of stochastic TFP, is introduced in the model we study in Section \ref{sec:Model}.

\begin{definition}[Equilibrium]
An equilibrium in this economy is a set of policies such that i) all agents optimize; ii) all active firms make no loss; iii) inactive firms would make a loss upon entry and iv) all markets clear. 
\end{definition}

This economy admits an aggregate production function representation which we characterize in the following lemma.

\begin{lemma}[Aggregate Production Function \label{lemma: agg_pf}]
The aggregate production function is given by \[ F(\Lambda, K, n\left(\Lambda,K\right))= \Phi(\Lambda,n\left(\Lambda,K\right)) \, F(K,L), \]
where $\Lambda$ is the technology set (as defined above), $n$ is the mass of active firms, and $\Phi(\cdot)$ is aggregate TFP. Finally $F(K,L)$ is the CRS production function introduced above.\footnote{Note that $L$ is a function of the set of state variables $\left(\Lambda,K\right)$. For ease of notation we suppress these. }
\end{lemma}
\begin{proof}
See Appendix \ref{appendix:proofs_section_2}.
\end{proof}

Aggregate TFP $\Phi(\Lambda,n\left(\Lambda,K\right))$ reflects two terms: a weighted average of firm level productivity $\gamma_{ij}$ and love for variety. From the aggregate production function it is possible to characterize the economy's inverse demand for capital. Let $\Omega$ denote the aggregate factor share (i.e. the ratio of total labor and capital payments over gross output $Y$). As shown in Appendix \ref{appendix:proofs_section_2},  the equilibrium rental rate can be written as
\begin{align} \label{eq:rr_map}
R(\Lambda,K) \; =  \; \Omega(\Lambda,n\left(\Lambda,K\right)) \, \Phi(\Lambda,n\left(\Lambda,K\right)) \,  F_{K}\big(K, L \big) . 
\end{align} 
It is convenient to define $\Theta\left(\Lambda,n\right)\coloneqq\Omega(\Lambda,n) \, \Phi(\Lambda,n)$, which represents a measure of aggregate factor prices (Appendix \ref{appendix:proofs_section_2}).
\footnote{This is equal to the Lagrange multiplier of the cost minimization problem for a firm with unit productivity.}
Given the demographic structure of this economy, the long-run supply of capital is infinitely elastic and given by\footnote{This can be obtained by evaluating the stationary Euler equation of the representative household.}
\begin{align}
R^{*} = \beta^{-1} - \left(1-\delta\right).
\end{align}
Therefore, the economy features multiple steady-states if the following equation admits more than one solution
\begin{align}
    R(\Lambda,K) = R^{*} .
    \label{rmap}
\end{align}
The red curve in Figure \ref{fig:multiplicity_figure} represents the capital demand schedule in eq. (\ref{eq:rr_map}) for a particular economy. Assuming that the Inada conditions are satisfied, we have $R(\Lambda,0)=\infty$ and $R(\Lambda,\infty)=0$. Therefore, multiple steady-states occur only if (\ref{eq:rr_map}) features at least one increasing part. As explained in Section \ref{appendix:generalframework} of the Supplementary Material, there are different mechanisms that can make $R\left(\cdot\right)$ locally increasing in $K$.
%\footnote{They can be grouped into three broad sets of mechanisms: reallocation, love for variety and market power. We exclude, by assumption, increasing returns in $F\left(\cdot\right)$ and backward bending labor supply. See Section \ref{appendix:generalframework} of the Supplementary Material.}
For example, suppose that firm entry increases in capital, so that competition and the aggregate factor share $\Omega(\Lambda,n)$ are also increasing in $K$. Then, if $\Omega(\Lambda,n)$ increases sufficiently fast in $K$ in some region, it can counteract decreasing returns $F_{K}\left(\cdot\right)$ and make $R(\cdot)$ locally increasing. In Figure \ref{fig:multiplicity_figure}, the economy in red contains two stable steady-states, $K_{1}^{S}$ and $K_{2}^{S}$, and an unstable one, $K_{1}^{U}$. The initial capital stock determines the unique path that the economy follows and the steady-state to which it converges.\footnote{When the economy starts on the left of $K_{1}^{U}$ it reaches $K_{1}^{S}$, otherwise it achieves $K_{2}^{S}$. Multiple paths would be possible if the curve in Figure \ref{fig:multiplicity_figure} was a correspondence, and not a function. In this section, we exclude multiple paths by assumption.} We are particularly interested in the possibility of downward transitions across steady-states. Note that, if the economy starts close to the high steady-state $K_{2}^{S}$, a transition to $K_{1}^{S}$ occurs if the economy is hit by a shock that destroys a fraction $1 - K_{1}^{U}/K_{2}^{S}$ of its capital stock. Thus, the likelihood of a downward transition depends on the distance between $K_{1}^{U}$ and $K_{2}^{S}$. For example, under the alternative economy represented in blue, a smaller fraction of the capital stock needs to be destroyed for a downward transition to take place, $1 - \tilde{K}^U_{1}/\tilde{K}^S_{2}$. This second economy is characterized by a lower capital demand schedule for sufficiently high values of $K$. This suggests that a reduction in the aggregate demand for capital can be associated with a higher likelihood of downward transitions across steady-states. We next formalize the concept of \textit{fragility} and explore different mechanisms that, by decreasing the aggregate demand for capital, can result in more likely downward transitions.

\begin{figure}[htb]
    \centering
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=1pt,y=1pt,yscale=-.75,xscale=.75]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Axis 2D [id:dp775497830869011] 
\draw [line width=3]  (15.6,253.42) -- (641.6,253.42)(78.2,27.52) -- (78.2,278.52) (634.6,248.42) -- (641.6,253.42) -- (634.6,258.42) (73.2,34.52) -- (78.2,27.52) -- (83.2,34.52)  ;
%Straight Lines [id:da9277312210637947] 
\draw [line width=3]  [dash pattern={on 7.88pt off 4.5pt}]  (79,151) -- (616.6,151.52) ;
%Curve Lines [id:da6180121553167277] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=3]    (96.6,57.52) .. controls (107.6,98.52) and (185.6,179.52) .. (216.6,199.52) ;
%Curve Lines [id:da05797439702758567] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=3]    (215,199.52) .. controls (243.6,177.52) and (257.6,168.52) .. (296.6,105.52) ;
%Curve Lines [id:da5620343829511387] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=3]    (295,105.52) .. controls (368.6,137.52) and (484.6,195.52) .. (577.6,217.52) ;


%Curve Lines [id:da333283432121507] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=3]    (112.6,56.52) .. controls (123.6,97.52) and (201.6,178.52) .. (232.6,198.52) ;
%Curve Lines [id:da4772784121211848] 

\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=3]    (231,198.52) .. controls (254.6,181) and (257.6,186) .. (302.6,126) ;
%Curve Lines [id:da8188162523653961] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=3]    (301,126) .. controls (374.6,158) and (492.6,216) .. (583.6,238) ;

% Text Node
\draw (623,269.4) node [anchor=north west][inner sep=0.75pt]    {$K$};
% Text Node
\draw (32,24.4) node [anchor=north west][inner sep=0.75pt] {$R(K)$};
% Text Node
\draw (50,143.4) node [anchor=north west][inner sep=0.75pt] {$R^{*}$};


%% STEADY STATES
%Straight Lines [id:da6720868559709041] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (161,150) -- (160.6,254.52) ;
%Straight Lines [id:da006637350827901178] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (265,151) -- (264.6,255.52) ;
%Straight Lines [id:da7659322515454083] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (396,151) -- (395.6,255.52) ;
% Text Node
\draw (145,263) node [color={rgb, 255:red, 208; green, 2; blue, 27 }][anchor=north west][inner sep=0.75pt]    {$K_{1}^{S}$};
% Text Node
\draw (249,263) node [color={rgb, 255:red, 208; green, 2; blue, 27 }][anchor=north west][inner sep=0.75pt]    {$K_{1}^{U}$};
% Text Node
\draw (387,263) node [color={rgb, 255:red, 208; green, 2; blue, 27 }][anchor=north west][inner sep=0.75pt]    {$K_{2}^{S}$};


%Straight Lines [id:da6720868559709041] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (181,150) -- (180.6,254.52) ;
%Straight Lines [id:da006637350827901178] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (285,151) -- (284.6,255.52) ;
%Straight Lines [id:da7659322515454083] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (366,151) -- (365.6,255.52) ;
% Text Node
\draw (175,263) node [color={rgb, 255:red, 74; green, 144; blue, 226 }][anchor=north west][inner sep=0.75pt]    {$\tilde{K}_{1}^{S}$};
% Text Node
\draw (283,263) node [color={rgb, 255:red, 74; green, 144; blue, 226 }][anchor=north west][inner sep=0.75pt]    {$\tilde{K}_{1}^{U}$};
% Text Node
\draw (353,263) node [color={rgb, 255:red, 74; green, 144; blue, 226 }][anchor=north west][inner sep=0.75pt]    {$\tilde{K}_{2}^{S}$};


\draw[fill={rgb, 255:red, 208; green, 2; blue, 27 },opacity=.3] (265,151) -- (264.6,255.52) -- (395.6,255.52)--  (396,151)  -- cycle;

\draw[fill={rgb, 255:red, 74; green, 144; blue, 226 },opacity=.3]  (285,151) -- (284.6,255.52) -- (365.6,255.52) -- (366,151) -- cycle;

\end{tikzpicture}
    \caption{Steady-state multiplicity}
    \label{fig:multiplicity_figure}
\end{figure}
\subsection{Technological Change and Fragility}
% Let $\mathcal{K}$ be the ordered set of capital levels in steady-states and $\mathcal{K^U}$ the collection of even elements of $\mathcal{K}$, which represent capital levels in unstable steady-states.\footnote{Note that we use even and odd elements as they correspond to unstable and stable steady-states, which are defined according to the local slope of $R(\cdot)$. }
We start by defining the concept of fragility, which is central to our analysis. Let $\mathcal{K}$ denote the ordered set of all steady-states capital levels. Let $\mathcal{K^S}$ be the collection of stable steady-states and $\mathcal{K^U}$ be the collection of unstable steady-states in $\mathcal{K}$. %\footnote{Note that $\mathcal{K^U}$ and $\mathcal{K^A}$ are respectively given by the set odd and even elements of $\mathcal{K}$)}
%\begin{definition}[Steady-States Transitions]\label{defitinitionSS}
%Define an upward transition as the economy moving from the $n-1^{th}$ element of the set $\mathcal{K}$ to the $n+1^{th}$ element, $\forall n \text{ even}$. Define a downward transition as the economy moving from the $n+1^{th}$ element of the set $\mathcal{K}$ to the $n-1^{th}$ element, $\forall n $ even. 
%\end{definition}
Recall that, in our setting, the economy can be hit by a one time unexpected shock that destroys a fraction $1-\chi$ of the capital stock.\footnote{The intuition behind all our results carries through under more general shock structures, with some adjustments. In general the capital level in a steady state depends on the shock realization. This would significantly increase the difficulty in defining a norm between $\mathcal{K}_{n}$ and $\mathcal{K}_{n-1}$, since their distance would become a random variable itself.} Our measure of fragility captures the proximity of a \textit{stable} steady-state $\mathcal{K}^S_{n}$ to the preceding \textit{unstable} steady-state $\mathcal{K}^{U}_{n-1}$. The closer these two steady-states are to each other, the lower is the minimum shock needed to trigger a downward transition.

\begin{definition}[Fragility]\label{definitionfragility}
Let $\chi_{n}\in[0,1]$ be defined as $\chi_{n} \coloneqq \mathcal{K}^U_{n-1} / \mathcal{K}^S_{n}$. It follows that $1 - \chi_{n}$ is the minimum size shock needed to make the economy move from $\mathcal{K}^S_{n}$ to $\mathcal{K}^S_{n-1}$. We call an increase in $\chi_{n}$ an increase in fragility. 
\end{definition}

%\begin{definition}[Fragility]\label{definitionfragility}
%Let $\chi_{n+1}\in[0,1]$ be defined as $\chi_{n+1} \coloneqq \mathcal{K}^U_n / \mathcal{K}_{n+1}$. It follows that $1 - \chi_{n+1}$ is the minimum size shock needed to trigger a downward transition from $\mathcal{K}_{n+1}$. We call an increase in $\chi_{n+1}$ an increase in fragility. 
%\end{definition}
Two further observations should be made. First, our main focus is on \textit{fragility}, which is different from the \textit{existence} of multiplicity. Although the first requires the second, these are different concepts. Second, the notion of \textit{fragility} is related to, but distinct from, the idea of the \textit{stability} of a steady-state. We think of \textit{fragility} as the possibility of downward transitions only. This is the size of the left partition of the basin of attraction of the steady-state, which is given by $\mathcal{K}^S_{n}-\mathcal{K}^U_{n-1}$. The notion of stability, instead, relates to the size of the whole basin of attraction and also accounts for the possibility of upward transitions.

The fundamental question which interests us is how a change in a technology parameter, $\partial \lambda$, affects $\chi_{n}$. In Proposition \ref{propcompstatexrc} we state a sufficient condition for a technology shift to increase fragility, i.e. $\partial  \chi_{n}/{d \lambda}>0$. This condition says that fragility increases when the rental rate decreases for intermediate values of $K$ (i.e. in the region between steady-states). This depends on the response of $\Theta\left(\cdot\right)$ to a technology shift.

\begin{prop}[Comparative Statics]\label{propcompstatexrc}
Let $\mathcal{K}^S_{n}$ be a stable steady-state and consider a technological shift $ d \lambda $. Then $\partial \chi_{n}/{d \lambda}>0$, i.e. the stable steady-state $\mathcal{K}^S_{n}$ becomes more fragile, if for $ K=\{\mathcal{K}^U_{n-1}, \, \mathcal{K}^S_{n}\} $
\begin{align}\nonumber
    &\frac{\partial}{ \partial  \lambda} \Theta\left(\Lambda,n\left(\Lambda,K\right)\right) = \Theta_{\lambda}\left(\Lambda,n\left(\Lambda,K\right)\right)+\Theta_{n}\left(\Lambda,n \left(\Lambda,K\right)\right)n_{\lambda}\left(\Lambda,K\right)   <0.
\end{align}
Using the definition of $\Theta(\cdot)$ we note that this is equivalent to
\begin{align}\nonumber
\hspace{-1cm}
\underbrace{\Omega(\Lambda,n)\Phi_{\lambda}(\Lambda,n)}_{\Delta \: \textrm{TFP}} \; + \;
\underbrace{\Omega_{\lambda}(\Lambda,n)\Phi(\Lambda,n)}_{\Delta \: \textrm{factor share}} \; + \;
\underbrace{\left[\Omega_{n}(\Lambda,n)\Phi(\Lambda,n) +
\Omega(\Lambda,n)\Phi_{n}(\Lambda,n)\right]n_{\lambda}\left(\Lambda,K\right)}_{\Delta \: \textrm{number of firms}} \; < \; 0 .
\end{align}
The first two terms characterize the direct effect of $ d \lambda $ on aggregate TFP and the factor share. The last term describes the effect of changes in the number of active firms. 

\end{prop}

\begin{proof}
See Appendix \ref{appendix:proofs_section_2}
\end{proof}

Proposition \ref{propcompstatexrc} provides a sufficient condition for a (technology-driven) increase in fragility. There are three main channels highlighted in this result: i) changes in aggregate TFP $\left(\Phi\right)$, ii) changes in the factor share $\left(\Omega\right)$ and iii) changes in the number of firms $\left(n\right)$.\footnote{We study these channels in detail in the Supplementary Materials through Remarks \ref{fixedfirms}, \ref{fixedaggTFP} and \ref{loveforvariety}.} To connect this result to the empirical patterns discussed in the introduction, we can think of $\partial  \lambda$ as an increase in firm level heterogeneity. Through the lens of Proposition \ref{propcompstatexrc} such an increase can trigger higher fragility by reducing the factor share (due to greater market power), via the reallocation of activity towards less productive firms or by reducing the number of active firms. If firms' market shares are increasing in their productivity, as heterogeneity increases three things happen: \textit{i)} a mechanical efficiency gain due to large firms becoming more productive and through positive reallocation; \textit{ii)} a compression of factor shares as large firms can exert more market power; \textit{iii)} entry is harder for firms outside the market, which can generate a loss of varieties and higher market power. 
Intuitively, if the anti-competitive forces \textit{ii)} and \textit{iii)} dominate the efficiency gains from higher heterogeneity \textit{i)}, the return to capital decreases and it becomes harder to sustain a high steady-state. 

The intuition behind the result described in Proposition \ref{propcompstatexrc} is similar in spirit to the findings of \cite{baqaee2020productivity} and \cite{EMX} relating dispersion and aggregate TFP. As will become clearer in the model presented in Section \ref{sec:Model}, we put forth the additional effect on the stability of the economy with respect to aggregate fluctuations. Our economy features an endogenous amplification mechanism that can trigger non-linearities in the response to shocks. As firms become more heterogeneous these non-linearities become more salient and the economy can be more likely to experience quasi-permanent slumps. To dig deeper into the forces underlying the effect of heterogeneity on fragility we specify a RBC model in which firms compete oligopolistically. This additional structure allows us to provide sharper theoretical and quantitative results.


%Any of these channels is theoretically sufficient to make the economy more fragile. In the next section we specify a model in which to address the problem quantitatively. We embed the workhorse oligopolistic competition model of \cite{AB} in an otherwise standard RBC setting. 

==> submitted_version/3_model3.tex <==
\section{A Model with Firm Heterogeneity and Variable Markups\label{sec:Model}}
The model presented in this section builds upon the neoclassical growth model, with a representative household that supplies labor and capital. The technology side is comprised of a large number of product markets, where firms compete oligopolistically as in \cite{AB}.
We start by describing the demand side and the technology structure. Then we analyze the equilibrium of a particular product market (taking aggregate variables as given). Finally, we characterize the general equilibrium.
\subsection{Preferences}
Time is discrete and indexed by $t=0,1,2,\ldots$.
There is a representative, infinitely-lived household with lifetime utility
\begin{align}
U_{t}=\mathbb{E}\sum_{t=0}^{\infty}\:\beta^{t}\:U\left(C_{t},L_{t}\right),
\end{align}
where $0 < \beta < 1$ is the discount factor, $C_{t} \geq 0$ is consumption of the final good and $L_{t} \geq 0$ is labor.
We adopt the period utility function as in \cite{GHH}
\begin{align}
U\left(C_{t},L_{t}\right)=\dfrac{1}{1-\psi}\left(C_{t}-\dfrac{L_{t}^{1+\nu}}{1+\nu}\right)^{1-\psi},
\label{eq:HH_utility}
\end{align}
where $0 \leq \psi \leq 1$ is the inverse of the intertemporal elasticity of substitution and $\nu>0$ is the inverse of the Frisch elasticity of labor supply. 
% we should probably mention what psi and nu are. i know we do it later, but still

The representative household contains many individual members, which are denoted by $j$. Each individual member can run a firm in the corporate sector. We assume that if two or more individuals run a firm in the same product market, they behave in a non-cooperative way \textendash{} i.e. they compete against each other and do not collude. Nevertheless, all individuals pool together the profits they make. Hence there is a single dynamic budget constraint\footnote{We assume that the economy features perfect financial markets. There is a stock market where individuals can trade firms (whose price equals the NPV of profits). Since stocks and capital must offer the same expected return $E_{t} \{R_{t+1}\}$, firm transactions among individuals do not affect the aggregate budget constraint.}
\begin{align}
K_{t+1}=\left[R_{t}+\left(1-\delta\right)\right]K_{t}+W_{t}L_{t}+\Pi^{N}_{t}-C_{t},
\label{eq:budget_constraint}
\end{align}
where $K_t$ is capital, $R_t$ is the rental rate, $W_{t}$ is the wage rate and $\Pi^{N}_{t}=\sum_{j} \Pi_{jt}^{N}$ are the profits from all firms $j$ net of fixed costs. Capital depreciates at rate $0\leq\delta\leq1$ and factor prices $R_{t}$ and $W_{t}$ are taken as given. The representative household maximizes (\ref{eq:HH_utility}) subject to (\ref{eq:budget_constraint}). Our choice of GHH preferences implies that the aggregate labor supply is given by $L^{S}_{t} = W_{t}^{1/\nu}$.
%\footnote{
%From the perspective of the household, labor and entrepreneurial decisions are separable. We abstract from an occupational decision problem (becoming an entrepreneur \textit{versus} working) for simplicity. This assumption does not however imply that there is a fixed supply of entrepreneurs, since the equilibrium number of firms/entrepreneurs will be endogenous.}

\subsection{Technology}

There is a final good (the \textit{numeraire}), which is a CES aggregate of $I$ different product markets $ Y_{t}=\left(\sum_{i=1}^{I}{\vphantom{\Pi^P}y}_{it}^{\rho}\right)^{1/\rho}, $ where $y_{it}$ is the quantity of product market $i$, and $\sigma_{I} = {1}/{(1-\rho)}>1$ is the elasticity of substitution across product markets. $I$ is assumed to be large, so that each individual product market has a negligible size in the economy. The output of each product market $i\in\left\{1,\ldots,I\right\}$ is itself a CES
composite of differentiated goods or varieties $ y_{it}=\left(\sum_{j=1}^{n_{it}}{\vphantom{\Pi^P}y}_{jit}^{\eta}\right) ^{1/\eta}, $ where $n_{it}$ is the number of active firms in product market $i$ at time $t$ (to be determined endogenously) and $\sigma_{G} = 1/(1-\eta) > 1$ is the within product market
elasticity of substitution. Following \cite{AB},
we assume that goods are more easily substitutable within product market than across product markets: 
%\begin{assumptionf} 
$0<\rho<\eta\leq1$.
%\end{assumptionf} 
Given these assumptions, the inverse demand for each variety $j$ in product market $i$ is given by
\begin{align}
p_{ijt}=\left(\dfrac{Y_{t}}{y_{it}}\right)^{1-\rho}\left(\dfrac{y_{it}}{y_{ijt}}\right)^{1-\eta}.\label{eq:inv_demand_good}
\end{align}
We assume that in every product market $i$ there is a maximum number of entrepreneurs $M \in \mathbb{N}$, so that $n_{it} \leq M$. Entrepreneur $j$ can produce her variety
by combining capital $k_{ijt}$ and labor $l_{ijt}$ through a CRS
technology
\begin{align}
y_{it}=\underbrace{{A_t}\;\gamma_{ij}}_{\tau_{ijt}}\left(k_{ijt}\right)^{\alpha}\left(l_{ijt}\right)^{1-\alpha}.\label{eq:CD_pf}
\end{align}
Note that the productivity of each entrepreneur $\tau_{ijt}$ is the product of two terms (i) a time-varying aggregate component $A_t$
(common to all product markets and types) and (ii) a time-invariant idiosyncratic
term $\gamma_{ij}$. We refer to $A_{t}$ as aggregate productivity and to $\gamma_{ij}$ as $j$'s idiosyncratic productivity. Aggregate productivity follows an auto-regressive process
$\log A_{t}=\phi_{A}\log A_{t-1}+\varepsilon_{t}$,
with $\varepsilon_{t}\sim N \left(0,\sigma_{\varepsilon}^{2}\right)$. Without loss of generality,
we order idiosyncratic productivities according to $\gamma_{i1}\geq\gamma_{i2}\geq\cdots.$ 
Labor is hired at the competitive wage $W_{t}$ and capital at the
rental rate $R_{t}$. Entrepreneur $j$ can thus produce
her variety at a marginal cost $\Theta_{t} / \tau_{ijt}$,
where 
\begin{align}
\Theta_{t}\coloneqq\left(\frac{R_{t}}{\alpha}\right)^{\alpha}\left(\frac{W_{t}}{1-\alpha}\right)^{1-\alpha}
\label{eq:factor_price_index}
\end{align}
is the marginal cost function for a Cobb-Douglas technology with unit
productivity. We refer to $\Theta_{t}$ as the \textit{factor
price index}. In addition to all variable costs, the production of each variety entails a fixed production cost $c_{i} \geq 0$ per period (which may be different across product markets). Such a cost is in units of the \textit{numeraire}.\footnote{This implies that fixed costs do not change with factor prices. We modify this assumption in Section \ref{subsec:robustness}.}


\subsection{Market Structure \label{subsec:Market-Structure}}

We assume that all firms that enter (and thus incur the fixed cost $c_{i}$) play a static Cournot game: they simultaneously announce quantities,
taking the output of the other competitors as given.\footnote{We follow \cite{AB} and assume
that firms enter sequentially in decreasing order of TFP.} 
Therefore, each entrepreneur $j$ solves 
\begin{align}
\underset{y_{ijt}}{\textrm{max}}\quad\left(p_{ijt}-\dfrac{\Theta_{t}}{\tau_{ijt}}\right)y_{ijt}\qquad\text{s.t.}\;  p_{ijt}=\left(\dfrac{Y_{t}}{y_{it}}\right)^{1-\rho}\left(\dfrac{y_{it}}{y_{ijt}}\right)^{1-\eta} \text{ and }
\quad y_{it}=\left(\sum\limits_{k=1}^{n_{it}}y_{kit}^{\eta}\right)^{\frac{1}{\eta}}.
\label{eq:Cournot_problem}
\end{align}
The solution to (\ref{eq:Cournot_problem}) yields a system of $n_{it}$ non-linear equations in $\left\{ p_{ijt}\right\}_{j=1}^{n_{it}}$ (one for each firm)\footnote{
This system of first order conditions admits a close-form solution only in the limit case in which there is no differentiation within an product market ($\eta = 1$), as shown in the Section \ref{proofs_appendixB}.}
\begin{align}
p_{ijt} = \underbrace{\dfrac{1}{\eta-\left(\eta-\rho\right)s_{ijt}}}_{\mu_{ijt}} \,  \dfrac{\Theta_{t}}{\tau_{ijt}},\label{eq:firm_FOC}
\end{align}
where $s_{ijt}$ is the market share of firm $j=1,\ldots,n_{it}$ and $\mu_{ijt}$ is the markup. Eq. (\ref{eq:firm_FOC}) establishes a positive relationship between market shares and markups. This follows from firms internalizing the impact of their size on the price they charge $\left(p_{ijt}\right)$; large firms end up restricting output disproportionately more (relative to productivity), thereby charging a high markup. 
Rearranging (\ref{eq:firm_FOC}), one can also see that market shares are a positive function of revenue TFP $\left(p_{ijt} \: \tau_{ijt}\right)$. Our model thus features a positive association between revenue productivity, size and markups. A shock that increases dispersion in revenue TFP is also associated with greater dispersion in market shares and markups.

To conclude the description of the product market equilibrium, we need to determine the number of active firms $n_{it}$. To this end, let $ \Pi\left(j ,n_{it},\Gamma_{it},X_{t}\right) \coloneqq \left(p_{ijt}-{\Theta_{t}}/{\tau_{ijt}}\right)y_{ijt}$ denote the gross profits of firm $j\leq n_{it}$ in product market $i$, when there are $n_{it}$
active firms, given a productivity distribution $\Gamma_{i} \coloneqq \left\{ \gamma_{i1} \, , \, \gamma_{i2} \, , \, \ldots \right\}$ and a vector of aggregate variables $X_{t} \coloneqq \left[ A_{t} \, , \, Y_{t} \, , \, \Theta_{t} \right]$. The equilibrium number of firms must be such that (i) the profits of each active firm are not lower than the fixed cost $c_{i}$ and (ii) if an additional firm were to enter, its profits would be lower than the fixed cost. Formally, an interior solution $n^{*}_{it} < M$ to the equilibrium number of firms must satisfy
\begin{align}
\left[\Pi\left({\color{blue}n_{it}^{*}},{\color{blue}n_{it}^{*}},\Gamma_{i},X_{t}\right)-c_{i}\right] \, \left[\Pi\left({\color{blue}n_{it}^{*}+1},{\color{blue}n_{it}^{*}+1},\Gamma_{i},X_{t}\right)-c_{i}\right] \; \leq \; 0, \quad   \forall i = 1,\ldots,I .\label{eq:eqm_n_firm}
\end{align}
Lemma \ref{lemma:(Profit-Function)} in Appendix \ref{proofs_appendixB} provides an analytical characterization of the profit function under the special case of $\eta=1$. We show that the profits of any firm $j$ i) increase in its own idiosyncratic productivity $\gamma_{ij}$ and ii) decrease in the idiosyncratic productivity
of all the other firms $\gamma_{ik}$. This means that, as top firms become more productive, small firms make lower profits and become closer to their exist threshold (\textit{ceteris paribus}). This is key to understanding some of the aggregate results that we describe next on the behavior of the economy under higher firm heterogeneity.

\subsection{General Equilibrium}
\paragraph{Equilibrium Definition}
We start by defining an equilibrium for this economy. Denoting the history of
aggregate productivity shocks by $ A^{t} = \{ A_{t}, A_{t-1}, ...\} $ we have the following definition.
\begin{definition}[Equilibrium]
An equilibrium is a sequence of policies  $ \left\{ C_{t}\left(A^{t}\right),  K_{t+1}\left(A^{t}\right),
L_{t}\left(A^{t}\right)\right\}_{t=0}^{\infty} $ for the household, firm policies $ \left\{ y_{ijt}\left(A^{t}\right),  k_{ijt}\left(A^{t}\right), l_{ijt}\left(A^{t}\right)\right\}_{t=0}^{\infty}  $, and a set of active firms $\left\{ n_{it}\left(A^{t}\right)\right\}_{t=0}^{\infty}$ with $\forall i\in\left\{1,\ldots,I\right\}$ such that i) households optimize; ii) all active firms optimize; iii) the slackness free entry condition in eq. (\ref{eq:eqm_n_firm}) holds; iv) capital and labor markets clear.
\end{definition}


\subsubsection{Static Equilibrium}
We now describe the general equilibrium of this economy. We start by focusing on a static equilibrium, in which production and labor supply decisions are described, taking the aggregate level of capital $K_{t}$ as given. Later on, we describe the equilibrium dynamics.
\paragraph{Aggregate Production Function} 
Given a $\left(I\times M\right)$
matrix of idiosyncratic productivity draws $\mathbf{\Gamma}$ and a vector of active firms
$\mathbf{N}_{t} \coloneqq \left\{ n_{it}\right\}_{i=1}^{I}$, aggregate output can be written as 
\begin{align}
Y_{t}={A}_{t}\,\Phi\left(\mathbf{\Gamma},\mathbf{N}_{t} \right)\;L_{t}^{1-\alpha}K_{t}^{\alpha} .\label{eq:agg_prod_fct}  
\end{align}
The term $\Phi\left(\cdot\right)$ 
represents the endogenous component of aggregate TFP and is a function of the number of active firms, individual productivities and market shares. An analytic expression for $\Phi\left(\mathbf{\Gamma},\mathbf{N}_{t}\right)$ is provided in Section \ref{sec:GEderivations}.
\paragraph{Aggregate Factor Share} 
Let $\mathbb{C}_t\coloneqq W_{t}\,L_{t} + R_{t}\,K_{t}$ represent aggregate variable costs. We can write the aggregate factor share $\Omega\left(\cdot\right) \coloneqq \mathbb{C}_t /Y_{t} $ as a function of individual markups and market shares\footnote{The aggregate factor share is equal to the inverse of the aggregate markup $\mu\left(\cdot\right) \coloneqq Y_{t} / \mathbb{C}_t $.}
\begin{align}
\Omega\left(\mathbf{\Gamma},\mathbf{N}_{t}\right) = \sum\limits _{i=1}^{I}\sum\limits _{j=1}^{n_{it}}s_{it}\;s_{ijt}\;\mu_{ijt}^{-1}.
\label{eq:agg_factor_share}
\end{align}
Combining (\ref{eq:agg_factor_share}) and (\ref{eq:firm_FOC}) we can write the aggregate factor share as a decreasing function of all product market-level Herfindahl-Hirschman index (HHI) of concentration
%
\begin{align}
\Omega\left(\mathbf{\Gamma},\mathbf{N}_{t}\right) = \sum\limits _{i=1}^{I}\;s_{it}\;\left[\eta-\left(\eta-\rho\right)\,HHI_{it}\right].
\label{eq:agg_factor_share_HHI}
\end{align}
where $HHI_{it} \coloneqq \sum _{j=1}^{n_{it}}\;s_{ijt}^2$.
This result, which is identical to the findings of \cite{grassi2017io} and \cite{AVB}, highlights two important relationships. First, product markets with higher concentration have larger markups. Second, when highly concentrated product markets have large shares in the economy (large $s_{it}$) the economy's average markup is also high. 
\paragraph{Factor Prices and Factor Markets}
We can write the aggregate demand schedules for labor $L_t$ and capital $K_t$, the analogs of eq. (\ref{eq:rr_map}), as
\begin{align}
     W_{t} \; = &  \left(1-\alpha\right)\; \Theta\left(\mathbf{\Gamma},\mathbf{N}_{t}\right) \; L_{t}^{-\alpha}\,K_{t}^{\alpha}, \\[1ex]
     R_{t} \; = & \alpha\; \Theta\left(\mathbf{\Gamma},\mathbf{N}_{t}\right)\;L_{t}^{1-\alpha}\,K_{t}^{\alpha-1}.
\label{eq:factor_demand}  
\end{align}
It is convenient to write the factor price index as the product between the aggregate factor share and aggregate TFP. Combining eqs. (\ref{eq:factor_price_index}), (\ref{eq:agg_prod_fct}) and (\ref{eq:factor_demand}), we have
\begin{align}
\Theta\left(\mathbf{\Gamma},\mathbf{N}_{t}\right)\;=\;\underbrace{\Omega\left(\mathbf{\Gamma},\mathbf{N}_{t}\right)}_{\substack{\text{aggregate} \\ \\ \text{factor share}}
} \; \underbrace{ \: {A}_{t} \: \Phi\left(\mathbf{\Gamma},\mathbf{N}_{t}\right)}_{\text{aggregate TFP}}.
\label{eq:agg_cost_decomposition}
\end{align}

Aggregating over all firms' first order condition (\ref{eq:firm_FOC}), we can express $\Theta\left(\mathbf{\Gamma},\mathbf{N}_{t}\right)$ as a function of the number of active firms $(n_{it})$, markups $(\mu_{ijt})$ and individual TFP $(\gamma_{ij})$
\begin{align}
\Theta\left(\mathbf{\Gamma},\mathbf{N}_{t}\right)=A_{t} \, \left\{ \sum_{i=1}^{I}\left[\sum_{j=1}^{n_{it}}\left(\dfrac{\gamma_{ijt}}{\mu_{ijt}}\right)^{\frac{\eta}{1-\eta}}\right]^{\frac{1-\eta}{\eta}\frac{\rho}{1-\rho}}\right\} ^{\frac{1-\rho}{\rho}}.\label{eq:agg_cost}
\end{align}
There are two aspects of eq. (\ref{eq:agg_cost}) that are worth highlighting. First, factor prices are decreasing in markups (holding the number of firms constant): higher markups drive a reallocation of income from factors of production to rents, resulting in lower $\Theta\left(\cdot\right)$. Second, factor prices are increasing in the number of active firms, which happens through two channels: \textit{directly} through the increase in $n_{it}$ (i.e. holding markups fixed) and \textit{indirectly} through the decrease in markups.

The factor demand schedules in (\ref{eq:factor_demand}) can be combined with the labor and capital supplies
\begin{align}
     L_{t}^{S} = W_{t}^{1 / \nu}  \quad \text{and} \quad K_{t}^{S} = K_{t} 
\label{eq:factor_supply}  
\end{align}
to determine the factor market equilibrium. Combining eqs. (\ref{eq:factor_demand}) and (\ref{eq:factor_supply})  with (\ref{eq:agg_prod_fct}), we can write aggregate labor and output as a function of the aggregate capital stock $K_t$, the productivity distribution $\mathbf{\Gamma}$ and the set of active firms $\mathbf{N}_{t}$
\begin{align}
L_{t} \; = & \;  \left[\left(1-\alpha\right)\Theta\left(\mathbf{\Gamma},\mathbf{N}_{t}\right)\right]^{\frac{1}{\nu+\alpha}}K_{t}^{\frac{\alpha}{\nu+\alpha}},\\
Y_{t} \; = & \; A_{t}\,\Phi\left(\mathbf{\Gamma},\mathbf{N}_{t}\right)\:\left[\left(1-\alpha\right)\Theta\left(\mathbf{\Gamma},\mathbf{N}_{t}\right)\right]^{\frac{1-\alpha}{\nu+\alpha}}\:K_{t}^{\alpha\frac{1+\nu}{\nu+\alpha}}.
\label{eq:agg_output_capital}
\end{align}
Both aggregate labor $L_{t}$ and output $Y_{t}$ are increasing in the factor price index. Higher factor prices result in higher wages (through (\ref{eq:factor_demand})) and hence a larger labor supply (through \ref{eq:factor_supply}). We conclude the characterization of the static equilibrium by determining the set of active firms $\mathbf{N}_{t}$.

\paragraph{Equilibrium Set of Firms}

The number of active firms in each product market $i$ is  jointly determined by eqs. (\ref{eq:agg_cost}),  (\ref{eq:agg_output_capital}) and the set of inequalities defined in (\ref{eq:eqm_n_firm}). Such a joint system does not admit a general analytical characterization. Nonetheless, we can characterize the particular case in which $\eta=1$ and all product markets are identical.\footnote{The special case with $\eta=1$ implies that goods are perfect substitutes within a product market.} Proposition \ref{A-symmetric-equilibrium} states the conditions for a symmetric equilibrium across product markets.

\begin{prop}[Existence and Uniqueness of a Symmetric Equilibrium]
\label{A-symmetric-equilibrium}

Suppose that $\eta=1$ and that all product markets have the same distribution of idiosyncratic productivities $\Gamma_{i}=\Gamma$. Then there exist two positive values $\underline{K}\left(\Gamma,n\right)$ and $ \overline{K}\left(\Gamma,n\right)$, with $\underline{K}\left(\Gamma,n\right)< \overline{K}\left(\Gamma,n\right)$ such that when $K_t\in[\,\underline{K}\left(\Gamma,n\right),\overline{K}\left(\Gamma,n\right)\,]$ the economy can sustain a symmetric equilibrium with $n$ firms in every product market. Furthermore, if the following holds
%
\[
\dfrac{\Phi\left(\Gamma,n\right)}{\Phi\left(\Gamma,n+1\right)}>\left[\dfrac{\Theta\left(\Gamma,n\right)}{\Theta\left(\Gamma,n+1\right)}\right]^{\frac{\rho}{1-\rho}-\frac{1-\alpha}{\nu+\alpha}}\, \quad \forall n,
\]
%
then there is a unique symmetric equilibrium in $[\,\underline{K}\left(\Gamma,n\right),\overline{K}\left(\Gamma,n\right)\,], \: \forall n$. When there are no productivity differences across firms, this condition is equivalent to $\frac{\rho}{1-\rho}>\frac{1-\alpha}{\nu+\alpha}$.

% Further, the bounds $\overline{K}\left(\Gamma,n\right)$ and $\underline{K}\left(\Gamma,n\right)$ are both increasing in $n$.

%\textbf{CHANGE TO BOUNDS} Suppose that all product markets have the same distribution of idiosyncratic productivities $\Gamma_{i}=\Gamma$. Then, there can be a symmetric equilibrium with $n$ firms per product market if $K_{t}$ is such that 
%\[
%\underline{K}\left(\Gamma,n\right)\leq K_{t}\leq\overline{K}\left(\Gamma,n\right),
%\]
%where the bounds $\overline{K}\left(\cdot\right)$ and $\underline{K}\left(\cdot\right)$ are both increasing in $n$.
\end{prop}
\begin{proof}
See Appendix \ref{Proofs-Additional-Results}.
\end{proof}
Intuitively, $K_{t}$ must be sufficiently large so that all existing $n$ firms can break even, but cannot be too high, for otherwise an additional firm could profitably enter in at least one product market. Figure \ref{fig:Static-Equilibrium} illustrates the static equilibrium when all product markets are (ex-ante) identical. When capital is within the bounds $\left[\underline{K}\left(1\right), \overline{K}\left(1\right)\right]$, the economy is characterized by a monopoly in every product market $(n=1)$; both labor and capital increase in the capital stock, but in a concave fashion (because of decreasing returns). When capital is above $\overline{K}\left(1\right)$, at least one product market can sustain a duopoly $(n=2)$. The increase in competition translates into a higher factor price index and a higher labor supply. For this reason, output is locally convex on capital when $K_{t}\in\left[\overline{K}\left(1\right),\underline{K}\left(2\right)\right]$.\footnote{In the regions $\left[\overline{K}\left(n\right), \underline{K}\left(n+1\right)\right]$, the economy is characterized by an asymmetric equilibrium in which some product markets have $n$ firms, and some others have $n+1$ firms. The number of product markets with $n+1$ firms is such that the last firm exactly breaks even. See Section \ref{sec:GEderivations} for details.}

\begin{figure}[ht]
\centering{}%
\begin{tabular}{ccc}
	\hspace{-1cm} \includegraphics*[scale=0.385]{input/static_eqm_theta} &  
	\hspace{0.25cm}
	\includegraphics*[scale=0.385]{input/static_eqm_labor}
	\hspace{0.25cm} 
	\includegraphics*[scale=0.385]{input/static_eqm_output} & 
\end{tabular}
\caption{Static equilibrium \protect \\ {Note: \small{} the figure shows how the factor price index, aggregate labor and output move with capital. Solid segments represent a regions with a symmetric equilibrium across product markets, while dotted segments represent non-symmetric regions. We use $\alpha \, = \, 1/3 \,$, $\rho \, = \, 3/4 \,$, $\eta \, = \, 1 \,$, $\nu \, = \, 2/5 \,$, $\gamma_{ij} \, = \, 1 \,$ and $ c_{i} \, = \, 0.015 \,$.}} 
\label{fig:Static-Equilibrium}
\end{figure}

The last part of the proposition provides a condition for uniqueness of symmetric equilibria, in the special case in which firms are identical. If the across product market elasticity of substitution $\sigma_I = 1/\left(1-\rho\right)$ is high, if the capital elasticity $\alpha$ is large or if the inverse Frisch elasticity $\nu$ is large, it is easier for the condition for uniqueness to be satisfied. We return to the discussion on uniqueness in the calibrated version of our model. 

\subsubsection{Equilibrium Dynamics}
We next explore the dynamic properties of our economy. Denoting by $s_{t}$ is the aggregate savings rate (from the household maximization problem), we can write the capital law of motion as 
\begin{align}
    K_{t+1} = \left(1-\delta\right) K_{t} + s_{t} \cdot Y_{t}. \label{eq:law-of-motion}
\end{align}
Even though we cannot provide an analytical characterization of $s_t$, we can establish that, in a steady-state, it is proportional to the aggregate factor share $\Omega\left(\mathbf{\Gamma},\mathbf{N}\right)$. Lemma \ref{lemma:savings_rate} establishes that a more competitive market structure, by resulting in a larger factor share $\Omega\left(\mathbf{\Gamma},\mathbf{N}\right)$, leads to a higher steady-state savings rate (and hence capital supply).
\begin{lemma}[Steady-State Savings Rate] \label{lemma:savings_rate}
In a steady-state, the following holds:
\begin{align}
s^{*}= \dfrac{\beta \, \delta}{1-\left(1-\delta\right)\beta}\;\underbrace{\alpha\;\Omega\left(\mathbf{\Gamma},\mathbf{N}\right)}_{\text{capital share}}.
\end{align}
Furthermore, as a consequence of Lemma \ref{aggregate_factor_share_lem}, $s^*$ is increasing in the number of firms.
\end{lemma}

\begin{proof}
See Appendix \ref{Proofs-Additional-Results}
\end{proof}


\begin{figure}[htb]
\centering{}
\hspace{-0.2cm}
 \includegraphics*[scale=0.475]{input/LOM_baseline}
 \hspace{0.4cm}
 \includegraphics*[scale=0.475]{input/RR_baseline}
\caption{Law of Motion and Rental Rate Map \label{fig:Law-of-Motion}
\protect \\ {Note: \small{}This example features two stable steady states and an unstable one. We use $\psi \, = \, 1 \,$,  $\rho \, = \, 3/4 \,$, $\eta \, = \, 1 \,$, $\alpha \, = \, 1/3 \,$, $\delta \, = \, 1 \,$, $\nu \, = \, 2/5 \,$ and $ c_{i} \, = \, 0.015 \,$.}} 
\end{figure}
The left panel of Figure \ref{fig:Law-of-Motion} represents the law of motion (\ref{eq:law-of-motion}) for a particular parameter combination. For the sake of exposition, we assume again that all product markets are (ex-ante) identical and that the economy is subject only to one time unexpected shocks (we relax these assumptions in the quantitative model). 
First, note that $K_{t+1}$ is not globally concave in $K_{t}$. Second, the economy features  multiple steady-states: there are two stable steady-states, $K^{*}_{1}$ and $K^{*}_{2}$, and an unstable one, $K_{U}$.\footnote{It is important to note that this map is a function, rather than a correspondence, which would signal the possibility of dynamic multiplicity. In this setting the initial conditions fully determine the steady-state the economy will converge to.} The shape of the law of motion (and the existence of multiple steady-states) can be explained by the interaction between competition, factor prices and factor supply. Within the colored regions, the economy is characterized by the same market structure (same number of firms $n_{t+1}$). This ensures that the law of motion is concave within these regions, as in a standard neoclassical growth model. However, in the regions coinciding with changes in the market structure, the law of motion is convex. To understand this, consider again eq. (\ref{eq:law-of-motion}). The law of motion can be convex in capital if at least one of two conditions holds: i) $Y_{t}$ is convex in $K_{t}$ or ii) $s_{t}$ increases sufficiently fast in $K_{t}$. As already highlighted in Figure \ref{fig:Static-Equilibrium}, $Y_{t}$ can be convex in $K_{t}$ because of the positive impact of competition on labor supply. On the other hand, more intense competition can also result in a larger savings rate $s_t$ and hence a larger supply of capital. 
To sum up, relative to $K^{*}_{1}$, steady-state $K^{*}_{2}$ is characterized by a more competitive market structure, and hence a larger supply of labor and capital by the representative household.

The right panel of Figure \ref{fig:Law-of-Motion} represents the rental rate map of this economy. As discussed in Section \ref{sec: general framework text}, multiple steady-states occur whenever this map crosses the steady-state rental rate multiple times. A steady-state is characterized by a constant rental rate equal to $ R^{*} = \beta^{-1} - \left(1-\delta\right).$ Proposition \ref{prop:multiplicity} characterises the conditions for the existence of multiple steady-states.

\begin{prop}[Existence of Multiple Steady States]\label{prop:multiplicity} Suppose that all product markets have the same distribution of idiosyncratic productivities $\Gamma_{i}=\Gamma$.
The economy features multiple symmetric steady states if and only if there exists an $n\in \mathbb{N}$ such that
\begin{align}
    \Theta\left(\Gamma,n\right)^{\frac{1+\nu}{\nu+\alpha}}\:\overline{K}\left(\Gamma,n\right)^{-\nu\frac{1-\alpha}{\nu+\alpha}}<\dfrac{\beta^{-1}-\left(1-\delta\right)}{\alpha\;\left(1-\alpha\right)^{\frac{1-\alpha}{\nu+\alpha}}}<\;\Theta\left(\Gamma,n+1\right)^{\frac{1+\nu}{\nu+\alpha}}\:\underline{K}\left(\Gamma,n+1\right)^{-\nu\frac{1-\alpha}{\nu+\alpha}}.
\end{align}
where $ \underline{K}\left(\Gamma,n\right)$ and $ \overline{K}\left(\Gamma,n\right)$ are defined in Appendix \ref{Proofs-Additional-Results}.
%Furthermore, fixing $n$, since both $\overline{K}(\Gamma,n)$ and $\underline{K}(\Gamma,n+1)$ are strictly increasing in the fixed cost $c$, there exists a set $(\underline{c},\overline{c}): \forall c\notin (\underline{c},\overline{c})$ the steady state of the economy is unique.
\end{prop}
\begin{proof}
See Appendix \ref{Proofs-Additional-Results}.
\end{proof}
Proposition \ref{prop:multiplicity} formalizes the idea that multiplicity obtains if there exists an increasing segment of the rental rate map and this segment crosses the steady-state interest rate $R^*=\beta^{-1} - (1-\delta)$. This condition depends on fundamental parameters such as the productivity distribution or the fixed production cost. For example, both $\underline{K}(\Gamma,n+1)$ and $\overline{K}(\Gamma,n)$ are strictly increasing in the fixed cost $c$. Therefore, as fixed costs change, the economy may enter/exit a region of steady-state multiplicity. Throughout this section, we assume that product markets are ex-ante symmetric and that the condition of Proposition \ref{prop:multiplicity} is satisfied, so that multiple steady-states exist. In Section \ref{sec:Quantitative-Evaluation}, we relax the assumption of product market symmetry and assess whether multiple steady-states arise or not under different calibrations of our model.

Finally, applying the definition of \textit{fragility} from Section \ref{sec: general framework text} to this particular economy, we have $\chi_{2} \; = \; {K_{U}}/{K^{*}\left(2\right)}$.
We next ask how changes in the technology set of the economy can affect \textit{fragility}. We consider two comparative statics exercises: a mean-preserving spread (MPS) to the productivity distribution of active firms and an increase in fixed costs. These technological shifts can explain some of the micro trends that have taken place since the 1980s (e.g. rising concentration or markups). Next, we study the aggregate consequences of rising heterogeneity and fixed costs, with a particular focus on the likelihood of persistent transitions.


\subsection{Comparative Statics}

In the special case of $\eta=1$ and symmetric product markets we can characterize two important results about the aggregate factor share, which we formalize in the next lemma.  
\begin{lemma}[Aggregate Factor Share]\label{aggregate_factor_share_lem}
Suppose that $\eta=1$ and all product markets are
identical and have $n$ firms. Let  $\Gamma_n=\left\{\gamma_1,\ldots,\gamma_n\right\}$ be the productivity vector of $n$ the active firms. Then, the following holds:
\begin{enumerate}[label=\alph*)]
    \item $\Omega\left({\Gamma_n},n+1\right)>\Omega\left({\Gamma_n},n\right)$,
    \item $\Omega\left({\tilde\Gamma_n},n\right)<\Omega\left({\Gamma_n},n\right)$ if $\tilde\Gamma_n$ is a mean-preserving spread of $\Gamma_n$ .
\end{enumerate}
\end{lemma}
\begin{proof}
See Appendix \ref{Proofs-Additional-Results}.
\end{proof}
Part $a)$ of the Lemma states that increasing the number of firms in the economy increases the aggregate factor share. This intuitive result goes through the competitive effect of a larger number of firms, which compresses markups and the profit share and therefore increases the factor share. Part $b)$ of the lemma states that economies characterized by higher firm level heterogeneity feature lower factor shares. Suppose we increase firm heterogeneity by increasing the productivity of the best firm in a product market. This implies a reallocation of market shares from low to high productivity firms. In our model this also implies a change in markups. As a consequence of the reallocation and markup response, the average markup increases and the factor share decreases. 



\paragraph*{Firm Heterogeneity}

We start by studying the impact of an MPS in the distribution of productivities on \textit{fragility}. The next results obtain under two assumptions, which are necessary to have an analytical characterization of the model's steady-state(s) i) all product markets are ex-ante identical and ii) $\eta = 1$ (i.e. no within product market differentiation). We dispense with both assumptions in our quantitative application. We start by characterizing the response of the factor price index $\Theta\left(\cdot\right)$ to a productivity spread. %Note that, as eq. (\ref{eq:factor_demand}) highlights, $\Theta\left(\cdot\right)$ is important to characterize $R_t$ and hence the distance between steady-states.

\begin{lemma}[Mean Preserving Spread and Factor Prices]
\label{lemma:MPS_theta} Let $\eta = 1$ and suppose that all product markets are identical and have $n$ firms. Let $\Gamma_n=\left\{\gamma_1,\ldots,\gamma_n\right\}$ be the productivity vector of the $n$ active firms and $\tilde\Gamma_n$ be a mean-preserving spread on $\Gamma_n$. Then
%\begin{align}
$\Theta(\tilde\Gamma_n,n)<\Theta(\Gamma_n,n).$
%\end{align}
\end{lemma}
\begin{proof}
See Appendix \ref{Proofs-Additional-Results}.
\end{proof}

%This result is the partial analog to Proposition \ref{propcompstatexrc}. 
This result states that, in a symmetric steady state with $n$ firms, a spread of the productivity distribution decreases the aggregate factor price index. As formalized by the first part of Proposition \ref{prop:MPS}, this is a sufficient condition for the stable steady-state level of capital to decrease.

\begin{prop} [Firm Heterogeneity and Fragility] \label{prop:MPS} Let $\eta = 1$ and suppose that all product markets are identical. Let ${K}^{*}\left(n\right)$ be a stable steady-state with $n$ firms in every product market. Let $\Gamma_n=\left\{\gamma_1,\ldots,\gamma_n\right\}$ be the productivity vector of the $n$ active firms and $\tilde\Gamma_n$ be a mean-preserving spread on $\Gamma_n$. The following holds
\begin{enumerate}[label=\alph*)]
    \item $K^{*}(\tilde\Gamma_n,n)<K^{*}(\Gamma_n,n)$.\label{mps_a}
    \item If $n=2$ and $\rho>1-\dfrac{\nu\left(1-\alpha\right)}{1+\nu\alpha}$, then
    $K_U(\tilde\Gamma_2)>K_U(\Gamma_2)$. \label{mps_b}
\end{enumerate}
%\[ \dfrac{\partial {K}^{*}\left(n\right)}{\partial\lambda} \leq 0. \]
\end{prop}
\begin{proof}
See Appendix \ref{Proofs-Additional-Results}.
\end{proof}
\begin{corollary}\label{mps_fragility}
If the condition in Proposition \ref{prop:MPS}\ref{mps_b} is satisfied, the highest steady state $K^*(\tilde\Gamma_2,2)$ becomes more fragile after a mean-preserving spread. Formally, $\chi_2(\tilde\Gamma_2)>\chi_2(\Gamma_2).$
\end{corollary}
Proposition \ref{prop:MPS} is the analog of Proposition \ref{propcompstatexrc} in Section \ref{sec: general framework text}. Before explaining its results, let us start by discussing the distributional consequences of an MPS. Fixing the number of firms, an MPS of idiosyncratic productivities, by increasing product market concentration, results in a lower factor share (eq. \ref{eq:agg_factor_share_HHI}). This pushes the factor price index down, for a given level of aggregate TFP, as eq. (\ref{eq:agg_cost_decomposition}) highlights. This is a \textit{market power effect} associated with higher firm heterogeneity, which results in lower factor prices. However, aggregate TFP is likely to increase after an MPS: large, high productivity firms become even more productive and increase their market shares. This pushes the factor price index up (eq. \ref{eq:agg_cost_decomposition}). This is an \textit{allocative efficiency effect}, which results in higher factor prices. The impact of an MPS on factor prices depends on the relative strength of these two forces. These effects are the more precise characterizations of the elements highlighted in Section \ref{sec: general framework text}. Proposition \ref{prop:MPS} specifies the result from Proposition \ref{propcompstatexrc} under an MPS of productivities.


\begin{figure}[ht!]
\hspace{-0.0cm}
\begin{minipage}[b]{.5\linewidth}
\centering\includegraphics*[scale=0.5]{input/RR_MPS.eps}\subcaption{Effect of an MPS on capital demand} \label{fig:RR_MPS}
\end{minipage}
\vspace{0.75cm}
\begin{minipage}[b]{.5\linewidth}
\centering\includegraphics*[scale=0.5]{input/RR_cf.eps}\subcaption{Effect of $\uparrow c$ on capital demand} \label{fig:LOM_MPS}
\end{minipage}
\begin{minipage}[b]{.5\linewidth}
\centering\includegraphics*[scale=0.5]{input/LOM_MPS.eps}\subcaption{Effect of an MPS on the law of motion} \label{fig:RR_cf}
\end{minipage}
\begin{minipage}[b]{.5\linewidth}
\centering\includegraphics*[scale=0.5]{input/LOM_cf.eps}\subcaption{Effect of $\uparrow c$ on the law of motion} \label{fig:LOM_cf}
\end{minipage}
\caption{Comparative Statics \protect \\ {\small{} Panels (a) and (c) represent the effect of an MPS on capital demand and the law of motion of capital (in an economy with two steady-states). Panels (b) and (d) represent the effect of an increase in fixed costs. We use $\rho \, = \, 3/4 \,$, $\eta \, = \, 1 \,$,  $\alpha \, = \, 1/3 \,$ and $\nu \, = \, 2/5 \,$.}} \label{fig:Comparative-Statics}
\end{figure}

% \begin{figure}[ht!]
% \centering{}%
% \begin{tabular}{cc}
% 	\hspace{-1cm} \includegraphics*[scale=0.45]{input/RR_MPS} &  \hspace{-0.2cm}
% 	\includegraphics*[scale=0.45]{input/RR_cf} \\
% 	\hspace{-1cm} 
% 	\includegraphics*[scale=0.45]{input/LOM_MPS.eps} & 
% 	\hspace{-0.2cm}
% 	\includegraphics*[scale=0.45]{input/LOM_cf}
% \end{tabular}
% \caption{Comparative Statics \protect \\ {Note: \small{} The left panels represent the effect of an MPS on the rental rate and the law of motion of capital (in an economy with two steady-states). The right panels represent the effect of an increase in fixed costs. We use $\rho \, = \, 3/4 \,$, $\eta \, = \, 1 \,$,  $\alpha \, = \, 1/3 \,$ and $\nu \, = \, 2/5 \,$.}} 
% \label{fig:Comparative-Statics}
% \end{figure}

Proposition \ref{prop:MPS} formalizes two results. The first is that, if there exists a steady-state where all product markets are identical and have $n$ firms, the steady-state level of capital necessarily shrinks after an MPS of the productivities of these $n$ firms. This happens because the \textit{market power effect} always dominates, so that $\Theta\left(\cdot\right)$ declines. The steady-state level must shrink, so that eq. (\ref{eq:factor_demand}) holds at the same $R^{*}$.
The second part of Proposition \ref{prop:MPS} characterizes the behavior of the unstable steady-state $K_{U}$. It provides a sufficient condition under which the unstable steady-state moves rightward after an MPS. As the rental rate map is upward slopping at $K_{U}$, this steady-state moves rightward whenever the rental rate falls. This is illustrated in the left panels of Figure \ref{fig:Comparative-Statics}. Panel (a) shows that capital demand decreases for sufficiently high values of $K_t$. This translates into a higher proximity between the unstable steady-state $K_U$ and the highest stable steady-state $K^{*}\left(2\right)$, as illustrated in panel (c). Proposition \ref{prop:MPS}\ref{mps_b} provides a sufficient condition under which the rental rate falls in the region in which it is increasing. The difficulty in establishing a result for this region is that, even when all product markets are ex-ante identical, there are ex-post differences: some have $n$ firms, while others feature $n-1$ firms. For tractability reasons, Proposition \ref{prop:MPS}\ref{mps_b} focuses on the case of $n=2$. Proposition \ref{prop:MPS_BA_n} in Appendix \ref{Proofs-Additional-Results} provides a result for general $n$.
Proposition \ref{prop:MPS}\ref{mps_b} states that $K_{U}$ increases when $\rho$ is sufficiently high. A high value of $\rho$ means that the degree of cross product market differentiation and of average markups are relatively low. Small productivity differences are magnified and entry becomes more difficult for a second player (which brings down aggregate factor shares and factor prices).

Taken together, as highlighted in Corollary \ref{mps_fragility}, the two parts of Proposition \ref{prop:MPS} provide a sufficient condition under which fragility increases after an MPS. 
%Note that $\chi$ captures the proximity between steady-states. Provided that large shocks are less likely than small ones, then $\chi$ is a sufficient statistic for the probability of downward transitions.\footnote{More formally, this follows from the size of capital adjustment being a strictly increasing function of the absolute value of the shock. Hence if large shocks are less likely so are large changes in capital and therefore transitions between steady-states.}
% \begin{remark}[Fragility and Distance between Steady-States]
% Provided that the PDF of the stochastic process is decreasing away from zero, then $\chi$ is a sufficient statistic for the probability of downward transitions. An increase in $\chi$ implies an increase in the probability of moving to lower steady-states.
% \end{remark}
%In summary, if the condition in Proposition \ref{prop:MPS}\ref{mps_b} is verified, higher firm heterogeneity makes persistent recessions more likely.
Finally, Proposition \ref{prop:MPS} focuses on the consequences of an MPS with $n=2$. By construction, we increase the productivity of the top firm and reduce the productivity of the second one, keeping their average unchanged. However, fragility can also increase if we increase the productivity of the top firm, leaving the productivity of the second firm unchanged.\footnote{Figure \ref{fig:Law-of-Motion-MIS} in Supplementary Material Section \ref{appendix:baseline-model} shows one such example.}

\paragraph*{Rising Fixed Costs} The decline in product market competition since the 1980s may also be explained, through the lens of our model, by rising fixed costs.\footnote{This channel is also studied in \cite{de2021quantifying}.} As fixed costs rise, they drive out of the market those firms that exactly break even. This results in higher markups and concentration. Their effect on the capital demand schedule can be understood in two steps. First, in a steady-state with $n$ firms where all firms make strictly positive profits, the capital level of such a steady-state $\left(K^{SS}_{n}\right)$ is unaffected by a marginal increase in $c_f$. On the other hand, the larger fixed costs result in a rightward shift of the unstable steady-state. Recall that $K_U$ belongs to a region where some firms are breaking even. These firms can break even with a higher fixed cost only if the capital stock is higher.
%This means that rising fixed costs also make the highest steady-state more fragile, so that now even relatively small shocks can trigger a transition to the low competition trap.
Proposition \ref{prop:basin_attraction_cf} and Corollary \ref{mps_fixed_cost} formalize these results. Differently from Proposition \ref{prop:MPS} we make no assumption of symmetry across product markets or perfect substitution.

\begin{prop}[Fixed Costs and Fragility] \label{prop:basin_attraction_cf} Let ${K}^{*}\left(\mathbf{\Gamma}, \mathbf{N}\right) $ be a stable steady-state with a set of active firms $\mathbf{N}$. Then the following holds
\begin{enumerate}[label=\alph*)]
    \item $\dfrac{\partial K^*(\mathbf{\Gamma}, \mathbf{N})}{\partial c}\leq0$ .\label{cf_a}
    \item $\dfrac{\partial K_U(\mathbf{\Gamma}, \mathbf{N})}{\partial c}>0$. \label{cf_b}
\end{enumerate}
\end{prop}
\begin{proof} See Appendix \ref{Proofs-Additional-Results}.
\end{proof}
\begin{corollary}\label{mps_fixed_cost}
When fixed costs increase, any stable steady-state becomes more fragile: $\dfrac{\partial \chi(\mathbf{\Gamma}, \mathbf{N})}{\partial c}>0$.
\end{corollary}
Panels (b) and (d) of Figure \ref{fig:Comparative-Statics} illustrate the effect of an increase in fixed costs. We represent again an economy where all product markets are ex-ante identical (same distribution of productivities and identical fixed costs). The two declining segments of the rental rate map represent a situation of full monopoly and full duopoly; since all firms make strictly positive profits in these regions, the equilibrium is unchanged as $c$ increases marginally. In the increasing segment, where some firms are exactly breaking even, some are driven out of the market. The rental rate decreases and the unstable steady-state increases. As a result, the economy becomes more fragile (Corollary \ref{mps_fixed_cost}).

These results also shed light on the conditions of Proposition \ref{prop:multiplicity}.A change in fixed costs can affect the existence of multiple steady-states. This is made clear in Figure \ref{fig:Comparative-Statics}: a sufficiently large increase in fixed costs can shift the rental rate map downward such that it crosses $R^{*}$ only once. In such a case, only one steady-state exists, where all product markets are monopolies $\left(K^{*}\left(1\right)\right)$. The level of capital $K^{*}\left(2\right)$ is no longer a steady-state. The opposite would happen if fixed costs were to experience a sufficiently large decrease. In such a case, only $K^{*}\left(2\right)$ would be a steady-state.\footnote{Figure \ref{fig:Law-of-Motion-existence} in Supplementary Material Section \ref{appendix:baseline-model} shows one such example.}

\paragraph{Discussion}
We conclude by summarizing two keys insights of our theory, which are relevant to understanding the US growth experience after 2008. The first is that a complementarity between competition and factor supply can generate multiple competition regimes or steady-states. A transition from a high competition to a low competition regime can in many aspects describe the 2008 recession and the subsequent great deviation. The second insight is that changes in technology that result in larger market power (e.g. larger productivity differences across firms or larger fixed costs) make high competition regimes more difficult to sustain, and transitions to low competition traps more likely to occur. Our model therefore suggests that the US economy, experiencing a long-run increase in markups and concentration since the 1980s, became increasingly vulnerable to transitions like the one observed after 2008.

In the next section, we use a calibrated version of our model and study its quantitative predictions. We then ask whether it can replicate the behavior of the US economy in the aftermath of the 2008 crisis and finally study the welfare gain of policy interventions.


==> submitted_version/4_quantitative_model.tex <==
\section{Quantitative Results \label{sec:Quantitative-Evaluation}}
The goal of this section is to develop a quantitative version of the model built in Section \ref{sec:Model}. We use it to provide a quantification of the forces described earlier, and to evaluate policy counterfactuals.

There are two objects that we need to parametrize: the distributions of idiosyncratic productivities $\gamma_{ij}$ and of fixed costs $c_i$. We assume that firms draw their idiosyncratic productivities from a log normal distribution with standard deviation $\lambda$, i.e. $\log \gamma_{ij} \sim \textrm{N}\left( 0, \lambda \right).$ Each product market $i$ is characterized by $M$ such draws. Since $M$ is a finite number, product markets have different ex-post distributions of idiosyncratic productivities $\left\{ \gamma_{ij} \right\}_{j=1}^{M}$.

Furthermore, we assume that there are two types of product markets: a fraction $f\in\left(0,1\right)$ of all product markets face a fixed cost $c_{i} = c > 0$, whereas the remaining fraction $1 - f$ faces a zero fixed cost $c_{i} = 0$. We refer to the first as \textit{concentrated} and the second as \textit{unconcentrated} product markets. In product markets with a zero fixed cost, the extensive margin is muted as all potential $M$ entrants are always active. However, these product markets do not necessarily operate close to perfect competition, as there can be large productivity differences across firms, resulting in high concentration and large markups for productive firms.
Importantly, even if idiosyncratic productivities are drawn from the same distribution, there will be ex-post differences in productivity draws. This heterogeneity acts against the existence of steady-state multiplicity.\footnote{We assume that there is a common fixed cost $c$ among all \textit{concentrated} product markets. %Although we make this assumption mostly for simplicity, we should highlight that it is not completely innocuous. In particular, when there are differences in fixed costs within these product markets, and if these differences are large, multiplicity may disappear \textendash{} since for multiplicity to arise, we need a sufficiently large number of product markets that move together.
%Recall however that, even if they share the same fixed cost $c>0$, \textit{concentrated} 
These product markets differ in their distributions of idiosyncratic TFP draws $\left\{ \gamma_{ij} \right\}_{j=1}^{M}$ and may display a different number of active firms.}

\subsection{Calibration}
The model is calibrated at a quarterly frequency. Our calibration strategy relies on the interpretation that, if two or more steady-states exist, the economy starts in the highest one. Some parameters are standard and taken from the literature. For the preference parameters, we set $\beta = 0.99$ and $\psi=1$ to have log utility. We set $\nu = 0.352$, which implies a Frisch elasticity of 2.84; this corresponds to the average macro elasticity of hours reported by \cite{CGMW}. We set the number of product markets at $I=10,000$ and the maximum number of firms per product market at $M=20$.\footnote{Contrarily to \cite{de2021quantifying} we fix this parameter across the different calibrations. We have also considered $M=50$ and $M=100$ and the results were identical.}
For technology parameters, we set the capital elasticity to $\alpha = 0.3$ and the depreciation rate to $\delta= 0.025$. There are 5 parameters that we need to calibrate internally: the within and across product market elasticities of substitution ($\sigma_G$ and $\sigma_I$), the standard deviation of the log-normal productivity distribution for the pool of potential entrants $\left(\lambda\right)$, the fixed cost for the \textit{concentrated} sector $\left(c\right)$, and the fraction of \textit{concentrated} product markets $\left(f\right)$.

Before describing in detail our calibration strategy we briefly discuss our algorithm, which is similar to \cite{de2021quantifying}. We begin by drawing productivity values for all $20\times10,000$ potential firms in the economy. For the product markets without entry costs, these also represent the number of active firms, while for the product markets with $c_i>0$ the free entry condition might not hold. To check that the slackness free entry condition holds at each pair of state variables $\left(K_t, A_t\right)$, we start with a full matrix of firms. If any firm makes negative profits, we eliminate the firm with the largest negative value and recompute the equilibrium. We do so until all firms make non-negative profits. This procedure is more computationally demanding than the alternative one in which we start with an empty matrix and fill it with firms as long as they make positive profits. The reason behind our choice is that iterative deletion implies, in the case of multiple equilibria, we consistently select the one with the highest number of active firms. 
%For the simpler case in which $\eta=1$ and firms are symmetric across sectors we can show that the static equilibrium is unique, however, for this much more general model such result needs not to hold. 
We view our approach as being conservative since the mechanism we propose has the largest potential effect when few firms are active in the market. Therefore our equilibrium selection algorithm provides us with a lower bound on the strength of our mechanism in case there are multiple static equilibria. The condition for static uniqueness presented in Proposition \ref{A-symmetric-equilibrium} was derived in the special case of $\eta=1$ and product market and firm symmetry \textendash{} which are not satisfied in this calibrated version of the model. The introduction of product market and firm heterogeneity makes uniqueness more likely to obtain.

We provide three different calibrations of our economy, where we target the same moments in different points in time: 1975, 1990 and 2007. Our calibration relies on the assumption that the elasticities $\sigma_G$ and $\sigma_I$ are time-invariant, while the other 3 parameters are allowed to vary over time. This allows us to compare features of the model in economies with different levels of firm heterogeneity and fixed costs.
We target 4 moments in each of the three calibration years. We thus have 12 moments for 11 parameters (2 elasticities and 3x3 time-varying parameters). This gives us an over-identified system, which we calibrate jointly.

% We chose moments that do not depend on assumptions about a particular level of aggregation (e.g. 4-digit versus 6-digit). We do so because we want to think of a product market $i$ as a market at the lowest possible level of aggregation.

% We design our calibration so that we do not have to commit to what a product market in our model maps to in the data. This has the great advantage that we do not have to specify what is the competitive market in the data. Clearly, while for some tradable firms the relevant competitive market might be a global product market, for very local service provider it might be as narrow as a neighborhood. Our calibration choices imply that we need not to take a stance on this and that we can think of the product markets in our model as a combination of \textit{product market}$\times$\textit{relevant competitive market} in the data. 
Importantly, we design our calibration so that it does not depend on assumptions about a particular level of aggregation, i.e. how to map a market $i$ in our model to a market $i$ in the data. While for some tradeable-good firms the relevant competitive market might be a global 10-digit industry, for local service providers it might be as narrow as a neighborhood. Our calibration choices imply that we need not take a stance on this mapping and that we can think of some product markets in our model as a combination of \textit{product market}$\times$\textit{location} in the data \citep[see][for a more complete discussion]{eeckhoutcomment, product_market_concentration}.\footnote{As \cite{product_market_concentration} report, some industries can be too broad for some products (e.g. NAICS 325620 contains products such as after-shave, mouthwash or sunscreen). In other cases, highly substitutable products belong to different industries (e.g. metal cans or glass bottles).}
For the two elasticities of substitution, we assume that they are time-invariant and calibrate them to match the sales-weighted average markup of public firms \citep[as reported by ][]{LEU}. Conditional on the other time-varying parameters, the elasticities are informative about the level of markups charged by firms in the economy.
We calibrate the standard deviation of the exogenous productivity distribution $\left(\lambda\right)$ to match dispersion in firm size. %Intuitively, conditional on the elasticities discussed above, the dispersion of market share is informative about the dispersion of the underlying productivity distribution.  
Specifically, we compute the standard deviation of log revenues for all firms in our economy and use as a target the corresponding moment in COMPUSTAT. Even though COMPUSTAT is not a representative sample of firms for the whole economy, we choose this dataset for two reasons. First, it covers all sectors in the economy (and is not restricted to specific sectors, such as manufacturing). Second, being a firm-level dataset, it allows us to obtain a measure of firm-level dispersion that does not depend on a particular level of aggregation (e.g. 4-digit NAICS).\footnote{Some aggregate datasets, such as the BLS Multifactor Productivity Database, provide statistics on firm-level differences. However, these differences are computed within a 4-digit industry and data is restricted to the set of manufacturing industries.}
Figure \ref{intro_figure_2} shows the evolution of our dispersion measure in COMPUSTAT.
We calibrate the fixed cost parameter to match the average ratio of fixed to total costs in COMPUSTAT. Following \cite{GW}, we define fixed costs as sum of `Selling, General and Administrative Expenses', `R\&D Expenditures' and `Advertisement Expenses'. We obtain a target level of 24.4\% for 1975, 35.5\% for 1990 and 41.4\% for 2007 (see Figure \ref{fig:fixed_total_costs}). 
To calibrate $f$, we target the fraction of aggregate employment in highly concentrated industries. In the calibrated model, \textit{concentrated} product markets have fewer than 4 firms. In an ideal setting, we would have direct information on the aggregate employment share of markets with 4 or fewer firms. As discussed above, we think of an product market in our model as a market at the highest level of disaggregation (e.g. 10-digit NAICS or, in some case, as a product market-location pair). However, we only have information of concentration metrics at the 6-digit NAICS level. Since this will understate concentration levels in finer markets, we scale the market share of the 4 largest firms in 6-digit NAICS, by the share of the largest 8 firms. Then, we define an product market as \textit{concentrated} if the share of the top 4 to top 8 is above 90\%.\footnote{Alternative thresholds for the ratio of the top 4 to the top 8 (80\% and 95\%) yield identical results.} Using data from the US Census, we find that 6.33\% of aggregate employment is allocated to such 6-digit industries in 2007. 

We also need to calibrate the two parameters governing the dynamics of aggregate productivity: the autocorrelation parameter $\phi_z$ and the standard deviation of the innovations $\sigma_{\varepsilon}$. We do so by targeting the first order autocorrelation and the standard deviation of  output.\footnote{We compute these moments for the entire postwar period 1947\textendash{}2019. Consistent with our interpretation that the US economy moved to a different regime after 2008, we remove a linear trend computed for the period 1947\textendash{}2007.} We calibrate these parameters using our 2007 model, and keep them unchanged in the 1975 and 1990 models.


\begin{table}[ht!]
\setlength{\tabcolsep}{0.2cm} \begin{center} \resizebox{14.5cm}{6cm} {  \begin{tabular}{lccccl}
\thickhline
\\[-1ex]
{\large Description} & {\large Parameter} & \multicolumn{3}{c}{{\large Value}} & {\large Source/Target} \\[1ex] \thickhline
\\[-1ex]
[A] External Parameters \\ \\[-1ex] \hline
\\[-1ex]
Capital elasticity & $\alpha$ & \multicolumn{3}{c}{0.3} & Standard value \\
\\[-1ex]
Depreciation rate & $\delta$ & \multicolumn{3}{c}{0.025} & Standard value \\
\\[-1ex]
Discount factor & $\beta$ & \multicolumn{3}{c}{0.99} & Standard value \\
\\[-1ex]
Inverse of Frisch elasticity& $\nu$ & \multicolumn{3}{c}{0.352} & \cite{CGMW}\\
\\[-1ex]
Coefficient of risk aversion & $\psi$ & \multicolumn{3}{c}{1} & log utility \\
\\[-1ex]
Max number of firms per product market & $M$ & \multicolumn{3}{c}{20} & \\
\\[-1ex]
Number of product markets & $I$ & \multicolumn{3}{c}{10,000} & \\
\\[-1ex]
\hline
\\[-1ex]
[B.1] Calibrated Parameters: Fixed \\ \\[-1ex]
\hline
\\[-1ex]
Between product markets ES & $\sigma_{I}$ & \multicolumn{3}{c}{1.38} & Sales-weighted average markup\\
\\[-1ex]
Within product market ES & $\sigma_{G}$ & \multicolumn{3}{c}{11.13} & Sales-weighted average markup\\
\\[-1ex]
Persistence of $z_t$  & $\rho_{z}$ & \multicolumn{3}{c}{0.950} & Autocorrelation of log $Y_t$ \\
\\[-1ex]
Standard deviation of $\varepsilon_t$ & $\sigma_{\varepsilon}$ & \multicolumn{3}{c}{0.003} & Standard deviation of log $Y_t$ \\ 
\\[-1ex] \hline
\\[-1ex]
[B.2] Calibrated Parameters: Variable & & 1975 & 1990 & 2007 & \\ \\[-1ex] \hline
\\[-1ex]
Fraction of product markets with $c_{i}>0$ & $f$ & 0.110 & 0.135 & 0.140 &  Emp share concentrated industries \\
\\[-1ex]
Standard deviation of $\gamma_{ij}$ & $\lambda$ & 0.190 & 0.283 & 0.328 & Std log revenues \\
\\[-1ex]
Fixed cost ($\times 10^{-3}$) & $c$ & 0.47 & 0.96 & 1.34 & Average ratio fixed/total costs \\
\\[-1ex]
\thickhline
\end{tabular}  
} \end{center}
\caption{Parameter Values\label{tab:parameter_values}}
\end{table}


\begin{table}[ht]
\setlength{\tabcolsep}{0.2cm}  
\begin{center}
\resizebox{12.5cm}{3cm} {
\begin{tabular}{lcccccccc} 		\thickhline 
\\[-2ex]
& \multicolumn{2}{c}{1975} & & \multicolumn{2}{c}{1990} & & \multicolumn{2}{c}{2007} \\
\\[-1ex] 
& Data & Model & & Data & Model & & Data & Model \\ \hline  
\\[-1ex] 
Sales-weighted average markup & 1.28 & 1.26 & & 1.37 & 1.38 & & 1.46 & 1.44 \\
\\[-1ex]
Std log revenues & 1.67 & 1.65 & & 2.47 & 2.42 & & 2.79 & 2.83 \\
\\[-1ex]
Average fixed to total cost ratio & 0.244 & 0.271 & & 0.355 & 0.376 & & 0.414 & 0.397 \\
\\[-1ex]
Emp share \textit{concentrated} product markets & - & 0.066 & & - & 0.071 & & 0.063 & 0.068 \\
\\[-1ex] \hline 
\\[-1ex]
Autocorrelation log GDP  &  &  & &  &  & & 0.978* & 0.975 \\
\\[-1ex]
Standard deviation log GDP &  &  & &  &  & & 0.061* & 0.062 \\
\\[-1ex]
\thickhline
\\[-1ex]
\multicolumn{6}{l}{*computed over 1947:Q1-2019:Q4} \\
\end{tabular} } \end{center}
\caption{Targeted moments and model counterparts\label{tab:targeted_moments}}
\end{table}

Table \ref{tab:parameter_values} reports our parameter values, while Table \ref{tab:targeted_moments} reports our targeted moments, with their model counterparts. We obtain a value of 1.38 for the cross product market elasticity of substitution, and a value of 11.25 for the within product market elasticity. These are in line with the estimates from similar studies using US data, such as \cite{EMX}. The model is successful at matching the sales-weighted markups and dispersion in revenues in all three years. We slightly over-estimate the fixed cost ratio in 1975 and 1990 while we underestimate it in 2007.

\begin{table}[ht]
\setlength{\tabcolsep}{0.2cm}  
\begin{center} \resizebox{12cm}{3cm} {
\begin{tabular}{lcccccccc} 		\thickhline 
\\[-2ex]
& \multicolumn{2}{c}{1975} & &
\multicolumn{2}{c}{1990} & &
\multicolumn{2}{c}{2007} \\
\\[-1ex] 
& Data & Model & & Data & Model & & Data & Model
\\ \hline
\\[-1ex]
[A] Total Economy
\\[-1ex] \\ \hline
\\[-1ex]
Cost-weighted average markup & 1.16 & 1.24 & & 1.20 & 1.30 & & 1.25 & 1.34 \\
\\[-1ex]
Aggregate TFP (log) & 0.00 & 0.00 & &  0.091 & 0.098 & & 0.296 & 0.167 \\
% \\[-1ex]
% Output per hour (log) & 0.00 & 0.00 & & 0.100 & & & 0.285  \\
\\[-1ex] \hline
\\[-1ex]
[B] Concentrated product markets
\\[-1ex] \\ \hline
\\[-1ex]
Number of firms per product market & & 1.97 & & & 1.60 & & & 1.47 \\
\\[-1ex]
Sales-weighted average markup & & 1.74 & & & 2.32 & & & 2.59 \\
\\[-1ex]
\thickhline
\end{tabular} }\end{center}
\caption{Non-targeted moments
\protect \\ {Note: \small{} The cost-weighted average markup is from \cite{EMX}. Aggregate TFP is from \cite{F}. The value of log TFP in 1975 is normalized to zero.}
\label{tab:nontargeted_moments}}
\end{table}
% \begin{table}[ht!]
% \setlength{\tabcolsep}{0.3cm}  
% \begin{center}
% \begin{tabular}{lccc} 		\thickhline 
% \\[-1ex]
% Concentrated product markets & 1985 & 2007 \\ \hline
% \\[-1ex] 
% Number of firms per product market & 1.72 & 1.40 \\
% \\[-1ex]
% Average markup (simple average) & 1.96 & 2.58 \\
% % \\[-2ex]
% % Average markup (sales-weighted) & 2.08 & 2.80 \\
% % \\[-2ex]
% \\[-2ex]
% \thickhline
% \end{tabular} \end{center}
% \caption{product markets with $c>0$ (model moments) \label{tab:markups_moments}}
% \end{table}
Part [A] of Table \ref{tab:nontargeted_moments} reports the evolution of some non-targeted moments. When computing aggregate markups with cost-weights, we find an average of 1.24 in the 1975 economy, and an average of 1.34 in 2007. While these values are slightly above the recent estimates by \cite{EMX}, the time variation is similar in the model and in the data (10pp increase in the model, against 9pp increase in the data). To characterize some of the aggregate consequences of the change in the three structural parameters $\left(\lambda,c,f\right)$, we also report the evolution of aggregate TFP. Our model predicts an 16.7\% increase in aggregate TFP, which represents roughly half of the 29.6\% increase observed in the data.



Product markets facing positive fixed costs play an important role in our mechanism. Part [B] of Table \ref{tab:nontargeted_moments} provides a characterization of these product markets in the three calibrated economies. Product markets with positive fixed costs consist mostly of monopolies and duopolies \textemdash{} the average number of firms is 1.97 in the 1975 economy, 1.60 in 1990 and 1.47 in 2007. This implies an average markup of 1.75 in 1975, 2.32 in 1990 and of 2.59 in 2007 in these product markets. These values are within the bounds of estimates for the markup distribution of US firms. For example, \cite{LEU} report that the 90th percentile of the (sales-weighted) markup distribution increased from 1.57 in 1975 to 2.25 in 2007. Concentrated product markets represent 6.8\% of aggregate employment in the 2007 model, so approximately 1/15 of aggregate employment is concentrated in monopolist or duopolist firms. We regard these numbers are reasonable for two reasons. First, in our model a market can be as disaggregated as narrow product market-location pair. Second, the right tail of the empirical markup distribution displays levels consistent with monopolies and duopolies, given our calibrated elasticities, which are similar to the values found in other studies.

Table \ref{tab:HHI_distribution} shows the  distribution of HHIs obtained under the 2007 calibration. We also show the same moments reported by \cite{product_market_concentration}, who estimate concentration metrics for narrowly defined consumption-based product markets. The model closely matches both the 50th and the 90th percentiles of the empirical distribution of HHIs. An HHI of 0.5 is the one that would be obtained under a symmetric duopoly. This implies that both in our model and in the data 10\% of the markets have concentration metrics equal or higher than that of a symmetric duopoly. Therefore, even if we do not impose a particular level of aggregation in our calibration, the model can replicate the distribution of concentration for consumption-based product markets.

\begin{table}[ht]
\setlength{\tabcolsep}{0.2cm}  
\begin{center} \resizebox{14cm}{1.85cm} {
\begin{tabular}{ c c c c c c }
\thickhline
\\[-1ex]
 & $p\left(10\right)$ & $p\left(25\right)$ & $p\left(50\right)$ & $p\left(75\right)$ & $p\left(90\right)$ \\[2ex] \hline
 \\[-1ex]
model & 0.135 & 0.160 & 0.200 & 0.271 & 0.501 \\[2ex]
Data: local market \citep{product_market_concentration} & 0.0852 & 0.140 & 0.220 & 0.335 & 0.484 \\[2ex]
Data: national 
market \citep{product_market_concentration} & 0.0863 & 0.132 & 0.214 & 0.319 & 0.456 \\
\\[-1ex]
\thickhline 
\end{tabular} } \end{center}
\caption{Distribution of HHI within product markets: model \textit{versus} data
\label{tab:HHI_distribution}}
\end{table}

%Given that a market in our model can be as disaggregated as a product market-location pair, we regard these numbers as reasonable.

% In this sense we regard our calibration result that some of these \textit{product market}$\times$\textit{relevant competitive market} pairs are highly uncompetitive as a reasonable outcome.

\subsection{Quantitative Results}
%We start by comparing the steady-states of the 1985 and 2007 economies.

%We also include a parameterization for the years 1990, 1995 and 2000, assuming that average markups and markup dispersion  follow a linear trend between 1985 and 2007. Figure \ref{fig:ss_transition} shows the steady-state values of output per hour, aggregate TFP, the labor share and aggregate markups for the five different parameterizations.\footnote{In each of the five calibrations, the economy features two steady-states and is at the highest one.} Our model predicts an overall increase in aggregate output per hour between 1985 and 2007 of roughly 30\%. Aggregate TFP increases by 26\%. Note that the increase in both output per hour and aggregate TFP are driven by the increase in the tail of the Pareto distribution \textendash{} which results in a larger production possibility frontier.
%When looking at the data counterparts, we observe that real output per hour increases by 50\%, while aggregate TFP increases by 26\%. Therefore, through the lens of our model, the increase in the Pareto tail of the distribution of idiosyncratic draws can explain 60\% of the increase in real output per hour. Our model replicates, however, the evolution of aggregate TFP, which is a non-targeted moment. Regarding the labor share, our model predicts a 3.9 percentage point decline in the aggregate labor share (from 0.564 to 0.525). In the data, it falls by only 2 percentage points (from 0.615 to 0.595). Note that the labor share in our model is about 5 to 6 percentage points lower than the one observed in the data. Therefore, our model underestimates the level of the labor share, but overestimates its decline. Such a discrepancy can be explained by the fact that we target average markups for public firms, which tend to display larger profit shares (and hence lower labor shares) than the average firm in the economy.
%\begin{figure}[ht!]
%\centering{}\includegraphics*[scale=0.95]{input/model_data_ss_transition.eps}\caption{Model \textit{versus} data: 1985-2007.\protect \\ {Note: \small{} The data series are respectively (i) Business Sector: Real Output Per Hour of All Persons (from BLS), (ii) Aggregate TFP from \cite{F}, (iii) Business Sector: Labor Share (from BLS), and (iv) Aggregate Markup from \cite{LEU}.}} \label{fig:ss_transition}
%\end{figure}
Having calibrated the model, we solve the full dynamic problem, approximating the policy function of the household, by iterating on
the Euler equation. We describe the algorithm in Section \ref{sec:Quantitative-Model}. 
We start by comparing the dynamic properties of the 1975, 1990 and 2007 economies. Figure \ref{fig:businesscycle} shows the ergodic distribution of log output; the distributions are centered around the highest mode, so that the horizontal axis represents output in percentage deviation from the highest steady-state. We highlight three important observations. First, while the ergodic distribution of the 1975 economy is unimodal, the other two economies feature bimodal distributions, implying that these two economies are characterized by multiple (stochastic) steady-states. Through the lens of our model, multiple competition regimes are possible in economies characterized by levels of markups and fixed costs observed in 1990 and 2007, but not in 1975, when markups and fixed costs were lower.\footnote{As highlighted in discussion of Proposition \ref{prop:multiplicity} and later of Figure \ref{fig:Comparative-Statics}, changes in fixed costs can affect the condition for the existence of multiple steady-states.}
Second, relative to the 1990 economy, the 2007 model features a larger probability mass on the left, suggesting that the economy on average spends more time on the lowest regime, characterized by lower competition and output. Third, in the 2007 distribution, the two steady-states are also closer to each other \textemdash{} a transition from the high to the low regime implies a 19\% reduction in output in 2007, as opposed to approximately 30\% in 1990.
While this means that transitions are less pronounced in 2007, it also implies that they are substantially more likely in 2007 than in 1990, as we discuss below. The 1975 economy, instead, behaves similarly to a standard RBC model. This economy can suffer temporary recessions, but these will not have long-lasting consequences.
%Recall that the 1985 and the 2007 economies differ in the productivity dispersion parameter $\lambda$ and the fixed production cost in the \textit{concentrated} sector. In particular, the 2007 economy exhibits a more dispersed log normal distribution and larger fixed costs. These facts imply that, in 2007, the smallest firms in the \textit{concentrated} sector will be more sensitive to aggregate fluctuations. 
Table \ref{tab:business_cycle_moments} provides business cycle moments for the three economies.

\begin{figure}[htbp]
\hspace{-1cm}
\begin{minipage}[b]{.33\linewidth}
\centering\includegraphics*[scale=0.365]{input/hist_1975.eps}\subcaption{1975} \label{fig:y_dist_1975}
\end{minipage}%
\begin{minipage}[b]{.33\linewidth}
\centering\includegraphics*[scale=0.365]{input/hist_1990.eps}\subcaption{1990} \label{fig:y_dist_1990}
\end{minipage}
\begin{minipage}[b]{.33\linewidth}
\centering\includegraphics*[scale=0.365]{input/hist_2007.eps}\subcaption{2007} \label{fig:y_dist_2007}
\end{minipage}
\caption{Ergodic distribution of output \protect \\ {Note: \small{}\small{} This figure shows the distribution of log output for the 1975, 1990 and the 2007 economies. We simulate each economy for 10,000,000 periods and plot output in deviation from the high steady state.}} \label{fig:businesscycle}
\end{figure}
%
We next study the probabilities of deep recessions in the three economies. We simulate each economy 100,000 times for 40 and 100 quarters. We compute the fraction of simulations in which output experiences 10\%, 15\% or 20\% drop relative to the high steady state level (for at least 4 consecutive quarters). The results are shown in Table \ref{tab:ss_transition}. When running the 2007 economy for 40 quarters, output drops by at least 10\% in 19.3\% of the simulations, whereas the same figure for the 1990 economy is 9.6\%. In the 1975 economy this type of deep recession is extremely rare as it only occurs in 0.7\% of our simulations. Relative to 1990, the 2007 economy is approximately twice as likely to experience a 10\% fall in output over a 10-year period. Over 100 quarters, the 2007 economy appears about 1.67 times more likely to experience a 10\% recession (35\% probability in 2007, against 21.5\% probability in 1990). The same probability for the 1975 economy is 3.4\%. 
This implies that, in expectation, the 2007 economy experiences a recession larger than 10\% every 75 years, the 1990 economy does so every 120 years and the 1975 economy every 735 years. When focusing on larger recessions, the difference is even starker: the 1975 economy never has output drops larger than 15\%, while these events remain somewhat likely in the 2007 and 1990 economies. As a final remark on the ergodic properties of these economies, recall that the exogenous aggregate shocks process in unchanged across the three calibrations. The large observed differences in the ergodic behavior is fully driven by the endogenous response of the economies. The three calibrations only differ in parameters related to the firm heterogeneity and market structure. Therefore we attribute the observed differences in the business cycle properties of the three economies to the heterogeneity in  competitive structure. 
%This exercise suggests that the economy is between five to nine times more likely to experience large recessions in 2007 than the 1985 economy.
%To further illustrate the dynamic properties of our calibrated economies we next describe the response of several variables to exogenous TFP shocks.

\begin{table}[htbp]
\setlength{\tabcolsep}{0.2cm}  
\begin{center}
\resizebox{14cm}{1.85cm} {
\begin{tabular}{lccccccccc} 		\thickhline 
\\[-1.5ex]
&&  \multicolumn{2}{c}{1975 Model} & & \multicolumn{2}{c}{1990 Model} & & \multicolumn{2}{c}{2007 Model} \\ [0.5ex]
\hline  
\\ [-1ex]
& & T = 40 & T = 100 & & T = 40 & T = 100 & & T = 40 & T = 100
\\[-2ex]
\\ \hline
\\[-1ex] 
$\textrm{Pr} \big[$ 10\% recession $\big]$ & & 0.007 & 0.034 & & 0.096 & 0.215 & & 0.193 & 0.350 \\
\\[-1.75ex]
$\textrm{Pr} \big[$ 15\% recession $\big]$ & & 0.000 & 0.000 & & 0.018 & 0.082 & & 0.068 & 0.206 \\
\\[-1.75ex]
$\textrm{Pr} \big[$ 20\% recession $\big]$ & & 0.000 & 0.000 & & 0.002 & 0.035 & & 0.011 & 0.104 \\
\\[-1.75ex]
\thickhline
\end{tabular}} \end{center}
\caption{Probability of deep recessions \protect \\ {\small{} This table shows the probabilities of deep recessions in the 1975, 1990 and 2007 economies. Each economy starts in the highest steady-state and is simulated for $T=40$ and $T=100$ quarters. Each simulation is repeated 100,000 times. The table reports the fraction of simulations in which output is $ \kappa \%$ below the initial value for at least 4 consecutive quarters.} \label{tab:ss_transition}}
\end{table}
%
%
\begin{comment}
\begin{table}[htbp]
\setlength{\tabcolsep}{0.3cm}  
\begin{center}
\begin{tabular}{lccc} 		\thickhline 
\\[-1.5ex]
& 1975 Model & 1990 Model & 2007 Model
\\[1ex] \hline
\\[-1ex] 
mean & 3.90 & 4.17 & 4.37
 \\[1.5ex]
highest mode & 3.90 & 4.22 & 4.49
 \\[1.5ex]
standard deviation & 0.045 &	0.116	& 0.136
 \\[1ex]
\thickhline
\end{tabular} \end{center}
\caption{Simulated distribution of $\log \left(Y_t\right)$ \protect \\ {\small{} This table shows moments of the simulated distribution of $\log \left(Y_t\right)$. Each economy has been simulated for 10,000,000 periods.} \label{tab:y_dist_moments}}
\end{table}
\end{comment}
%
The likelihood of a transition is related to the distance between the steady states of the economy. It is possible that, while slumps are more frequent in the 2007 economy, they are associted with lower drops in output, relative to the 1990 economy. It is not ex-ante clear which effect dominates and therefore whether the 2007 economy should be more or less volatile than the 1990 one. To investigate this, we report additional moments of our simulated economies in Table \ref{tab:y_dist_moments}. The first row reports the average deviation of log output from the highest mode of the ergodic distribution. Since the 1975 distribution is symmetric around its unique mode, this deviation is zero. The 1990 and 2007 economies, on the other hand, feature sizeable deviations as they have multiple steady staes. In these economies, output is on average 5\% and 12\% below their respective high steady state. %As shown in Table \ref{tab:nontargeted_moments}, the increase of heterogeneity also implies level effects on productivity.\footnote{This effect is a combination of selection and shifting distribution. First, by changing $\lambda$, the parameter governing the productivity dispersion, while fixing the location parameter $\mu=0$, we are changing the average draw of the distribution. Secondly, the selection effect, namely that the best firms operate, implies that with higher dispersion the selected firms have a higher productivity.} As a consequence aggregate TFP is higher in 2007 than in 1990 and 1975. In the second row, we report the deviations of average log output from the 1975 average. Average outpuput is 27\% higher in 1990 economy and 47\% in 2007. This effect is due solely to the changes in the parameters governing the market structure, as discussed above. 
%Relative to 1990, the 2007 economy features a smaller distance between the two stochastic steady-states. However, as shown in Table \ref{tab:ss_transition}, the probability of transitions is considerably higher in 2007. Therefore, it is ex-ante unclear whether output volalitility should be higher in the 2007 economy relative to 1990. 
The second row of Table \ref{tab:y_dist_moments} shows that higher firm heterogeneity and fixed costs result in higher volatility. The higher likelihood of transitions dominates and relative 1975, the 1990 and 2007 economies are 2.5 and 3 times more volatile. 
%
\begin{table}[ht]
\setlength{\tabcolsep}{0.3cm}  
\begin{center}
\begin{tabular}{lccc} 		\thickhline 
\\[-1.5ex]
& 1975 Model & 1990 Model & 2007 Model
\\[1ex] \hline
\\[-1ex] 
$\overline{\log Y}-{\log Y^H}$ & 0.00 & -0.05 & -0.12
% \\[1.5ex]
%$\overline{\log Y}-{\log Y_{1975}^H}$ & 0.00 & 0.27 & 0.47
 \\[1.5ex]
$\sigma_{\log Y}$ & 0.045 &	0.116	& 0.136
 \\[1ex]
\thickhline
\end{tabular} \end{center}
\caption{Simulated distribution of $\log \left(Y_t\right)$ \protect \\ {\small{} This table shows moments of the simulated distribution of $\log \left(Y_t\right)$. Each economy has been simulated for 10,000,000 periods. $\overline{\log Y}-{\log Y^H}$ is the average log deviation of output from the high steady state output. %Similarly, $\overline{\log Y}-{\log Y_{1975}^H}$ compares the average log deviation of output from the steady state of the 1975 economy.
Lastly, $\sigma_{\log Y}$ is the standard deviation of log output.} \label{tab:y_dist_moments}}
\end{table}

% \begin{table}[htbp]
% \setlength{\tabcolsep}{0.3cm}  
% \begin{center}
% \begin{tabular}{lccccccccc} 		\thickhline 
% \\[-1.5ex]
% &&  \multicolumn{2}{c}{1975 Model} & & \multicolumn{2}{c}{1990 Model} & & \multicolumn{2}{c}{2007 Model} \\ [0.5ex]
% \hline  
% \\ [-1ex]
% & & T = 40 & T = 100 & & T = 40 & T = 100 & & T = 40 & T = 100
% \\[-2ex]
% \\ \hline
% \\[-1ex] 
% $\textrm{Pr} \big[$ 10\% recession $\big]$ & & 0.002 & 0.018 & & 0.065 & 0.173 & & 0.148 & 0.305 \\
% \\[-1.75ex]
% $\textrm{Pr} \big[$ 15\% recession $\big]$ & & 0.000 & 0.000 & & 0.009 & 0.063 & & 0.046 & 0.177 \\
% \\[-1.75ex]
% $\textrm{Pr} \big[$ 20\% recession $\big]$ & & 0.000 & 0.000 & & 0.000 & 0.026 & & 0.004 & 0.085 \\
% \\[-1.75ex]
% \thickhline
% \end{tabular} \end{center}
% \caption{Probability of deep recessions \protect \\ {\small{} This table shows the probabilities of deep recessions in the 1975, 1990 and 2007 economies. Each economy starts in the high steady-state and is simulated for $T=40$ and $T=100$ quarters. Each simulation is repeated 100,000 times. The table reports the fraction of simulations in which output is $ \kappa \%$ the initial value for at least 8 consecutive quarters.} \label{tab:ss_transition_2}}
% \end{table}

%There is one aspect about our calibration strategy that should be discussed. In particular, the parameters determining the dynamics of TFP shocks ($\rho_{z}$ and $\sigma_{\varepsilon}$) are the same in the two economies. We do not change these parameters because we want to focus on the role of the parameters determining the unconcentrated structure of the economy ($\lambda$, $c$ and $f$).\footnote{There are however reasons to think that $\rho_{z}$ and $\sigma_{\varepsilon}$ changed over time. We will return to this point later.}



\paragraph{Impulse Response Functions: Small Negative Shock}
We characterize the reaction of the economy to a small negative shock. We consider a shock to the innovation of the exogenous TFP process that is equal to $\varepsilon_t = - \sigma_{\varepsilon}$  and lasts for four quarters. Figure \ref{fig:IRF_small_shock} shows the impulse responses for 1975, 1990 and the 2007 economy. The simulation of the transition dynamics covers 100 quarters.  This shock generates different responses for the three economies. The 2007 economy exhibits both greater amplification and persistence.  First, the 1975 economy experiences a 3.8\% reduction in aggregate output after 5 quarters, against a 4.7\% in 1990 and a 5.7\% reduction in the 2007 economy. Second, after 100 quarters, the 1975 economy is 1.0\% below the steady-state, while the 1990 economy is 2.5\% below trend and the 2007 economy has a much more prolonged downturn, being still 5.6\% below pre-crisis output. Eventually they converge back to the initial level.

The mechanism underlying such increased amplification and persistence can be understood by looking at the bottom panel, which plots the transition dynamics of the number of firms in \textit{concentrated} product markets. In 2007, there is a much more significant reduction in the number of firms, due to the mechanisms outlined above: increased productivity dispersion and larger fixed costs make small, unproductive firms more sensitive to aggregate shocks. This additional action in the extensive margins generates both additional amplification and persistence. Quantitatively we have that on impact, in 1975, about 0.35\% of firms in concentrated product markets exit, while this number is 5.9\% for 2007. The slow net entry as the economy goes back to the original steady state drives the large persistence of the contraction.


\paragraph{Impulse Response Functions: Large Negative Shock}

The shock introduced above was small enough to make all three economies converge back to their initial steady-states, albeit in very different time horizons. We now study the effect of a larger shock. We repeat the same exercise for the three economies, but now introduce a negative shock $\varepsilon_t = - 2 \sigma_{\varepsilon}$, which lasts for six quarters. The dynamics are shown in Figure \ref{fig:IRF_big_shock}. As before, there is greater amplification and persistence in the 2007 economy. However, this economy now experiences a permanent drop in aggregate output, i.e. it transitions to a lower steady-state. In the example we consider, after 100 quarters, output is 12.2\% below its initial value. Note, however, that the gap is still widening at the end of the sample. This is due to a permanent loss of 13.9\% of active firms in concentrated product markets. The 1975 and 1990 economies, on the other hand, converge back to the pre-crisis levels of both firms and output.
%
\begin{figure}[ht]
\hspace{-0.0cm}
\begin{minipage}[b]{.5\linewidth}
\centering\includegraphics*[scale=0.75]{input/IRF_small_shock.eps}\subcaption{Small Negative Shock} \label{fig:IRF_small_shock}
\end{minipage}%
\hspace{-0.75cm}
\begin{minipage}[b]{.5\linewidth}
\centering\includegraphics*[scale=0.75]{input/IRF_big_shock.eps}\subcaption{Large Negative Shock} \label{fig:IRF_big_shock}
\end{minipage}
\caption{Impulse Response Functions\protect \\ {Note: \small{} The graphs show the IRFs to an exogenous TFP shock. In panel (a), we feed a shock $\varepsilon_t = - \sigma_{\varepsilon}$ that lasts for four quarters. In panel (b), we feed $\varepsilon_t = - 2 \, \sigma_{\varepsilon}$ during six quarters.}} \label{fig:IRF_figure}
\end{figure}


These results suggest that rising firm differences and fixed costs are a source non-linearity in the economy's response to aggregate shocks. This may appear to be inconsistent with the idea of a \textit{great moderation} \textemdash{} namely, the fact that the volatility of aggregate output declined between 1980 and 2007. Note, however, that aggregate volatility in our economy is the product of two forces \textemdash{} exogenous volatility (TFP shocks) and endogenous amplification and persistence. If exogenous volatility declined over time, it is possible that aggregate volatility also declined in spite of larger amplification. There are reasons to think that exogenous aggregate volatility may have decreased over time \textendash{} for example, because of demographic shifts \citep{JS_AER} or a rising share of low-volatility industries \citep{GC}.

We next use our model as a laboratory to study the 2008 recession.

==> submitted_version/5_2008_crisis.tex <==


\section{The 2008 Recession and Its Aftermath}\label{sec:aggregatefacts}
In this section, we take a closer look at the 2008 recession and its aftermath. The left panel of Figure \ref{fig:GR_data_model} shows the behavior of four aggregate variables from 2006 to 2019 \textemdash{} real GDP, real gross private investment and total hours (all in per capita terms), as well as aggregate TFP. All variables are in logs, detrended (with a linear trend computed over 1985\textendash{}2007) and centered on 2007Q4. The four variables decline on impact and do not rebound to their pre-recession trends. For example, in the first quarter of 2019, real GDP per capita is 14.2\% below trend (Table \ref{tab:great-recession}). Aggregate TFP experienced a 8.2\% negative deviation from trend. Investment declines by more than 40\% on impact, and then stabilizes at approximately 15-20\% below the pre-crisis trend.

\begin{figure}[ht]
\begin{minipage}[b]{.5\linewidth}
\centering{}\includegraphics*[scale=0.525]{input/GR_transition_data.eps}\subcaption{Data \label{fig:GR_data}}
\end{minipage}%
\begin{minipage}[b]{.5\linewidth}
\centering{}\includegraphics*[scale=0.525]{input/GR_transition_2007.eps}\subcaption{2007 Model \label{fig:GR_model}}
\end{minipage}
\caption{The great recession and its aftermath \protect \\ {Note: \small{} The figure shows the evolution of key macro aggregates in the aftermath of the 2008 recession in the data (Panel a) and the model (Panel b). The model is subjected to a sequence of six quarter shocks $\left\{\varepsilon_{t}\right\}$ to match the dynamics of aggregate TFP in the data between 2008Q1:2009Q2. See Appendix \ref{sec:Data-Appendix} for data definitions.}} \label{fig:GR_data_model}
\end{figure}

\begin{table}[ht]
\setlength{\tabcolsep}{0.4cm} \begin{center} \resizebox{17cm}{2.15cm} {
\begin{tabular}{c c c c || c c c c} \thickhline
& & & & & & \\[-1.5ex]
& \multicolumn{3}{c||}{\Large Data} & \multicolumn{4}{c}{\Large Model} \\[1ex]
& {\large 2009Q4} & {\large 2015Q1} & {\large 2019Q1} & {\large 2009Q4} & {\large 2015Q1} & {\large 2019Q1} & {\large 2040Q1} \\
\\[-2.25ex]
\thickhline
& & & & & & \\[-1.25ex]
{\large Output} & -0.088 & -0.126 & -0.142 & -0.107 & -0.118 & -0.123 & -0.142 \\[1ex]
{\large TFP} & -0.045 & -0.026 & -0.082 & -0.039 & -0.023 & -0.019 & -0.018 \\[1ex]

{\large Hours} & -0.130 & -0.078 & -0.055 & -0.086 & -0.094 & -0.098 & -0.113 \\[1ex]
{\large Investment} & -0.340 & -0.109 & -0.147 & -0.247 & -0.169 & -0.151 & -0.157 \\[1ex]

\thickhline 
\end{tabular}}
\end{center}

\caption{The great recession and its aftermath \label{tab:great-recession}}
\end{table}


We then ask whether our model can replicate the behavior of these four variables. To this end, we feed the model a sequence of shocks $\varepsilon_{t}$ (i.e. the innovation of $A_t$) that lasts for six quarters (2008Q1:2009Q2); these shocks are calibrated so that aggregate measured TFP in our model (i.e. $A_{t} \: \Phi_{t}$) matches the dynamics of its data counterpart over the same period. The economy starts at the high steady-state
(with $z_{t}=0$). We set the innovations to productivity to zero after 2009Q2 and let the economy recover. The right panel of Figure \ref{fig:GR_data_model} shows the implied responses of output, aggregate TFP, employment and investment, generated by our model. As the figure shows, this series of shocks triggers a transition to the low steady-state. Our model provides a very good description of the evolution of the four variables. Output experiences a decline of 12.3\% after 10 years, whereas hours drop by 9.8\% (Table \ref{tab:great-recession}). Both reactions are of the same order of magnitude as observed in the data.\footnote{In the data, hours worked seem to recover faster than output, which seems inconsistent with a jobless recovery. Note, however, that i) we are showing variables in deviation from trend and that ii) hours worked were characterized by slower growth (and hence a flatter trend) before the crisis. For example, total hours worked were stagnant between 2000-2007.} Additionally,  our model predicts a 24.7\% decline on impact for investment, and a 15.1\% drop by 2019 (14.7\% in the data). Finally, we observe a long-run decline of aggregate TFP, representing approximately 1/5 of the drop in the data (1.6\% in the model, 8.2\% in the data). We discuss the mechanisms underlying this result in the next section. The crisis experiment in our model can also replicate the still widening gap between output and its trend throughout our sample. Importantly, the model economy after 30 years shows a permanent deviation from the pre-crisis trend (last column of Table \ref{tab:great-recession}). Output is 14.2\% lower while hours and investment are 11.3 and 15.7\% below trend. The economy therefore features a change in steady-state to one with lower output and competition.
%In summary, our model can successfully replicate the 2008 crisis and its persistent effects and predicts a permanent deviation even after more than 30 years.

%We ask whether these effects should be attributed to the nature and magnitude of the shock or to the features of the underlying economy.
%Next, we ask whether the behavior of the US economy after 2008 has been mostly a reaction to an unusually large shock, or can also be attributed of its technological features.
Next, as our first counterfactual, we ask whether the same sequence of aggregate TFP shocks used in the 2007 economy can also trigger a transition to the low steady-state in the 1975 and 1990 economies. We study this experiment to ask whether the deviation our model predicts for the 2007 economy is driven by an unusually large shock or by inherent fragility of the economy itself. Figure  \ref{fig:GR_data_model_85_1} and Table \ref{tab:great-recession-counterfactual-models} show the transitional dynamics. Both economies exhibit substantially less amplification, and, importantly, they also revert to their pre-crisis steady-states. 
\begin{figure}[ht!]
\begin{minipage}[b]{.5\linewidth}
\centering{}\includegraphics*[scale=0.525]{input/GR_transition_1975.eps}\subcaption{1975 Model \label{fig:GR_1975}}
\end{minipage}%
\begin{minipage}[b]{.5\linewidth}
\centering{}\includegraphics*[scale=0.525]{input/GR_transition_1990.eps}\subcaption{1990 Model \label{fig:GR_1990}}
\end{minipage}
\caption{The \textit{great recession} in the 1975 and 1990 models \protect \\ {Note: \small{}This figure shows the response of the 1975 and 1990 economies to the sequence of shocks used in Figure \ref{fig:GR_model}} \label{fig:GR_data_model_85_1}}
\end{figure}
%
\begin{table}[ht!]
\setlength{\tabcolsep}{0.4cm} \begin{center} \resizebox{16cm}{2.15cm} {
\begin{tabular}{c c c c || c c c} \thickhline
& & & & & & \\[-1.5ex]
& \multicolumn{3}{c||}{\Large 1975 Model} & \multicolumn{3}{c}{\Large 1990 Model} \\[1ex]
& {\large 2009Q4} & {\large 2019Q1} & {\large 2040Q1} & {\large 2009Q4} & {\large 2019Q1} & {\large 2040Q1} \\
\\[-2.25ex]
\thickhline
& & & & & & \\[-1.25ex]
{\large Output} & -0.065 & -0.038 & -0.010 & -0.089 & -0.072 & -0.037 \\[1ex]
{\large TFP} & -0.025 & -0.003 & -0.000 & -0.033 & -0.009 & -0.003 \\[1ex]

{\large Hours} & -0.048 & -0.028 & -0.007 & -0.069 & -0.056 & -0.029 \\[1ex]
{\large Investment} & -0.148 & -0.035 & -0.006 & -0.205 & -0.079 & -0.032 \\[1ex]

\thickhline 
\end{tabular}}
\end{center}

\caption{The great recession and its aftermath \label{tab:great-recession-counterfactual-models}}
\end{table}
In economies with the 1975 and 1990 features, a negative aggregate shock of the magnitude required in our model to generate the 2008-2009 recession would not be large enough to induce a persistent deviation from trend. These economies would have experienced a faster reversal to trend. For example, as of 2019, output would be 3.8\% and 7.2\% below trend (in the 1975 and 1990 economies, respectively), against 12.3\% of the 2007 model and 14.2\% as observed in the data. When we evaluate the longer run behavior in 2040, we find that the 1975 economy would experience a 1\% drop, while for the 1990 economy this figure is 3.7\%. We conclude that the structural differences between the 1975, 1990 and the 2007 economies (namely larger productivity differences and higher fixed costs) are key to understanding the 2008 crisis and the subsequent \textit{great deviation}. Next we provide empirical evidence consistent with our proposed mechanism both at the aggregate and industry level.


\subsection{Empirical Evidence}

According to our model, a transition between steady-states is driven by a change in the competitive regime of the economy. We now provide evidence consistent with our model's mechanism. In particular, we show that after 2008 the US economy experienced i) a persistent decline in the number of active firms, ii) a persistent decline in the aggregate labor share and iii) acceleration in the aggregate profit share and markup. Furthermore, the model has stark predictions about how product markets starting with different levels of concentration should feature different responses to the negative shock. The extensive margin is more elastic in product markets with higher concentration to begin with; as a consequence, we should observe that these product markets experience a larger drop in output. We provide cross-industry evidence corroborating this prediction.


\subsubsection{Aggregate Level Evidence}
We begin by reviewing the evidence at the aggregate level on the number of firms in the economy, the behavior of markups, labor and profit shares and the dynamics of aggregate TFP.

\paragraph{Number of Firms}
Firms in our model are single-product and operate in only one market. This contrasts with the definition of firms in the data, which are often multi-product and operate in several markets (e.g. geographic segmentation). As a consequence, studying the dynamics of the number of firms probably provides a lower bound on the effects through the extensive margin as some firms might remain in market but remove products or close establishments. With this caveat in mind, we ask whether the evolution of the number of firms in the data qualitatively matches the prediction of our model. Figure \ref{fig:nfirms_total} shows the evolution of the number of active firms (with at least one employee). As the figure shows, the number of active firms experiences a persistent deviation from trend after 2007. As of 2016, the number of active firms was 0.151 log points below trend. Such a persistent decline can also be observed within most sectors of activity (Section \ref{sec:numberfirms}). %As we show below, the decline in the number of firms was more pronounced in industries featuring initially higher concentration.
With the caveat that a firm in our model do not necessarily represents a firm in the data, we report the evolution of the number of firms in the \textit{concentrated} sector. As shown in Table \ref{tab:great-recession-labor-share}, this sector experiences a persistent decline in the number of firms of 0.134 log points.
%
\begin{figure}[ht]
\begin{centering}
\includegraphics*[scale=0.485]{input/nfirms_total} 
\par\end{centering}
\caption{\textbf{Number of Firms: 1978-2018}\protect \\ {Note: \small{} The red line shows the number of firms with at least one employee (in logs). The dashed grey line shows a linear trend computed for the period 1978-2007. Data is from the US Business Dynamics Statistics. \label{fig:nfirms_total}}}
\end{figure}

We think that alternative models could replicate this figure only if they featured an active extensive margin, multiple steady states and predicted a transition during the 2007-08 recession. We argue that these features and the changes in the market structure, which we discuss next, corroborate our proposed mechanism.
\paragraph{Aggregate Markups, Labor and Profit Shares}
We now ask how our model compares to the data regarding the evolution of labor and profit shares after 2008. Figure \ref{fig:US-LS-Markup-Trend} shows the evolution of the labor share, the profit share (both computed for the US business sector) and the aggregate markup series for publicly listed firms from \cite{LEU}. The grey dashed lines represent linear trends computed for the period 1975\textendash{}2007.


\begin{figure}[ht!]
\centering
\includegraphics*[scale=1.1]{input/US_ls_markup_trend}\caption{\textbf{Aggregate Markup and Labor and Profit Share: 1975-2019}\protect \\ {Note: \small{}This figure shows (i) labor share of the US business sector (from the BLS), (ii) the profit share of the US business sector (defined in Appendix \ref{sec:Data-Appendix}) and (iii) the aggregate markup series for COMPUSTAT firms from \cite{LEU}. The dashed grey lines represent linear trends computed for the 
period 1975\textendash{}2007.\label{fig:US-LS-Markup-Trend}}}
\end{figure}

Table \ref{tab:great-recession-labor-share} compares the evolution between 2007 and 2016 observed in the data and obtained in our model.\footnote{The aggregate profit share in our model is net of fixed production costs.} Our model predicts a 0.6pp decline in the aggregate labor share, approximately 17\% of the observed decline between 2007 and 2016. If we account for a pre-crisis trend, we explain 22\% of the deviation in 2016. For the profit share, we can explain 30\% of its 3pp increase from trend. Markups increase by 4.1 points in our model, which represents 29\% of the observed increase (14.2 points) and 64\% of the deviation from the pre-crisis trend (6.4 points).\footnote{ Other studies have also documented a sharp rise in markups in the post-crisis years. For example, \cite{rising_markups} use US product-level data and document a 25\% increase in markups between 2006 and 2019.}

\begin{table}[ht!]
\setlength{\tabcolsep}{0.2cm} \begin{center}
\begin{tabular}{cc|cc} \thickhline
& & & \\[-1.25ex]
& Model & \multicolumn{2}{c}{Data} \\[1ex]
& $\Delta_{2007-2016}$ & $\Delta_{2007-2016}$ & $\Delta_{2007-2016} - \Delta_{\textrm{trend}}$ \\[1ex]
\hline
& & & \\[-1.25ex]
(log) Number of Firms  & -0.134 & -0.014 & -0.151 \\[0.25ex]
(\textit{concentrated} product markets)  & & & \\[1ex]
& & & \\[-1.25ex]
Labor Share & -0.005 & -0.029 & -0.023 \\[1ex]
Profit Share & 0.009 & 0.032 & 0.030 \\[1ex]
Aggregate Markup & 4.1 & 14.2 & 6.4 \\[1ex]
\thickhline 
\end{tabular}
\end{center}
\vspace{-0.5cm}
\caption{Change in the number of firms and in income shares: model \textit{versus} data \label{tab:great-recession-labor-share}}
\end{table}

\paragraph{Aggregate Productivity}\label{aggrtfp}

As shown in Figure \ref{fig:GR_data_model}, the post-2008 growth experience has also been characterized by a persistent decline of aggregate TFP from trend. Our model predicts a persistent fall in aggregate TFP (though of smaller magnitude than the one observed in the data). In our model, this happens in spite of the exit of unproductive firms, which results in higher average firm-level TFP, the ``cleansing effect of recessions'' (see Figure \ref{fig:TFP_Model_transition}).
There are two reasons explaining the decline in aggregate TFP. First, there is a \textit{love-for-variety} effect, associated with the reduction in the number of firms. This can best be seen in the limit case in which all product markets have $n$ firms with identical productivity $\tau$. In such a case, aggregate TFP is equal to $\Phi=I^{\frac{1-\rho}{\rho}}n^{\frac{1-\eta}{\eta}}\tau$. Second, in a low competition trap, there is higher cross product market misallocation. This happens because markets with a larger contraction are the ones with positive fixed costs $c>0$, i.e. whose output is already low.\footnote{Figure \ref{fig:output_dispersion_transition} (Section \ref{sec:Quantitative-Model}) shows that the standard deviation of  outputs, $\text{std}_i \left( \log y_{it} \right)$, increases.}

% In summary, our model provides two possible reasons why aggregate TFP may have experienced a permanent drop after 2008.
% Consistent with the model, such a drop in aggregate TFP may have occurred in spite of the exit of low productivity firms.\footnote{\cite{FGH} show that, as in previous recessions, manufacturing firms exiting during the great recession were on average less productive.}

The macro trends discussed above suggest that, consistent with our model, market power accelerated after 2008. Alternative models would be able to generate these empirical pattern if they featured cyclical changes in the level of competition, so that, over the business cycle profit and factor shares would move. 
We next review the cross-sectional implications of our model and test them in the data.


\subsubsection{Industry Level Evidence}\label{sec:empiricalevidence}
According to our model, product markets featuring a larger concentration in 2007 should have experienced a larger contraction in 2008. This prediction follows from equation (\ref{eq:firm_FOC}), which establishes a positive link between productivity, market shares and markups (for a given number of active firms). Therefore, if we take two markets with the same number of firms, the one featuring a more uneven distribution of productivities will have a larger dispersion in market shares and hence a larger concentration. In these markets, firms at the bottom of the distribution will be smaller and charge lower markups, and will hence be more likely to exit upon a negative shock. This prediction holds for a given number of firms $n_{it}$, so that, when measuring the correlation between concentration in 2007 and the size of the contraction in 2008, we must control for the number of firms in the industry.

We build a dataset combining the 2002 and 2007 US Census data on industry concentration to the Statistics of US Businesses (SUSB) and the Bureau of Labor Statistics (BLS) to obtain outcomes as employment, total wage bill and the number of firms at the industry level (6-digits NAICS). The final dataset includes 791 6-digit industries. In 2016, the median industry had 1,316 firms, 36,910 workers and a total payroll of \$1,880 million.

To assess whether industries with a larger concentration before the crisis experienced a larger post-crisis decline, we estimate the following regression 
\[
\dfrac{\Delta y_{i,07-16}}{y_{i,07}}=\beta_{0}+\beta_{1}\;\textrm{concent}_{i,07}+\beta_{2}\; \log \textrm{firms}_{i,07} +\beta_3 \dfrac{\Delta y_{i,03-07}}{y_{i,03}} + a_s \mathbbm{1}\{i\in s\}+u_{i}.
\]
$y_i$ is an outcome for industry $i$ (for example total employment, total wage bill or total number of firms) and $\textit{concent}_i$ is the share of the 4 largest firms (scaled by the share of the largest 50); we also control for the number of firms before the crisis ($\textrm{firms}_{i,07}$). Importantly, to control for possible differences in the pre-crisis dynamics, e.g. different growth opportunities in different industries, we include pre-trends in the regression. The outcomes always take the form of the annualized growth rate between 2007 and 2016 in a specific industry. In all regressions, we will also include sector fixed effects $\left(a_s\right)$. The unit of observation is a 6-digit industry.


We start by studying the correlation between the change in employment between 2008 and 2016 and concentration in 2007. The results are compactly presented in Table \ref{empirics_main} and robustness are shown in Appendix \ref{sec:reg-tables}. We find that more concentrated industries experienced lower employment growth in the aftermath of the great recession. Quantitatively, a 1pp higher pre-crisis concentration is associated with a 2pp lower employment growth rate between 2007 and 2016. This pattern holds irrespective of the inclusion of the number of firms in 2007. To address the concern that industries with larger concentration in 2007 could have already exhibited lower growth before the crisis, we include cumulative employment growth between 2003 and 2007 as a control; the results do not change. Finally, the results are also robust to the inclusion of sector fixed effects. While these results concern the evolution of employment growth, a similar pattern is found if we use the total wage bill instead . We also study the correlation between concentration and net entry after the crisis . Our findings suggest that a 1pp increase in the concentration measure is associated with a 2-3pp decrease in the post-crisis net entry.
These results suggest that industries with larger concentration in 2007 experienced a larger contraction in activity after the crisis. 
%They do not tell us however whether these industries experienced a larger increase in profit margins or a larger decline in labor shares.


\begin{table}[ht]
\setlength{\tabcolsep}{0.1cm}  \begin{center}
\scalebox{.8}{\begin{tabular}{lcccc} 				\thickhline
			\\[-2ex]
			 & (1) & (2) & (3) & (4) \\
			 \\[-1.5ex]
			VARIABLES & $\Delta \log \textrm{emp}_{07-16}$ & $\Delta \log \textrm{payroll}_{07-16}$ & $\Delta \log \textrm{firms}_{07-16}$ & $\Delta \textrm{labor share}_{07-16}$ \\
			\\[-1.5ex]
            \thickhline
			&  &  &  \\
			$ \textrm{concent}_{07} $ & -0.0177*** & -0.0189*** &-0.0406*** & -0.0314*\\
			& (0.00682) & (0.00697)&(0.00635)&(0.0167) \\
			&  &  &  & \\
			$ \log \textrm{firms}_{07} $ & 0.00193*** &0.00164** &0.00119* &-0.00120 \\
			&   (0.000706) & (0.000725)&(0.000661) & (0.00240)\\
			&  &  &  & \\
			$\Delta \log \textrm{y}_{03-07}$ &  0.0984***  &0.0823*** &0.0881*** &0.169*\\
			&   (0.0241) & (0.0219)&(0.0270)&(0.0867) \\
			&  &  &  &  \\
			Observations & 769 &773 & 791&98\\
			R-squared  & 0.050 & 0.043& 0.078&0.075 \\
			\\[-2ex] \thickhline
			\\[-2ex]
			\multicolumn{5}{c}{ Standard errors in parentheses} \\
			\multicolumn{5}{c}{ *** p$<$0.01, ** p$<$0.05, * p$<$0.1} \\
\end{tabular} }
\caption{Cross-industry regressions\protect \\ {Note: \small{} the table shows the results of regressing the growth rate of sectoral employment, payroll, number of firms and labor share between 2007 and 2016 on the measure of concentration in 2007 and controls. Robustness on these regressions are displayed in Appendix \ref{sec:reg-tables}.}}
\label{empirics_main}
\end{center}
\end{table}

We conclude this section by providing evidence on the evolution of the labor share across industries. While the US census of firms provides data on total employment and the total number of firms for all 6-digit industries, it does not contain data on the labor share. We rely on data from the BLS `Labor Productivity and Cost' programme (see Appendix \ref{sec:Data-Appendix} for details). This database, however, only provides data on the labor share for a restricted group of industries. We find a negative relationship between the post-crisis change in the labor share and the pre-crisis level of concentration. Industries with larger concentration in 2007 experienced a larger drop in labor share between 2008 and 2016.

In summary, these results suggest that the structure of US product markets in 2007 is important to understand the consequences of the 2008 crisis. The results presented are purely cross-sectional \textemdash{} industries with a larger concentration in 2007, displayed a larger post-crisis contraction. We think, however, that they support one of the main insights of the model \textemdash{} rising concentration can have made the US economy more vulnerable to aggregate shocks.

Taken together we view the empirical evidence reported here as corroborating our proposed mechanism. The aggregate economy shows a long-lasting deviation and a widening gap from the pre-crisis trend and a change in the distribution of incomes from factor suppliers to firms, suggestive of an increase in market power. At the industry level we observe that industries respond differentially depending on the pre-existing market structure. Our model shows that the latter observation and its implications for the distribution of rents in the economy can explain the quasi-permanent deviation at the macro level.

\subsection{Robustness Checks}\label{subsec:robustness}

In the previous section we described how a calibrated version of the model admits multiple stochastic steady states and performs well when tasked with replicating the behavior of the US economy in the aftermath of the 2008 recession. In this section we study two robustness checks on our model. First we subject the same economies to the aggregate shocks needed to match the 1990 recession. Next we check whether our modelling choices on the structure of the fixed cost, which is expressed in terms of the \textit{numeraire} output good, matter for our results.

\paragraph{The 1990 Recession}
Through the lens of our model, the 2008 crisis made the US economy transition to a new steady-state. This fact has not been observed after any other postwar recession. This raises a natural question: what was special about the 2008 crisis? Was the shock hitting the economy in 2008 larger than in previous recessions? Or was the economy more fragile in 2008 and therefore more prone to experience a transition even for moderate shocks? Earlier in this section we showed that the same shocks underlying the 2008 recession in our model do not trigger transitions in the 1975 and 1990 economies. We show that this holds for other recessions. We repeat the experiment of Section \ref{sec:aggregatefacts} using the 1990 crisis. We feed the 1990 economy a sequence of shocks that replicates the dynamics of aggregate TFP during the 1990\textendash{}1991 recession (1990Q3:1991Q1). We then take this same sequence of exogenous shocks and apply them to the 2007 economy.
The results of this experiment are shown in the Supplementary Material Section \ref{sec:90_recession}. When looking at the response of the 1990 economy, we observe a temporary decline in all variables, but followed by a gradual recovery to the previous steady-state.
%\footnote{The recovery seems to be slower than in the actual data. Note, however, that by design we are shutting down possible positive shocks hitting the economy in 1991 and afterwards.}
This contrasts with the response of the 2007 economy, which eventually experiences a transition to the lower steady-state. These results suggest that, rather than the consequence of an unusually large shock, the post-2008 deviation can be linked to an underlying market structure that made the US economy more fragile to negative shocks.











%\paragraph{Alternative values for the elasticity of substitution} The first robustness check we carry out is a different parametrization of the key elasticities in our model. In particular, we use the values from \cite{de2021quantifying} and set the cross-industry elasticity at $\sigma_{I} = 1.2$ and the within-industry elasticity of at $\sigma_{G} = 5.75$. The model retains multiplicity of steady states. As in our benchmark model, when hit with the aggregate shocks to generate the 2007 TFP response, we find that the 1985 converges to the same steady state while the 2007 economy falls in a low competition trap. The calibration, the ergodic distribution and the crisis experiment are all reported in Section \ref{subsec:new-calibration-ES}.



\paragraph{Variable fixed costs}

In the model presented so far firms pay a fixed cost $c>0$ in units of the final good. This assumption implies that the cost of entry is independent of the state of the economy and, hence, of its competition regime and of factor prices. If fixed costs were to change with factor prices, entry could be cheaper (more expensive) in a low (high) competition regime, which could in principle eliminate steady-state multiplicity. To address this concern, we let firms hire labor and capital to pay the fixed cost. In particular we assume production entails a fixed cost $ c \, = \, k_c^\alpha \, l_c^{1-\alpha}$. 
Under this assumption, firms pay an effective fixed cost $\Theta_{t} \cdot c$. Since the factor cost index $\Theta_t$ is increasing in the number of active firms, entry becomes more expensive as firms enter. 
%We update the labor and capital market clearing conditions accordingly.
Appendix \ref{sec:var_fixed_costs} shows the results for this version of the model. The existence of two competition regimes is preserved under this alternative assumption (for the 1990 and 2007 calibrations). We also obtain responses for the crisis experiment performed above and the results are qualitatively and quantitatively similar to the benchmark model.


==> submitted_version/6_policy_experiment.tex <==


\section{Policy Experiment}\label{policy}

We conclude by studying the role of policy in our model. In this economy, in addition to the standard (static) inefficiencies associated with markups and markup dispersion, market power carries additional negative consequences as it can trap the economy in a low competition regime.

We consider a government which grants an entry subsidy equal to a fraction $\tau_f\in\left[0,1\right]$ of the fixed cost, while
levying a tax $\tau_{\pi}\in\left[0,1\right]$ on net profits $\tilde{\Pi}_{ijt} \coloneqq \Pi_{ijt} - \left(1-\tau_f\right)c_{i}$ to balance the budget. 
First, note that by design the entry subsidy affects only \textit{concentrated} product markets. Secondly, since the government is taxing only the amount of profits in excess of fixed costs, the tax $\tau_\pi>0$ does not create a disincentive to entry. It also does not distort firm size conditional on the market structure, since firms' optimal size is given by the zero marginal profit condition $\pi^\prime = 0 = (1-\tau_{\pi})\pi^\prime$.
Finally, a positive entry subsidy will reduce the entry productivity thresholds. The planner faces, however, one key trade-off when subsidizing entry: while having more firms in the economy reduces markups and increases available varieties, it also implies that more resources are spent in fixed costs and that less productive firms enter the market.

We report welfare calculations for different levels of the entry subsidy in Figure \ref{fig:welfare_tau} for our three economies. The analysis suggests that, in the 2007 economy, the government would find a subsidy of around 70\% of the fixed cost optimal, implying a welfare gain of approximately 21\% (in consumption equivalent terms). This value is within the range of estimates reported by the literature for the cost of markups. For example, \cite{BGM2} find a cost as high as 25\%, while \cite{EMX} find a welfare loss of 23.6\% for an average cost-weighted markup of 1.25. For the 1990 economy the welfare effect of the policy takes a similar shape but the impact peaks at around 12\%, while for 1975 the maximum welfare improvement is about 2\% CEV.

\begin{figure}[ht]
\centering{}\includegraphics*[scale=0.5]{input/welfare_tau_plot.eps}
\caption{Welfare: consumption equivalent gain
\protect \\ {Note:  \small{} the figure shows the welfare impact (in consumption equivalent gains) of an entry subsidy equal to a fraction $\tau_f$ of fixed costs. For each level of  $\tau_f$, we simulate the economy 100,000 times and calculate average welfare.}}
\label{fig:welfare_tau}
\end{figure}
It should be noted that the policy experiment we consider does not implement the first best allocation. We evaluate a simple firm subsidy and do not consider size-dependent taxes/subsidies that might be necessary to eliminate markup distortions. Furthermore, as mentioned earlier, we highlight another cost of market power: the fact that it can generate quasi-permanent recessions. Interestingly, Figure \ref{fig:welfare_tau} suggests that welfare is very steep around $\tau_f=0$, implying that relatively small entry subsidies can have a sizeable impact on welfare. For example, a 10\% entry subsidy would be enough to generate a 8\% gain in consumption equivalent terms. The reason is that even a relatively small subsidy can significantly shift the probability mass from the low to the high steady state. This intuition explains why the effect is partially and fully muted in the 1990 and 1975 economies. As the likelihood of moving to a low competition regime reduces, the welfare gain from the policy declines. In the 1975 economy, where the probability of quasi-permanent recessions is zero to begin with, the welfare effects are solely driven by trading off lower markups and more varieties with the more resources absorbed by fixed costs. Interestingly, the three economies also differ in terms of the welfare costs associated to an entry tax. In particular, such tax can have two complementary effects: i) it can force the economy in the low competition regime and ii) it can worsen the welfare in the low steady state as fewer firms are able to survive. This rationale explains the large costs for the 1990 economy. Recall that in this calibration quasi-permanent recessions are unlikely but feature large output losses relative to the high steady state. These welfare costs are smaller for the 2007 economy as downward transitions entail smaller output losses and are more likely even before the tax.

Lastly, one can think about the optimal state-dependent subsidy. If the economy is hit by a large negative shock that triggers a steady state transition, the welfare benefit of such a subsidy can be very large. On the other hand, during a recession, profits are reduced, thereby making the budget constraint tighter. If the government could borrow intertemporally it would have large incentives to do so and to finance entry during downturns and pay back debt during booms. This suggests that, through the lens of our model, countercyclical firm subsidies can alleviate downturns by preventing the economy from falling into quasi-permanent recessions.

% Discuss the last paragraph


==> submitted_version/7_conclusions.tex <==

\section{Conclusion \label{sec:Conclusion}}
The US economy appears to have experienced a fundamental change over the past decades, with several studies and data sources indicating a reallocation of activity towards large, high markup firms. This observation has raised concerns in academic and policy circles about increasing market power, and it has been proposed as an explanation for recent macroeconomic \textit{puzzles}, such as low aggregate investment, low wage growth or declining labor shares. Our model suggests that, besides their impact on factor shares and factor prices, that rising firm differences and greater market power can also have an impact on business cycles and provide an amplification and persistence mechanism to aggregate fluctuations. In particular, larger firm heterogeneity may have rendered the US economy more vulnerable to aggregate shocks and more likely to experience quasi-permanent slumps. Through the lens of our theory, such increased fragility may have been difficult to identify, as it manifests itself only in reaction to large shocks.

%In broader terms, our theory indicates that the firm size/markup distribution can be an important determinant of the response of the economy to aggregate shocks. This observation suggests that product market considerations should gain relevance within macroeconomic research and policy analysis. In particular, the standard toolkits used by macroeconomists should increasingly incorporate a realistic characterization of product market frictions.

% We conclude by mentioning two extensions we are considering in our future work. First, we are planning to introduce endogenous growth to research the dynamic interplay between market power and innovation in a context of multiple competition regimes. As documented in Figure \ref{fig:great_deviation_figure}, both real GDP per capita and aggregate TFP have experienced a widening deviation from trend after 2008, which indicates that growth rates have become persistently lower. We think that an extended version
% of our model with endogenous R\&D has the potential to account for this. In a world where firms conduct R\&D because of an \textit{escape-from-competition}
% effect, a decrease in product market competition will likely reduce
% firms' incentives to innovate.

% Second, we also plan to consider a setup with nominal rigidities to think about the monetary policy implications of increasing firm differences and of rising market power. Our theory suggests at least two relevant insights for the design of monetary policy. First, as industries become more concentrated, firms' pricing decisions are likely to become increasingly rigid and less sensitive to aggregate fluctuations. This suggests that the degree of price rigidity may endogenously respond to changes in the product market structure, which has obvious implications for the effects of monetary policy. Second, market power can have a negative impact on interest rates and hence be associated with the greater likelihood of a binding zero lower bound. The examination of these two hypotheses is an important avenue for future research.

Our work also provides further motive for policies that curb market power. As we have shown, the endogenous response of the market structure to aggregate shocks act as an accelerant. On top of the standard static effects, any policy that reduces market power can have dynamic benefits in terms of the persistence and amplitude of aggregate fluctuations. These effects are particularly large if the economy is at risk of quasi-permanent slumps.

To keep the analysis simple, we have abstracted from a number of important features. One such example is that, in our model, firms solve a static problem and their productivity is permanent. The interaction between endogenous growth through innovation, market power and fragility is a natural next step for this area of research. Further, our model features one-sided market power. Recent models of oligopoly \citep[see][]{azar2021general} lend themselves to the study of the interaction between two-sided market power and the likelihood of quasi-permanent slumps. Lastly, recent work studies the interplay between competition and monetary policy \citep[see][]{mongey2017market,wang2020dynamic,fabianiJMP}. The question of how monetary policy, by changing the market structure, shapes the dynamic properties of an economy is an avenue for future research. 

==> submitted_version/SupplementaryMaterial.tex <==
\newpage
\begin{center}
    
{\huge {Appendix B} \\\large{Supplementary Material for \\\textit{Firm Heterogeneity, Market Power and Macroeconomic Fragility} }\\ Not for Publication}
\end{center}


\raggedright
\justify



\setcounter{page}{1}
\setcounter{section}{0}
\setcounter{figure}{0}
\setcounter{table}{0}
\setcounter{lemma}{0}
\newcounter{mysection}
\makeatletter
\@addtoreset{section}{mysection}
\makeatother

\renewcommand{\thesection}{B.\arabic{section}}
\renewcommand{\thetable}{B.\arabic{table}}
\renewcommand{\theprop}{B.\arabic{prop}}
\renewcommand{\thecor}{B.\arabic{cor}}
\renewcommand{\theremark}{B.\arabic{remark}}
\renewcommand{\thefigure}{B.\arabic{figure}}

\renewcommand{\thelemma}{B.\arabic{lemma}}



\input{derivations}


\section{The Quantitative Model \label{sec:Quantitative-Model}}

\subsection{Calibration \label{subsec:Calibration} }

\paragraph{Steady-State}

We perform three different calibrations of our model \textendash{} to match the average level of markups and its dispersion in 1975, 1990 and in 2007. We need to calibrate five technology parameters: the elasticity of substitution $\sigma_{I}$ and $\sigma_{G}$ (which are time-invariant), the log-normal standard deviation $\lambda$, the fixed production cost $c$ and the fraction of industries with zero fixed cost $f_{comp}$ (which are allowed to vary over time).

We start by specifying a grid with possible values for $\sigma_{I}$ and $\sigma_{G}$. Then, for each pair $\left(\sigma_{I} , \sigma_{G}\right)$, we specify a triplet $\left(\lambda, c, f_{comp} \right)$, as well as a grid with values for the aggregate capital stock $K$. We then compute the aggregate equilibrium for each parameter combination $\left(\sigma_{I}, \sigma_{G}, \lambda, c, f_{comp} \right)$
and for each value $K$.\footnote{Aggregate TFP $e^{z_{t}}$ is assumed to be constant and equal to one.} We start by assuming that all firms are active, so that there are $N$ firms in each of the $I$ industries. We compute the aggregate equilibrium using equations (\ref{eq:agg_tfp}) and (\ref{eq:agg_cost}). We then compute the profits net of the fixed cost that each firm makes
\[
\left(p_{ijt} - \dfrac{\Theta_{t}}{\tau_{ijt}} \right)\:y_{ijt} - c_{i}
\]
and identify the firm with the largest negative value. We exclude this firm and recompute the aggregate equilibrium. We repeat this iterative procedure until all firms have non-negative profits (net of the fixed production cost). If equilibrium multiplicity arises, this algorithm allows us to consistently select the equilibrium that features the largest number of  firms.

For each triplet $\left(\lambda, c, f_{comp} \right)$, we then have the general equilibrium computed for all possible capital values. The steady-state(s) of our economy correspond to the value(s) of $K$ for with the rental rate $R_{t}$ is equal to $\dfrac{1}{\beta}-\left(1-\delta\right)$. 

When multiple steady-states arise (as in the 1990 and 2007 economies), we compute model moments in the highest steady-state.

\paragraph{Data Definitions}

For the sales weighted-average markup, we use the series computed by \cite{LEU}. 
The authors calculate price-cost markups for the universe of public firms, using data from COMPUSTAT. The markup of a firm $j$ in a 2-digit NAICS sector $s$ at time $t$ is calculated as
\[
\mu_{sjt} = \xi_{st} \cdot \dfrac{\textrm{sale}_{sjt}}{\textrm{cogs}_{sjt}}
\]
where $ \xi_{st}$ is the elasticity of sales to the total variable input bundle, $\textrm{sale}_{sjt}$ is sales and $\textrm{cogs}_{sjt}$ is the cost of the goods sold, which measures total variable costs.

% To measure markup dispersion, we compute the standard deviation of markups within 2-digit NAICS sectors. Treating $ \xi_{st}$ as constant within a sector $s$ and time $t$, we can measure markup dispersion within this sector as

% \[
% \textrm{sd}_{s}\left[\textrm{log}\left(\mu_{sjt}\right)\right] = \textrm{sd}_{s}\left[\textrm{log}\left(\dfrac{\textrm{sale}_{sjt}}{\textrm{cogs}_{sjt}}\right)\right]
% \]

% We calculate this measure for all 23 sectors (2-digit NAICS). We then compute an average across all such sectors, weighted by the sector sales. Figure \ref{fig:Markup-Dispersion} shows the evolution of this measure.

% In our model, we compute the standard deviation of (log) markups across all firms in the economy, i.e. we do not compute it industry by industry. We think of an industry in our model as a market at the possible level of disaggregation (e.g. 10-digit NAICS). We cannot however observe data at such a fine level of disaggregation \textendash{} first because most data sets only provide industry information at the 6-digit, second because many large firms are multi-product an operate in different markets. We hence think of our final good $Y_t$ as one big-sector.

% \begin{figure}[H]
% \centering{}%
% \includegraphics*[scale=0.6]{input/sd_log_markup}\tabularnewline
% \caption{Markup Dispersion\protect \\ {Note: \small{} the figure shows the evolution of markup dispersion computed from COMPUSTAT data for 2-digit industries.}
% \label{fig:Markup-Dispersion}}
% \end{figure}


\subsection{Solution Algorithm for the Dynamic Optimization Problem}

We now explain the algorithm we use for the dynamic optimization problem of the representative household. We take the calibrated parameters $\left(\lambda, c \right)$ and form a grid for aggregate capital with $n_K = 70 $ points. This grid is centered around the highest steady-state $K^{\text{ss}}_H$, with a lower-bound $0.5 \times K^{\text{ss}}_H$ and upper bound $1.5 \times K^{\text{ss}}_H$. We also form a grid for aggregate TFP, $A$. We use Tauchen's algorithm with $n_A = 11$ points, autocorrelation parameter $\phi_A$ and standard deviation for the innovations $\sigma_{\varepsilon}$ (the last two parameters are calibrated, as explained in the main text). We compute the aggregate equilibrium for each value of $K$ and $A$. 

We next compute a numerical approximation for the household policy function, by iterating on the Euler equation. We start by making a guess for the savings rate
\[
s\left(X_t\right) \coloneqq \dfrac{C\left(X_t\right) }{Y\left(X_t\right) }
\]
for every combination of the vector of state-variables $X_t \coloneqq \left(K_t, A_t\right)$. Given a guess $s^{\left(n\right)}\left(X_{t}\right) \; \forall X_t$ for the savings rate, we use the Euler equation to obtain a new guess $s^{\left(n+1\right)}\left(X_{t}\right)$ as follows
\begin{comment}
\[
\dfrac{1}{C_{t}-\dfrac{L_{t}^{1+\nu}}{1+\nu}}=\mathbb{E}_{t}\left\{ \dfrac{\beta\left[R_{t+1}+\left(1-\delta\right)\right]}{C_{t+1}-\dfrac{L_{t+1}^{1+\nu}}{1+\nu}}\right\} 
\]
\end{comment}

{\footnotesize
\[
\begin{array}{rl}
 & \dfrac{1}{\left(1-s^{\left(n+1\right)}\left(X_{t}\right)\right)Y\left(X_{t}\right)-\dfrac{W\left(X_{t}\right)^{\left(1+\nu\right)/\nu}}{1+\nu}}=\mathbb{E}_{t}\left\{ \dfrac{\beta\left[R\left(X_{t+1}\right)+\left(1-\delta\right)\right]}{\left(1-s^{\left(n\right)}\left(X_{t+1}\right)\right)Y\left(X_{t+1}\right)-\dfrac{W\left(X_{t+1}\right)^{\left(1+\nu\right)/\nu}}{1+\nu}}\right\} \\[8ex]
\Leftrightarrow & s^{\left(n+1\right)}\left(X_{t}\right)=1-\dfrac{1}{Y\left(X_{t}\right)}\left\{ \dfrac{W\left(X_{t}\right)^{\left(1+\nu\right)/\nu}}{1+\nu}+\left[\mathbb{E}_{t}\left\{ \dfrac{\beta\left[R\left(X_{t+1}\right)+\left(1-\delta\right)\right]}{\left(1-s^{\left(n\right)}\left(X_{t+1}\right)\right)Y\left(X_{t+1}\right)-\dfrac{W\left(X_{t+1}\right)^{\left(1+\nu\right)/\nu}}{1+\nu}}\right\} \right]^{-1}\right\}.
\end{array}
\]
}
We iterate on this procedure until

\[
\left|s^{\left(n+1\right)}\left(X_{t}\right)- s^{\left(n\right)}\left(X_{t}\right) \right| \; < \;  \epsilon \quad \forall X_t .
\]

\subsection{Business Cycle Moments \label{subsec:business_cycle_moments}}

\begin{table}[H]
\setlength{\tabcolsep}{0.4cm}  
\begin{center}
\begin{tabular}{lccccc} 		\thickhline
\\[-2ex]
& Output & Consumption & Investment & Hours & TFP \\ \thickhline
\\[-2ex]
& \multicolumn{4}{c}{Correlation with Output} \\
\\[-2ex]
Data: 1947-2019 & 1.00 & 0.95 & 0.76 & 0.67 & 0.71 \\[0.25ex]
Model: 1975 calibration & 1.00 & 0.99 & 0.92 & 1.00 & 0.83 \\[0.25ex]
Model: 1990 calibration & 1.00 & 1.00 & 0.96 & 1.00 & 0.88 \\[0.25ex]
Model: 2007 calibration & 1.00 & 1.00 & 0.96 & 1.00 & 0.89  \\ 
\\
& \multicolumn{4}{c}{Standard Deviation Relative to Output} \\
\\[-2ex]
Data: 1947-2019 & 1.00 & 0.90 & 2.04 & 0.98 & 0.95 \\[0.25ex]
Model: 1975 calibration & 1.00 & 0.95 & 1.54 & 0.74 & 0.25 \\[0.25ex]
Model: 1990 calibration & 1.00 & 0.97 & 1.23 & 0.78 & 0.17 \\[0.25ex]
Model: 2007 calibration & 1.00 & 0.98 & 1.20 & 0.79 & 0.15  \\ 
\\[-2ex]\thickhline
\end{tabular} \end{center}
\caption{Business Cycle Moments. All variables are in logs. Data variables are in per capita terms (except TFP) and in deviation from a linear trend computed over 1947-2007.} \label{tab:business_cycle_moments}
\end{table}

Table \ref{tab:business_cycle_moments} shows some business cycle moments for our two calibrated economies, as well as their data counterparts.
To be consistent with our interpretation that the US economy transitioned to a lower steady-state after 2008, all data variables are in deviation from a linear trend computed over 1947-2007. This fact explains the large empirical correlation between consumption and output. 
Comparing our two calibrated economies, we see that both economies display the same correlations of consumption and hours with output. The 2007 economy displays, however, a significantly lower correlation of investment with output. %This is explained by the fact the investment appears to be more volatile in the 2007 economy.

% \subsection{Impulse Responses: Other Variables \label{subsec:IRF_other}}

% In figures \ref{fig:IRF_other_1980} and \ref{fig:IRF_other_2007} we plot the responses of the gross investment rate $I_{t} / Y_{t}$, the rental rate, the labor share and the (sales-weighted) average markup.\footnote{In our setup, the steady-state rental rate is independent of the regime of the economy, as it is pinned down by the discount factor of the representative household.}
% With respect to the behavior of the investment rate, there is one difference that is worth highlighting. In the 1985 economy, the investment rate suffers a significant drop on impact, but ultimately recovers and overshoots its steady-state level \textendash{} so that the capital stock can recover to its long-run value. This is not true for the 2007 economy. As the economy is converging to a lower steady state, during the transition there is ``too much'' capital in the system, which yields a gradual reduction of the stock through a depressed investment rate over the transition.
% Aggregate markups increase on impact as there is firm exit. In the 1985 economy, this increase is reabsorbed as the economy transitions back to its steady state and firms enter the market. In the 2007 economy, such absorption does not take place since the number of firms never goes back to the previous level. Not surprisingly, the labor share exhibits the opposite behavior. In the 1985 economy, the reduction quickly reverts, while the 2007 economy experiences a 0.5 pp permanent drop in the labor share. 

% \begin{figure}[H]
% \begin{minipage}[b]{.5\linewidth}
% \centering{}\includegraphics*[scale=0.725]{input/IRF_big_shock_other_80.eps}\subcaption{1985 Economy \label{fig:IRF_other_1980}}
% \end{minipage}%
% \begin{minipage}[b]{.5\linewidth}
% \centering{}\includegraphics*[scale=0.725]{input/IRF_big_shock_other_07.eps}\subcaption{2007 Economy \label{fig:IRF_other_2007}}
% \end{minipage}
% \caption{IRF (Large Shock)\protect \\ {Note: \small{the figure shows the impulse responses of additional variables to a large shock to aggregate TFP for the 1985 (Panel (a)) and the 2007 (Panel (b)) economies.}}}\label{fig:IRF_other_variables}
% \end{figure}


\subsection{Aggregate Productivity \label{subsec:agg_TFP}}

\subsubsection*{Average Firm Level TFP}

\begin{figure}[H]
\centering
\includegraphics*[scale=0.8]{input/IRF_firm_tfp.eps}\caption{Aggregate TFP versus Average Firm Level TFP \protect \\
{Note: \small{}The left panel shows aggregate TFP. The right panel shows a sales-weighted average of firm level revenue TFP $p_{ijt}\cdot\tau_{ijt}$.
\label{fig:TFP_Model_transition}}}
\end{figure}

Figure \ref{fig:TFP_Model_transition} reports a sales-weighted average of firm level revenue TFP. A similar pattern emerges if one uses physical TFP instead.

\subsubsection*{Dispersion in Industry Output}

\begin{figure}[H]
\centering
\includegraphics*[scale=0.5]{input/output_dispersion}\caption{Dispersion in $\log\left(y_{it}\right)${\small{} \label{fig:output_dispersion_transition}}}
\end{figure}





%\subsection{The Great Recession}
% \subsection{Welfare \label{subsec:welfare_GR}}
% \begin{figure}[H]
% \centering
% \includegraphics*[scale=0.7]{input/GR_welfare_model}\caption{The great recession and its aftermath: welfare \label{fig:GR_welfare_model}}
% \end{figure}


\section{The 1990 Recession \label{sec:90_recession}}

\subsubsection*{The response in the 1990 economy}

\begin{figure}[H]
\begin{minipage}[b]{.5\linewidth}
\centering{}\includegraphics*[scale=0.5]{input/data_90_recession.eps}\subcaption{1990-1991 recession (data) \label{fig:data_90_recession}}
\end{minipage}
\begin{minipage}[b]{.5\linewidth}
\centering{}\includegraphics*[scale=0.5]{input/1990_recession_1990_model.eps}\subcaption{The 1990-1991 shock in the 1990 model \label{fig:85_model_82_crisis}}
\end{minipage}
\caption{The 1990-1991 recession \label{fig:90_crisis}}
\end{figure}

\subsubsection*{The response in the 2007 economy}

\begin{figure}[H]
\centering{}\includegraphics*[scale=0.65]{input/1990_recession_2007_model.eps}
\caption{The 1990-1991 shock in the 2007 model
\label{fig:07_model_90_crisis}}
\end{figure}




\section{Number of Firms per Sector}
\label{sec:numberfirms}
\begin{figure}[H]
\begin{centering}
\includegraphics*[scale=0.9]{input/nfirms_sector} 
\par\end{centering}
\caption{\textbf{Number of Firms per Sector: 1980-2018}\protect \\
{\small{}Each panel shows the number of firms with at least one employee in each sector (in logs). For
each series, the dashed grey line shows a linear trend computed over the 1980-2007 period. Data is from the US Business Dynamics Statistics\label{fig:nfirms_sector}}}
\end{figure}

% \section{Size Dispersion} \label{sec:std_log_ms}
% \begin{figure}[H]
% \centering{}%
% \includegraphics*[scale=0.7]{input/std_log_ms}\tabularnewline
% \caption{Standard Deviation of Log Revenues \\ This figure shows the standard deviation of log revenues (COMPUSTAT item SALE), computed on a yearly basis, for all firms in COMPUSTAT.
% \label{fig:std_log_ms}}
% \end{figure}

\section{Fixed Costs}\label{sec:fixed_costs_data}
\begin{figure}[H]
\centering{}%
\includegraphics*[scale=0.7]{input/ratio_fixed_costs}\tabularnewline
\caption{Ratio of fixed to total costs \\ This figure shows the average ratio of fixed to total costs for COMPUSTAT firms. Following \cite{GW}, we define fixed costs as the sum of `Selling, General and Administrative Expenses' (COMPUSTAT item XSGA), `Advertising Expenses'
(Compustat item XAD) and `R\&D Expenditures'  (Compustat item XRD). Total costs are the sum of fixed costs and variable costs, where the latter correspond to the `Cost of Goods Sold' (Compustat item COGS).
\label{fig:fixed_total_costs}}
\end{figure}




% \section{Robustness: Different Elasticities of Substitution \label{subsec:new-calibration-ES}}

% \subsubsection*{Calibration}
% Parameters not reported are as in the baseline calibration (Table \ref{tab:parameter_values}).
% \begin{table}[H]
% \setlength{\tabcolsep}{0.2cm} \begin{center} \resizebox{14cm}{5cm} {  \begin{tabular}{lccl}
% \thickhline
% \\[-1ex]
% {\large Description} & {\large Parameter} & {\large Value} & {\large Source/Target} \\[1ex] \thickhline
% \\[-1ex]
% Between-industry ES & $\sigma_{I}$ & 1.2 & \cite{de2021quantifying} \\
% \\[-1ex]
% Within-industry ES & $\sigma_{G}$ & 5.75 & \cite{de2021quantifying} \\
% \\[-1ex]
% \hline
% \\[-1ex]
% Calibrated Parameters: 2007 \\ \\[-1ex] \hline
% \\[-2ex]
% Standard deviation $\gamma$ & $\lambda$ & 0.280 & Sales-weighted average markup\\
% \\[-1ex]
% Fixed cost & $c$ & 0.0034 & Average ratio fixed/total costs \\
% \\[-1ex]
% Fraction of industries with $c_{i}>0$ & $f$ & 0.080 &  Emp share concentrated industries \\
% \\[-1ex]
% Persistence of $z_t$  & $\rho_{z}$ & 0.900 & Autocorrelation of log Y \\
% \\[-1ex]
% Standard deviation of $\varepsilon_t$ & $\sigma_{\varepsilon}$ & 0.0035 & Standard deviation of log Y \\ 
% \\[-1ex]
% \hline
% \\[-1ex]
% Calibrated Parameters: 1985 \\ \\[-1ex] \hline
% \\[-2ex]
% Standard deviation $\gamma$ & $\lambda$ & 0.140 & Sales-weighted average markup\\
% \\[-1ex]
% Fixed cost & $c$ & 0.0004 & Average ratio fixed/total costs \\
% \\[-1ex]
% Fraction of industries with $c_{i}>0$ & $f$ & 0.110 &  Emp share concentrated industries \\
% \\[-1ex]
% \thickhline
% \end{tabular}  
% } \end{center}
% \caption{Parameter Values\label{tab:parameter_values_ES}}
% \end{table}


% \begin{table}[H]
% \setlength{\tabcolsep}{0.35cm}  
% \begin{center}
% \begin{tabular}{lccccc} 		\thickhline 
% \\[-2ex]
% & \multicolumn{2}{c}{1985} & & \multicolumn{2}{c}{2007} \\
% \\[-1ex] 
% & Data & Model & & Data & Model
% \\ \hline  
% \\[-1ex] 
% Sales-weighted average markup & 1.27 & 1.25 & & 1.46 & 1.43 \\
% \\[-1ex]
% Average fixed to total cost ratio & 0.343 & 0.370 & & 0.414 & 0.479 \\
% \\[-1ex]
% Employment share in \textit{concentrated} industries & - & 0.058 & & 0.063 & 0.037 \\
% \\[-1ex] \hline 
% \\[-1ex]
% Autocorrelation log GDP  & 0.978* & 0.953 & & 0.978* & 0.956 \\
% \\[-1ex]
% Standard deviation log GDP & 0.061* & 0.040 & & 0.061* & 0.059 \\
% \\[-1ex]
% \thickhline
% \\[-1ex]
% \multicolumn{6}{l}{*computed over 1947:Q1-2019:Q4} \\
% \end{tabular} \end{center}
% \caption{Targeted moments and model counterparts}
% \end{table}


% \subsubsection*{Ergodic Distributions}

% \begin{figure}[H]
% \hspace{-1cm}
% \begin{minipage}[b]{.55\linewidth}
% \centering\includegraphics*[scale=0.5]{input/hist_1985_ES.eps}\subcaption{Output Distribution: 1985} \label{fig:y_dist_1985_ES}
% \end{minipage}%
% \hspace{-0.5cm}
% \begin{minipage}[b]{.55\linewidth}
% \centering\includegraphics*[scale=0.5]{input/hist_2007_ES.eps}\subcaption{Output Distribution: 2007} \label{fig:y_dist_2007_ES}
% \end{minipage}
% \caption{Ergodic distribution of output \protect \\ {\small{} This figure shows the distribution of log output for the 1985 and the 2007 economies. We simulate each economy for 10,000,000 periods and plot output in deviation from the high steady state.}}
% \end{figure}

% \subsubsection*{The 2008 Crisis}

% \begin{figure}[H]
% \begin{minipage}[b]{.5\linewidth}
% \centering{}\includegraphics*[scale=0.55]{input/GR_transition_2007_ES.eps}\subcaption{2007 Model  \\ This figures replicates Figure \ref{fig:GR_model} \label{fig:GR_model_07_ES}}
% \end{minipage}%
% \hspace{0.5cm}
% \begin{minipage}[b]{.5\linewidth}
% \centering{}\includegraphics*[scale=0.55]{input/GR_transition_1985_ES.eps}\subcaption{1985 Model  \\ This figures replicates Figure \ref{fig:GR_data_model_85_1} \label{fig:GR_model_85_ES}}
% \end{minipage}
% \caption{The \textit{great recession} and its aftermath}\label{fig:GR_data_model_ES}
% \end{figure}

% \newpage

\section{Robustness: Variable Fixed Costs} \label{sec:var_fixed_costs}

We assume that, each period, a fixed amount $c_f$ of firms' output is lost
\begin{align*}
    c_f=k_c^\alpha l_c^{1-\alpha}
\end{align*}

Given these assumptions, firms need to pay a per per period fixed cost
\[
\Theta_{t} \cdot c_f
\]
where $\Theta_{t} $ is the factor price index.

Denoting by $L_{yt}$ and $K_{yt}$ the aggregate stocks of labor and capital used in the production, we have the following market clearing conditions for labor and capital
\begin{align*}
    L_{t} = L_{yt} + N^{c}_{t} \cdot l_c \\
    K_{t} = K_{yt} + N^{c}_{t} \cdot k_c
\end{align*}
where $N^{c}$ denotes the number of firms incurring $c_f$. Note that the optimal mix of $l_c$ and $k_c$ chosen by each individual firm satisfies
\begin{align*}
    \dfrac{k_c}{l_c} = \dfrac{K_{yt}}{L_{yt}}
\end{align*}

\subsubsection*{Calibration}
Parameters not reported are as in the baseline calibration (Table \ref{tab:parameter_values}).
\begin{table}[ht!]
\setlength{\tabcolsep}{0.2cm} \begin{center} \resizebox{16cm}{3.7cm} {  \begin{tabular}{lccccl}
\thickhline
\\[-1ex]
{\large Description} & {\large Parameter} & \multicolumn{3}{c}{{\large Value}} & {\large Source/Target} \\[1ex] \thickhline
\\[-1ex]
[A.1] Calibrated Parameters: Fixed \\ \\[-1ex]
\hline
\\[-1ex]
Between-industry ES & $\sigma_{I}$ & \multicolumn{3}{c}{1.33} & Sales-weighted average markup\\
\\[-1ex]
Within-industry ES & $\sigma_{G}$ & \multicolumn{3}{c}{12.5} & Sales-weighted average markup \\
\\[-1ex]
Persistence of $z_t$  & $\rho_{z}$ & \multicolumn{3}{c}{0.950} & Autocorrelation of log $Y_t$ \\
\\[-1ex]
Standard deviation of $\varepsilon_t$ & $\sigma_{\varepsilon}$ & \multicolumn{3}{c}{0.003} & Standard deviation of log $Y_t$ \\ 
\\[-1ex] \hline
\\[-1ex]
[A.2] Calibrated Parameters: Variable & & 1975 & 1990 & 2007 & \\ \\[-1ex] \hline
\\[-1ex]
Fraction of industries with $c_{i}>0$ & $f$ & 0.105 & 0.140 & 0.130 &  Emp share concentrated industries \\
\\[-1ex]
Standard deviation of $\gamma_{ij}$ & $\lambda$ & 0.193 & 0.252 & 0.304 & Std log market share \\
\\[-1ex]
Fixed cost ($\times 10^{-4}$) & $c$ & 3.03 & 5.66 & 7.82 & Average ratio fixed/total costs \\
\\[-1ex]
\thickhline
\end{tabular}  
} \end{center}
\caption{Parameter Values\label{tab:parameter_values_vfc}}
\end{table}

\begin{table}[ht]
\setlength{\tabcolsep}{0.25cm}  
\begin{center}
\resizebox{16cm}{3.7cm} {
\begin{tabular}{lcccccccc} 		\thickhline 
\\[-2ex]
& \multicolumn{2}{c}{1975} & & \multicolumn{2}{c}{1990} & & \multicolumn{2}{c}{2007} \\
\\[-1ex] 
& Data & Model & & Data & Model & & Data & Model \\ \hline  
\\[-1ex] 
Sales-weighted average markup & 1.28 & 1.26 & & 1.37 & 1.38 & & 1.46 & 1.44 \\
\\[-1ex]
Std log revenues & 1.67 & 1.74 & & 2.47 & 2.36 & & 2.79 & 2.92 \\
\\[-1ex]
Average fixed to total cost ratio & 0.244 & 0.259 & & 0.355 & 0.390 & & 0.414 & 0.420 \\
\\[-1ex]
Emp share \textit{concentrated} industries & - & 0.067 & & - & 0.072 & & 0.063 & 0.060 \\
\\[-1ex] \hline 
\\[-1ex]
Autocorrelation log GDP  &  &  & &  &  & & 0.978* & 0.976 \\
\\[-1ex]
Standard deviation log GDP &  &  & &  &  & & 0.061* & 0.056 \\
\\[-1ex]
\thickhline
\\[-1ex]
\multicolumn{6}{l}{*computed over 1947:Q1-2019:Q4} \\
\end{tabular}} \end{center}
\caption{Targeted moments and model counterparts\label{tab:targeted_moments_vfc}}
\end{table}

\subsubsection*{Ergodic Distributions}

\begin{figure}[H]
\hspace{-1cm}
\begin{minipage}[b]{.33\linewidth}
\centering\includegraphics*[scale=0.325]{input/hist_1975_vfc.eps}\subcaption{1975} \label{fig:y_dist_1975_vfc}
\end{minipage}%
\begin{minipage}[b]{.33\linewidth}
\centering\includegraphics*[scale=0.325]{input/hist_1990_vfc.eps}\subcaption{1990} \label{fig:y_dist_1990_vfc}
\end{minipage}
\begin{minipage}[b]{.33\linewidth}
\centering\includegraphics*[scale=0.325]{input/hist_2007_vfc.eps}\subcaption{2007} \label{fig:y_dist_2007_vfc}
\end{minipage}
\caption{Ergodic distribution of output \protect \\ {Note: \small{}\small{} This figure shows the distribution of log output for the 1975, 1990 and the 2007 economies. We simulate each economy for 10,000,000 periods and plot output in deviation from the high steady state.}} \label{fig:businesscycle_vfc}
\end{figure}

\subsubsection*{The 2008 Crisis}

\begin{figure}[H]
\begin{minipage}[b]{.33\linewidth}
\centering{}\includegraphics*[scale=0.325]{input/GR_transition_1975_vfc.eps}\subcaption{1975 Model \label{fig:GR_1975_vfc}}
\end{minipage}%
\begin{minipage}[b]{.33\linewidth}
\centering{}\includegraphics*[scale=0.325]{input/GR_transition_1990_vfc.eps}\subcaption{1990 Model \label{fig:GR_1990_vfc}}
\end{minipage}
\begin{minipage}[b]{.33\linewidth}
\centering{}\includegraphics*[scale=0.325]{input/GR_transition_2007_vfc.eps}\subcaption{2007 Model \label{fig:GR_2007_vfc}}
\end{minipage}
\caption{The \textit{great recession} in the 1975, 1990 and 2007 models \protect \\ {Note: \small{}The 2007 model is subjected to a sequence of six quarter shocks $\left\{\varepsilon_{t}\right\}$ to match the dynamics of aggregate TFP in the data between 2008Q1:2009Q2. This sequence of shocks is then fed in the 1975 and 1990 economies.}}
\end{figure}

==> submitted_version/derivations.tex <==
\section[No Product Differentiation]{Industry Equilibrium with $\eta=1$}\label{proofs_appendixB}

\paragraph{Equilibrium Price and Output}
Suppose that $\eta=1$. When $n$ firms produce, we have a system of $n$ first order conditions
\begin{align}
p\left[1-\left(1-\rho\right)s_{j}\right]=\dfrac{\Theta}{\gamma_{j}}
\end{align}
Dividing the first order condition of firm $j$ by that of firm $1$
we obtain
\begin{align}
 %& \dfrac{1-\left(1-\rho\right)s_{j}}{1-\left(1-\rho\right)s_{1}}=\dfrac{\gamma_{1}}{\gamma_{j}}\\
%\Leftrightarrow & 1-\left(1-\rho\right)s_{j}=\dfrac{\gamma_{1}}{\gamma_{j}}\left[1-\left(1-\rho\right)s_{1}\right]\\
%\Leftrightarrow & 
s_{j}=\dfrac{1}{\left(1-\rho\right)}\left\{ 1-\dfrac{\gamma_{1}}{\gamma_{j}}\left[1-\left(1-\rho\right)s_{1}\right]\right\} 
\end{align}
Note that
\begin{align}
  \stackrel[k=1]{n}{\sum}s_{k}=1
 %\\
%\Leftrightarrow & \stackrel[k=1]{n}{\sum}\dfrac{1}{\left(1-\rho\right)}\left\{ 1-\dfrac{\gamma_{1}}{\gamma_{k}}\left[1-\left(1-\rho\right)s_{1}\right]\right\} =1\\
%\Leftrightarrow & n-\gamma_{1}\left[1-\left(1-\rho\right)s_{1}\right]\stackrel[k=1]{n}{\sum}\dfrac{1}{\gamma_{k}}=1-\rho\\
\Rightarrow  \dfrac{n-\left(1-\rho\right)}{\stackrel[k=1]{n}{\sum}\dfrac{1}{\gamma_{k}}}=\gamma_{1}\left[1-\left(1-\rho\right)s_{1}\right]
\end{align}
Plugging the last equation into the first order condition of firm
$1$ we obtain
\begin{align}
 %& p\dfrac{n-\left(1-\rho\right)}{\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}}=\Theta\\
%\Leftrightarrow &
p=\dfrac{\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}}{n-\left(1-\rho\right)}\Theta
\end{align}
Total output is hence equal to 
\begin{align}
 & y=p^{-\frac{1}{1-\rho}}Y=\left[\dfrac{\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}}{n-\left(1-\rho\right)}\Theta\right]^{-\frac{1}{1-\rho}}Y
\end{align}

\paragraph{Market Shares}

Plugging the previous equation into the first order condition of firm
$j$ we have
\begin{align}
% & 1-\left(1-\rho\right)s_{j}=\dfrac{n-\left(1-\rho\right)}{\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}}\dfrac{1}{\gamma_{j}}\\
%\Leftrightarrow & 
s_{j}=\dfrac{1}{1-\rho}\left[1-\dfrac{n-\left(1-\rho\right)}{\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}}\dfrac{1}{\gamma_{j}}\right]
\end{align}
It is easy to verify that each firm's market share decreases in the
total number of active firms. To see this, suppose that the number
of firms increases from $n$ to $n+1$. The new entrant will have
a market share
\begin{align}
s_{n+1}=\dfrac{1}{1-\rho}\left[1-\dfrac{n+1-\left(1-\rho\right)}{\sum\limits_{k=1}^{n+1}\dfrac{1}{\gamma_{k}}}\dfrac{1}{\gamma_{n+1}}\right]
\end{align}
which is non-negative provided that
\begin{equation}
\gamma_{n+1}\sum_{k=1}^{n+1}\dfrac{1}{\gamma_{k}}>n+1-\left(1-\rho\right)\label{eq:cond_mg_1}
\end{equation}
and below one given that
\begin{equation}
\gamma_{n+1}\sum_{k=1}^{n+1}\dfrac{1}{\gamma_{k}}<\dfrac{1}{\rho}\left[n+1-\left(1-\rho\right)\right]\label{eq:cond_mg_2}
\end{equation}
If we compare the market share of firm $j$ when there $n$ and $n+1$
firms in the market, we have
\begin{align}
 & s_{j}\left|_{n+1}\right.<s_{j}\left|_n\right.
%\Leftrightarrow & \dfrac{1}{1-\rho}\left[1-\dfrac{n+1-\left(1-\rho\right)}{\sum\limits_{k=1}^{n+1}\dfrac{1}{\gamma_{k}}}\dfrac{1}{\gamma_{j}}\right]<\dfrac{1}{1-\rho}\left[1-\dfrac{n-\left(1-\rho\right)}{\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}}\dfrac{1}{\gamma_{j}}\right]\\
%\Leftrightarrow & \dfrac{n-\left(1-\rho\right)}{\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}}<\dfrac{n+1-\left(1-\rho\right)}{\sum\limits_{k=1}^{n+1}\dfrac{1}{\gamma_{k}}}\\
%\Leftrightarrow & \left[n-\left(1-\rho\right)\right]\left(\dfrac{1}{\gamma_{n+1}}+\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}\right)<\left[n+1-\left(1-\rho\right)\right]\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}\\
%\Leftrightarrow & \left[n-\left(1-\rho\right)\right]\dfrac{1}{\gamma_{n+1}}<\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}\\
\Leftrightarrow  \gamma_{n+1}\sum\limits_{k=1}^{n+1}\dfrac{1}{\gamma_{k}}>n-\left(1-\rho\right)
\end{align}
Note that the last condition is implied by (\ref{eq:cond_mg_1}).

\paragraph{Profits}%\label{subsec:Profits}}

When there are $n$ active firms, type $\gamma_{j}$ makes production profits
\begin{align}
\Pi\left(\gamma_{j},n,\Gamma,\Theta,Y\right) %& =\left(p-\dfrac{\Theta}{\gamma_{j}}\right)s_{j}\:y_{j} \\
 & = \underbrace{\dfrac{1}{1-\rho}\left[1-\dfrac{n-\left(1-\rho\right)}{\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}}\dfrac{1}{\gamma_{j}}\right]^{2}\left[\dfrac{n-\left(1-\rho\right)}{\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}}\right]^{\frac{\rho}{1-\rho}}}_{\equiv \varLambda\left(\gamma_{j},n,\Gamma\right)}\Theta^{-\frac{\rho}{1-\rho}}Y
\end{align}
\begin{lemma}
\label{lemma:(Profit-Function)} When $\eta=1$, the profit function \textup{$\Pi\left(j,n_{it},\Gamma_{i},X_{t}\right)$}
satisfies
\begin{align} 
1) & \dfrac{\partial\Pi\left(j,n_{it},\Gamma_{i},X_{t}\right)}{\partial Y_{t}}\vphantom{\vphantom{\dfrac{\dfrac{1}{1}}{\frac{_{1}}{1}}}}>0  \qquad 
2) & \dfrac{\partial\Pi\left(j,n_{it},\Gamma_{i},X_{t}\right)}{\partial n_{it}}\vphantom{\vphantom{\dfrac{\dfrac{1}{1}}{\frac{_{1}}{1}}}}<0  \quad,\;n_{it}>j \\
3) & \dfrac{\partial\Pi\left(j,n_{it},\Gamma_{i},X_{t}\right)}{\partial\gamma_{ij}}\vphantom{\dfrac{\dfrac{1}{1}}{\frac{_{1}}{1}}}>0 \qquad
4) & \dfrac{\partial\Pi\left(j,n_{it},\Gamma_{i},X_{t}\right)}{\partial\gamma_{ik}}\vphantom{\vphantom{\dfrac{\dfrac{1}{1}}{\frac{_{1}}{1}}}}<0  \quad,\;\forall k\neq j.
\end{align}
\end{lemma}
\begin{proof} [Proof of Lemma \ref{lemma:(Profit-Function)}]
We start by showing that $\Pi\left(\cdot\right)$ increases in $\gamma_{j}$
\begin{align}
 & 2\left[1-\dfrac{n-\left(1-\rho\right)}{\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}}\dfrac{1}{\gamma_{j}}\right]^{-1}\left\{ -\dfrac{-\left[n-\left(1-\rho\right)\right]\left[-\left(\dfrac{1}{\gamma_{j}}\right)^{2}\right]}{\left(\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}\right)^{2}}\dfrac{1}{\gamma_{j}}+\dfrac{n-\left(1-\rho\right)}{\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}}\left(\dfrac{1}{\gamma_{j}}\right)^{2}\right\} + \\
 & \dfrac{\rho}{1-\rho}\left[\dfrac{n-\left(1-\rho\right)}{\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}}\right]^{-1}\dfrac{-\left[n-\left(1-\rho\right)\right]\left[-\left(\dfrac{1}{\gamma_{j}}\right)^{2}\right]}{\left(\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}\right)^{2}}>0\\
%\Leftrightarrow & 2\left[1-\dfrac{n-\left(1-\rho\right)}{\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}}\dfrac{1}{\gamma_{j}}\right]^{-1}\left\{ -\dfrac{1}{\left(\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}\right)^{2}}\dfrac{1}{\gamma_{j}}+\dfrac{1}{\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}}\right\} + \\
%& \dfrac{\rho}{1-\rho}\left[\dfrac{n-\left(1-\rho\right)}{\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}}\right]^{-1}\dfrac{1}{\left(\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}\right)^{2}}>0\\
%\Leftrightarrow & 2\left[1-\dfrac{n-\left(1-\rho\right)}{\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}}\dfrac{1}{\gamma_{j}}\right]^{-1}\left\{ -\dfrac{1}{\gamma_{j}}+\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}\right\} +\dfrac{\rho}{1-\rho}\left[\dfrac{n-\left(1-\rho\right)}{\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}}\right]^{-1}\dfrac{1}{\left(\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}\right)^{2}}>0\\
\Leftrightarrow & 2\left[1-\dfrac{n-\left(1-\rho\right)}{\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}}\dfrac{1}{\gamma_{j}}\right]^{-1}\left(\sum\limits_{k\neq j}^{n}\dfrac{1}{\gamma_{k}}\right)+\dfrac{\rho}{1-\rho}\left[\dfrac{n-\left(1-\rho\right)}{\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}}\right]^{-1}>0
\end{align}
To prove points (ii) and (iii) it suffices to show that $\varLambda\left(\cdot\right)$
is decreasing in $[{n-\left(1-\rho\right)}]/\left[{\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}}\right]$
\begin{align}
 & 2\left[1-\dfrac{n-\left(1-\rho\right)}{\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}}\dfrac{1}{\gamma_{j}}\right]^{-1}\left(-\dfrac{1}{\gamma_{j}}\right)+\dfrac{\rho}{1-\rho}\left[\dfrac{n-\left(1-\rho\right)}{\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}}\right]^{-1}<0\\
%\Leftrightarrow & \dfrac{\rho}{1-\rho}\left[1-\dfrac{n-\left(1-\rho\right)}{\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}}\dfrac{1}{\gamma_{j}}\right]<2\left[\dfrac{n-\left(1-\rho\right)}{\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}}\right]\dfrac{1}{\gamma_{j}}\\
%\Leftrightarrow & \dfrac{\rho}{1-\rho}<\left(2+\frac{\rho}{1-\rho}\right)\left[\dfrac{n-\left(1-\rho\right)}{\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}}\right]\dfrac{1}{\gamma_{j}}\\
%\Leftrightarrow & \rho<\left(2-\rho\right)\left[\dfrac{n-\left(1-\rho\right)}{\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}}\right]\dfrac{1}{\gamma_{j}}\\
\Leftrightarrow & \gamma_{j}\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}<\dfrac{2-\rho}{\rho}\left[n-\left(1-\rho\right)\right]
\end{align}
The last condition is implied by (\ref{eq:cond_mg_2}).
\end{proof}



\section{Derivations: General Equilibrium}\label{sec:GEderivations}

\subsection{Aggregate TFP \label{subsec:Aggregate-TFP} }
Aggregate TFP is given by
\begin{equation}
\Phi\left(\mathbf{\Gamma},\mathbf{N}_{t}\right)=\left[\sum_{i=1}^{I}\left(\sum_{j=1}^{n_{it}}\omega_{ijt}^{\eta}\right)^{\frac{\rho}{\eta}}\right]^{\frac{1}{\rho}}\left(\sum_{i=1}^{I}\sum_{j=1}^{n_{it}}\dfrac{\omega_{ijt}}{\tau_{ijt}}\right)^{-1},\label{eq:agg_tfp}
\end{equation}
where
\begin{align}
\omega_{ijt}\coloneqq\left[\sum_{k=1}^{n_{it}}\left(\dfrac{\mu_{ikt}}{\tau_{ikt}}\right)^{\frac{\eta}{1-\eta}}\right]^{\frac{\eta-\rho}{\eta}\frac{1}{1-\rho}}\left(\dfrac{\tau_{ijt}}{\mu_{ijt}}\right)^{\frac{1}{1-\eta}}.
\end{align}


\subsection{Factor Prices and Factor Shares \label{subsec:Factor-Prices} }
We can aggregate firms' best responses, given by equation (\ref{eq:firm_FOC}), to find an expression for the aggregate factor cost index. Given a $\left(I\times M\right)$
matrix of productivity draws $\mathbf{A}_{t}$ and a vector of active firms $\mathbf{N}_{t} \equiv \left\{ n_{it}\right\}_{i=1}^{I}$, the equilibrium factor cost index is equal to
\begin{equation}
\Theta\left(\mathbf{A}_{t},\mathbf{N}_{t}\right)=\left\{ \sum_{i=1}^{I}\left[\sum_{j=1}^{n_{it}}\left(\dfrac{\tau_{ijt}}{\mu_{ijt}}\right)^{\frac{\eta}{1-\eta}}\right]^{\frac{1-\eta}{\eta}\frac{\rho}{1-\rho}}\right\} ^{\frac{1-\rho}{\rho}}.
\end{equation}

The aggregate factor share $\Omega\left(\cdot\right) = \left(W_{t}\,L_{t} + R_{t}\,K_{t} \right)/Y_{t} $ is equal to
\begin{equation}
\Omega\left(\mathbf{A}_{t},\mathbf{N}_{t}\right) = \dfrac{\Theta\left(\mathbf{A}_{t},\mathbf{N}_{t}\right)}{\Phi\left(\mathbf{A}_{t},\mathbf{N}_{t}\right)} .
\end{equation}


% \subsection{Static Equilibrium Characterization \label{subsec:Static-Equilibrium-Characterization}}

% Figure \ref{fig:Static-Equilibrium} illustrates these results. It shows aggregate output, the profit share, and the equilibrium wage and rental rate as a function of aggregate capital $K_{t}$. In the regions represented by the full line, the economy features a symmetric equilibrium  (all industries have the same number of firms). In the regions represented by the dashed line, not all industries have the same number of firms. When the capital stock is such that $\underline{K}\left(1\right)\leq\overline{K}\leq\left(1\right)$, the economy can accommodate only one firm per industry \textendash{} it will consist of a collection of identical monopolies. As capital increases and surpasses $\overline{K}\left(1\right)$, then some industries will have a second player. When it achieves $\underline{K}\left(2\right)$, all industries will have two players. As one can see, output $Y_t$ is not globally concave in the capital stock $K_t$. This fact is explained by a complementarity between firm entry and labor supply. As the average number of firms increases (say from $n=1$ to $n=2$), competition becomes more intense and the profit share decreases (top right panel). This translates into a larger factor share and a disproportionately larger wage (bottom left panel) and labor supply (through equation (\ref{eq:factor_supply})). The fact that factor shares increase as the economy transitions into a more competitive regime also explains why, as in the case represented in Figure \ref{fig:Static-Equilibrium}, the rental rate $R_t$ is not strictly decreasing in the aggregate capital stock $K_t$.\footnote{Such a result helps us understand how multiple steady-states can occur. Note that the steady-state rental rate is pinned down by the household's discount factor $\beta$. If the the steady-state rental rate is such that it crosses the map represented in  Figure \ref{fig:Static-Equilibrium} more than once, then steady-state multiplicity occurs as we will see in the next subsection.}.



% \begin{figure}[ht!]
% \centering{}%
% \begin{tabular}{cc}
% 	\hspace{-1cm} \includegraphics*[scale=0.45]{input/production_function_ue} &  \hspace{-0.2cm}
% 	\includegraphics*[scale=0.45]{input/profit_share_ue} \\
% 	\hspace{-1cm} 
% 	\includegraphics*[scale=0.45]{input/wage_ue.eps} & 
% 	\hspace{-0.2cm}
% 	\includegraphics*[scale=0.45]{input/rental_rate_ue}
% \end{tabular}
% \caption{Static equilibrium \protect \\ {Note: \small{} the figure shows how output, the profit share and input prices move with capital. Solid segments represent economies with symmetric market structure (same number of firms), while dotted segments represent non-symmetric equilibria. We use $\alpha \, = \, 1/3 \,$, $\rho \, = \, 0.6 \,$, $\eta \, = \, 1 \,$, $\nu \, = \, 0.4 \,$, $\gamma_{ij} \, = \, 1 \,$ and $ c_{i} \, = \, 0.015 \,$.}} 
% \end{figure}

% To conclude, note that in this example of the equilibrium is always unique, i.e. the aggregate capital stock $\left(K_{t}\right)$ pins down the number of firms per industry $\left(n_{t}\right)$ and all other equilibrium variables. However, if the complementarity between firm entry and labor supply is strong enough, there can be generate multiple equilibria, results on this are available upon request.



\begin{comment}

\subsection{Law of Motion: Stochastic Productivity \label{law-of-motion-stochastic-productivity}}

Suppose for simplicity that $z_{t}$ can take three values: a low value $z_{L}$, an intermediate value $z_{M}$ and
a high value $z_{H}$. Figure \ref{fig:Law-of-Motion-Homog-UE-stochastic}
represents the law of motion under each value of aggregate productivity.

\begin{figure}[H]
\begin{minipage}[b]{.5\linewidth}
\centering{}\includegraphics*[scale=0.475]{input/lom_stochastic.eps}\subcaption{Baseline \label{fig:Law-of-Motion-Homog-UE-stochastic}}
\end{minipage}%
\begin{minipage}[b]{.5\linewidth}
\centering{}\includegraphics*[scale=0.475]{input/lom_stochastic_heterog.eps}\subcaption{Effect of an increase in $\gamma$ \label{fig:Law-of-Motion-Heterog-stochastic}}
\end{minipage}
\caption{Law of motion with stochastic productivity\protect \\ {Note: \small{} the figure shows the law of motion of capital for different levels of aggregate productivity (Panel (a)) and how it changes when the most productivity firm becomes even more productive (Panel (b)). }}\label{fig:lom_stochastic}
\end{figure}


As one can see, when aggregate productivity is low and equal to $z_{L}$, the economy exhibits a unique steady-state where all industries are a monopoly ($K_{L}^{*}$). Under $z_{H}$, on the other hand, there is only a unique steady-state where all industries are a duopoly ($K_{H}^{*}$). Finally, when aggregate productivity takes the intermediate value $z_{M}$, the economy exhibits two steady-states: a low one where all industries are a monopoly ($K_{M1}^{*}$) and a high one where all industries are a duopoly ($K_{M2}^{*}$).

To exemplify the dynamics of the model, suppose that aggregate productivity
starts at $z_{H}$ and that the economy is at the steady-state
$K_{H}^{*}$. Suppose now that there is a negative aggregate
productivity shock, which reduces aggregate productivity permanently to $z_{M}$. After this shock, the economy will converge to
the new steady-state $K_{M2}^{*}$. Output is lower than
before, but the market structure is identical \textendash{} all sectors are still a duopoly.

Now suppose that, instead of falling permanently to $z_{M}$, aggregate productivity falls first to $z_{L}$, and later increases to $z_{M}$. Suppose further that aggregate productivity remains at $z_{L}$ for sufficiently large period, so that the economy approaches the low steady-state $K_{L}^{*}$. Then, as aggregate productivity increases to $z_{M}$, the economy will approach $K_{M1}^{*}$. Note now that in the new steady-state all sectors are a monopoly. The economy therefore experiences a persistent transition to a regime featuring a more concentrated market structure.

Figure \ref{fig:Law-of-Motion-Heterog-stochastic} shows the effect of an increase in the productivity of the top firm ($\gamma$). The main
difference with respect to Figure \ref{fig:Law-of-Motion-Homog-UE-stochastic}
is that now, for the intermediate value of aggregate productivity
$z_{M}$, there is only one steady-state \textendash{}  it becomes increasingly more difficult to sustain
a duopoly and, as a consequence, the steady-state $K_{M2}^{*}$
disappears. Note that the two steady-states $K_{L}^{*}$
and $K_{H}^{*}$ are larger after the increase in the leaders'
productivity. The same happens with the low steady-state when aggregate
productivity is equal to $z_{M}$ ($K_{M1}^{*}$). This
result is not surprising. Keeping the market structure constant (for
example, a monopoly in every industry), the higher the productivity
of the leader, the higher is aggregate output.
\end{comment}

% \subsection{Factor Costs and Factor Shares \label{subsec:Aggregate-Factor-Share}}

% \subsubsection*{Aggregate TFP}

% Suppose all industries are identical and that $\eta=1$. Let $s_{j}$ denote the market
% share of firm $j$ and let $v_{j}$ denote its input share within
% the industry. Note that firm $j$ produces $\dfrac{s_{j}}{s_{1}}$
% as much output as firm $1$ and uses $\dfrac{s_{j}}{s_{1}}\dfrac{\gamma_{1}}{\gamma_{j}}$
% as many inputs. We have that
% \begin{align}
% \begin{array}{cl}
%  & \sum\limits_{k=1}^{n}v_{k}=1%\\
% %\Leftrightarrow & v_{1}\dfrac{\gamma_{1}}{s_{1}}\sum\limits_{k=1}^{n}\dfrac{s_{k}}{\gamma_{k}}=1\\
% \Leftrightarrow  v_{1}=\dfrac{s_{1}}{\gamma_{1}}\left(\sum\limits_{k=1}^{n}\dfrac{s_{k}}{\gamma_{k}}\right)^{-1}
% \end{array}
% \end{align}
% Note that we can write aggregate output as
% \begin{align}
% \begin{array}{rl}
%  Y_{t}=\left[\sum\limits_{i=1}^{I}\left(\sum\limits_{k=1}^{n}y_{k}\right)^{\rho}\right]^{\frac{1}{\rho}}%\\
% %\Leftrightarrow & Y_{t}=I^{\frac{1}{\rho}}\sum\limits_{k=1}^{n}y_{k}\\
% %\Leftrightarrow & Y_{t}=I^{\frac{1}{\rho}}\sum\limits_{k=1}^{n}\gamma_{k}\left(v_{k}I^{-1}L\right)^{1-\alpha}\left(v_{k}I^{-1}K\right)^{\alpha}\\
% %\Leftrightarrow & Y_{t}=I^{-\frac{1-\rho}{\rho}}\left(\sum\limits_{k=1}^{n}\gamma_{k}v_{k}\right)L^{1-\alpha}K^{\alpha}\\
% %\Leftrightarrow & Y_{t}=I^{-\frac{1-\rho}{\rho}}\left(\sum\limits_{k=1}^{n}\gamma_{k}\dfrac{s_{k}}{s_{1}}\dfrac{\gamma_{1}}{\gamma_{k}}v_{1}\right)L^{1-\alpha}K^{\alpha}\\
% %%\Leftrightarrow & Y_{t}=I^{-\frac{1-\rho}{\rho}}\Big(\dfrac{\gamma_{1}}{s_{1}}v_{1}\underbrace{\sum\limits_{k=1}^{n}s_{k}}_{=1}\Big)L^{1-\alpha}K^{\alpha}\\
% %\Leftrightarrow & Y_{t}=I^{-\frac{1-\rho}{\rho}}\left(\sum\limits_{k=1}^{n}\dfrac{s_{k}}{\gamma_{k}}\right)^{-1}L^{1-\alpha}K^{\alpha}\\
% %\Leftrightarrow & Y_{t}
% =\underbrace{I^{-\frac{1-\rho}{\rho}}\left\{ \sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}\dfrac{1}{1-\rho}\left[1-\dfrac{n-\left(1-\rho\right)}{\sum\limits_{h=1}^{n}\dfrac{1}{\gamma_{h}}}\dfrac{1}{\gamma_{k}}\right]\right\} ^{-1}}_{\coloneqq\Phi\left(n\right)}L^{1-\alpha}K^{\alpha}
% \end{array}
% \end{align}

% In this particular case, in which all industries are identical and $\eta=1$, aggregate productivity decreases in the number of active firms. This result simply reflects the fact that firms enter in reverse order of productivity. To prove it, note the each firm's market share decreases in the number
% of active firms in its industry. We hence have that $s_{k}<\tilde{s}_{k}\:,\:\forall k$
% and that $\gamma_{n+1}<\gamma_{k}\:,\:\forall k\leq n$ . These facts imply
% that
% \begin{align}
% \sum\limits_{k=1}^{n}s_{k}\dfrac{1}{\gamma_{k}}<\left(\sum\limits_{k=1}^{n}\tilde{s}_{k}\dfrac{1}{\gamma_{k}}\right)+\tilde{s}_{n+1}\dfrac{1}{\gamma_{n+1}}
% \end{align}

% \subsubsection*{Aggregate Factor Cost Index}
% Suppose all industries are identical and that $\eta=1$.
% When there are $n$ firms in every industry we have
% \begin{align}
% \Theta\left(n\right)=\dfrac{n-\left(1-\rho\right)}{\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}}
% \end{align}
% We can show that $\Theta\left(n\right)$ is increasing in $n$. To see this, note that
% \begin{align}
% \begin{array}{cl}
%  & \dfrac{n+1-\left(1-\rho\right)}{\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}+\dfrac{1}{\gamma_{n+1}}}>\dfrac{n-\left(1-\rho\right)}{\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}}\\
% %\Leftrightarrow & \dfrac{n+1-\left(1-\rho\right)}{n-\left(1-\rho\right)}>\dfrac{\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}+\dfrac{1}{\gamma_{n+1}}}{\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}}\\
% %\Leftrightarrow & \dfrac{1}{n-\left(1-\rho\right)}>\dfrac{\dfrac{1}{\gamma_{n+1}}}{\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}}\\
% \Leftrightarrow & \gamma_{n+1}\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}>n-\left(1-\rho\right)
% \end{array}
% \end{align}
% The last condition is implied by (\ref{eq:cond_mg_1}).


% \subsection{Multiple Equilibria \label{subsec: Static-Multiplicity}} 

% In the example of Figure \ref{fig:Static-Equilibrium} the equilibrium is always unique, i.e. the aggregate capital stock $K_{t}$ pins down the number of firms per industry $n_{t}$ and all other equilibrium variables. This happens because the bounds $\overline{K}\left(\cdot\right)$ and $\underline{K}\left(\cdot\right)$ satisfy
% \begin{align}
% \overline{K}\left(\Gamma,n\right)<\underline{K}\left(\Gamma,n+1\right)\quad,\qquad\forall n
% \end{align}
% However, if the above condition is not satisfied, there can be multiple equilibria. Suppose that the bounds $\overline{K}\left(\cdot\right)$ and $\underline{K}\left(\cdot\right)$ satisfy
% \begin{align}
% \underline{K}\left(\Gamma,n+1\right)<\overline{K}\left(\Gamma,n\right) \quad,\qquad \text{ for some } n
% \end{align}
% When $K_{t}\in\left[\underline{K}\left(\Gamma,n+1\right), \overline{K}\left(\Gamma,n\right)\right]$, the economy features multiple equilibria: it can feature a symmetric equilibrium with $n$ firms per industry, a symmetric equilibrium with $n+1$ per industry, and also an asymmetric equilibrium with $n$ firms in some industries and $n+1$ in some others. Figure \ref{fig:Static-Multiplicity-Figure} shows aggregate output $Y_t$ as a function of the aggregate capital stock $K_t$ for an economy in which (static) multiplicity can occur. 

% \begin{figure}[ht!]
% \centering{}%
% \includegraphics*[scale=0.6]{input/production_function_me}\tabularnewline
% \caption{Static
% Multiplicity\protect \\ {Note: \small{} the figure represents the relation between capital and output. Solid lines depict symmetric equilibria, while dotted lines are asymmetric ones.}}
% \label{fig:Static-Multiplicity-Figure}
% \end{figure}

% The full lines represent symmetric equilibria in which all industries are identical, whereas the dashed lines represent asymmetric equilibria.
% Note that (static) multiplicity arises because of a positive complementarity between competition and labor supply. For a given capital stock level $K_{t}$ there can be an equilibrium featuring a large number of active firms, and hence high factor shares, high wages and high labor supply; and another possible equilibrium with a lower number of firms, and hence low factor shares, low wages and a depressed labor supply. The following proposition provides the conditions for (static) multiplicity.

% \begin{prop}
%  (Static Multiplicity)\label{(static-multiplicity)} Suppose that
% an equilibrium with \textup{$n$} firms per industry is possible at
% time $t$. An equilibrium with \textup{$n+1$} firms is also possible
% provided that
% \begin{align}
% \dfrac{\Phi\left(\Gamma,n\right)}{\Phi\left(\Gamma,n+1\right)}<\left[\dfrac{\Theta\left(\Gamma,n\right)}{\Theta\left(\Gamma,n+1\right)}\right]^{\frac{\rho}{1-\rho}-\frac{1-\alpha}{\nu+\alpha}}
% \end{align}
% \end{prop}
% \begin{proof}[Proof of Proposition \ref{(static-multiplicity)}]
% Suppose that 
% \begin{align}
% \underline{K}\left(\Gamma,n\right)\leq K_{t}\leq\overline{K}\left(\Gamma,n\right)
% \end{align}
% so that a symmetric equilibrium with $n$ firms in every industry
% is possible. A symmetric equilibrium with $n+1$ firms will also be
% possible provided that 
% \begin{align}
% \begin{array}{cl}
%  & \underline{K}\left(\Gamma,n+1\right)<\overline{K}\left(\Gamma,n\right)\\begin{align}2ex]
% \Leftrightarrow & \dfrac{c_{i}}{\varLambda\left(n+1,\gamma_{n+1}\right)}\dfrac{\left[\Theta\left(\Gamma,n+1\right)\right]^{\frac{\rho}{1-\rho}-\frac{1-\alpha}{\nu+\alpha}}}{\Phi\left(\Gamma,n+1\right)} < \dfrac{c_{i}}{\varLambda\left(n+1,\gamma_{n+1}\right)}\dfrac{\left[\Theta\left(\Gamma,n\right)\right]^{\frac{\rho}{1-\rho}-\frac{1-\alpha}{\nu+\alpha}}}{\Phi\left(\Gamma,n\right)}\\begin{align}2ex]
% \Leftrightarrow & \dfrac{\Phi\left(\Gamma,n\right)}{\Phi\left(\Gamma,n+1\right)}<\left[\dfrac{\Theta\left(\Gamma,n\right)}{\Theta\left(\Gamma,n+1\right)}\right]^{\frac{\rho}{1-\rho}-\frac{1-\alpha}{\nu+\alpha}}
% \end{array}
% \end{align}\end{proof}
% %
% \begin{cor}
% (Static Multiplicity with No Productivity Differences)\label{corollarypropa1} When all firms
% are equally productive there can be equilibrium multiplicity if and
% only if
% \begin{align}
% \dfrac{\rho}{1-\rho}<\dfrac{1-\alpha}{\nu+\alpha}
% \end{align}
% \end{cor}

% \begin{proof}[Proof of Corollary \ref{corollarypropa1}]
% when there are no productivity differences, the condition
% becomes
% \begin{align}
% \begin{array}{cl}
%  & \left[\dfrac{\Theta\left(\Gamma,n\right)}{\Theta\left(\Gamma,n+1\right)}\right]^{\frac{\rho}{1-\rho}-\frac{1-\alpha}{\nu+\alpha}}>1%\\begin{align}1.5ex]
% %\Leftrightarrow & \dfrac{\rho}{1-\rho}-\dfrac{1-\alpha}{\nu+\alpha}<0\\begin{align}1.5ex]
% %\Leftrightarrow & \dfrac{\rho}{1-\rho}<\dfrac{1-\alpha}{\nu+\alpha}\\begin{align}1.5ex]
% %\Leftrightarrow & \rho<\dfrac{1-\alpha}{\nu+\alpha}\left(1-\rho\right)\\begin{align}1.5ex]
% \Leftrightarrow  \dfrac{\rho}{1-\rho}<\dfrac{1-\alpha}{\nu+\alpha}
% \end{array}
% \end{align}
% \end{proof}

% As the above corollary makes it clear, in the limit case in which firms are equally productive, static multiplicity
% depends on three main parameters: $\rho$, $\nu$ and $\alpha$. In
% particular, when there are no productivity differences, static multiplicity
% arises whenever (i) $\rho$ is low (so that differentiation across
% varieties is large and markups/factor shares display a high responsiveness
% to changes in the number of firms), (ii) the wage elasticity of labor
% supply $\dfrac{1}{\nu}$ is large or (iii) when the labor elasticity
% of output $1-\alpha$ is large. Note that in the limit case of perfect
% competition ($\rho=1$, $c_{i}=0$ and no productivity differences),
% static multiplicity can never arise.


\subsection{Asymmetric Equilibrium\label{subsec:Asymmetric Equilibrium}}

When
\begin{align}
\overline{K}\left(\Gamma,n\right) <  K < \underline{K}\left(\Gamma,n+1\right)
\end{align}
there will be an asymmetric equilibrium at time $t+1$:
some industries will contain $n$ firms, whereas some industries will
contain $n+1$ firms. The fraction of industries with $n+1$ will
be pinned down by a zero profit condition for the marginal entrant
in an industry with $n+1$ firms
\begin{align}
\varLambda\left(\Gamma,\gamma_{n+1},n+1\right)\Theta^{-\frac{\rho}{1-\rho}}Y=c_{i}
\end{align}


The equilibrium is characterized by 4 variables: 
the fraction of the industries
with $n+1$ firms ($\eta$), aggregate output ($Y$), aggregate productivity ($\Phi$) and the aggregate cost index ($\Theta$). These 4 variables are pinned down by the following 4 equations

\begin{align}
Y=\Phi\left[\left(1-\alpha\right)\Theta\right]^{\frac{1-\alpha}{\nu+\alpha}}K^{\alpha\frac{1+\nu}{\nu+\alpha}}\\
\Phi=\dfrac{\left\{ \left(1-\eta\right)\left[\dfrac{n-\left(1-\rho\right)}{\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{1k}}}\right]^{\frac{\rho}{1-\rho}}+\eta\left[\dfrac{n+1-\left(1-\rho\right)}{\sum\limits_{k=1}^{n+1}\dfrac{1}{\gamma_{2k}}}\right]^{\frac{\rho}{1-\rho}}\right\} ^{\frac{1}{\rho}}}{\left(1-\eta\right)\left[\dfrac{n-\left(1-\rho\right)}{\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{1k}}}\right]^{\frac{1}{1-\rho}}\left(\sum\limits_{k=1}^{n}\dfrac{s_{1k}}{\gamma_{1k}}\right)+\eta\left[\dfrac{n+1-\left(1-\rho\right)}{\sum\limits_{k=1}^{n+1}\dfrac{1}{\gamma_{2k}}}\right]^{\frac{1}{1-\rho}}\left(\sum\limits_{k=1}^{n+1}\dfrac{s_{2k}}{\gamma_{2k}}\right)\vphantom{\left[\dfrac{\dfrac{\sum\limits_{k}^{n}\dfrac{1}{\gamma}}{1}}{\dfrac{\sum\limits_{k}^{n}\dfrac{1}{\gamma}}{1}}\right]}}\\
\Theta=\left\{ \left(1-\eta\right)\left[\dfrac{n-\left(1-\rho\right)}{\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}}\right]^{\frac{\rho}{1-\rho}}+\eta\left[\dfrac{n+1-\left(1-\rho\right)}{\sum\limits_{k=1}^{n+1}\dfrac{1}{\gamma_{k}}}\right]^{\frac{\rho}{1-\rho}}\right\} ^{\frac{1-\rho}{\rho}}\vphantom{\left[\dfrac{\dfrac{\sum\limits_{k}^{n}\dfrac{1}{\gamma}}{1}}{\dfrac{\sum_{k}^{n}\dfrac{1}{\gamma}}{1}}\right]}\\
\varLambda\left(\Gamma,\gamma_{n+1},n+1\right)\Theta^{-\frac{\rho}{1-\rho}}Y=c_{i}
\end{align}

$s_{1k}$ is the market share of firm $k$ in an industry with $n$ firms, whereas $s_{2k}$ is the market share of firm $k$ in an industry with $n+1$ firms. They are defined in Appendix
\ref{proofs_appendixB}.


% \subsection{Basins of Attraction} \label{subsec:basin_attraction}

% In a steady-state with a constant productivity distribution $\mathbb{Z}_{\tau}$ and a set of active firms $\left\{ n_{i}\right\} _{i=1}^{I}$, the aggregate savings rate is equal to
% \begin{align}
% s=\dfrac{\beta\delta}{1-\left(1-\delta\right)\beta}\:\alpha\:\Omega\left(\mathbb{Z}_{\tau t},\left\{ n_{i}\right\} _{i=1}^{I}\right)
% \end{align}
% Recall that we also have
% \begin{align}
% Y=\Phi\left(\mathbb{Z}_{\tau },\left\{ n_{i}\right\} _{i=1}^{I}\right)\left[\left(1-\alpha\right)\Theta\left(\mathbb{Z}_{\tau},\left\{ n_{i}\right\} _{i=1}^{I}\right)\right]^{\frac{1-\alpha}{\nu+\alpha}}K^{\alpha\frac{1+\nu}{\nu+\alpha}}
% \end{align}
% We can combine the above two equations with
% \begin{align}
% \delta  K = s Y
% \end{align}
% to write
% \begin{align}
% \begin{array}{rl}
%  & Y=\Phi\left(\mathbb{Z}_{\tau},\left\{ n_{i}\right\} _{i=1}^{I}\right)\left[\left(1-\alpha\right)\Theta\left(\mathbb{Z}_{\tau},\left\{ n_{i}\right\} _{i=1}^{I}\right)\right]^{\frac{1-\alpha}{\nu+\alpha}}\left[\dfrac{\beta}{1-\left(1-\delta\right)\beta}\:\alpha\:\Omega\left(\mathbb{Z}_{\tau},\left\{ n_{i}\right\} _{i=1}^{I}\right)Y\right]^{\alpha\frac{1+\nu}{\nu+\alpha}}\\
% %\Leftrightarrow & Y^{\frac{\nu-\alpha\nu}{\nu+\alpha}}=\Phi\left(\mathbb{Z}_{\tau},\left\{ n_{i}\right\} _{i=1}^{I}\right)\left[\left(1-\alpha\right)\Theta\left(\mathbb{Z}_{\tau},\left\{ n_{i}\right\} _{i=1}^{I}\right)\right]^{\frac{1-\alpha}{\nu+\alpha}}\left[\dfrac{\beta}{1-\left(1-\delta\right)\beta}\:\alpha\:\Omega\left(\mathbb{Z}_{\tau},\left\{ n_{i}\right\} _{i=1}^{I}\right)\right]^{\alpha\frac{1+\nu}{\nu+\alpha}}\\
% %\Leftrightarrow & Y=\left[\Phi\left(\mathbb{Z}_{\tau},\left\{ n_{i}\right\} _{i=1}^{I}\right)\right]^{\frac{\nu+\alpha}{\nu-\alpha\nu}}\left[\left(1-\alpha\right)\Theta\left(\mathbb{Z}_{\tau},\left\{ n_{i}\right\} _{i=1}^{I}\right)\right]^{\frac{1-\alpha}{\nu-\alpha\nu}}\left[\dfrac{\beta}{1-\left(1-\delta\right)\beta}\:\alpha\:\Omega\left(\mathbb{Z}_{\tau},\left\{ n_{i}\right\} _{i=1}^{I}\right)\right]^{\alpha\frac{1+\nu}{\nu-\alpha\nu}}\\
% %\Leftrightarrow & Y=\left[\Phi\left(\mathbb{Z}_{\tau},\left\{ n_{i}\right\} _{i=1}^{I}\right)\right]^{\frac{\nu+\alpha}{\nu-\alpha\nu}-\alpha\frac{1+\nu}{\nu-\alpha\nu}}\left[\Theta\left(\mathbb{Z}_{\tau},\left\{ n_{i}\right\} _{i=1}^{I}\right)\right]^{\frac{1-\alpha}{\nu-\alpha\nu}+\alpha\frac{1+\nu}{\nu-\alpha\nu}}\left(1-\alpha\right)^{\frac{1-\alpha}{\nu-\alpha\nu}}\left[\dfrac{\beta\alpha}{1-\left(1-\delta\right)\beta}\right]^{\alpha\frac{1+\nu}{\nu-\alpha\nu}}\\
% \Leftrightarrow & Y=\Phi\left(\mathbb{Z}_{\tau},\left\{ n_{i}\right\} _{i=1}^{I}\right)\left[\Theta\left(\mathbb{Z}_{\tau},\left\{ n_{i}\right\} _{i=1}^{I}\right)\right]^{\frac{1+\alpha\nu}{\nu\left(1-\alpha\right)}}\left(1-\alpha\right)^{\frac{1-\alpha}{\nu-\alpha\nu}}\left[\dfrac{\beta\alpha}{1-\left(1-\delta\right)\beta}\right]^{\alpha\frac{1+\nu}{\nu-\alpha\nu}}
% \end{array}
% \end{align}

\section{The Baseline Model}\label{appendix:baseline-model}

\subsection*{Comparative Statics with $\uparrow \gamma_{1}$ and $\leftrightarrow \gamma_{2}$ (mean-increasing spread)}
\begin{figure}[H]
\centering{}
\hspace{-0.2cm}
 \includegraphics*[scale=0.475]{input/LOM_MIS}
 \hspace{0.4cm}
 \includegraphics*[scale=0.475]{input/RR_MIS}
\caption{Law of Motion and Rental Rate Map \label{fig:Law-of-Motion-MIS}
\protect \\ {This example features two stable steady states and an unstable one. We use $\psi \, = \, 1 \,$,  $\rho \, = \, 3/4 \,$, $\eta \, = \, 1 \,$, $\alpha \, = \, 1/3 \,$, $\delta \, = \, 1 \,$, $\nu \, = \, 2/5 \,$ and $ c_{i} \, = \, 0.015 \,$.}} 
\end{figure}

\subsection*{Steady-State Multiplicity}
\begin{figure}[H]
\centering{}
\hspace{-0.2cm}
 \includegraphics*[scale=0.475]{input/LOM_cf_existence}
 \hspace{0.4cm}
 \includegraphics*[scale=0.475]{input/RR_cf_existence}
\caption{Law of Motion and Rental Rate Map \label{fig:Law-of-Motion-existence}
\protect \\ {This example features two stable steady states and an unstable one. We use $\psi \, = \, 1 \,$,  $\rho \, = \, 3/4 \,$, $\eta \, = \, 1 \,$, $\alpha \, = \, 1/3 \,$, $\delta \, = \, 1 \,$ and $\nu \, = \, 2/5 $.}} 
\end{figure}

==> submitted_version/proofs.tex <==

\section{Proofs and Additional Results for Section \ref{sec:Model} \label{Proofs-Additional-Results}}


\subsubsection*{Proof of Lemma \ref{aggregate_factor_share_lem}}
\begin{proof}
Using equation (\ref{eq:agg_factor_share_HHI}) and imposing $\eta=1$ and symmetry we obtain $\Omega(\Gamma_n, n)=1-(1-\rho)HHI_t$ where $HHI_t$ is the Herfindhal-Hirschman Index of the economy. As $\rho<1$ the aggregate factor share decreases in concentration, as measured by HHI. The latter is trivially decreasing in $n$, which proves the first part of the lemma.
Furthermore, a mean-preserving spread of productivity, holding $n$ fixed, implies a spread of the market shares distribution. Since HHI is a convex function of market shares, it necessarily increases after a spread of the productivity distribution. The statement follows. 
\end{proof}

% \begin{lemma}[Labor Response]\label{lemma:signL}
% If the labor supply is upward sloping and wages increase in $\Theta\left(\cdot\right)$ (for fixed $K$), the labor response to changes in the technology fundamental $\lambda$ has the same sign as the effect on the function $\Theta(\cdot): \sgn\{L_\lambda\}=\sgn\{\Theta_\lambda\}.$
% \end{lemma}

% \begin{proof}[Proof of Lemma \ref{lemma:signL}]
% We want to sign $L_\lambda$. We start by noting that $L_\lambda=L_w w_\lambda$. Note that we can write the equivalent of equation \ref{rmap} for the wage: $ w=\Theta(\Lambda,n)F_L$, where $F=F(K,L)$.  Further, $\sgn\{w_\lambda\}=\sgn\{\Theta_\lambda\}$. Therefore, provided that $L_w>0$ the statement follows.
% \end{proof}


\subsubsection*{Proof of Proposition \ref{A-symmetric-equilibrium}}


\begin{proof}
Suppose $\eta=1$.When there are $n$ active firms in a given industry, the profits of a firm with productivity $\gamma_{j}$ are equal to
\begin{align}
\Pi\left(\gamma_{j},n,\Gamma,\Theta,Y\right) = \varLambda\left(\gamma_{j},n,\Gamma\right) \Theta^{-\frac{\rho}{1-\rho}}Y
\end{align}
where
$\varLambda\left(\gamma_{j},n,\Gamma\right)$ has been defined in Appendix \ref{proofs_appendixB}. A symmetric equilibrium with $n$ firms per industry is possible provided that
\begin{align*}
    \varLambda\left(\gamma_{n},n,\Gamma\right) \Theta^{-\frac{\rho}{1-\rho}}Y & \geq c \\
    \varLambda\left(\gamma_{n+1},n+1,\Gamma\right) \Theta^{-\frac{\rho}{1-\rho}}Y & \leq c
\end{align*}
Using equation (\ref{eq:agg_output_capital}), we can write the above inequalities as 
\begin{align}
\underline{K}\left(\Gamma,n\right)\leq K_{t}\leq\overline{K}\left(\Gamma,n\right),
\end{align}
where
\begin{align}
\underline{K}\left(\Gamma,n\right) = \left\{ \dfrac{c}{\varLambda\left(\gamma_{n},n,\Gamma\right)}\left(1-\alpha\right)^{-\frac{1-\alpha}{\nu+\alpha}}\left[\Phi\left(\Gamma,n\right)\right]^{-1}\left[\Theta\left(\Gamma,n\right)\right]^{\frac{\rho}{1-\rho}-\frac{1-\alpha}{\nu+\alpha}}\right\} ^{\frac{\nu+\alpha}{\alpha\left(1+\nu\right)}} \\
\overline{K}\left(\Gamma,n\right) = \left\{ \dfrac{c}{\varLambda\left(\gamma_{n+1},n+1,\Gamma\right)}\left(1-\alpha\right)^{-\frac{1-\alpha}{\nu+\alpha}}\left[\Phi\left(\Gamma,n\right)\right]^{-1}\left[\Theta\left(\Gamma,n\right)\right]^{\frac{\rho}{1-\rho}-\frac{1-\alpha}{\nu+\alpha}}\right\} ^{\frac{\nu+\alpha}{\alpha\left(1+\nu\right)}}.
\end{align}

The condition on uniqueness can be derived by noting that it arises if and only if the following holds $\forall n$
\[
\begin{array}{cl}
 & \underline{K}\left(\Gamma,n+1\right)>\overline{K}\left(\Gamma,n\right)\\[2ex]
\Leftrightarrow & \left[\Phi\left(\Gamma,n+1\right)\right]^{-1}\left[\Theta\left(\Gamma,n+1\right)\right]^{\frac{\rho}{1-\rho}-\frac{1-\alpha}{\nu+\alpha}}>\left[\Phi\left(\Gamma,n\right)\right]^{-1}\left[\Theta\left(\Gamma,n\right)\right]^{\frac{\rho}{1-\rho}-\frac{1-\alpha}{\nu+\alpha}}\\[2ex]
\Leftrightarrow & \dfrac{\Phi\left(\Gamma,n\right)}{\Phi\left(\Gamma,n+1\right)}>\left[\dfrac{\Theta\left(\Gamma,n\right)}{\Theta\left(\Gamma,n+1\right)}\right]^{\frac{\rho}{1-\rho}-\frac{1-\alpha}{\nu+\alpha}}
\end{array}
\]
Therefore, when there are no productivity differences across firms, the condition becomes
\[
\begin{array}{cl}
 & \left[\dfrac{\Theta\left(\Gamma,n\right)}{\Theta\left(\Gamma,n+1\right)}\right]^{\frac{\rho}{1-\rho}-\frac{1-\alpha}{\nu+\alpha}}<1\\[2ex]
\Leftrightarrow & \dfrac{\rho}{1-\rho}-\dfrac{1-\alpha}{\nu+\alpha}>0\\[2ex]
\Leftrightarrow & \dfrac{\rho}{1-\rho}>\dfrac{1-\alpha}{\nu+\alpha}
\end{array}
\]
since $\Theta\left(\Gamma,n+1\right)>\Theta\left(\Gamma,n\right)$.
\end{proof}

%\subsection{Savings Rate Lemmas \label{subsec:Proof-prop}}

\subsubsection*{Proof of Lemma \ref{lemma:savings_rate}}

\begin{proof}
In a steady-state we have a constant rental rate
\begin{align}
R^{*} = \beta^{-1} - \left(1-\delta\right)
\end{align}
and
\begin{align}
\delta  K = s Y
\end{align}
Combining these two equations with equation (\ref{eq:factor_demand}) we obtain
\begin{align}\nonumber
 & \beta^{-1}-\left(1-\delta\right)=\alpha\;\Omega\left(\mathbf{\Gamma},\mathbf{N}\right)\;\dfrac{Y^{*}}{K^{*}}\\\nonumber
\Leftrightarrow & \beta^{-1}-\left(1-\delta\right)=\alpha\;\Omega\left(\mathbf{\Gamma},\mathbf{N}\right)\;\dfrac{\delta}{s^{*}}\\
\Leftrightarrow & s^{*}=\dfrac{\delta\;\alpha}{\beta^{-1}-\left(1-\delta\right)}\Omega\left(\mathbf{\Gamma},\mathbf{N}\right)
\end{align}
\end{proof}


\subsubsection*{Proof of Proposition \ref{prop:multiplicity}}
\begin{proof}
We have
\[
R_{t}\;=\;\alpha\;\left(1-\alpha\right)^{\frac{1-\alpha}{\nu+\alpha}}\;\Theta\left(\mathbf{\Gamma},\mathbf{N}_{t}\right)^{\frac{1+\nu}{\nu+\alpha}}\:K_{t}^{-\nu\frac{1-\alpha}{\nu+\alpha}}.
\]
Let $\underline{R}\left(\Gamma,n\right)$ and $\overline{R}\left(\Gamma,n\right)$ be the rental rates at $\underline{K}\left(\Gamma,n\right)$ and $\overline{K}\left(\Gamma,n\right)$ respectively. Then, multiplicity obtains if there exists an $n \in \mathbb{N}$ such that

\[
\begin{array}{rl}
 & \overline{R}\left(\Gamma,n\right)<\underbrace{\beta^{-1}-\left(1-\delta\right)}_{R^{*}}<\underline{R}\left(\Gamma,n+1\right)\\[1ex]
\Leftrightarrow & \;\Theta\left(\Gamma,n\right)^{\frac{1+\nu}{\nu+\alpha}}\:\overline{K}\left(\Gamma,n\right)^{-\nu\frac{1-\alpha}{\nu+\alpha}}<\dfrac{\beta^{-1}-\left(1-\delta\right)}{\alpha\;\left(1-\alpha\right)^{\frac{1-\alpha}{\nu+\alpha}}}<\;\Theta\left(\Gamma,n+1\right)^{\frac{1+\nu}{\nu+\alpha}}\:\underline{K}\left(\Gamma,n+1\right)^{-\nu\frac{1-\alpha}{\nu+\alpha}}.
\end{array}
\]


% Part 2: both bounds are strictly decreasing in the fixed cost so define c lowerbar and c upperbar such that the inequality stated becomes equality on either side
\end{proof}

\subsubsection*{Proof of Lemma \ref{lemma:MPS_theta}}

\begin{proof}
When all industries are identical and have $n$ firms, the factor price index is equal to
\begin{align}
\Theta\left(\Gamma_n,n\right)=\dfrac{n-\left(1-\rho\right)}{\sum\limits_{k=1}^{n}\dfrac{1}{\gamma_{k}}}
\end{align}
As $\Theta$ is a concave function of $\gamma_k$, by the definition of MPS, we have that if $\tilde \Gamma$ is a MPS of $\Gamma$, then $\Theta(\tilde \Gamma,n)<\Theta(\Gamma,n)$.
\end{proof}

% \begin{lemma}
% \label{prop:The-aggregate-factor-share} Let $\Omega\left(\Gamma,n\right)$ be the aggregate factor share in a symmetric equilibrium in which all industries are identical (have the the same productivity distribution $\Gamma$ and the same number of firms $n$). We have that 

% 1. $\Omega\left(\Gamma,n\right)$ increases in $n$: $\Omega\left(\Gamma,n+1\right)>\Omega\left(\Gamma,n\right). $

% 2. Let $\pi_{j}$ be an idiosyncratic productivity type such that
% $\pi_{j}\geq\dfrac{1}{n}\sum\limits_{k=1}^{n}\pi_{k}$. Suppose
% that $\pi_{j}$ increases to $\pi^{\prime}_{j}>\pi_{j}$ in all industries but all
% other types remain unchanged. Then, the new distribution $\Gamma^{\prime}$
% is such that$ \Omega\left(\Gamma^{\prime},n\right)<\Omega\left(\Gamma,n\right).$
% \end{lemma}


% %\subsubsection*{Proof of Lemma \ref{prop:The-aggregate-factor-share}}


% \begin{proof}[Proof of Lemma \ref{prop:The-aggregate-factor-share}]

% The aggregate factor share can be written as the ratio of the aggregate factor cost index and aggregate TFP.
% \begin{align}
% \Omega\left(\Gamma,n\right)=\dfrac{\Theta\left(\Gamma,n\right)}{\Phi\left(\Gamma,n\right)}
% \end{align}
% Assume that all industries are identical (same distribution of idiosyncratic productivities $\Gamma$ and same number of active firms $n$) and that $\eta=1$. As shown in online appendix \ref{subsec:Aggregate-Factor-Share} the aggregate factor cost index $\Theta\left(\Gamma,n\right)$
% is increasing in $n$, and aggregate TFP $\Phi\left(\Gamma,n\right)$
% is decreasing in $n$. This implies that $\Omega\left(\Gamma,n\right)$ is increasing in the number of firms per industry $n$.

% %The second part of the proposition is proved in online appendix \ref{subsec:Aggregate-Factor-Share}.
% %\end{proof}
% % Recall that the aggregate factor share is equal to
% % \begin{align}
% % \Omega\left(\Gamma,n\right)=\dfrac{\Theta\left(\Gamma,n\right)}{\Phi\left(\Gamma,n\right)}
% % \end{align}
% % As we have seen before, the aggregate factor cost index $\Theta\left(\Gamma,n\right)$
% % is increasing in $n$, and aggregate TFP $\Phi\left(\Gamma,n\right)$
% %is decreasing in $n$. 
% To prove the second part of the proposition, note that the aggregate factor share can be written as
% \begin{align}
% \Omega\left(\Gamma,n\right)=\left(\dfrac{n}{1-\rho}-1\right)\left\{ \sum\limits_{k=1}^{n}\dfrac{\dfrac{1}{\pi_{k}}}{\sum\limits_{h=1}^{n}\dfrac{1}{\pi_{h}}}\left[1-\left[n-\left(1-\rho\right)\right]\dfrac{\dfrac{1}{\pi_{k}}}{\sum\limits_{h=1}^{n}\dfrac{1}{\pi_{h}}}\right]\right\} 
% \end{align}
% Take some $j<n$ such that $\pi_{j}\geq\dfrac{1}{n}\sum\limits_{h=1}^{n}\pi_{h}$.
% First note that we must have that
% %\begin{align}
% %\dfrac{\dfrac{1}{\pi_{j}}}{\dfrac{1}{n}\sum\limits_{h=1}^{n}\dfrac{1}{\pi_{h}}}\leq1
% %\end{align}
% %To see this, note that
% \begin{align}
% \begin{array}{cl}
%  & \dfrac{1}{\pi_{j}}\leq\dfrac{1}{n}\sum\limits_{h=1}^{n}\dfrac{1}{\pi_{h}}%\\
% %\Leftrightarrow & 1\leq\dfrac{1}{n}\sum\limits_{h=1}^{n}\dfrac{\pi_{j}}{\pi_{h}}\\
% %\Leftrightarrow & 1\leq\dfrac{1}{n}\sum\limits_{h=1}^{n}\dfrac{\pi_{j}}{\dfrac{1}{n}\sum\limits_{k=1}^{n}\pi_{k}}\dfrac{\dfrac{1}{n}\sum\limits_{k=1}^{n}\pi_{k}}{\pi_{h}}\\
% \Leftrightarrow  1\leq\underbrace{\dfrac{\pi_{j}}{\dfrac{1}{n}\sum\limits_{k=1}^{n}\pi_{k}}}_{\geq1}\underbrace{\vphantom{\dfrac{\pi_{j}}{\dfrac{1}{n}\sum\limits_{k=1}^{n}\pi_{k}}}\dfrac{1}{n}\sum\limits_{h=1}^{n}\dfrac{\dfrac{1}{n}\sum\limits_{k=1}^{n}\pi_{k}}{\pi_{h}}}_{\geq1}
% \end{array}
% \end{align}
% Now suppose that $\pi_{j}$ increases to $\tilde{\pi}_{j}>\pi_{j}$.
% We want to show that $\Omega\left(\mathcal{\tilde{F}},n\right)<\Omega\left(\Gamma,n\right)$, this holds if

% \begin{align}
% \begin{array}{cl}
%  & \sum\limits_{k=1}^{n}\dfrac{\dfrac{1}{\tilde{\pi}_{k}}}{\sum\limits_{h=1}^{n}\dfrac{1}{\tilde{\pi}_{h}}}\left[1-\left[n-\left(1-\rho\right)\right]\dfrac{\dfrac{1}{\tilde{\pi}_{k}}}{\sum\limits_{h=1}^{n}\dfrac{1}{\tilde{\pi}_{h}}}\right]<\sum\limits_{k=1}^{n}\dfrac{\dfrac{1}{\pi_{k}}}{\sum\limits_{h=1}^{n}\dfrac{1}{\pi_{h}}}\left[1-\left[n-\left(1-\rho\right)\right]\dfrac{\dfrac{1}{\pi_{k}}}{\sum\limits_{h=1}^{n}\dfrac{1}{\pi_{h}}}\right]\\
% %\Leftrightarrow & \sum\limits_{k=1}^{n}\dfrac{1}{\tilde{\pi}_{k}}\left[\sum\limits_{h=1}^{n}\dfrac{1}{\tilde{\pi}_{h}}-\left[n-\left(1-\rho\right)\right]\dfrac{1}{\tilde{\pi}_{k}}\right]<\dfrac{\sum\limits_{h=1}^{n}\dfrac{1}{\tilde{\pi}_{h}}}{\sum\limits_{h=1}^{n}\dfrac{1}{\pi_{h}}}\sum\limits_{k=1}^{n}\dfrac{1}{\pi_{k}}\left[\sum\limits_{h=1}^{n}\dfrac{1}{\tilde{\pi}_{h}}-\left[n-\left(1-\rho\right)\right]\dfrac{\sum\limits_{h=1}^{n}\dfrac{1}{\tilde{\pi}_{h}}}{\sum\limits_{h=1}^{n}\dfrac{1}{\pi_{h}}}\dfrac{1}{\pi_{k}}\right]\\
% %\Leftrightarrow & \sum\limits_{k=1}^{n}\dfrac{1}{\tilde{\pi}_{k}}\left[\sum\limits_{h=1}^{n}\dfrac{1}{\tilde{\pi}_{h}}-\left[n-\left(1-\rho\right)\right]\dfrac{1}{\tilde{\pi}_{k}}\right]<\left[1+\dfrac{\dfrac{1}{\tilde{\pi}_{j}}-\dfrac{1}{\pi_{j}}}{\sum\limits_{h=1}^{n}\dfrac{1}{\pi_{h}}}\right] \cdot \\
% %& \cdot \sum\limits_{k=1}^{n}\dfrac{1}{\pi_{k}}\left\{ \sum\limits_{h=1}^{n}\dfrac{1}{\tilde{\pi}_{h}}-\left[n-\left(1-\rho\right)\right]\left[1+\dfrac{\dfrac{1}{\tilde{\pi}_{j}}-\dfrac{1}{\pi_{j}}}{\sum\limits_{h=1}^{n}\dfrac{1}{\pi_{h}}}\right]\dfrac{1}{\pi_{k}}\right\} \\
% \Leftrightarrow & \sum\limits_{k=1}^{n}\dfrac{1}{\tilde{\pi}_{k}}\left[\sum\limits_{h=1}^{n}\dfrac{1}{\tilde{\pi}_{h}}-\left[n-\left(1-\rho\right)\right]\dfrac{1}{\tilde{\pi}_{k}}\right]<\sum\limits_{k=1}^{n}\dfrac{1}{\pi_{k}}\left[\sum\limits_{h=1}^{n}\dfrac{1}{\tilde{\pi}_{h}}-\left[n-\left(1-\rho\right)\right]\dfrac{1}{\pi_{k}}\right]+\\
%  & +\dfrac{\dfrac{1}{\tilde{\pi}_{j}}-\dfrac{1}{\pi_{j}}}{\sum\limits_{h=1}^{n}\dfrac{1}{\pi_{h}}}\sum\limits_{k=1}^{n}\dfrac{1}{\pi_{k}}\left\{ \sum\limits_{h=1}^{n}\dfrac{1}{\tilde{\pi}_{h}}-\left[n-\left(1-\rho\right)\right]\left[1+\dfrac{\dfrac{1}{\tilde{\pi}_{j}}-\dfrac{1}{\pi_{j}}}{\sum\limits_{h=1}^{n}\dfrac{1}{\pi_{h}}}\right]\dfrac{1}{\pi_{k}}\right\} -\sum\limits_{k=1}^{n}\dfrac{1}{\pi_{k}}\left\{ \left[n-\left(1-\rho\right)\right]\dfrac{\dfrac{1}{\tilde{\pi}_{j}}-\dfrac{1}{\pi_{j}}}{\sum\limits_{h=1}^{n}\dfrac{1}{\pi_{h}}}\dfrac{1}{\pi_{k}}\right\} \\
% %\Leftrightarrow & \dfrac{1}{\tilde{\pi}_{j}}\left[\sum\limits_{h=1}^{n}\dfrac{1}{\tilde{\pi}_{h}}-\left[n-\left(1-\rho\right)\right]\dfrac{1}{\tilde{\pi}_{j}}\right]<\dfrac{1}{\pi_{j}}\left[\sum\limits_{h=1}^{n}\dfrac{1}{\tilde{\pi}_{h}}-\left[n-\left(1-\rho\right)\right]\dfrac{1}{\pi_{j}}\right]+\\
%  %& +\dfrac{\dfrac{1}{\tilde{\pi}_{j}}-\dfrac{1}{\pi_{j}}}{\sum\limits_{h=1}^{n}\dfrac{1}{\pi_{h}}}\sum\limits_{k=1}^{n}\dfrac{1}{\pi_{k}}\left\{ \sum\limits_{h=1}^{n}\dfrac{1}{\tilde{\pi}_{h}}-\left[n-\left(1-\rho\right)\right]\left[1+\dfrac{\dfrac{1}{\tilde{\pi}_{j}}-\dfrac{1}{\pi_{j}}}{\sum\limits_{h=1}^{n}\dfrac{1}{\pi_{h}}}\right]\dfrac{1}{\pi_{k}}\right\} -\left[n-\left(1-\rho\right)\right]\dfrac{\dfrac{1}{\tilde{\pi}_{j}}-\dfrac{1}{\pi_{j}}}{\sum\limits_{h=1}^{n}\dfrac{1}{\pi_{h}}}\sum\limits_{k=1}^{n}\left(\dfrac{1}{\pi_{k}}\right)^{2}\\
% %\Leftrightarrow & \left(\dfrac{1}{\tilde{\pi}_{j}}-\dfrac{1}{\pi_{j}}\right)\sum\limits_{h=1}^{n}\dfrac{1}{\tilde{\pi}_{h}}-\left[n-\left(1-\rho\right)\right]\left[\left(\dfrac{1}{\tilde{\pi}_{j}}\right)^{2}-\left(\dfrac{1}{\pi_{j}}\right)^{2}\right]<\\
%  %& <\dfrac{\dfrac{1}{\tilde{\pi}_{j}}-\dfrac{1}{\pi_{j}}}{\sum\limits_{h=1}^{n}\dfrac{1}{\pi_{h}}}\sum\limits_{k=1}^{n}\dfrac{1}{\pi_{k}}\left\{ \sum\limits_{h=1}^{n}\dfrac{1}{\tilde{\pi}_{h}}-\left[n-\left(1-\rho\right)\right]\left[1+\dfrac{\dfrac{1}{\tilde{\pi}_{j}}-\dfrac{1}{\pi_{j}}}{\sum\limits_{h=1}^{n}\dfrac{1}{\pi_{h}}}\right]\dfrac{1}{\pi_{k}}\right\} -\left[n-\left(1-\rho\right)\right]\dfrac{\dfrac{1}{\tilde{\pi}_{j}}-\dfrac{1}{\pi_{j}}}{\sum\limits_{h=1}^{n}\dfrac{1}{\pi_{h}}}\sum\limits_{k=1}^{n}\left(\dfrac{1}{\pi_{k}}\right)^{2}\\
% %\Leftrightarrow & \sum\limits_{h=1}^{n}\dfrac{1}{\tilde{\pi}_{h}}-\left[n-\left(1-\rho\right)\right]\left(\dfrac{1}{\pi_{j}}+\dfrac{1}{\tilde{\pi}_{j}}\right){\color{blue}>}\\
% % & {\color{blue}>}\dfrac{1}{\sum\limits_{h=1}^{n}\dfrac{1}{\pi_{h}}}\sum\limits_{k=1}^{n}\dfrac{1}{\pi_{k}}\left\{ \sum\limits_{h=1}^{n}\dfrac{1}{\tilde{\pi}_{h}}-\left[n-\left(1-\rho\right)\right]\left[1+\dfrac{\dfrac{1}{\tilde{\pi}_{j}}-\dfrac{1}{\pi_{j}}}{\sum\limits_{h=1}^{n}\dfrac{1}{\pi_{h}}}\right]\dfrac{1}{\pi_{k}}\right\} -\left[n-\left(1-\rho\right)\right]\dfrac{\sum\limits_{k=1}^{n}\left(\dfrac{1}{\pi_{k}}\right)^{2}}{\sum\limits_{h=1}^{n}\dfrac{1}{\pi_{h}}}
% %\end{array}
% %\end{align}
% %\begin{align}
% %\begin{array}{cl}
% \Leftrightarrow & \sum\limits_{h=1}^{n}\dfrac{1}{\tilde{\pi}_{h}}-\left[n-\left(1-\rho\right)\right]\left(\dfrac{1}{\pi_{j}}+\dfrac{1}{\tilde{\pi}_{j}}\right)>\underbrace{\dfrac{\sum\limits_{k=1}^{n}\dfrac{1}{\pi_{k}}}{\sum\limits_{h=1}^{n}\dfrac{1}{\pi_{h}}}}_{=1}\sum\limits_{h=1}^{n}\dfrac{1}{\tilde{\pi}_{h}}-\dfrac{n-\left(1-\rho\right)}{\sum\limits_{h=1}^{n}\dfrac{1}{\pi_{h}}}\left[2+\dfrac{\dfrac{1}{\tilde{\pi}_{j}}-\dfrac{1}{\pi_{j}}}{\sum\limits_{h=1}^{n}\dfrac{1}{\pi_{h}}}\right]\sum\limits_{k=1}^{n}\left(\dfrac{1}{\pi_{k}}\right)^{2}\\
% %\Leftrightarrow & -\left[n-\left(1-\rho\right)\right]\left(\dfrac{1}{\pi_{j}}+\dfrac{1}{\tilde{\pi}_{j}}\right)>-\dfrac{n-\left(1-\rho\right)}{\sum\limits_{h=1}^{n}\dfrac{1}{\pi_{h}}}\left[2+\dfrac{\dfrac{1}{\tilde{\pi}_{j}}-\dfrac{1}{\pi_{j}}}{\sum\limits_{h=1}^{n}\dfrac{1}{\pi_{h}}}\right]\sum\limits_{k=1}^{n}\left(\dfrac{1}{\pi_{k}}\right)^{2}\\
% %\Leftrightarrow & \dfrac{1}{\pi_{j}}+\dfrac{1}{\tilde{\pi}_{j}}{\color{blue}<}\dfrac{1}{\sum\limits_{h=1}^{n}\dfrac{1}{\pi_{h}}}\left[2+\dfrac{\dfrac{1}{\tilde{\pi}_{j}}-\dfrac{1}{\pi_{j}}}{\sum\limits_{h=1}^{n}\dfrac{1}{\pi_{h}}}\right]\sum\limits_{k=1}^{n}\left(\dfrac{1}{\pi_{k}}\right)^{2}\\
% %\Leftrightarrow & 1+\dfrac{\pi_{j}}{\tilde{\pi}_{j}}<\dfrac{\sum\limits_{k=1}^{n}\left(\dfrac{\pi_{j}}{\pi_{k}}\right)^{2}}{\sum\limits_{h=1}^{n}\dfrac{\pi_{j}}{\pi_{h}}}\left(2+\dfrac{\dfrac{\pi_{j}}{\tilde{\pi}_{j}}-1}{\sum\limits_{h=1}^{n}\dfrac{\pi_{j}}{\pi_{h}}}\right)\\
% \Leftrightarrow & \tilde{\pi}_{j}+\pi_{j}<2\tilde{\pi}_{j}\dfrac{\sum\limits_{k=1}^{n}\left(\dfrac{\pi_{j}}{\pi_{k}}\right)^{2}}{\sum\limits_{h=1}^{n}\dfrac{\pi_{j}}{\pi_{h}}}-\left(\tilde{\pi}_{j}-\pi_{j}\right)\dfrac{\sum\limits_{k=1}^{n}\left(\dfrac{\pi_{j}}{\pi_{k}}\right)^{2}}{\left(\sum\limits_{h=1}^{n}\dfrac{\pi_{j}}{\pi_{h}}\right)^{2}}\\
% %\Leftrightarrow & \pi_{j}\left[1-\dfrac{\sum\limits_{k=1}^{n}\left(\dfrac{\pi_{j}}{\pi_{k}}\right)^{2}}{\left(\sum\limits_{h=1}^{n}\dfrac{\pi_{j}}{\pi_{h}}\right)^{2}}\right]<\tilde{\pi}_{j}\left[2\dfrac{\sum\limits_{k=1}^{n}\left(\dfrac{\pi_{j}}{\pi_{k}}\right)^{2}}{\sum\limits_{h=1}^{n}\dfrac{\pi_{j}}{\pi_{h}}}-\dfrac{\sum\limits_{k=1}^{n}\left(\dfrac{\pi_{j}}{\pi_{k}}\right)^{2}}{\left(\sum\limits_{h=1}^{n}\dfrac{\pi_{j}}{\pi_{h}}\right)^{2}}-1\right]\\
% \Leftrightarrow & \dfrac{\pi_{j}}{\tilde{\pi}_{j}}<\dfrac{2\dfrac{\sum\limits_{k=1}^{n}\left(\dfrac{\pi_{j}}{\pi_{k}}\right)^{2}}{\sum\limits_{h=1}^{n}\dfrac{\pi_{j}}{\pi_{h}}}-\dfrac{\sum\limits_{k=1}^{n}\left(\dfrac{\pi_{j}}{\pi_{k}}\right)^{2}}{\left(\sum\limits_{h=1}^{n}\dfrac{\pi_{j}}{\pi_{h}}\right)^{2}}-1}{1-\dfrac{\sum\limits_{k=1}^{n}\left(\dfrac{\pi_{j}}{\pi_{k}}\right)^{2}}{\left(\sum\limits_{h=1}^{n}\dfrac{\pi_{j}}{\pi_{h}}\right)^{2}}}
% \end{array}
% \end{align}
% It  suffices to show that the right hand side of the above inequality
% is greater than one
% \begin{align}
% \begin{array}{cl}
%  & 2\sum\limits_{k=1}^{n}\left(\dfrac{\pi_{j}}{\pi_{k}}\right)^{2}\left(\sum\limits_{h=1}^{n}\dfrac{\pi_{j}}{\pi_{h}}\right)-\sum\limits_{k=1}^{n}\left(\dfrac{\pi_{j}}{\pi_{k}}\right)^{2}-\left(\sum\limits_{h=1}^{n}\dfrac{\pi_{j}}{\pi_{h}}\right)^{2}>\left(\sum\limits_{h=1}^{n}\dfrac{\pi_{j}}{\pi_{h}}\right)^{2}-\sum\limits_{k=1}^{n}\left(\dfrac{\pi_{j}}{\pi_{k}}\right)^{2}\\
% %\Leftrightarrow & 2\sum\limits_{k=1}^{n}\left(\dfrac{\pi_{j}}{\pi_{k}}\right)^{2}\left(\sum\limits_{h=1}^{n}\dfrac{\pi_{j}}{\pi_{h}}\right)-\left(\sum\limits_{h=1}^{n}\dfrac{\pi_{j}}{\pi_{h}}\right)^{2}>\left(\sum\limits_{h=1}^{n}\dfrac{\pi_{j}}{\pi_{h}}\right)^{2}\\
% %\Leftrightarrow & \sum\limits_{k=1}^{n}\left(\dfrac{\pi_{j}}{\pi_{k}}\right)^{2}\left(\sum\limits_{h=1}^{n}\dfrac{\pi_{j}}{\pi_{h}}\right)>\left(\sum\limits_{h=1}^{n}\dfrac{\pi_{j}}{\pi_{h}}\right)^{2}\\
% %\Leftrightarrow & \sum\limits_{k=1}^{n}\left(\dfrac{\pi_{j}}{\pi_{k}}\right)^{2}\left(\sum\limits_{h=1}^{n}\dfrac{\pi_{j}}{\pi_{h}}\right)>\left(\sum\limits_{h=1}^{n}\dfrac{\pi_{j}}{\pi_{h}}\right)\left(\sum\limits_{h=1}^{n}\dfrac{\pi_{j}}{\pi_{h}}\right)\\
% \Leftrightarrow & \sum\limits_{h=1}^{n}\left(\dfrac{\pi_{j}}{\pi_{h}}\right)^{2}>\sum\limits_{h=1}^{n}\dfrac{\pi_{j}}{\pi_{h}}
% \end{array}
% \end{align}
% It is easy to prove that the last inequality is satisfied provided
% that $\pi_{j}\geq\dfrac{1}{n}\sum\limits_{k=1}^{n}\pi_{k}$. Note that
% \begin{align}
% \begin{array}{cl}
%  & \sum\limits_{h=1}^{n}\dfrac{\dfrac{1}{n}\sum\limits_{k=1}^{n}\pi_{k}}{\pi_{h}}\dfrac{\pi_{j}}{\pi_{h}}>\sum\limits_{h=1}^{n}\dfrac{\pi_{j}}{\pi_{h}}
% \Leftrightarrow  \left(\sum\limits_{h=1}^{n}\dfrac{\pi_{j}}{\pi_{h}}\right)+\left(\sum\limits_{h=1}^{n}\dfrac{\dfrac{1}{n}\sum_{k\neq h}^{n}\pi_{k}}{\pi_{h}}\dfrac{\pi_{j}}{\pi_{h}}\right)>\sum\limits_{h=1}^{n}\dfrac{\pi_{j}}{\pi_{h}}
% \end{array}
% \end{align}
% \end{proof}

% \vspace{1cm}

\subsubsection*{Proof of Proposition \ref{prop:MPS}}

\begin{proof}
a) Let $K^{*}_n$ be a steady-state where all industries are have $n$ firms and common productivity distribution $\Gamma_n$. Using equation (\ref{eq:factor_demand}), we can define $K^{*}_n$ as
\begin{align}
R^{*}\:=\:\alpha\:\left(1-\alpha\right)^{\left(1-\alpha\right)/\left(\nu+\alpha\right)}\:\Theta\left(\Gamma_n,n\right)^{\left(\nu+1\right)/\left(\nu+\alpha\right)}\:\left(K^{*}_n\right)^{-\nu\left(1-\alpha\right)/\left(\nu+\alpha\right)}
\end{align}
Recall from Lemma \ref{lemma:MPS_theta} that $\Theta\left(\Gamma_n,n\right)$ declines after a MPS on $\Gamma_n$. Then $K^{*}_n$ must also decline.

b)
We provide a sufficient condition under which the unstable steady-state increases after an MPS. Note that the unstable steady-state increases whenever the increasing segment of the rental rate map lies strictly underneath the original one.

We know from the proof of Proposition \ref{prop:MPS}.a that the new rental rate at $\underline{K}\left(2\right)$ is strictly lower than before. The proof involves two steps

[A] We derive a sufficient condition under which the new rental rate at $\overline{K}\left(1\right)$ is lower than before

[B] We show that the increasing segment of the rental rate map after an MPS cannot cross the previous one more than once. Thus, if the new segment starts and ends below the previous one, it can never go above it.

\subsubsection*{Proof of Part A}

The free entry condition is
\begin{align}
\Lambda\left(n\right)\Theta\left(n-1\right)^{-\frac{\rho}{1-\rho}}\:\Phi\left(n-1\right)K^{\alpha}\:L^{1-\alpha}\;=\;c_{f}
\end{align}
Using
\begin{align}
L=\left[\left(1-\alpha\right)\Theta\left(n-1\right)\right]^{\frac{1}{\nu+\alpha}}K^{\frac{\alpha}{\nu+\alpha}}
\end{align}
we can rewrite the free-entry condition as
\begin{align}\nonumber
 & \Lambda\left(n\right)\Theta\left(n-1\right)^{-\frac{\rho}{1-\rho}}\:\Phi\left(n-1\right)\;K^{\alpha}\:\left[\left(1-\alpha\right)\Theta\left(n-1\right)\right]^{\frac{1-\alpha}{\nu+\alpha}}K^{\alpha\frac{1-\alpha}{\nu+\alpha}}\;=\;c_{f}\\\nonumber
\Leftrightarrow & \Lambda\left(n\right)\Theta\left(n-1\right)^{-\frac{\rho}{1-\rho}}\:\Phi\left(n-1\right)\left[\left(1-\alpha\right)\Theta\left(n-1\right)\right]^{\frac{1-\alpha}{\nu+\alpha}}K^{\alpha\frac{\nu+1}{\nu+\alpha}}\;=\;c_{f}\\
\Leftrightarrow & K\;=\;\left[\dfrac{c_{f}\left(1-\alpha\right)^{-\frac{1-\alpha}{\nu+\alpha}}}{\Lambda\left(n\right)\Theta\left(n-1\right)^{\frac{1-\alpha}{\nu+\alpha}-\frac{\rho}{1-\rho}}\:\Phi\left(n-1\right)}\right]^{\frac{1}{\alpha}\frac{\nu+\alpha}{\nu+1}}
\end{align}
The interest rate is
\begin{align}\nonumber
R= & \alpha\:\Theta\left(n-1\right)\:K^{\alpha-1}\:L^{1-\alpha}\\\nonumber
= & \alpha\:\Theta\left(n-1\right)\:K^{\alpha-1}\:\left[\left(1-\alpha\right)\Theta\left(n-1\right)\right]^{\frac{1-\alpha}{\nu+\alpha}}K^{\alpha\frac{1-\alpha}{\nu+\alpha}}\\
= & \alpha\:\left(1-\alpha\right)^{\frac{1-\alpha}{\nu+\alpha}}\:\Theta\left(\mathbf{\Gamma},\mathbf{N}_{t}\right)^{\frac{\nu+1}{\nu+\alpha}}\:K^{\nu\frac{\alpha-1}{\nu+\alpha}}
\end{align}
Putting the two together
\begin{equation}
R=\alpha\:\left(1-\alpha\right)^{\frac{1-\alpha}{\nu+\alpha}}\:\Theta\left(n-1\right)^{\frac{\nu+1}{\nu+\alpha}}\:\left(\dfrac{\Lambda\left(n\right)\Theta\left(n-1\right)^{\frac{1-\alpha}{\nu+\alpha}-\frac{\rho}{1-\rho}}\:\Phi\left(n-1\right)}{c_{f}\left(1-\alpha\right)^{-\frac{1-\alpha}{\nu+\alpha}}}\right)^{\frac{\nu}{\nu+1}\frac{1-\alpha}{\alpha}}\label{eq:R_1}
\end{equation}
implying
\begin{align}
R^{\frac{\nu+1}{\nu}\frac{\alpha}{1-\alpha}}=\propto\:\Theta\left(n-1\right)^{\frac{\nu+1}{\nu}\frac{\alpha}{1-\alpha}\frac{\nu+1}{\nu+\alpha}}\:\Lambda\left(n\right)\Theta\left(n-1\right)^{\frac{1-\alpha}{\nu+\alpha}-\frac{\rho}{1-\rho}}\:\Phi\left(n-1\right)
\end{align}
where
\begin{align}
\Theta\left(n\right)= & g\left(n\right)\\
\Phi\left(n\right)= & \dfrac{1}{\sum\limits _{j=1}^{n}\dfrac{s_{j}}{\pi_{j}}}\\
\Lambda\left(n\right)= & s_{n}^{2}\left[g\left(n\right)\right]^{\frac{\rho}{1-\rho}}
\end{align}
We can thus rewrite (\ref{eq:R_1}) as
\begin{equation}
R^{\frac{\nu+1}{\nu}\frac{\alpha}{1-\alpha}}=g\left(n-1\right)^{\frac{\nu+1}{\nu}\frac{\alpha}{1-\alpha}\frac{\nu+1}{\nu+\alpha}+\frac{1-\alpha}{\nu+\alpha}}\:\dfrac{s_{n}^{2}\left[\dfrac{g\left(n\right)}{g\left(n-1\right)}\right]^{\frac{\rho}{1-\rho}}}{\sum\limits _{j=1}^{n-1}\dfrac{\hat{s}_{j}}{\pi_{j}}}\label{eq:R_2}
\end{equation}
where $\hat{s}_{j}$ is the market share of firm $j$ in an industry
with $n-1$ firms and $s_{j}$ is the market share of that firm when
there are $n$ player in the industry. We want to show that the expression
in (\ref{eq:R_2}) goes down when we do an MPS on $n$ firms. The
challenge is in the fact that the expression involves terms that refer
to $n-1$ industries.

Under $n=2$, we have
\begin{align}
g\left(1\right)= & \rho\,\pi_{1}\\
g\left(2\right)= & \dfrac{1+\rho}{\dfrac{1}{\pi_{1}}+\dfrac{1}{\pi_{2}}}
\end{align}
so that
\begin{align}\nonumber
R^{\frac{\alpha}{1-\alpha}}= & \left(\rho\,\pi_{1}\right)^{\frac{\nu+1}{\nu}\frac{\alpha}{1-\alpha}\frac{\nu+1}{\nu+\alpha}+\frac{1-\alpha}{\nu+\alpha}-\frac{\rho}{1-\rho}}\:\left(\dfrac{1+\rho}{\dfrac{1}{\pi_{1}}+\dfrac{1}{\pi_{2}}}\right)^{\frac{\rho}{1-\rho}}\dfrac{\left[1-\dfrac{1+\rho}{\dfrac{1}{\pi_{1}}+\dfrac{1}{\pi_{2}}}\dfrac{1}{\pi_{2}}\right]^{2}}{\dfrac{1}{\pi_{1}}}\\
%= & \propto\:\pi_{1}^{\frac{\nu+1}{\nu}\frac{\alpha}{1-\alpha}\frac{\nu+1}{\nu+\alpha}+\frac{1-\alpha}{\nu+\alpha}-\frac{\rho}{1-\rho}}\:\pi_{1}\left[1-\dfrac{1+\rho}{\dfrac{1}{\pi_{1}}+\dfrac{1}{\pi_{2}}}\dfrac{1}{\pi_{2}}\right]^{2}\left[\dfrac{1+\rho}{\dfrac{1}{\pi_{1}}+\dfrac{1}{\pi_{2}}}\right]^{\frac{\rho}{1-\rho}}\\
%= & \propto\pi_{1}^{\frac{\nu+1}{\nu}\frac{\alpha}{1-\alpha}\frac{\nu+1}{\nu+\alpha}+\frac{1-\alpha}{\nu+\alpha}-\frac{\rho}{1-\rho}}\:\dfrac{\pi_{1}^{2}}{\pi_{1}}\left[1-\dfrac{1+\rho}{\dfrac{\pi_{2}}{\pi_{1}}+1}\right]^{2}\left[\dfrac{1+\rho}{\dfrac{1}{\pi_{1}}+\dfrac{1}{\pi_{2}}}\right]^{\frac{\rho}{1-\rho}}\\
%= & \propto\pi_{1}^{\frac{\nu+1}{\nu}\frac{\alpha}{1-\alpha}\frac{\nu+1}{\nu+\alpha}+\frac{1-\alpha}{\nu+\alpha}-\frac{\rho}{1-\rho}-1}\:\left[\pi_{1}-\pi_{1}\dfrac{1+\rho}{\dfrac{\pi_{2}}{\pi_{1}}+1}\right]^{2}\left[\dfrac{1+\rho}{\dfrac{1}{\pi_{1}}+\dfrac{1}{\pi_{2}}}\right]^{\frac{\rho}{1-\rho}}\\
%= & \propto\pi_{1}^{\frac{\nu+1}{\nu}\frac{\alpha}{1-\alpha}\frac{\nu+1}{\nu+\alpha}+\frac{1-\alpha}{\nu+\alpha}-\frac{\rho}{1-\rho}-1}\:\left[\pi_{1}-\pi_{1}\dfrac{1+\rho}{\dfrac{2x-\pi_{1}}{\pi_{1}}+1}\right]^{2}\left[\dfrac{1+\rho}{\dfrac{1}{\pi_{1}}+\dfrac{1}{\pi_{2}}}\right]^{\frac{\rho}{1-\rho}}\\
= & \propto\pi_{1}^{\frac{\nu+1}{\nu}\frac{\alpha}{1-\alpha}\frac{\nu+1}{\nu+\alpha}+\frac{1-\alpha}{\nu+\alpha}-\frac{\rho}{1-\rho}-1}\:\left[\pi_{1}-\pi_{1}\dfrac{1+\rho}{\dfrac{2x}{\pi_{1}}}\right]^{2}\left[\dfrac{1+\rho}{\dfrac{1}{\pi_{1}}+\dfrac{1}{2x-\pi_{1}}}\right]^{\frac{\rho}{1-\rho}}
\end{align}
The last term is decreasing on an MPS, since it is simply $g\left(2\right)$.
The first term is decreasing on an MPS provided that
\begin{align}
1+\dfrac{\rho}{1-\rho}>\dfrac{\nu+1}{\nu}\dfrac{\alpha}{1-\alpha}\dfrac{\nu+1}{\nu+\alpha}+\dfrac{1-\alpha}{\nu+\alpha}
%\Leftrightarrow & \dfrac{1}{1-\rho}>\dfrac{\alpha\left(\nu+1\right)^{2}+\left(1-\alpha\right)^{2}\nu}{\nu\left(1-\alpha\right)\left(\nu+\alpha\right)}\\
%\Leftrightarrow & \dfrac{1}{1-\rho}>\dfrac{\alpha\left(\nu+1\right)^{2}+\left(1-\alpha\right)^{2}\nu}{\nu\left(1-\alpha\right)\left(\nu+\alpha\right)}\\
%\Leftrightarrow & \rho>1-\dfrac{\nu\left(1-\alpha\right)\left(\nu+\alpha\right)}{\alpha\left(\nu+1\right)^{2}+\left(1-\alpha\right)^{2}\nu}\\
%\Leftrightarrow & \rho>1-\nu\dfrac{1-\alpha}{1+\nu\alpha}\\
\Leftrightarrow  \alpha<\dfrac{\nu+\rho-1}{\nu\left(2-\rho\right)}
\end{align}
since this MPS must result in higher $\pi_{1}$. We just need to evaluate
the term in the middle. Note that we can rewrite it as
\begin{align}
\pi_{1}-\pi_{1}^{2}\dfrac{1+\rho}{2x}
\end{align}
where $2x\equiv\pi_{1}+\pi_{2}$ is fixed by construction. The derivative
of the expression above is
\begin{align}
\dfrac{\partial}{\partial\pi_{1}}= & 1-2\pi_{1}\dfrac{1+\rho}{2x}\\
= & 1-\underbrace{\dfrac{\pi_{1}}{x}}_{>1}\left(1+\rho\right)<0
\end{align}
Therefore, for $n=2$, the interest rate is always declining on an
MPS provided that
\begin{align}
\rho>1-\nu\dfrac{1-\alpha}{1+\nu\alpha}
\end{align}

\subsubsection*{Proof of Part B}
Recall that the free entry condition is
\begin{align}
\Lambda_{j}\Theta^{-\frac{\rho}{1-\rho}}\:\Phi\:K^{\alpha}\:L^{1-\alpha}=c_{f}
\end{align}

Aggregate TFP can be written as
\hspace{-5cm}
\begin{align*}
\Phi= & \dfrac{\left\{ \left(1-m\right)\left[g\left(n-1\right)\right]^{\frac{\rho}{1-\rho}}+m\left[g\left(n\right)\right]^{\frac{\rho}{1-\rho}}\right\} ^{\frac{1}{\rho}}}{\left(1-m\right)\left[g\left(n-1\right)\right]^{\frac{1}{1-\rho}}h\left(n-1\right)+m\left[g\left(n\right)\right]^{\frac{1}{1-\rho}}h\left(n\right)} \\
& = \dfrac{\Theta^{\frac{1}{1-\rho}}}{\left(1-m\right)\left[g\left(n-1\right)\right]^{\frac{1}{1-\rho}}h\left(n-1\right)+m\left[g\left(n\right)\right]^{\frac{1}{1-\rho}}h\left(n\right)}
\end{align*}
where
\begin{align}
g\left(n\right)= & \dfrac{n-\left(1-\rho\right)}{\sum\limits _{j=1}^{n}\dfrac{1}{\pi_{j}}}\\
h\left(n\right)= & \sum\limits _{j=1}^{n}\dfrac{s_{j}}{\pi_{j}}
\end{align}
Now suppose that we do the MPS and have $\tilde{\Theta}=\Theta$ at
the same $K$.\footnote{We also have $\tilde{L}=L$, since $L$ is a function of $\Theta$
and $K$.} From the free entry condition and the expression for $\Phi$, this
is possible if
\begin{align}\nonumber
 & \dfrac{\Lambda_{j}}{\tilde{\Lambda}_{j}}=\dfrac{\left(1-{\color{red}m}\right)\left[g\left(n-1\right)\right]^{\frac{1}{1-\rho}}h\left(n-1\right)+{\color{red}m}\left[g\left(n\right)\right]^{\frac{1}{1-\rho}}h\left(n\right)}{\left(1-{\color{red}\tilde{m}}\right)\left[\tilde{g}\left(n-1\right)\right]^{\frac{1}{1-\rho}}\tilde{h}\left(n-1\right)+{\color{red}\tilde{m}}\left[\tilde{g}\left(n\right)\right]^{\frac{1}{1-\rho}}\tilde{h}\left(n\right)}\\
\Leftrightarrow & \dfrac{\Lambda_{j}}{\tilde{\Lambda}_{j}}=\dfrac{\left[g\left(n-1\right)\right]^{\frac{1}{1-\rho}}h\left(n-1\right)+{\color{red}m}\left\{ \left[g\left(n\right)\right]^{\frac{1}{1-\rho}}h\left(n\right)-\left[g\left(n-1\right)\right]^{\frac{1}{1-\rho}}h\left(n-1\right)\right\} }{\left[\tilde{g}\left(n-1\right)\right]^{\frac{1}{1-\rho}}\tilde{h}\left(n-1\right)+{\color{red}\tilde{m}}\left\{ \left[\tilde{g}\left(n\right)\right]^{\frac{1}{1-\rho}}\tilde{h}\left(n\right)-\left[\tilde{g}\left(n-1\right)\right]^{\frac{1}{1-\rho}}\tilde{h}\left(n-1\right)\right\} }
\end{align}
Rearranging this equation, we can write
\begin{equation}
\tilde{m}=a_{1}+b_{1}\cdot m\label{eq:eq_1}
\end{equation}
where $a_{1}$ and $b_{1}$ are some numbers (independent of $K$).

Furthermore, from $\tilde{\Theta}=\Theta$ we have
\begin{align}\nonumber
 & \left(1-{\color{red}m}\right)\left[g\left(n-1\right)\right]^{\frac{\rho}{1-\rho}}+{\color{red}m}\left[g\left(n\right)\right]^{\frac{\rho}{1-\rho}}=\left(1-{\color{red}\tilde{m}}\right)\left[\tilde{g}\left(n-1\right)\right]^{\frac{\rho}{1-\rho}}+{\color{red}\tilde{m}}\left[\tilde{g}\left(n\right)\right]^{\frac{\rho}{1-\rho}}\\
\Leftrightarrow & \left[g\left(n-1\right)\right]^{\frac{\rho}{1-\rho}}+{\color{red}m}\left\{ \left[g\left(n\right)\right]^{\frac{\rho}{1-\rho}}-\left[g\left(n-1\right)\right]^{\frac{\rho}{1-\rho}}\right\} =\left[\tilde{g}\left(n-1\right)\right]^{\frac{\rho}{1-\rho}}+{\color{red}\tilde{m}}\left\{ \left[\tilde{g}\left(n\right)\right]^{\frac{\rho}{1-\rho}}-\left[\tilde{g}\left(n-1\right)\right]^{\frac{\rho}{1-\rho}}\right\} 
\end{align}
Rearranging this equation, we can write
\begin{equation}
\tilde{m}=a_{2}+b_{2}\cdot m\label{eq:eq_2}
\end{equation}
Combining (\ref{eq:eq_1}) and (\ref{eq:eq_2}), there is at most
one pair $\left(m,\tilde{m}\right)$ such that $\tilde{\Theta}=\Theta$.
This establishes that $\tilde{\Theta}$ cannot cross $\Theta$ twice.
\end{proof}


\begin{prop}[Mean Preserving Spread and Fragility, general $n$] \label{prop:MPS_BA_n}

Let $\eta = 1$ and suppose that all industries are identical to start ($\gamma_{ij} = \gamma_{j} \; \forall i$). Let ${K}^{*}\left(n\right)$ be a steady-state with $n$ firms. Let $\lambda$ be a mean-preserving spread on the distribution $\left\{\gamma_1,\ldots,\gamma_n\right\}$ of active firms, such that for any $j=1,\ldots,n-1$, $\gamma_{1}/\gamma_{j}$ is unchanged. Then, if
\begin{align}
\rho>\dfrac{1+\nu\alpha}{1+\nu}\end{align}
we have that
\begin{align} \dfrac{\partial \underline{B}\left(n\right)}{\partial\lambda} > 0. \end{align}
\end{prop}

\begin{proof}[Proof of Proposition \ref{prop:MPS_BA_n}]

Let us now provide a sufficient condition for general $n$. First
note that we can write (\ref{eq:R_2}) as
\begin{align}
R^{\frac{\nu+1}{\nu}\frac{\alpha}{1-\alpha}}=\underbrace{g\left(n-1\right)^{\frac{\nu+1}{\nu}\frac{\alpha}{1-\alpha}\frac{\nu+1}{\nu+\alpha}+\frac{1-\alpha}{\nu+\alpha}-\frac{\rho}{1-\rho}}g\left(n\right)^{\frac{\rho}{1-\rho}}}_{v}\underbrace{\dfrac{1}{\sum\limits _{j=1}^{n-1}\dfrac{\hat{s}_{j}}{\pi_{j}}}s_{n}^{2}}_{z}
\end{align}
\begin{align}
R^{\frac{\alpha}{1-\alpha}}=\underbrace{g\left(n-1\right)^{\frac{\alpha}{1-\alpha}-\frac{\rho}{1-\rho}}g\left(n\right)^{\frac{\rho}{1-\rho}}}_{v}\underbrace{\dfrac{1}{\sum\limits _{j=1}^{n-1}\dfrac{\hat{s}_{j}}{\pi_{j}}}s_{n}^{2}}_{z}
\end{align}
The first term $v$ is always decreasing on an MPS provided that

\begin{align}
 \dfrac{\rho}{1-\rho}>\dfrac{\nu+1}{\nu}\dfrac{\alpha}{1-\alpha}\dfrac{\nu+1}{\nu+\alpha}+\dfrac{1-\alpha}{\nu+\alpha}
%\Leftrightarrow & \dfrac{\nu\left(1-\alpha\right)\left(\nu+\alpha\right)}{\alpha\left(\nu+1\right)^{2}+\left(1-\alpha\right)^{2}\nu}>\dfrac{1-\rho}{\rho}\\
%\Leftrightarrow & \dfrac{\nu\left(1-\alpha\right)\left(\nu+\alpha\right)}{\alpha\left(\nu+1\right)^{2}+\left(1-\alpha\right)^{2}\nu}>\dfrac{1}{\rho}-1\\
%\Leftrightarrow & \dfrac{1}{\rho}<\nu\dfrac{1-\alpha}{1+\nu\alpha}+1\\
%\Leftrightarrow & \rho>\dfrac{1+\nu\alpha}{1+\nu}\\
\Leftrightarrow  \alpha<\dfrac{\rho\left(1+\nu\right)-1}{\nu}
\end{align}
To see it note that $g\left(n\right)$ is decreasing on an MPS. If
$g\left(n-1\right)$ is increasing on an MPS, it immediately follows
that $v$ decreases on an MPS when the above condition is satisfied.
If $g\left(n-1\right)$ is instead decreasing on an MPS, just rewrite
$v$ as
\begin{align}
v=g\left(n-1\right)^{\frac{\nu+1}{\nu}\frac{\alpha}{1-\alpha}\frac{\nu+1}{\nu+\alpha}+\frac{1-\alpha}{\nu+\alpha}}\left[\dfrac{g\left(n\right)}{g\left(n-1\right)}\right]^{\frac{\rho}{1-\rho}}
\end{align}

and note that $\dfrac{g\left(n\right)}{g\left(n-1\right)}$ decreases
on an MPS.

Thus, all we need to show is that $z$ is also decreasing on an MPS.
Note that we can write $z$ as
\begin{align}
z=\dfrac{s_{n}^{2}}{\sum\limits _{j=1}^{n-1}\dfrac{\hat{s}_{j}}{\pi_{j}}}=\dfrac{1}{\sum\limits _{j=1}^{n-1}\dfrac{\hat{s}_{j}}{\pi_{j}}\dfrac{1}{s_{n}^{2}}}
\end{align}
We know that $s_{n}$ is decreasing on an MPS. A sufficient condition
for $z$ to be decreasing on an MPS is that
\begin{align}
\dfrac{\hat{s}_{j}}{\pi_{j}}\dfrac{1}{s_{n}^{2}}
\end{align}
is increasing on an MPS for every $j=1,2,\ldots,n-1$.

Consider an MPS such that
\begin{align}
\widetilde{\pi}_{j}=\gamma\,\pi_{j}\quad\forall j=1,2,\ldots,n-1
\end{align}
and 
\begin{align}
 & \gamma\sum\limits _{j=1}^{n-1}\pi_{j}+\widetilde{\pi}_{n}=\sum\limits _{j=1}^{n-1}\pi_{j}+\pi_{n}\\
\Leftrightarrow & \widetilde{\pi}_{n}=\pi_{n}-\left(\gamma-1\right)\sum\limits _{j=1}^{n-1}\pi_{j}
\end{align}
In this case we have
\begin{align}
\dfrac{1}{\gamma}\underbrace{\dfrac{\hat{s}_{j}}{\pi_{j}}}_{\text{const}}\dfrac{1}{\widetilde{s}_{n}^{2}}
\end{align}
We need to show that 
\begin{align}
\gamma\underbrace{\left[1-\dfrac{n-\left(1-\rho\right)}{\sum\limits _{j=1}^{n-1}\dfrac{1}{\gamma\pi_{j}}+1}\dfrac{1}{\pi_{n}-\left(\gamma-1\right)\sum\limits _{j=1}^{n-1}\pi_{j}}\right]^{2}}_{\widetilde{s}_{n}}
\end{align}
decreases in $\gamma$. Note that we can rewrite it as
\begin{align}
 \gamma\underbrace{\left[1-\dfrac{n-\left(1-\rho\right)}{\sum\limits _{j=1}^{n-1}\dfrac{\pi_{n}-\left(\gamma-1\right)\sum\limits _{j=1}^{n-1}\pi_{j}}{\gamma\,\pi_{j}}+1}\right]^{2}}_{\tilde{s}_{n}}
%= & \gamma\underbrace{\left[1-\dfrac{n-\left(1-\rho\right)}{\dfrac{\pi_{n}-\left(\gamma-1\right)\sum\limits _{j=1}^{n-1}\pi_{j}}{\gamma}\sum\limits _{j=1}^{n-1}\dfrac{1}{\pi_{j}}+1}\right]^{2}}_{\tilde{s}_{n}}\\
%= & \gamma\underbrace{\left[1-\dfrac{n-\left(1-\rho\right)}{\left[\dfrac{\pi_{n}}{\gamma}-\left(1-\dfrac{1}{\gamma}\right)\sum\limits _{j=1}^{n-1}\pi_{j}\right]\sum\limits _{j=1}^{n-1}\dfrac{1}{\pi_{j}}+1}\right]^{2}}_{\tilde{s}_{n}}\\
= \gamma\underbrace{\left[1-\dfrac{n-\left(1-\rho\right)}{\left[\dfrac{1}{\gamma}\left(\pi_{n}+\sum\limits _{j=1}^{n-1}\pi_{j}\right)-\sum\limits _{j=1}^{n-1}\pi_{j}\right]\sum\limits _{j=1}^{n-1}\dfrac{1}{\pi_{j}}+1}\right]^{2}}_{\tilde{s}_{n}}
\end{align}
The derivative with respect to $\gamma$ is
\begin{align}
\tilde{s}_{n}^{2}+\gamma2\tilde{s}_{n}\left\{ -\left(-1\right)\left[n-\left(1-\rho\right)\right]\dfrac{\left(\pi_{n}+\sum\limits _{j=1}^{n-1}\pi_{j}\right)\sum\limits _{j=1}^{n-1}\dfrac{1}{\pi_{j}}\left(-\dfrac{1}{\gamma^{2}}\right)}{\left(\left[\dfrac{1}{\gamma}\left(\pi_{n}+\sum\limits _{j=1}^{n-1}\pi_{j}\right)-\sum\limits _{j=1}^{n-1}\pi_{j}\right]\sum\limits _{j=1}^{n-1}\dfrac{1}{\pi_{j}}+1\right)^{2}}\right\} 
\end{align}
which is lower than zero if
\begin{align}
 & \tilde{s}_{n}-\dfrac{2}{\gamma}\left[\dfrac{n-\left(1-\rho\right)}{\sum\limits _{j=1}^{n}\dfrac{\tilde{\pi}_{n}}{\gamma\pi_{j}}}\dfrac{1}{\sum\limits _{j=1}^{n}\dfrac{\tilde{\pi}_{n}}{\gamma\pi_{j}}}\left(\pi_{n}+\sum\limits _{j=1}^{n-1}\pi_{j}\right)\sum\limits _{j=1}^{n-1}\dfrac{1}{\pi_{j}}\right]<0
%\Leftrightarrow & 1-\dfrac{n-\left(1-\rho\right)}{\sum\limits _{j=1}^{n}\dfrac{\tilde{\pi}_{n}}{\pi_{j}}}-2\gamma\left[\dfrac{n-\left(1-\rho\right)}{\sum\limits _{j=1}^{n}\dfrac{\tilde{\pi}_{n}}{\pi_{j}}}\dfrac{1}{\sum\limits _{j=1}^{n}\dfrac{\tilde{\pi}_{n}}{\pi_{j}}}\left(\sum\limits _{j=1}^{n}\pi_{j}\right)\sum\limits _{j=1}^{n-1}\dfrac{1}{\pi_{j}}\right]<0\\
\Leftrightarrow  1-\underbrace{\dfrac{n-\left(1-\rho\right)}{\sum\limits _{j=1}^{n}\dfrac{\tilde{\pi}_{n}}{\pi_{j}}}}_{\left(a\right)}\left[1+2\gamma\underbrace{\dfrac{\sum\limits _{j=1}^{n}\pi_{j}}{\tilde{\pi}_{n}}}_{>n}\underbrace{\dfrac{\sum\limits _{j=1}^{n-1}\dfrac{1}{\pi_{j}}}{\sum\limits _{j=1}^{n}\dfrac{1}{\pi_{j}}}}_{\left(b\right)}\right]<0
\end{align}

If suffices to prove that $\left(a\right)>1/3$ and that $\left(b\right)>1/n$.

To prove the first, note that
\begin{align}
\tilde{s}_{n}=\dfrac{1}{1-\rho}\left[1-\dfrac{n-\left(1-\rho\right)}{\sum\limits _{j=1}^{n}\dfrac{\tilde{\pi}_{n}}{\pi_{j}}}\right]<\dfrac{1}{3}
%\Leftrightarrow & 1-\dfrac{n-\left(1-\rho\right)}{\sum\limits _{j=1}^{n}\dfrac{\tilde{\pi}_{n}}{\pi_{j}}}<\dfrac{1-\rho}{3}\\
%\Leftrightarrow & \dfrac{3-1+\rho}{3}<\dfrac{n-\left(1-\rho\right)}{\sum\limits _{j=1}^{n}\dfrac{\tilde{\pi}_{n}}{\pi_{j}}}\\
\Leftrightarrow  \underbrace{\dfrac{n-\left(1-\rho\right)}{\sum\limits _{j=1}^{n}\dfrac{\tilde{\pi}_{n}}{\pi_{j}}}}_{\left(a\right)}>\dfrac{2+\rho}{3}>\dfrac{1}{3}
\end{align}
To prove the second, note that
%
\begin{align}
 \dfrac{\sum\limits _{j=1}^{n-1}\dfrac{1}{\pi_{j}}}{\sum\limits _{j=1}^{n}\dfrac{1}{\pi_{j}}}>\dfrac{1}{n}
%\Leftrightarrow & n\sum\limits _{j=1}^{n-1}\dfrac{1}{\pi_{j}}>\sum\limits _{j=1}^{n}\dfrac{1}{\pi_{j}}\\
%\Leftrightarrow & n\left(\sum\limits _{j=1}^{n}\dfrac{1}{\pi_{j}}-\dfrac{1}{\pi_{n}}\right)>\sum\limits _{j=1}^{n}\dfrac{1}{\pi_{j}}\\
%\Leftrightarrow & \left(n-1\right)\sum\limits _{j=1}^{n}\dfrac{1}{\pi_{j}}>n\dfrac{1}{\pi_{n}}\\
\Leftrightarrow  \sum\limits _{j=1}^{n}\dfrac{\pi_{n}}{\pi_{j}}>\dfrac{n}{n-1}
\end{align}
%
The last equation is implied by the fact that
\begin{align}
  1-\dfrac{n-\left(1-\rho\right)}{\sum\limits _{j=1}^{n}\dfrac{\pi_{n}}{\pi_{j}}}>0 \Leftrightarrow  \sum\limits _{j=1}^{n}\dfrac{\pi_{n}}{\pi_{j}}>\underbrace{n-\left(1-\rho\right)}_{>2\;\text{under}\;n\geq3}
\end{align}
which is needed for $s_{n}>0$. This completes the proof.
\end{proof}

\subsubsection*{Proof of Proposition \ref{prop:basin_attraction_cf}}

\begin{proof}

% In a steady-state with identical industries and $n$ firms per industry we have that
% \begin{align}
% \begin{array}{rl}
% R^{*}= & \alpha\left(1-\alpha\right)^{\frac{1-\alpha}{\nu+\alpha}}\;\left[\Theta\left(n\right)\right]^{\frac{1+\nu}{\nu+\alpha}}\;\left[K^{*}\left(n\right)\right]^{\left(1-\alpha\right)\frac{-\nu}{\nu+\alpha}}\\
% R^{*}= & \beta^{-1}+\left(1-\delta\right)
% \end{array}
% \end{align}
% The first equation describes capital demand by fimrs, whereas the second evaluates the Euler equation (in a steady-state).
% $K^{*}\left(n\right)$ is therefore independent of $c_f$ \textendash{} provided that all $n$ make strictly positive profits, a marginal increase in $c_f$ will not drive any of them out of the market.

% Note furthermore that $\underline{K}\left(n\right)$ is increasing in $n$ (Appendix \ref{subsec:numb-active-firms}).
% \begin{align}
% \underline{K}\left(n\right) = \left\{ \dfrac{c} {\varLambda\left(n,n\right)} \left(1-\alpha\right)^{-\frac{1-\alpha}{\nu+\alpha}}\left[\Phi\left(n\right)\right]^{-1}\left[\Theta\left(n\right)\right]^{\frac{\rho}{1-\rho}-\frac{1-\alpha}{\nu+\alpha}}\right\} ^{\frac{\nu+\alpha}{\alpha\left(1+\nu\right)}} 
% \end{align}

From equation (\ref{eq:factor_demand}) we can write
\begin{align}
R_{t}\:=\:\alpha\:\left(1-\alpha\right)^{\left(1-\alpha\right)/\left(\nu+\alpha\right)}\:\Theta\left(\mathbf{\Gamma},\mathbf{N}_{t}\right)^{\left(\nu+1\right)/\left(\nu+\alpha\right)}\:K_{t}^{-\nu\left(1-\alpha\right)/\left(\nu+\alpha\right)}
\end{align}
where $\Theta \left(\mathbf{\Gamma}, \mathbf{N}_{t}\right) $ is increasing in the number of active firms (as explained above). For a given steady-state $K^*$, the slackness free entry condition may or may not hold exactly. If it does hold exactly then, in response to a marginal increase in $c$, the number of firms will necessarily decrease and so will the level of capital at the steady-state. If it does not hold exactly then the level of capital will be unchanged as no firm will leave the market. The statement of part a) follows.

Second, at an unstable steady-state $K_{U}$, the rental rate is increasing in the capital stock. For this to happen, $\Theta\left(\mathbf{\Gamma}, \mathbf{N}_{t}\right)$ must be increasing in $K$ at that point. Assuming $I$ large, this only happens if some firm is exactly breaking even. Therefore, the rental rate at an unstable steady-state $K_{U}$ necessarily declines after an increase in $c$, as stated in part b).




\end{proof}


==> submitted_version/section_2_new.tex <==
\section{General Framework}\label{sec: general framework text}
In this section we introduce the concept of macroeconomic fragility. We do so in the context of a general economy, featuring a representative household, endogenous factor supply, and a large number of product markets (characterized by an endogenous number of firms, variable markups and love-for-variety).
We proceed by first describing the economy. We then define macroeconomic fragility and study how it changes with firm-level heterogeneity. In Section \ref{sec:Model} we impose additional structure to this general framework, by developing an RBC model with oligopolistic competition.  This allows us to derive sharper predictions and analytical results.

\subsection{Primitives}\label{general_description}
\paragraph{Demographics}
The economy contains an infinitely-lived representative household, who has time separable utility $U = \sum_{t=0}^{\infty} \beta^{t}u\left(C_{t},L_{t}\right)$.  The household can save by investing in capital, which depreciates at rate $\delta$. The household earns rental and wage rates $R_{t}$ and $w_{t}$, determined in competitive factor markets.
\paragraph{Technology}
There is a final good (used for consumption and investment), which is given by a homothetic aggregator of different products or varieties.
The economy contains $I \in \mathbb{N}^{+}$ different categories of products. Within each category, there is a measure one of markets. For example, one possible product category is restaurants, within which there are many different geographic locations in which restaurants compete. %The economy contains a continuum of markets where each product category can be produced and consumed (e.g. one in every geographical location).
We think of goods sold in different markets as different products which enter the final good aggregator.\footnote{We adopt this formulation only for tractability reasons, to make the aggregate number of firms a continuously differentiable variable, in spite of the existence of a finite number of different types of markets $I$.}
All product markets are characterized by the same maximum number of players $M \in \mathbb{N}^{+}$, who produce differentiated varieties. Firms produce according to $\tilde{F}\left(\gamma,L,K\right) = \gamma \cdot F\left(L,K\right)$ where $\gamma$ is idiosyncratic TFP and $ F\left(L,K\right)$ is a constant returns to scale production function satisfying the Inada conditions. 
Operating in a product market of type $i$ requires a per period fixed cost $c_i$ (in units of the final good). Firms purchase factors of production in competitive factor markets, but imperfectly compete in product markets. Different product categories can be subject to different market structures (e.g. Cournot or Bertrand competition).
The technology can be summarized by a matrix of Hicks-neutral idiosyncratic productivities $\Gamma \coloneqq \big[\gamma_{ij}\big]_{\left(I\times M\right)}$ and a vector of fixed costs $\mathcal{C} \coloneqq \big[c_{i}\big]_{\left(I\times 1\right)}$. 
%The elements of each row of $\Gamma$ appear in decreasing order, so that $\gamma_{ij} \geq \gamma_{ij+1}$ (i.e. more productive firms are ranked first).\footnote{These assumptions are with no loss of generality. If an industry can only have a maximum of $M<N$ firms, this can be modeled as $\gamma_{ij}=0 \; \forall j \geq M+1$.} To simplify the exposition, we assume that firms have identical fixed costs $c_{ij} = c$ and that, within a market, firms enter sequentially in decreasing order of productivity.\footnote{Therefore, if firm $\gamma_{ij}$ is active, all firms $k$ with $\gamma_{ik}>\gamma_{ij}$ are also active.}
Given these definitions, the technology set is summarized by $\Lambda \coloneqq \left[\:\Gamma\,,\:\mathcal{C}\,\right]$.
The aggregate mass of firms can be written as $ n =
\sum_{i=1}^{I} \, \sum_{m=1}^{M} \, \eta_{im} \, m$, where $\eta_{im}\in\left[0,1\right]$ is the fraction of product markets $i$ with $m \leq M$ firms. We assume that firms enter sequentially and that firms making higher profits enter first. Given these assumptions, the aggregate mass of firms $n$ and the technology set $\Lambda$ fully characterize the set of active firms. For exposition purposes, we work with a deterministic setting subject to one time unexpected shocks. In particular, we think of the possibility of shocks that destroy a fraction $1 -\chi \in \left[0,1\right]$ of the capital stock. Aggregate uncertainty, by means of stochastic TFP, is introduced in the model we study in Section \ref{sec:Model}.

\begin{definition}[Equilibrium]
An equilibrium in this economy is a set of policies such that i) all agents optimize; ii) all active firms make no loss; iii) inactive firms would make a loss upon entry and iv) all markets clear. 
\end{definition}

This economy admits an aggregate production function, which we characterize in Lemma \ref{lemma: agg_pf}.

\begin{lemma}[Aggregate Production Function \label{lemma: agg_pf}]
The aggregate production function is given by \[ F(\Lambda, K, n\left(\Lambda,K\right))= \Phi(\Lambda,n\left(\Lambda,K\right)) \, F(K,L), \]
where $\Lambda$ is the technology set (as defined above), $n$ is the mass of active firms, and $\Phi(\cdot)$ is aggregate TFP. Finally $F(K,L)$ is the CRS production function introduced above.\footnote{Note that $L$ is a function of the set of state variables $\left(\Lambda,K\right)$. For ease of notation we suppress these. }
\end{lemma}
\begin{proof}
See Appendix \ref{appendix:proofs_section_2}.
\end{proof}

Aggregate TFP $\Phi(\Lambda,n\left(\Lambda,K\right))$ reflects two terms: a weighted average of firm level productivity $\gamma_{ij}$ and love for variety. From the aggregate production function it is possible to characterize the economy's inverse demand for capital. Let $\Omega$ denote the aggregate factor share (i.e. the ratio of total labor and capital payments over gross output $Y$). As shown in Appendix \ref{appendix:proofs_section_2},  the equilibrium rental rate can be written as
\begin{align} \label{eq:rr_map}
R(\Lambda,K) \; =  \; \Omega(\Lambda,n\left(\Lambda,K\right)) \, \Phi(\Lambda,n\left(\Lambda,K\right)) \,  F_{K}\big(K, L \big) . 
\end{align} 
It is convenient to define $\Theta\left(\Lambda,n\right)\coloneqq\Omega(\Lambda,n) \, \Phi(\Lambda,n)$, which represents a measure of aggregate factor prices (Appendix \ref{appendix:proofs_section_2}).
\footnote{This is equal to the Lagrange multiplier of the cost minimization problem for a firm with unit productivity.}
Given the demographic structure of this economy, the long-run supply of capital is infinitely elastic and given by\footnote{This can be obtained by evaluating the stationary Euler equation of the representative household.}
\begin{align}
R^{*} = \beta^{-1} - \left(1-\delta\right).
\end{align}
Therefore, the economy features multiple steady-states if the following equation admits more than one solution
\begin{align}
    R(\Lambda,K) = R^{*} .
    \label{rmap}
\end{align}
The red curve in Figure \ref{fig:multiplicity_figure} represents the capital demand schedule in eq. (\ref{eq:rr_map}) for a particular economy. Assuming that the Inada conditions are satisfied, we have $R(\Lambda,0)=\infty$ and $R(\Lambda,\infty)=0$. Therefore, multiple steady-states occur only if (\ref{eq:rr_map}) features at least one increasing part. As explained in Section \ref{appendix:generalframework} of the Supplementary Material, there are different mechanisms that can make $R\left(\cdot\right)$ locally increasing in $K$.
%\footnote{They can be grouped into three broad sets of mechanisms: reallocation, love for variety and market power. We exclude, by assumption, increasing returns in $F\left(\cdot\right)$ and backward bending labor supply. See Section \ref{appendix:generalframework} of the Supplementary Material.}
For example, suppose that firm entry increases in capital, so that competition and the aggregate factor share $\Omega(\Lambda,n)$ are also increasing in $K$. Then, if $\Omega(\Lambda,n)$ increases sufficiently fast in $K$ in some region, it can counteract decreasing returns $F_{K}\left(\cdot\right)$ and make $R(\cdot)$ locally increasing. In Figure \ref{fig:multiplicity_figure}, the economy in red contains two stable steady-states, $K_{1}^{S}$ and $K_{2}^{S}$, and an unstable one, $K_{1}^{U}$. The initial capital stock determines the unique path that the economy follows and the steady-state to which it converges.\footnote{When the economy starts on the left of $K_{1}^{U}$ it reaches $K_{1}^{S}$, otherwise it achieves $K_{2}^{S}$. Multiple paths would be possible if the curve in Figure \ref{fig:multiplicity_figure} was a correspondence, and not a function. In this section, we exclude multiple paths by assumption.} We are particularly interested in the possibility of downward transitions across steady-states. Note that, if the economy starts close to the high steady-state $K_{2}^{S}$, a transition to $K_{1}^{S}$ occurs if the economy is hit by a shock that destroys a fraction $1 - K_{1}^{U}/K_{2}^{S}$ of its capital stock. Thus, the likelihood of a downward transition depends on the distance between $K_{1}^{U}$ and $K_{2}^{S}$. For example, under the alternative economy represented in blue, a smaller fraction of the capital stock needs to be destroyed for a downward transition to take place, $1 - \tilde{K}^U_{1}/\tilde{K}^S_{2}$. This second economy is characterized by a lower capital demand schedule for sufficiently high values of $K$. This suggests that a reduction in the aggregate demand for capital can be associated with a higher likelihood of downward transitions across steady-states. We next formalize the concept of \textit{fragility} and explore different mechanisms that, by decreasing the aggregate demand for capital, can result in more likely downward transitions.

\begin{figure}[htb]
    \centering
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=1pt,y=1pt,yscale=-.75,xscale=.75]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Axis 2D [id:dp775497830869011] 
\draw [line width=3]  (15.6,253.42) -- (641.6,253.42)(78.2,27.52) -- (78.2,278.52) (634.6,248.42) -- (641.6,253.42) -- (634.6,258.42) (73.2,34.52) -- (78.2,27.52) -- (83.2,34.52)  ;
%Straight Lines [id:da9277312210637947] 
\draw [line width=3]  [dash pattern={on 7.88pt off 4.5pt}]  (79,151) -- (616.6,151.52) ;
%Curve Lines [id:da6180121553167277] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=3]    (96.6,57.52) .. controls (107.6,98.52) and (185.6,179.52) .. (216.6,199.52) ;
%Curve Lines [id:da05797439702758567] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=3]    (215,199.52) .. controls (243.6,177.52) and (257.6,168.52) .. (296.6,105.52) ;
%Curve Lines [id:da5620343829511387] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=3]    (295,105.52) .. controls (368.6,137.52) and (484.6,195.52) .. (577.6,217.52) ;


%Curve Lines [id:da333283432121507] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=3]    (112.6,56.52) .. controls (123.6,97.52) and (201.6,178.52) .. (232.6,198.52) ;
%Curve Lines [id:da4772784121211848] 

\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=3]    (231,198.52) .. controls (254.6,181) and (257.6,186) .. (302.6,126) ;
%Curve Lines [id:da8188162523653961] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=3]    (301,126) .. controls (374.6,158) and (492.6,216) .. (583.6,238) ;

% Text Node
\draw (623,269.4) node [anchor=north west][inner sep=0.75pt]    {$K$};
% Text Node
\draw (32,24.4) node [anchor=north west][inner sep=0.75pt] {$R(K)$};
% Text Node
\draw (50,143.4) node [anchor=north west][inner sep=0.75pt] {$R^{*}$};


%% STEADY STATES
%Straight Lines [id:da6720868559709041] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (161,150) -- (160.6,254.52) ;
%Straight Lines [id:da006637350827901178] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (265,151) -- (264.6,255.52) ;
%Straight Lines [id:da7659322515454083] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (396,151) -- (395.6,255.52) ;
% Text Node
\draw (145,263) node [color={rgb, 255:red, 208; green, 2; blue, 27 }][anchor=north west][inner sep=0.75pt]    {$K_{1}^{S}$};
% Text Node
\draw (249,263) node [color={rgb, 255:red, 208; green, 2; blue, 27 }][anchor=north west][inner sep=0.75pt]    {$K_{1}^{U}$};
% Text Node
\draw (387,263) node [color={rgb, 255:red, 208; green, 2; blue, 27 }][anchor=north west][inner sep=0.75pt]    {$K_{2}^{S}$};


%Straight Lines [id:da6720868559709041] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (181,150) -- (180.6,254.52) ;
%Straight Lines [id:da006637350827901178] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (285,151) -- (284.6,255.52) ;
%Straight Lines [id:da7659322515454083] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (366,151) -- (365.6,255.52) ;
% Text Node
\draw (175,263) node [color={rgb, 255:red, 74; green, 144; blue, 226 }][anchor=north west][inner sep=0.75pt]    {$\tilde{K}_{1}^{S}$};
% Text Node
\draw (283,263) node [color={rgb, 255:red, 74; green, 144; blue, 226 }][anchor=north west][inner sep=0.75pt]    {$\tilde{K}_{1}^{U}$};
% Text Node
\draw (353,263) node [color={rgb, 255:red, 74; green, 144; blue, 226 }][anchor=north west][inner sep=0.75pt]    {$\tilde{K}_{2}^{S}$};


\draw[fill={rgb, 255:red, 208; green, 2; blue, 27 },opacity=.3] (265,151) -- (264.6,255.52) -- (395.6,255.52)--  (396,151)  -- cycle;

\draw[fill={rgb, 255:red, 74; green, 144; blue, 226 },opacity=.3]  (285,151) -- (284.6,255.52) -- (365.6,255.52) -- (366,151) -- cycle;

\end{tikzpicture}
    \caption{Steady-state multiplicity}
    \label{fig:multiplicity_figure}
\end{figure}
\subsection{Technological Change and Fragility}
% Let $\mathcal{K}$ be the ordered set of capital levels in steady-states and $\mathcal{K^U}$ the collection of even elements of $\mathcal{K}$, which represent capital levels in unstable steady-states.\footnote{Note that we use even and odd elements as they correspond to unstable and stable steady-states, which are defined according to the local slope of $R(\cdot)$. }
We start by defining the concept of fragility, which is central to our analysis. Let $\mathcal{K}$ denote the ordered set of all steady-states capital levels. Let $\mathcal{K^S}$ be the collection of stable steady-states and $\mathcal{K^U}$ be the collection of unstable steady-states in $\mathcal{K}$. %\footnote{Note that $\mathcal{K^U}$ and $\mathcal{K^A}$ are respectively given by the set odd and even elements of $\mathcal{K}$)}
%\begin{definition}[Steady-States Transitions]\label{defitinitionSS}
%Define an upward transition as the economy moving from the $n-1^{th}$ element of the set $\mathcal{K}$ to the $n+1^{th}$ element, $\forall n \text{ even}$. Define a downward transition as the economy moving from the $n+1^{th}$ element of the set $\mathcal{K}$ to the $n-1^{th}$ element, $\forall n $ even. 
%\end{definition}
Recall that, in our setting, the economy can be hit by a one time unexpected shock that destroys a fraction $1-\chi$ of the capital stock.\footnote{The intuition behind all our results carries through under more general shock structures, with some adjustments. In general the capital level in a steady state depends on the shock realization. This would significantly increase the difficulty in defining a norm between $\mathcal{K}_{n}$ and $\mathcal{K}_{n-1}$, since their distance would become a random variable itself.} Our measure of fragility captures the proximity of a \textit{stable} steady-state $\mathcal{K}^S_{n}$ to the preceding \textit{unstable} steady-state $\mathcal{K}^{U}_{n-1}$. The closer these two steady-states are to each other, the lower is the minimum shock needed to trigger a downward transition.

\begin{definition}[Fragility]\label{definitionfragility}
Let $\chi_{n}\in[0,1]$ be defined as $\chi_{n} \coloneqq \mathcal{K}^U_{n-1} / \mathcal{K}^S_{n}$. It follows that $1 - \chi_{n}$ is the minimum size shock needed to make the economy move from $\mathcal{K}^S_{n}$ to $\mathcal{K}^S_{n-1}$. We call an increase in $\chi_{n}$ an increase in fragility. 
\end{definition}

%\begin{definition}[Fragility]\label{definitionfragility}
%Let $\chi_{n+1}\in[0,1]$ be defined as $\chi_{n+1} \coloneqq \mathcal{K}^U_n / \mathcal{K}_{n+1}$. It follows that $1 - \chi_{n+1}$ is the minimum size shock needed to trigger a downward transition from $\mathcal{K}_{n+1}$. We call an increase in $\chi_{n+1}$ an increase in fragility. 
%\end{definition}
Two further observations should be made. First, our main focus is on \textit{fragility}, which is different from the \textit{existence} of multiplicity. Although the first requires the second, these are different concepts. Second, the notion of \textit{fragility} is related to, but distinct from, the idea of the \textit{stability} of a steady-state. We think of \textit{fragility} as the possibility of downward transitions only. This is the size of the left partition of the basin of attraction of the steady-state, which is given by $\mathcal{K}^S_{n}-\mathcal{K}^U_{n-1}$. The notion of stability, instead, relates to the size of the whole basin of attraction and also accounts for the possibility of upward transitions.
%The fundamental question which interests us is how a change in a technology parameter, $\partial \lambda$, affects $\chi_{n}$. 
In Proposition \ref{propcompstatexrc} we state a sufficient condition for a technology shift to increase fragility, i.e. $\partial  \chi_{n}/{\partial\lambda}>0$. This condition says that fragility increases when the rental rate decreases for intermediate values of $K$ (i.e. in the region between steady-states). %This depends on the response of $\Theta\left(\cdot\right)$ to a technology shift.

\begin{prop}[Comparative Statics]\label{propcompstatexrc}
Let $\mathcal{K}^S_{n}$ be a stable steady-state and consider a technological shift $ \partial \lambda $. Then $\partial \chi_{n}/{\partial \lambda}>0$, i.e. the stable steady-state $\mathcal{K}^S_{n}$ becomes more fragile, if for $ K=\{\mathcal{K}^U_{n-1}, \, \mathcal{K}^S_{n}\} $
\begin{align}\nonumber
    &\frac{\partial}{ \partial  \lambda} \Theta\left(\Lambda,n\left(\Lambda,K\right)\right) = \Theta_{\lambda}\left(\Lambda,n\left(\Lambda,K\right)\right)+\Theta_{n}\left(\Lambda,n \left(\Lambda,K\right)\right)n_{\lambda}\left(\Lambda,K\right)   <0.
\end{align}
Using the definition of $\Theta(\cdot)$ we note that this is equivalent to
\begin{align}\nonumber
\hspace{-1cm}
\underbrace{\Omega(\Lambda,n)\Phi_{\lambda}(\Lambda,n)}_{\Delta \: \textrm{TFP}} \; + \;
\underbrace{\Omega_{\lambda}(\Lambda,n)\Phi(\Lambda,n)}_{\Delta \: \textrm{factor share}} \; + \;
\underbrace{\left[\Omega_{n}(\Lambda,n)\Phi(\Lambda,n) +
\Omega(\Lambda,n)\Phi_{n}(\Lambda,n)\right]n_{\lambda}\left(\Lambda,K\right)}_{\Delta \: \textrm{number of firms}} \; < \; 0 .
\end{align}
The first two terms characterize the direct effect of $ \partial \lambda $ on aggregate TFP and the factor share. The last term describes the effect of changes in the number of active firms. 

\end{prop}

\begin{proof}
See Appendix \ref{appendix:proofs_section_2}
\end{proof}

Proposition \ref{propcompstatexrc} provides a sufficient condition for a (technology-driven) increase in fragility. There are three main channels highlighted in this result: i) changes in aggregate TFP $\left(\Phi\right)$, ii) changes in the factor share $\left(\Omega\right)$ and iii) changes in the number of firms $\left(n\right)$.\footnote{We study these channels in detail in the Supplementary Materials through Remarks \ref{fixedfirms}, \ref{fixedaggTFP} and \ref{loveforvariety}.} To connect this result to the empirical patterns discussed in the introduction, we can think of $\partial  \lambda$ as an increase in firm level heterogeneity. Through the lens of Proposition \ref{propcompstatexrc} such an increase can trigger higher fragility by reducing the factor share (due to greater market power), via the reallocation of activity towards less productive firms or by reducing the number of active firms. If firms' market shares are increasing in their productivity, as heterogeneity increases three things happen: \textit{i)} a mechanical efficiency gain due to large firms becoming more productive and through positive reallocation; \textit{ii)} a compression of factor shares as large firms can exert more market power; \textit{iii)} entry is harder for firms outside the market, which can generate a loss of varieties and higher market power. 
Intuitively, if the anti-competitive forces \textit{ii)} and \textit{iii)} dominate the efficiency gains from higher heterogeneity \textit{i)}, the return to capital decreases and it becomes harder to sustain a high steady-state. 

The intuition behind the result described in Proposition \ref{propcompstatexrc} is similar in spirit to the findings of \cite{baqaee2020productivity} and \cite{EMX} relating dispersion and aggregate TFP. As will become clearer in the model presented in Section \ref{sec:Model}, we put forth the additional effect on the stability of the economy with respect to aggregate fluctuations. Our economy features an endogenous amplification mechanism that can trigger non-linearities in the response to shocks. As firms become more heterogeneous these non-linearities become more salient and the economy can be more likely to experience quasi-permanent slumps. To dig deeper into the forces underlying the effect of heterogeneity on fragility we specify a RBC model in which firms compete oligopolistically. This additional structure allows us to provide sharper theoretical and quantitative results.


%Any of these channels is theoretically sufficient to make the economy more fragile. In the next section we specify a model in which to address the problem quantitatively. We embed the workhorse oligopolistic competition model of \cite{AB} in an otherwise standard RBC setting. 
